Parametric Phase Tracking via Expectation Propagation

In this work we propose simple algorithms for signal detection in a single-carrier transmission corrupted by a strong phase noise. The proposed phase tracking algorithms are formulated within the framework of a parametric message passing (MP) which reduces the complexity of the Bayesian inference by using distributions from a predefined family; here, of Tikhonov distributions. This stays in line with previous works mainly inspired by the well-known Colavolpe-Barbieri-Caire (CBC) algorithm which gained popularity due to its simplicity and possibility for decoder-aided operation. In our work we mainly focus on practically relevant case of one-shot phase tracking that does not require decoder's feedback. Applying the principles of the expectation propagation (EP), we notably improve the performance of the phase tracking before the decoder's feedback can be even considered. The EP algorithms can be also integrated in the decoding loop in the spirit of joint decoding and phase tracking.

==> Includes/Algorithms.R1.v2.tex <==
%!TEX root =  ../Phase.Tracking.R1.v2.tex
\section{Phase tracking}\label{sec:phase.track}
%%%%%
%\subsection{Message passing on the graph}\label{Sec:MP.graph}
%%%%%%%%%%%%%%
\begin{figure}[bt]
\begin{center}
\scalebox{0.8}{\input{./figures/Graph.RRHARQ.x.2D.tex}}
\end{center}
\caption{Graph defining the relationship between the variables in the phase tracking problem used previously \eg in \cite[Fig.~2]{Colavolpe05}, \cite[Fig.~2]{Shayovitz16}; the messages exchanged between the nodes are shown together with the arrows indicating the direction of the exchange. When variable is connected to two functions, the message passes transparently through the variable node as in the case of probability $P_n(a)=\PR{x_n=a|\by}, a\in\mcA$ defining the distribution of the symbol $x_n$ via phase tracking, and its priori distribution $P_n^{\tr{a}}(a), a\in\mcA$  (obtained from the decoder).}
\label{fig:graph.tracking}
\end{figure}
%%%%%%%%%%%%%%%

Our goal now is to find $P_n(a), a\in\mcA$ exploiting the relationships between the involved random variables.  

As in \cite{Colavolpe05,Kreimer18}, we show in \figref{fig:graph.tracking} a graph which captures these relationships: the squares represent the functions taking as arguments the variables which, in turn, are represented by the directly connected circles. In particular
\begin{align}
\label{f.n.x}
g_n(\theta_n,x_n)  & \propto f(y_n|x_n,\theta_n) \\
&\propto \exp\left(-\SNRrv\Big|y_n-x_n\e^{\jmath\theta_n}\Big|^2\right)
\end{align}
corresponds to the relationship defined in \eqref{y.kn}, where we use $\pdf(\cd|\cd)$ to denote the conditional \gls{pdf}; the model \eqref{theta.Wiener} yields 
\begin{align}\label{p.w}
q(\theta_n,\theta_{n+1}) &\propto \pdf(\theta_n|\theta_{n+1})\propto\pdf( \theta_{n+1} | \theta_{n} )\\
&=\omega(\theta_n-\theta_{n+1}),
\end{align}
with
\begin{align}\label{Normal.pdf}
\omega(\theta)=\frac{1}{\sqrt{2\pi \sigma^2_w}}\sum_{k=-\infty}^{\infty}\exp\left(-\frac{(\theta-k2\pi)^2}{2\sigma^2_w}\right)
\end{align}
being a zero-mean, wrapped Gaussian distribution defined over any interval of length $2\pi$.

In \figref{fig:graph.tracking} we also show a shaded rectangle labeled as ``modulation/coding graph''; it also contains a graph which describes the relationship $\set{x_n}  \rightarrow \set{s_n} \rightarrow \set{c_n} \rightarrow \set{b_n}$, and its knowledge is used for the demodulation (to implement \eqref{lambda.n.l}) and for the decoding.

If the phase tracking has to be carried out and no decoding was not yet executed,  the payload symbols $x_n$ are assumed to be \gls{iid}, with non-informative a priori distribution over the transmitted symbols, \ie $P^{\tr{a}}_n(a)\propto 1$. In a case we would like  to perform the joint decoding/demodulation/phase tracking, as done, \eg in \cite{Colavolpe05,Kreimer18,Alfredsson19}, we use $P^{\tr{a}}_n(a)$ obtained from the decoding results. 

Thus, from the point of view of the phase tracking, the relationships induced by the modulation/coding graph are summarized by $P^{\tr{a}}_n(a)$. As a direct consequence, the graph we deal with in \figref{fig:graph.tracking} is a tree, \ie contain no loops. Therefore, the efficient marginalization can be done exactly by the \gls{mp} algorithm as follows \cite{Colavolpe05}, \cite{Shayovitz16}, \cite{Kreimer18}
\begin{align}\label{P.n.x}
P_n(a) \propto\int_{-\pi}^{\pi}  \alpha_n(\theta)  \beta_n(\theta) g_n(\theta,a ) \dd \theta,\quad a\in\mcA,
\end{align}
where
\begin{align}\label{alpha}
\alpha_n(\theta)&\propto \big(\alpha_{n-1}(\theta)  \gamma_{n-1}(\theta)\big) \convop 
\omega(\theta),\\
\label{beta}
\beta_n(\theta)&\propto \big(\beta_{n+1}(\theta) \gamma_{n+1}(\theta) \big) \convop 
\omega(\theta),\\
\label{gamma}
\gamma_n(\theta)&\propto\sum_{a\in\mcA} P^{\tr{a}}_n(a) g_{n}(\theta,a ),%=\sum_{x\in\mcA}  g_{n}(\theta,a ),
\end{align}
are (proportional to) the marginal distributions of the phase $\theta_n$ conditioned, respectively, on $y_0,\ld,y_{n-1}$, on $y_{n+1},\ld,y_{N}$, and  on $y_n$.\footnote{That is,
\begin{align}
\alpha_n(\theta)&\propto\pdf(\theta_n| y_0,\ld,y_{n-1})\\
\beta_n(\theta)&\propto\pdf(\theta_n| y_{n+1},\ld,y_{N})\\
g_n(\theta,a)&\propto\pdf(\theta_n| y_{n},a)
\end{align}
and thus the integrand in \eqref{P.n.x} is the posterior distribution of the phase
\begin{align}
\pdf(\theta_n | \by, a)&\propto
 \alpha_n(\theta)  \beta_n(\theta) g_n(\theta,a ) 
\end{align}
while $P_n(a)$ is given by \eqref{P.n.a.x}.

} All the distributions of the phase are periodic and so is the convolution in \eqref{alpha} and \eqref{beta}. 
%These equations are practically the same as those appearing in the \gls{bcjr} recursion \cite{BCJR} well known in the area of decoding of convolutional codes to obtain the distribution of the bits, which has discrete argument. Here, derived from the graph representation, they are applied to calculate the continuous-argument distributions of the phase. 

%%%%%%%%%
\section{Parametric message passing}\label{Sec:Parametric.MP}
The operations \eqref{P.n.x}-\eqref{gamma} which allow us to calculate $P_n(a)$ may be implemented on the discretized versions of the distributions $\alpha_n(\theta)$, $\beta_n(\theta)$, and $\gamma_n(\theta)$ defined over the samples of $\theta\in(-\pi, \pi]$. In such a \gls{dmp} the multiplications and additions are straightforward to implemented and the convolution is efficiently implemented via \gls{fft}. 

However, to ensure sufficient precision of the discretization, a large number of samples, $N_{\theta}$, may be needed.\footnote{\label{foot:N8} The literature often used $N_\theta=8M$ \eg \cite{Peleg00,Colavolpe05,Shayovitz16,Kreimer18} but finding the smallest $N_{\theta}$ which ensures the sufficient accuracy of the \gls{mp}, \eqref{alpha}-\eqref{gamma}, is difficult. 

The general rule is that all the distributions involved in the \gls{mp} should be represented without ``significant'' loss of accuracy so the sampling step should decrease when the spectral support of the distributions increases. 

Then, by approximating the distributions by Gaussians, we know that their spectral support is proportional to their precision (inverse of the variance). Thus, observing that the precision of $g_n(\theta,a)$ increases with the \gls{snr}, see also \eqref{f.n.x.Tikh}-\eqref{z.fn}, and the precision of $\omega(\theta)$ decreases with $\sigma_w^2$, we may conclude that the number of samples will grow when we increase the \gls{snr} or when we decrease the phase-noise level. These operational conditions are also required to transmit reliably high-order constellations. So, indeed, we should expect that the $N_\theta$ will grow with $M$ but we are not aware of any formal study backing up the heuristics $N_\theta=8M$ (that turned out unnecessarily conservative in our case, see Footnote~\ref{foot:DMP32} in \secref{example.start}.).
%, which is where the impact of the \gls{dmp} complexity will be the most notable. In such a case, the simplification may be sought by limiting the period over which the distribution must be represented \cite{ShahMohammadian18}.
}  Since this implies a large computational complexity as well as a storage requirements, many previous works have gone in the direction of parametric representation of the involved periodic distributions. Then, instead of tracking the samples in \gls{dmp}, we only need to track (a few) parameters which represent the distributions. 

We thus should find a family of the distributions, $\mcF$, on which the operations defined in \eqref{P.n.x}-\eqref{gamma} are easily dealt with. In particular, we have to handle multiplication of the periodic functions as well as, the convolution in \eqref{alpha} and \eqref{beta}; the integration in \eqref{P.n.x}, when done on the parametric forms of distributions, is usually straightforward.

%%%%%%%%%
%\subsection{Tikhonov distributions}\label{Sec:Tikh.dist}
In this work we consider a family of  Tikhonov distributions which were already used, \eg in \cite{Colavolpe05,Barbieri07,Shayovitz16}. Here, to simplify the notation we use unnormalized distributions 
\begin{align}\label{Tikh.definition}
\mcT(\theta; z)= \e^{\Re[z\e^{-\jj \theta}]},
\end{align}
where $\Re[\cd]$ denotes the real part and $z$ is a complex parameter whose phase is the circular mean of the underlying variable and the value of $|z|$ is, approximatively, a measure of precision \cite{Kurz16}.\footnote{The normalized distribution is obtained as
\begin{align}
\mcT^\text{norm}(\theta; z)=\frac{\mcT(\theta; z)}{\int_0^{2\pi}\mcT(\theta; z)\dd \theta}=\frac{\e^{\Re[z\e^{-\jj \theta}]}}{2\pi I_0(|z|)},
\end{align}
where $I_0(\cd)$ is the zero-th order modified Bessel function. 
}

The multiplications are trivial over $\mcF$ 
\begin{align}\label{Tikh.multiplication}
\mcT(\theta; z_1)\mcT(\theta; z_2)
&=%\frac{I_0(|z_1+z_2|)}{2\pi I_0(|z_1|)I_0(|z_2|)}
\mcT(\theta; z_1+z_2),
\end{align}
while the convolution with the Gaussian, appearing in \eqref{alpha} and \eqref{beta}, must be treated via  approximations as done before \cite[Appendix]{Colavolpe05} and also explained using the concept of a \gls{cmm} in \appref{conv.T.G}
\begin{align}\label{Tik.h.Normal.convolution}
\mcT(\theta; z)&\convop\omega(\theta)
\propto  \mcT\Big( \theta; \frac{z}{1+\sigma_w^2|z|} \Big).
\end{align}

We also note that $g_n(\theta,a) \in \mcF$, so \eqref{f.n.x} can be rewritten as
\begin{align}\label{f.n.x.Tikh}
g_n(\theta,a)&%\propto \e^{\xi_{g,n}(a)}\mcT\big(\theta; z_{g,n}(a)\big) \\
\propto \e^{-\SNRrv |a|^2}\mcT\big(\theta; z_{g,n}(a)\big) \\
\label{z.fn}
z_{g,n}(a)&=2\SNRrv ~y_n a^{*}.
%\label{xi.f.n}
%\xi_{g,n}(a)&=%\e^{ -\frac{|a|^2}{\No} }I_0\big(|z_{g,n}(a)|\big)=
%-\frac{|a|^2}{\No} +\hat{I}_0(|z_{g,n}(a)|),
\end{align}

Instead of Tikhonov family we might opt for the wrapped Gaussians \eqref{Normal.pdf} but 
\begin{itemize}
\item To  take care of their periodic nature, particular attention is required when dealing with multiplication  \cite[Sec.~II.B]{Kurz16}; this aspect is not always emphasized in the literature: in some works,  the Gaussian distributions are used without explicit wrapping. Ignoring the circularity, it produces an apparent closeness under multiplication but may lead to interpretation errors when ``locking'' on the wrong phase, see example in \cite[Fig.~1]{Kurz16}; 
\item We have to start using approximations already for $g_n(\theta,a)$; it can be done, of course, \eg as in \cite{Kreimer18}, but requires the introduction of additional layer of approximations before the \gls{mp} is derived. This stands in contrast with a natural representation of  $g_n(\theta,a)$ by a Tikhonov distribution in \eqref{f.n.x.Tikh},
and 
\item Comparing to the Tikhonov distributions, Gaussians are less well suited to represent the uniform or almost-uniform distributions of the phase (in Tikhonov family this is obtained by setting $z\approx 0$, while in Gaussian the variance must tend to infinity).
\end{itemize}

If $\alpha_n(\theta), \beta_n(\theta), \gamma_n(\theta), \omega(\theta)\in\mcF$  and $\mcF$ was closed under  multiplication and convolution, the parametric \gls{mp} would be immediately obtained. This condition,  however, does not materialize with the most popular circular distributions such as the wrapped Gaussian distributions or  the Tikhonov distributions \cite{Kurz16}. Namely, the space of wrapped Gaussian distributions is not closed under multiplications, while the Tikhonov space is not closed under convolution. 


We thus conclude that, independently of the family $\mcF$ we decide to use, approximations will be necessary. However, this is not the main issue in the parametric \gls{mp}; the main difficulty stems from the presence of $\gamma_n(\theta)$  which is a mixture of Tikhonov distributions which  we rewrite as
\begin{align}\label{gamma.def.mixture}
\gamma_n(\theta)&\propto\sum_{a\in\mcA}\e^{\eta_{g,n}(a)}\mcT\big(\theta;z_{g,n}(a )\big),\\
\label{eta.f.n}
\eta_{g,n}(a)&=-\SNRrv ~|a|^2+\hat{P}^{\tr{a}}_n(a),%+ \hat{I}_0\big(|z_{g,n}(a)|\big)
\end{align}
where we again use $\hat{P}^{\tr{a}}_n(a)=\log P^{\tr{a}}_n(a)$ because the logarithmic representation simplifies the implementation.

There are essentially two approaches that have been used in the literature to deal with this issues and we compare them in the following.

%%%
\subsection{Out-of recursion projection: \acrshort{cbc} algorithm}\label{Sec:Pre-MP}

Taking advantage of the fact that $\gamma_n(\theta)$ is not obtained recursively, its approximation, $\tilde{\gamma}_n(\theta)$ may be obtained \emph{before} the recursive steps of \gls{mp} \eqref{alpha}-\eqref{beta} are executed. This may be seen as the following approximation of the \gls{rhs} of \eqref{alpha}:
\begin{align}
\label{alpha.projection.preMP}
\alpha_n(\theta)&\propto \mcF\left[\big(\alpha_{n-1}(\theta)  \gamma_{n-1}(\theta)\big) \convop  \omega(\theta)\right]\\
\label{alpha.projection.preMP.1}
&\approx \mcF\left[\alpha_{n-1}(\theta)  \gamma_{n-1}(\theta)\right] \convop  \omega(\theta)\\
\label{alpha.projection.preMP.2}
&\approx \big(\alpha_{n-1}(\theta)  \mcF[\gamma_{n-1}(\theta)]\big) \convop  \omega(\theta)\\
\label{alpha.projection.preMP.3}
&= \big(\alpha_{n-1}(\theta)  \tilde\gamma_{n-1}(\theta)\big) \convop  \omega(\theta)
\end{align}
where, 
\begin{align}\label{gamma.projection.first}
\tilde{\gamma}_n(\theta)
&=\mcF[\gamma_n(\theta)]=\mcT\Big(\theta;  z_{\tilde{\gamma},n} \Big)\\
&=\mcF\Big[ \sum_{a\in\mcA}\e^{\eta_{g,n}(a)}\mcT\big(\theta;z_{g,n}(a )\big) \Big],
\end{align}
and, with a slight abuse of notation we use $\mcF[\cd]$ to denote the operator which  projects $\gamma_n(\theta)$ onto the Tikhonov family $\mcF$. To pass from \eqref{alpha.projection.preMP} to \eqref{alpha.projection.preMP.1} we used (approximate) closeness of $\mcF$ with respect to convolution and this approximation holds well. On the other hand, to pass from  \eqref{alpha.projection.preMP.1} to \eqref{alpha.projection.preMP.2} we used the   approximation $\mcF\left[\alpha_{n-1}(\theta)  \gamma_{n-1}(\theta)\right]\approx \alpha_{n-1}(\theta)\mcF\left[\gamma_{n-1}(\theta) \right]$ that holds only if $\gamma_n(\theta)\in\mcF$. This is not the case, of course, but in this way we can precalculate $\tilde{\gamma}_n(\theta)$ before the \gls{mp} recursion starts. This idea underlies the \acrfull{cbc} algorithm introduced in \cite{Colavolpe05}.

Next, since all the distributions are from the Tikhonov family, \ie $\alpha_n(\theta)=\mcT(\theta;z_{\alpha,n})$ and $\beta_n(\theta)=\mcT(\theta;z_{\beta,n})$, replacing $\gamma_n(\theta)$ with $\tilde{\gamma}_{n}(\theta)$ (as defined in  \eqref{gamma.projection.first})  and applying \eqref{Tikh.multiplication} and \eqref{Tik.h.Normal.convolution}, we obtain the following parametric \gls{mp} :
\begin{align}
\label{z.alpha.init}
z_{\alpha,0}&=0,\\
\label{z.alpha}
z_{\alpha,n}&= \frac{z_{\alpha,n-1} + z_{\tilde{\gamma},n-1}}{1+|z_{\alpha,n-1} + z_{\tilde{\gamma},n-1}|\sigma_w^2}, \quad n=1, \ld,N-1\\
\label{z.beta.init}
z_{\beta,N}&=0,\\
\label{z.beta}
z_{\beta,n}&= \frac{z_{\beta,n+1} + z_{\tilde{\gamma},n+1}}{1+|z_{\beta,n+1} + z_{\tilde{\gamma},n+1}|\sigma_w^2}, \quad n=N-1,\ld,1,
\end{align}
which is exactly equivalent to the \gls{cbc} algorithm defined in \cite[Eq.~(36)-(37)]{Colavolpe05} and  is provided for completeness and as a starting point for the discussion.

Using \eqref{Tikh.multiplication}  and \eqref{f.n.x.Tikh}--\eqref{z.fn} in \eqref{P.n.x}, the ``extrinsic'' symbol probabilities are also calculated as \cite[Eq.~(35)]{Colavolpe05}
\begin{align}\label{P.a.final}
P_n( a )&\propto \int_{0}^{2\pi} \mcT\big(\theta;z_{\Sigma,n}(a)\big)\e^{-\SNRrv|a|^2} \dd \theta,\\
\label{P.a.final.2}
\hat{P}_n( a )&=\log P_n( a )\\
&\propto -\SNRrv |a|^2 + \hat{I}_0\big(|z_{\Sigma,n}(a)|\big),
\end{align}
where
\begin{align}
\label{z.Sigma.n}
z_{\Sigma,n}(a)&=z_{\alpha,n}+z_{\beta,n}+z_{g,n}(a),%2\SNRrv~y_n a^{*},\\
\end{align}
and we avoid numerical issues due to the exponential grows of $I_0(\cd)$ by using its log-version
\begin{align}\label{hat.I0}
\hat{I}_0(x) &= \log I_0(x) = x  + \Delta(x),
\end{align}
with $\Delta(x)$ being the log-domain corrective factor.\footnote{The approximation $\Delta(x)\approx -\frac{1}{2}\log(2\pi x)$ is tight for large $x$ \cite[Eq.~(96)]{Shayovitz16}\cite[Eq.~(18)]{Pecorino15}  but does not apply for small arguments because $\Delta( 0 )=0$. Thus, for a better accuracy, $\Delta(x)$ may be implemented via lookup table. On the other hand, it is also possible to simply set $\Delta(x)\approx 0$.}

Further,  the log-probability $\hat{P}_n( a )$ should be used in \eqref{lambda.n.l}.  

Due to its simplicity the \gls{cbc} algorithm \eqref{z.alpha.init}-\eqref{z.beta}, should be treated as a ``canonical'' solution to the problem of phase tracking: it is explicit and requires no fine-tuning. This, and its historical precedence,  explains the considerable attention it received up to now.

The remaining issue is the projection in \eqref{gamma.projection.first} and \cite{Colavolpe05} proposed to approximate $\gamma_n(\theta)$ with $\tilde{\gamma}_n(\theta)\in\mcF$ by,  first matching a Gaussian to $\pdf(y_n|\theta_n,a)\propto g_n(\theta,a)$ from which a Tikhonov distribution was derived as \cite[Sec.~IV.B]{Colavolpe05}
\begin{align}
\label{hat.z.gamma}
\tilde{\gamma}_n(\theta)
&=\mcT\Big(\theta;  z_{\tilde{\gamma},n} \Big)\\
\label{gamma.GA.cases}
z_{\tilde{\gamma},n}&=
\begin{cases}
z_{g,n}(x_n)  & \text{if}\quad n= l L\\
2\frac{y_n\mfm_n^{*}}{\No+ \mfv_n}, & \text{if}\quad n\neq l L
\end{cases}
\end{align}
where 
\begin{align}
\label{m.n.A}
\mfm_n&=\sum_{a\in\mcA}  a P^{\tr{a}}_n(a) ,\quad%\label{v.n.A}
\mfv_n=\sum_{a\in\mcA}  |a|^2 P^{\tr{a}}_n(a)   -  |\mfm_n|^2,
\end{align}
are the mean and the variance of $x_n$. 

The approximation is needed only for the payload positions, $n\neq lL$. For the pilots $x_n, n=lL$, we have $\gamma_n(\theta)=g_{n}(\theta, x_{n} )$ so we can use directly the parameter of the Tikhonov distribution $z_{g,n}(x_n)$.

This \gls{ga} approach was often reused in the literature, \eg \cite{Barbieri07,Pecorino15,Alfredsson19} as the integral part of the \gls{cbc} algorithm. 

On the other hand, recognizing that the distribution \eqref{gamma.def.mixture} is circular, instead of the \gls{ga}  we may apply the \gls{cmm}. It relies on minimization of the \gls{kl} distance between $\tilde{\gamma}_n(\theta)$ and the mixture $\gamma_n(\theta)$, and changes the way the parameter $z_{\tilde{\gamma},n}$ is calculated, which we express as follows
\begin{align}
%\tilde{\gamma}_n(\theta)
%&=\mcT\Big(\theta;  z_{\tilde{\gamma},n} \Big)\\
%&=\mcF\Big[ \sum_{a\in\mcA}\e^{\eta_{g,n}(a)}\mcT\big(\theta;z_{g,n}(a )\big) \Big],\\
\label{gamma.projection.first.cases}
z_{\tilde{\gamma},n}
&=
\begin{cases}
z_{g,n}(x_{n}) &\text{if}\quad n= l L\\
\mf{CMM}\Big[ \big\{\eta_{g,n}(a), z_{g,n}(a)\big\}_{a\in\mcA}  \Big]&\text{if}\quad n\neq l L,
\end{cases}
\end{align}
where the dependence of $z_{\tilde{\gamma},n}$ on  $\eta_{g,n}(a)$ and $z_{g,n}(a)$, indexed by $a\in\mcA$  is defined in closed-form by a function $\mf{CMM}[\cd]$ shown in \appref{Sec:CMM}. %and which  follow closely \cite[Appendix~A]{Shayovitz16}. 

Before going further, we note that the difference between the original formulation of the \gls{cbc} algorithm in \cite{Colavolpe05} and this work appears in the way the approximate distribution $\tilde{\gamma}_n(\theta)$ is obtained, that is, whether we opt for the \gls{ga} \eqref{gamma.GA.cases}, or we use the \gls{cmm} from \eqref{gamma.projection.first.cases}. 

Although the \gls{cmm} was already used in the context of the phase tracking by \cite{Shayovitz16}, we are not aware of it being applied as a part of the \gls{cbc} algorithm. And while the implementation of the function $\mf{CMM}[\cd]$ is slightly less straightforward\footnote{Approximations of non-linear functions are involved, see \appref{Sec:CMM} and \appref{Sec:Bx}.} than the \gls{ga} shown in \eqref{hat.z.gamma}-\eqref{m.n.A}, it is worthwhile to evaluate the advantage of the former. 

An important observation, already made \eg in \cite[Sec.~I]{Shayovitz16} or \cite[Sec.~IV]{Pecorino15}, is that, using a non-informative prior $\hat{P}^{\tr{a}}(a)\propto 0$,  the approximation $\tilde{\gamma}_n(\theta)$ is also non-informative for the payload symbols; that is, \mbox{$z_{\tilde{\gamma},n}=0, n\neq lL$}.\footnote{If  the \gls{ga} \eqref{hat.z.gamma}-\eqref{m.n.A}, is used,  this is true, if the constellation $\mcA$ is zero mean, which is obvious from \eqref{m.n.A}. On the other hand, if the \gls{cmm} approach is used, this is true if the constellations $\mcA$ may be decomposed into constant modulus zero-mean sub-constellations; the demonstration is easy and omitted for sake of space. For the most popular constellations such as $M$-\gls{qam}, both conditions hold.}  Then, the only useful information is obtained from the non-zero $z_{\tilde{\gamma},n}$ (\ie from the pilots).

Thus,  the \gls{mp} in \eqref{z.alpha.init}-\eqref{z.beta} may be then seen as a \emph{pilot-only} based recursive estimation of the phase.  In fact, it is independent of the form of the constellation $\mcA$ used to modulate the payload symbols and this is why, in order to exploit the knowledge of $\mcA$, the \gls{cbc} phase tracking must be placed in the ``decoding-loop''. Known also as the joint phase tracking and decoding, it consists in alternate execution of  i)~the \gls{mp}  \eqref{z.alpha.init}-\eqref{z.beta} and ii)~the demodulation/decoding; the latter, providing an informative prior $\hat{P}^{\tr{a}}_n(a)$ on the payload symbols, improves the phase tracking, see \eg \cite{Colavolpe05,Barbieri07,Alfredsson19}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Intra-recursion projection: \gls{skr} algorithm}\label{Sec:Intra-MP}}

As we said, the disadvantage of the pre-\gls{mp} projection from \secref{Sec:Pre-MP} is that, without the decoder's feedback, the structure of the constellation $\mcA$ is ignored. In order to exploit the form of $\mcA$, Shayovitz and Raphaeli \cite{Shayovitz16}, as well as, Kreimer and Raphaeli \cite{Kreimer18} proposed to perform the projection on $\mcF$ \emph{after} the multiplications in \eqref{alpha}-\eqref{beta} are executed.  That is, the projections are carried out inside the \gls{mp} recursion.

From the perspective we adopted, the resulting \acrfull{skr} algorithms is obtained implementing  the approximations \eqref{alpha.projection.preMP.1}
\begin{align}\label{alpha.projection}
\alpha_n(\theta)&\propto 
\label{alpha.projection.3}
 \mcF\big[\alpha_{n-1}(\theta)\gamma_{n-1}(\theta)\big]\convop \omega(\theta)\\
&\approx \check{\alpha}_{n-1}(\theta) \convop \omega(\theta),\\
\label{beta.projection}
\beta_n(\theta)&\propto 
\mcF\big[\beta_{n+1}(\theta)\gamma_{n+1}(\theta)\big]  \convop  \omega(\theta)\\
&\approx\check{\beta}_{n+1}(\theta)\convop  \omega(\theta),
\end{align} 
where we define the ``auxiliary'' distributions obtained via projections
\begin{align}
\nonumber
\check{\alpha}_{n}(\theta)&=\mcT\big(\theta; z_{\check{\alpha},n}\big)\\%\mcF\big[\alpha_{n-1}(\theta)\gamma_{n-1}(\theta)\big]\\
\label{check.alpha}
&=\mcF\left[\sum_{a\in\mcA} P^{\tr{a}}_{n}(a) \alpha_{n}(\theta)g_{n}(\theta, a )\right]\\
\label{z.alpha.check}
z_{\check{\alpha},n}&=\mf{CMM}\Big[\big\{\eta_{g,n}(a), z_{\alpha,n}+z_{g,n}(a)\big\}_{a\in\mcA} \Big].
\end{align}
and
\begin{align}
\nonumber
\check{\beta}_{n}(\theta)&=\mcT\big(\theta; z_{\check{\beta},n}\big)\\%\mcF\big[\beta_{n+1}(\theta)\gamma_{n+1}(\theta)\big]\\
\label{check.beta}
&=\mcF\left[ \sum_{a\in\mcA} P^{\tr{a}}_{n}(a) \beta_{n}(\theta)g_{n}(\theta, a )  \right],\\
\label{z.beta.check}
z_{\check{\beta},n}&=\mf{CMM}\Big[\big\{\eta_{g,n}(a), z_{\beta,n}+z_{g,n}(a)\big\}_{a\in\mcA} \Big].
\end{align}

Using \eqref{Tik.h.Normal.convolution} in \eqref{alpha.projection.3} and \eqref{beta.projection} we obtain the following parametric \gls{mp}:
\begin{align}
z_{\alpha,0}&=0,\\
z_{\alpha,n}&= \frac{z_{\check{\alpha},n-1}}{1+|z_{\check{\alpha},n-1}| \sigma_w^2}, \quad n=1, \ld,N-1\\
z_{\beta,N}&=0,\\
z_{\beta,n}&= \frac{z_{\check{\beta},n-1}}{1+|z_{\check{\beta},n-1}| \sigma_w^2}, \quad n=N-1,\ld,1.
\end{align}

Comparing to the  \gls{cbc} algorithm from \secref{Sec:Pre-MP}, the \gls{skr} algorithms invokes the \gls{cmm} function twice for each time $n$ and this, even if no feedback is obtained from the decoder. This increases the computational burden comparing to the \gls{cbc} algorithm, which  invokes the \gls{cmm} function only once per $n$ (and does not need it at all in the case the decoder's feedback is not available). The hope is that, introducing approximations (projection) inside the \gls{mp} recursion will minimize the approximation errors.

Again, we can apply the \gls{skr} algorithm iteratively, using the decoder's feedback which is taken into account via $P^{\tr{a}}_n(a)$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\gls{skr} and \cite{Shayovitz16,Kreimer18}}\label{Sec:Intra.vs.Raphaeli}

The \gls{skr} algorithm should be seen as a ``canonical'' representation of the algorithms shown in \cite{Shayovitz16,Kreimer18}: it relies on the Tikhonov distribution as suggested by \cite{Shayovitz16}, while the projections defined in \eqref{alpha.projection.3} and \eqref{beta.projection} are the essence of the algorithm proposed in \cite{Kreimer18}.

The differences with respect to \cite{Shayovitz16,Kreimer18} lie in the fact that the family $\mcF$ used in the \gls[skr} algorithm is composed of Tikhonov distributions and this stands in contrast with i) \cite{Kreimer18} which used the Gaussian family $\mcF$, and ii) with \cite{Shayovitz16} where $\mcF$ was a \emph{mixture} of  Tikhonov distributions.

These differences, although simple, lead to a certain ambiguity of implementation of the algorithm from  \cite{Shayovitz16,Kreimer18}. Namely, 
\begin{itemize}
\item Since $\mcF$ which is a \emph{mixture} of  Tikhonov distributions in  \cite{Shayovitz16}, the projection requires clustering of the elements of the mixture. This is computationally complex procedure even for moderate-size problems.\footnote{This is because even if the order of the reduced mixture is fixed to $L<M$ clusters, there is a formidably large number of possible assignments of $M$ elements into $L$ groups and it is usually unfeasible to test all possibilities} The heuristics are thus required and depend very much on the implementation details (such as, for example, enumeration order of the elements of the mixture or the thresholds used in the clustering). Further, despite the heuristics, a non-negligible complexity is required by the algorithms proposed in \cite{Shayovitz16}. In the follow-up work \cite{Kreimer18} (by the same author as in \cite{Shayovitz16}) the mixture was replaced by single (Gaussian) distribution.\footnote{We can only conjecture that this excessive complexity is the very reason why the author of \cite{Kreimer18} refrained from showing the results of his own algorithm developed in \cite{Shayovitz16} for large $M$. In fact, \cite{Kreimer18} says about  \cite{Shayovitz16}  ``However, good results for high order constellations require much higher complexity and were not demonstrated.''}
\item Since  \cite{Kreimer18} uses the Gaussian family $\mcF$, as we already mentioned, the approximations must start already when representing $g_n(\theta,a)$. In fact,  \cite{Kreimer18} describes with much details different strategies for such approximations but there is no unique answer to how this should be done.
\end{itemize}

In other words, the \gls{skr} algorithms uses the parts of  \cite{Shayovitz16,Kreimer18} which lead to a clear and unambiguous implementation. 

However, there is one remaining question. The \gls{skr} algorithm is a particular case of the algorithm shown in \cite{Shayovitz16} (obtained if we force the family $\mcF$ to contain one Tikhonov distribution, which is a sort of  ``degenerate'' mixture), so we want to understand why \cite{Shayovitz16} did not show the results of the \gls{skr} algorithm based on the Tikhonov family which would be a sound base for comparison with more sophisticated (and complicated) approaches based on Tikhonov mixtures which \emph{are} shown in \cite{Shayovitz16}.

We elucidate this issue in \secref{example.start} by implementing the \gls{skr} algorithm using the projection formulas derived in \cite[Appendix A]{Shayovitz16}. These formulas are based on series of approximations  and their last step, expressed in \cite[Eq.~(102)]{Shayovitz16} is based on an assumption that all terms of the mixture have a similar circular mean. This assumption, does not materialize in practice and leads to significant approximation error. Removing it and implementing the approximation step defined in \cite[Eq.~(101)]{Shayovitz16} yields the results similar to those obtained by the \gls{skr} algorithm we defined in this work. This  observation is anecdotical but confirms the importance of developing the projection formulas and indicating where the approximations start; this is the goal of \appref{Sec:CMM}.

%%%%%%%%%%%%%%%%%%%%%
\section{Expectation Propagation:\\Self-iterations in the phase-tracking}\label{Sec:It.EP}


As we will see in \secref{example.start}, the performance of one-shot phase-tracking of the \gls{dmp}, indicates that satisfactory solutions may be obtained without relying on the decoders' feedback. Therefore, our goal should be to develop a  reliable parametric one-shot phase tracking by exploiting the form of the constellation $\mcA$. While this is what \gls{skr} does, more projetions are required increasing the complexity comparing to the \gls{cbc} algorithm. 

Here, we abandon the intra-recursive projections of the \gls{skr} algorithm. Instead,  motivated by the extreme simplicity of the forward-backward \gls{mp} \eqref{z.alpha.init}-\eqref{z.beta} which amounts to the non-linear recursive filtering, we will follow the idea of the \gls{cbc} algorithm. Thus, rather than moving the projection inside the \gls{mp} recursion, we want to enhance the approximations $\tilde{\gamma}_n(\theta)$ and preserve the structure of the \gls{mp} \eqref{z.alpha.init}-\eqref{z.beta}.

To do this, we will improve $\tilde{\gamma}_n(\theta)$ iteratively; this will be done with ``self-iterations", that is without any help from the decoder: the priors $\hat{P}^\tr{a}(a)$ will not change during the self-iterations. 

To explain why this can be done we note that, although the phase tracking \gls{mp} is defined on the tree (graph) that is known to yield the optimal solution in one run (backward-forward processing),  this is only  true for the \gls{dmp} which tracks the entire (discretized) distributions. On the other hand, the \gls{mp} in the \gls{cbc} algorithm is based on approximated distribution $\tilde{\gamma}_n(\theta)$ and, therefore, such a guarantee of optimality does not exist.

We follow here the \gls{ep} idea \cite[Ch.~3.2]{Minka01} which addresses the very problem of using approximate distributions in the \gls{mp}. We will apply the projection $\mcF[\cd]$ many times (iteratively) taking into account the results obtained in previous iterations.  Since most of the resulting operations are almost identical to those we already defined in the \gls{cbc} algorithm, we will use the parenthesized superscript $^{(i)}$ to denote the variables/functions obtained in the $i$-th iteration, where $i=1,\ld, I_\tr{ep}$ and $I_\tr{ep}$ is the maximum number of \gls{ep} iterations.

%\subsection{Expectation Propagation for the Phase Tracking}\label{Sec:EP.Ph.Track}
The \gls{ep} applied to our problem relies on the following idea: in the iteration $i$,  we find the approximation $\tilde{\gamma}^{(i)}_n(\theta)$ using the distributions $\alpha^{(i-1)}_n(\theta)$ and $ \beta^{(i-1)}_n(\theta)$ calculated in the previous iteration. This is done by exploiting the posterior distributions of $\theta_n$ after the iteration $i-1$ which is a mixture given by
\begin{align}
\nonumber
\label{posterior.i-1}
f^{(i-1)}_n(\theta)\propto \gamma_n(\theta)\big(\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)\big).
\end{align}

Our objective is to find $\tilde{\gamma}^{(i)}_n(\theta)\in\mcF$ which generates the approximate posterior
\begin{align}
\nonumber
\label{posterior.i-1}
\tilde{f}^{(i-1,i)}_n(\theta)\propto \tilde\gamma^{(i)}_n(\theta)\big(\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)\big)
\end{align}
close to $f^{(i-1)}_n(\theta)$, that is, we require
\begin{align}
\nonumber
\tilde{\gamma}^{(i)}_n(\theta)\big(\alpha^{(i-1)}_n(\theta)&\beta^{(i-1)}_n(\theta)\big)\\
\label{equal.proba.approx}
&\approx
\gamma_n(\theta)\big(\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)\big).
\end{align}

To satisfy \eqref{equal.proba.approx} we apply the projection, $\mcF[\cd]$ to its both sides. Since the \gls{lhs} contains the three terms from the family  $\mcF$, it is not affected by the projection (remember, the product of the Tikhonov distributions is a also a Tikhonov distribution), we obtain
\begin{align}\label{equal.proba.approx.2}
\tilde{\gamma}^{(i)}_n(\theta)
&\propto
\frac{\mcF\Big[\gamma_n(\theta)\big(\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)\big)\Big]}
{\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)}.
\end{align}

Of course, for $i=1$, we deal with non-informative distributions $\alpha^{(0)}(\theta)\propto 1$ and $\beta^{(0)}(\theta)\propto 1$, which reduces \eqref{equal.proba.approx.2} to  $\tilde{\gamma}^{(1)}_n(\theta)=\mcF\big[ \gamma_n(\theta)\big]$; this is what was done in \secref{Sec:Parametric.MP}, \ie  $\tilde{\gamma}_n^{(1)}(\theta)$ is the same as $\tilde{\gamma}_n(\theta)$ obtained in \eqref{gamma.projection.first}.\footnote{Similarly, if we want to apply the projection operator, $\mcF[\cd]$, to each of the terms under multiplication in the numerator in \eqref{equal.proba.approx.2}, the result will be the same as the original \gls{cbc} algorithm: the projection  $\mcF\Big[\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)\Big]=\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)$ will cancel out with the denominator and iterative improvement will not be possible. This ``transparency" to the presence of $\alpha_n(\theta)$ and $\beta_n(\theta)$ is thus nothing but the conventional projection characteristic of the \gls{cbc} and here it is not useful, although it may provide satisfactory results in other context, \eg \cite{Vannucci20}.}

For $i>1$, the informative distributions, $\alpha^{(i-1)}_n(\theta)$ and $\beta^{(i-1)}_n(\theta)$ are available so we have to calculate the \gls{rhs} of \eqref{equal.proba.approx}
\begin{align}
%\nonumber
\gamma_n(\theta)\Big(\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)\Big)
\label{apost.theta.i1}
&=
%\ls{\sum_{a\in\mcA} \e^{\eta^{(i-1)}_{\Sigma,n}(a)} \mcT\big(\theta; z^{(i-1)}_{\Sigma,n}(a) \big)},\\
\sum_{a\in\mcA} \e^{\eta_{g,n}(a)} \mcT\big(\theta; z^{(i-1)}_{\Sigma,n}(a) \big),
\end{align}
where, $z_{\Sigma,n}^{(i-1)}(a)=z_{\alpha,n}^{(i-1)}+z_{\beta,n}^{(i-1)}+z_{g,n}(a)$; we see that  $z_{\Sigma,n}^{(1)}(a)$ is the same as \eqref{z.Sigma.n}.
%\begin{align}
%\label{eta.Sigma.n.i1}
%\eta^{(i-1)}_{\Sigma,n}(a)&=-\SNRrv |a|^2+\hat{P}^{\tr{a}}_n(a)\\%+ \hat{I}_0\big(|z^{(i-1)}_{\Sigma,n}(a)|\big)
%&=\hat{P}^{(i-1)}_n(a)+\hat{P}^{\tr{a}}(a)
%\end{align}

Using \eqref{apost.theta.i1} in the numerator of \eqref{equal.proba.approx.2} yields
\begin{align}\label{EP.iterations}
\tilde{\gamma}^{(i)}_n(\theta) 
&=\mcT(\theta; z^{(i)}_{\tilde{\gamma},n})\\
\label{EP.division}
&\propto \frac
{\mcF\Big[\sum_{a\in\mcA} \e^{\eta_{g,n} (a)} \mcT\big(\theta; z^{(i-1)}_{\Sigma,n}(a) \big)\Big] }
{\mcT\big(\theta; z^{(i-1)}_{\alpha,n}+z^{(i-1)}_{\beta,n} \big)}\\
\label{EP.division.2}
&= \frac{ \mcT\Big(\theta; z^{(i)}_{\tr{post},n}\Big)  }{ \mcT\Big(\theta; z^{(i-1)}_{\alpha,n}+z^{(i-1)}_{\beta,n} \Big)},
\end{align}
where 
\begin{align}
z^{(i)}_{\tr{post},n} &=\mf{CMM}\Big[ \set{\eta_{g,n}(a), z^{(i-1)}_{\Sigma,n}(a)}_{a\in\mcA}  \Big]
\end{align}
and thus
\begin{align}
\label{z.gamma.i}
z^{(i)}_{\tilde{\gamma},n}&= z^{(i)}_{\tr{post},n}  - \big(z^{(i-1)}_{\alpha,n} + z^{(i-1)}_{\beta,n}\big).
\end{align}

%%%%%%%%%%%%%%%
\subsection{Pitfalls  and solutions}\label{Sec:Pitfalls}
The elegant formulation of  the \gls{ep} is indeed appealing but occasionally runs into difficulty due to the division of the distributions in \eqref{EP.division.2}, or equivalently, due to subtraction of the coefficients in \eqref{z.gamma.i}. The existence of a similar problem has been acknowledged in \cite[Sec.~3.2]{Minka01} in the context of the Gaussian \gls{ep}, where the division of the distributions may yield a ``Gaussian'' with negative variance, see also \cite[Sec.~IV.B]{Senst11} \cite[Sec.~IV.A]{Cespedes14}. Such results are usually uninterpretable so a workaround is needed. 

In the context of the \gls{ep} based on Tikhonov distributions $\mcT(\theta;z)$ which are defined by complex parameters $z$, the purely numerical issue of invalid parameters (such as a negative variance in  the Gaussian case) is avoided but the problem remains. To understand intuitively its source and devise a solution, we may look at the scenario where the problems materialize. 

\begin{example}[Pitfalls of EP]\label{Ex:Pitfall}
Assume that 
\begin{itemize}
\item The circular means of the approximate posterior distribution, $\mcT\big(\theta; z^{(i)}_{\tr{post},n}\big) $ and of the ``extrinsic'' distribution (defined by  the product $\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)$) coincide, that is,  $\angle z^{(i)}_{\tr{post},n} =\angle (z^{(i-1)}_{\alpha,n}+z^{(i-1)}_{\beta,n})$; (remember, the phase $\angle z^{(i)}_{\tr{post},n}$ defines the circular mean); and that
\item The variance of the posterior distribution is larger than the variance of the extrinsic distribution, \ie $|z^{(i)}_{\tr{post},n}|<|z^{(i-1)}_{\alpha,n}+z^{(i-1)}_{\beta,n}|$; this may occur because the distribution in the argument of $\mcF[\cd]$ in \eqref{EP.division} is obtained multiplying  the extrinsic distribution $\mcT\big(\theta; z^{(i-1)}_{\alpha,n}+z^{(i-1)}_{\beta,n}\big)$ with a mixture $\gamma_n(\theta)$; the variance of the resulting mixture (and thus of its projection result as well) may be larger than the variance of the extrinsic distribution. 
\end{itemize}

Then, carrying out the subtraction in \eqref{z.gamma.i} we will obtain
\begin{align}
z^{(i)}_{\tilde{\gamma},n}
&= (|z^{(i)}_{\tr{post},n}|  - |z^{(i-1)}_{\alpha,n} + z^{(i-1)}_{\beta,n}|\big)\e^{\jj \angle z^{(i)}_{\tr{post},n}}\\
&=|z^{(i-1)}_{\tilde{\gamma},n}|\e^{\jj(\angle z^{(i)}_{\tr{post},n}+\pi)}.
\end{align}
That is, the circular mean of the new distribution $\mcT(\theta; z^{(i)}_{\tilde{\gamma},n})$ will be  in disagreement (by the largest possible value of $\pi$) with the mean of the posterior and extrinsic distributions obtained from the previous iteration. Such a results, being an artefact of the way the \gls{ep} is defined \cite[Sec.~3.2]{Minka01} is clearly counterintuitive and simply wrong. 
\end{example}

This problem, characteristic of the \gls{ep} will affect first $\tilde{\gamma}_n(\theta)$ and,  propagating via the \gls{mp}, will have detrimental affects on $\alpha_n(\theta)$ and $\beta_n(\theta)$.

Heuristics were devised for the Gaussian \gls{ep} where the problem is clearly identified, \ie the variance of the distributions after division becomes negative. For example, \cite[Sec.~3.2]{Minka01} constrains the variance to be positive, while other proposed to identify the problematic cases (\ie the negative variance) and then, if necessary i)~eliminate the division of the distributions \cite[Sec.~IV.B]{Senst11}, which here would mean $z^{(i)}_{\tilde{\gamma},n}=z^{(i)}_{\tr{post},n}$, or ii)~remove the update \cite[Sec.~IV.A]{Cespedes14}, \ie $z^{(i)}_{\tilde{\gamma},n}=z^{(i-1)}_{\tilde{\gamma},n}$. 

On the other hand, instead of testing for the compliance with our prior requirements (that are not necessarily obvious to define),  we might ``smooth'' the obtained parameters via recursive filter \cite[Sec.~IV.A]{Cespedes14} , which would mean  replacing \eqref{z.gamma.i} with
\begin{align}\nonumber
z_{\tilde{\gamma},n}^{(i)} = \zeta \Big(z^{(i)}_{\tr{post},n}  - z^{(i-1)}_{\alpha,n} - z^{(i-1)}_{\beta,n}\Big)
&+(1-\zeta) z_{\tilde{\gamma},n}^{(i-1)}\\
\label{z.smoothing}
& i=2,\ld, I_\tr{ep},
\end{align}
where the smoothing parameter, $\zeta<1$, must be chosen heuristically to strike a balance between the new solution and the history accumulated in the previous estimate. In this way we avoid rapid changes in the the parameters $z_{\tilde{\gamma},n}^{(i)}$, regularizing the final solution. Note that the smoothing is not necessary in the first iteration, $i=1$, which is based solely on the information obtained from the pilots (and from the decoder if we allows for it). 

We applied this smoothing solution in our numerical experiments, and found $\zeta\approx 0.4$ yielding satisfactory results. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
\subsection{Summary of the algorithm}\label{Sec:Summary}
The proposed \gls{ep} phase tracking algorithm is now summarized as Algorithm~\ref{Algo:EP} where for simplicity we defined the set of indices to the payload symbols and to the pilots as
\begin{align}
\Natural_{\tr{pilots}}&=\set{0,L,2L,\ld, FL}\\
\Natural_{\tr{payload}}&=\set{1,\ld, N} \setminus \Natural_{\tr{pilots}}.
\end{align}
We also integrated the notation so that the \gls{cbc} algorithm is naturally the first iteration ($i=1$) of the \gls{ep} algorithm, \ie $z^{(0)}_{\Sigma,n}(a)=z_{g,n}(a)$ . The main distinction we need to make is that the smoothing \eqref{z.smoothing} is not applied for $i=1$, see lines \ref{i.if}--\ref{i.endif} of the algorithm. Note that the notation with the iteration index $^{(i)}$ may be removed (and the in-place calculation carried out) but we kept it for compatibility with the equations in the paper.

Last but not least, and at the risk of stating the obvious, we want to emphasize what the \gls{ep} algorithm is \emph{not} doing. Namely, it is not reusing the output ``extrinsic'' log-probabilities $\hat{P}_n(a)$ as if they were newly calculated prior log-probabilities $\hat{P}^{\tr{a}}_n(a)$. This is clearly seen in the description of the algorithm: the prior probability $\hat{P}^{\tr{a}}_n(a)$ affects the weighting factors $\eta_{g,n}(a)$ in line \ref{eta.gn.a} which remain unaltered throughout the \gls{ep} iterations; the \gls{ep} algorithm rather changes the parameters of the Tikhnov distributions $z^{(i)}_{\Sigma,n}(a)$.


% ------------------------------- algorithm -----------------------
\begin{algorithm}
    \caption{EP phase tracking} \label{Algo:EP}
\begin{algorithmic}[1]
\State Inputs:
\State $y_n, n\in\set{0,\ld,N}$ \Comment Received signal 
\State $x_n, n\in\Natural_{\tr{pilots}}$  \Comment Pilot symbols
\State $\hat{P}^{\tr{a}}_n(a)$\Comment Log-probabilities from the decoder
\State Initialization:
\State $z^{(i)}_{\tilde{\gamma},n}\gets 2\SNRrv~ y_n x_n^*,   \quad  n\in \Natural_{\tr{pilots}}, i\in{1,\ld, I_\tr{ep}}$\label{z.i.tilde.pilot}
\State $\eta_{g,n}(a) \gets -\SNRrv~|a|^2+\hat{P}^{\tr{a}}_n(a),\quad a\in\mcA, n\in\Natural_{\tr{payload}}$\label{eta.gn.a}
\State $z_{g,n}(a)\gets 2\SNRrv~y_n a^*,\quad a\in\mcA, n\in\Natural_{\tr{payload}}$\label{z.g.n.payload}
\State $z_{\Sigma,n}^{(0)}(a) \gets z_{g,n}(a), \quad n\in\Natural_{\tr{payload}}$
\State EP iterations:
\For{ $i\gets1,\ld, I_\tr{ep}$ }
	\State Pre-MP : Finds $\tilde{\gamma}^{(i)}_n(\theta)$
	\For {$n\gets \Natural_{\tr{payload}}$} 
		%\State $\eta^{(i-1)}_{\Sigma,n}(a) \gets -\frac{|a|^2}{\No}+ \hat{I}_0\big(|z^{(i-1)}_{\Sigma,n}(a)|\big)+\hat{P}^{\tr{a}}_n(a)$ \label{eta.Sigma.n}
		\State $z^{(i)}_{\tr{post},n}  \gets \mf{CMM}\Big[ \eta_{g,n}(a), \set{z^{(i-1)}_{\Sigma,n}(a)}_{a\in\mcA}  \Big]$
	\If {$i=1$} \label{i.if}
		\State $z^{(i)}_{\tilde{\gamma},n}\gets z^{(i)}_{\tr{post},n}$%  - z^{(i-1)}_{\alpha,n} - z^{(i-1)}_{\beta,n}$
	\Else
		\State $z_{\tilde{\gamma},n}^{(i)} \gets \zeta \Big(z^{(i)}_{\tr{post},n}  - z^{(i-1)}_{\alpha,n} - z^{(i-1)}_{\beta,n}\Big)$
		\State \qquad~ \qquad  ~ \qquad~ \qquad~ \qquad$+(1-\zeta) z_{\tilde{\gamma},n}^{(i-1)}$
	\EndIf  \label{i.endif}
	\EndFor
	\State MP recursive calculation:
	\State $z^{(i)}_{\alpha,0}\gets 0$	
	\For {$n\gets 1,\ld,N$} \Comment Finds $\alpha^{(i)}_n(\theta)$:
		\State $z^{(i)}_{\alpha,n} \gets \frac{z^{(i)}_{\alpha,n-1} + z^{(i)}_{\tilde{\gamma},n-1}}{1+\big|z^{(i)}_{\alpha,n-1} + z^{(i)}_{\tilde{\gamma},n-1}\big|\sigma_w^2}$
	\EndFor
   	\State $z^{(i)}_{\beta,N} \gets 0$
	\For {$n\gets N-1,\ld,0$} \Comment Finds $\beta^{(i)}_n(\theta)$:
		\State $z^{(i)}_{\beta,n} \gets  \frac{z^{(i)}_{\beta,n+1} + z^{(i)}_{\tilde{\gamma},n+1}}{1+\big|z^{(i)}_{\beta,n+1} + z^{(i)}_{\tilde{\gamma},n+1}\big|\sigma_w^2}$
	\EndFor
	\For {$n\gets \Natural_{\tr{payload}}$} %\Comment Prepare outputs
	\State $z^{(i)}_{\Sigma,n} \gets  z_{g,n}(a) +z^{(i)}_{\alpha,n}+ z^{(i)}_{\beta,n}$
	\EndFor
\EndFor % i
\State Output: log-probabilities to be used in \eqref{lambda.n.l}
\For {$n \gets \Natural_{\tr{payload}}$}
\State $\hat{P}_{n}( a ) \gets -\SNRrv |a|^2 + \hat{I}_0\big(|z^{(I_{\tr{ep}})}_{\Sigma,n}(a)|\big)$\label{P.n.a}
\EndFor
\end{algorithmic}
\end{algorithm}
% ------------------------------- end algorithm -------------------


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Numerical results}\label{example.start}

We considers transmission based on $16$-\gls{qam} constellation with Gray mapping \cite[Sec.~2.5.2]{Szczecinski_Alvarado_book}; the proprietary \gls{ldpc} encoder with the rate $r=\frac{7}{8}$ produces the block of $\Nc=4032$ bits. The pilot symbols are pseudo-randomly drawn from a $4$-\gls{qam} constellation; the pilot spacing is set to $L\in\set{17,25}$ which allows us to place $L-1\in\set{16,24}$ payload symbols between pilots, see \eqref{payload.1}, so dummy symbols are not needed to fill the frame of transmitted symbols $\set{x_n}$.\footnote{Instead of changing the pilot spacing, $L$, we might use a different coding rate $r$, change the phase-noise level $\sigma_w^2$, the constellation size $M$, or any combination of those. But changing these  parameters amounts to finding the scenarios in which the effect of the phase noise is more or less important.}  With this setting we thus have $F\in\set{64,43}$ pilots and total $N\in\set{1072,1051}$ symbols. The phase noise is generated with $\sigma_w^2=0.01~\tr{rad}^2$ or--equivalently, $\sigma_w=0.1~\tr{rad}\approx 5.7~\tr{deg}$. 

The demodulation/phase-tracking algorithms which use the decoder's feedback are referred to as ``iterative'' and those which don't -- as ``one shot" algorithms. \ls{Unless stated otherwise} in the iterative algorithms we deliberately limit our considerations to a particular form of scheduling of operations between the demodulator and the decoder: each demodulation operation is followed by one decoding iteration (where, the \gls{ep} phase tracking is iterative in itself). This is not necessarily the best solution but was extensively used in the literature, \eg \cite{Colavolpe05,Shayovitz16,Kreimer18} and thus constitues a well-accepted basis for comparison. The decoder's state (captured by the internal messages from the check to variables nodes) is preserved between iterations. 

The decoding is based on the min-sum algorithm\footnote{With scaling of the check-nodes messages by a constant factor equal to $\rho=0.7$, see \cite{Xu14}; then, a fraction of dB loss was observed when comparing to the sum-product algorithm in the \gls{awgn} channel.}  and, irrespectively of the scheduling, the total number of decoding iterations equals $I_\tr{dec}=10$. This means that the iterative receivers has to run the demodulation/phase tracking  $I_\tr{dec}$ times.

The \gls{dmp} is implemented using $N_\theta=64$ samples\footnote{\label{foot:DMP32}The numerical results obtained for $N_\theta\in\set{32,64,128}$ were practically indistinguishable while a significant deterioration of the results was observed for $N_\theta=16$. This indicates that the heuristics  $N_\theta=8M$ used \eg in \cite{Peleg00,Colavolpe05,Kreimer18}, may be too conservative but this issue is out of scope here.} and its \gls{per} curve is the performance limit for all  phase tracking algorithms.

The ``AWGN'' curve corresponds to a hypothetical scenario when the phase-noise is removed and we only deal with the \gls{awgn}. Such results are unattainable no matter how sophisticated the phase-tracking and decoding strategy are, and we show them to illustrate the impact of the phase noise.

As a reference  for the iterative receivers we use the curve ``All-pilots''. It is obtained assuming that, during the phase-tracking, all the symbols in $\set{x_n}$ are pilots. This corresponds to a hypothetical situation when the output of the decoder provides highly reliable information about the bits which gives certainty about the symbols $\bx$ (that is, $P^{\tr{a}}_n(a)\approx 1$ for $a=x_n$); these, in turn, become de facto pilots allowing for the best possible phase tracking.  

Then, when calculating $\hat{P}_n(a)$, the only uncertainty about the symbol $x_n$ is caused by the \gls{awgn} as well as  by the residual phase noise -- this part of it which cannot be estimated from other symbols $x_l, l\neq n$. The ``All-pilots" curve is a performance limit for all joint phase-tracking and demodulation/decoding algorithms we study here.\footnote{More precisely, for all those algorithms which do not use the decoder's feedback in the \gls{llr} calculation in \eqref{lambda.n.l}; see comments at the end of \secref{sec:model}.} If the iterative \gls{dmp} is too complex to implement, the ``All-pilots" curve may be treated as its proxy. ``All-pilots'' results are the virtually the same irrespectively of the pilot spacing $L$.


The \acrfull{per} is estimated after transmitting $10^5$ blocks or after occurence of $100$ blocks in error, whichever comes first. %Thus, below $10^{-4}$ the \gls{per}  cannot be considered a reliable estimate but some tendency may be deduced even from these results -- mainly about the error floor.


%%%%%%%%%%%%%%
\begin{figure}[bt]
\begin{center}
\psfrag{DMPXXXX}[lc][lc][\siz]{DMP}
\psfrag{EP2-02}[lc][lc][\siz]{EP $\zeta=0.2$}
\psfrag{EP2-04}[lc][lc][\siz]{EP $\zeta=0.4$}
\psfrag{EP2-06}[lc][lc][\siz]{EP $\zeta=0.6$}
\psfrag{EP2-08}[lc][lc][\siz]{EP $\zeta=0.8$}
\psfrag{EP2-10}[lc][lc][\siz]{EP, $\zeta=1.0$}
\psfrag{ylabel}[lc][lc][\siz]{$\PER$}
\psfrag{xlabel}[lc][lc][\siz]{$\SNRrv$ [dB]}
\scalebox{\sizf}{\includegraphics[width=\linewidth]{./figures/PER_EP_OneShot_Rev.eps}}
\end{center}
\caption{\gls{per} vs. \gls{snr} for one-shot \gls{ep} phase tracking algorithms with $I_\tr{ep}=2$ (solid lines) and $I_\tr{ep}=3$ (dashed-dotted lines),  and different values or the smoothing parameter $\zeta$. The thick lines indicate the results obtained for \mbox{$\zeta=0.4$} which is retained for further analysis.}\label{fig:PER.EP.OneShot}
\end{figure}
%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{One-shot receivers}
We analyze first non-iterative receivers which means that the \gls{mp} phase tracking algorithm is run only once and has no prior information about the symbols, \ie $\hat{P}^{\tr{a}}_n(a)\propto 0$. In the case of the \gls{cbc} algorithm, it means that the phase reference for all the symbols is obtained using only the pilots.

We start showing in \figref{fig:PER.EP.OneShot} the results produced by the \gls{ep} algorithm with different values of the smoothing parameter $\zeta$ used in \eqref{z.smoothing}. The best performance is obtained for $\zeta=0.4$ which will be used in all the remaining examples. This result confirm the existence of the problems we delineated in \secref{Sec:Pitfalls} and, since it produces erroneous estimation of the phase distribution, it is what \cite{Shayovitz16} calls a ``phase-slip''. We discuss this concept in \secref{Sec:Phase.slip}.

%%%%%%%%%%%%%%
\begin{figure}[bt]
\begin{center}
\psfrag{DMPXXX}[lc][lc][\siz]{DMP}
\psfrag{CBC}[lc][lc][\siz]{CBC}
\psfrag{AWGN}[lc][lc][\siz]{AWGN}
\psfrag{Intra-MP}[lc][lc][\siz]{\gls{skr}}
\psfrag{Intra-Sh}[lc][lc][\siz]{\gls{skr}+\cite{Shayovitz16}}
\psfrag{EP2}[lc][lc][\siz]{EP, $I_\tr{ep}=2$}
\psfrag{EP3}[lc][lc][\siz]{EP, $I_\tr{ep}=3$}
\psfrag{ylabel}[lc][lc][\siz]{$\PER$}
\psfrag{xlabel}[lc][lc][\siz]{$\SNRrv$ [dB]}
\scalebox{\sizf}{\includegraphics[width=\linewidth]{./figures/PER_Tikh_OneShot_Rev.eps}}
\end{center}
\caption{\gls{per} vs. \gls{snr} for one-shot phase tracking algorithms; two pilot spacings $L=17$ (dashed) and $L=25$ (solid), are considered. The  ``AWGN" curve assumes no phase noise. The results ``\gls{skr}+\cite{Shayovitz16}''  correspond to the \gls{skr} algorithm based on the \gls{cmm} defined by \cite[Eq.~(102)]{Shayovitz16}.}\label{fig:PER.OneShot}
\end{figure}
%%%%%%%%%%%%%%

The results of the \gls{dmp}, \gls{cbc}, \gls{skr} and \gls{ep} are shown in \figref{fig:PER.OneShot} where we observe that 
\begin{enumerate}
\item The performance decreases notoriously with the increased pilot spacing for all the algorithm but for the \gls{dmp}, where the effect is much less notable. This suggests that the projection on $\mcF$ is the principal source of degradation of the parametric phase tracking algorithm.

\item The \gls{per} curves show a tendency to display the error floor in high \gls{snr} (increasing the \gls{snr} yields small \gls{per} gains) where the phase noise is a dominating distortion.\footnote{No error floor is observed for the \gls{dmp} due to the limitation of the simulations we can carry out.} This effect is especially notable for a large pilot spacing, $L=25$. This was expected but the reasons behind the error floor are not exactly the same in all algorithms. In particular
\begin{itemize}
\item In the one-shot \gls{cbc}, the mixture reduction for the payload symbols is trivial (\ie $z_{\tilde{\gamma},n}=0$) so the uncertainty about the phase depends only on the pilots. 
\item  The mixture reduction in the \gls{skr} and the \gls{ep} algorithms relies on non-trivial operations based on  the \gls{cmm}
which are prone to errors: the projection may over-emphasize one of the components $g_n(\theta,a)$ which does not represent the actual phase distribution (that is, when the component $g_n(\theta,a)$ dominating the mixture is the one with $a\neq x_n$); this is the phase-slip phenomenon, we already mentioned.
\end{itemize}

 
This algorithmic phase-slip phenomenon also explains why the \gls{skr} algorithm which, at each time $n$, exploits the form of the constellation $\mcA$, may be outperformed (for $L=17$ in \figref{fig:PER.OneShot}) by the \gls{cbc} algorithm which is merely based on the pilots and ignores the form of $\mcA$. In fact, this very dependence on the pilots \emph{only} is the source of robustness of the \gls{cbc} algorithm: that eventual discrepancy between the estimated phase distribution and the actual one is only tributary to the noise at the pilots.

\item 
The one-shot \gls{ep} algorithm outperform notably the \gls{skr} phase-tracking closing gap to the \gls{dmp}. The performance is particularly impressive  for $L=17$ where in the displayed range of the \gls{per} the gap to the \gls{dmp} is smaller than $0.5$dB. Again, the reason for the difference between the \gls{skr} and \gls{ep} algorithms should be sought in their different propensity to phase-slip phenomenon, which may be due to the following:
\begin{itemize}
\item In the \gls{ep} algorithm, at the iteration $i$, the projection of $\gamma_n(\theta)$ on $\mcF$ relies \emph{both} on $\alpha^{(i-1)}(\theta)$ and on $\beta^{(i-1)}_n(\theta)$, see \eqref{equal.proba.approx.2}. On the other hand, the \gls{skr} performs a projection to obtain $\alpha_n(\theta)$ (or $\beta_n(\theta)$), but uses only the previously calculated message $\alpha_{n-1}(\theta)$ (or $\beta_{n+1}(\theta)$), see \eqref{z.alpha.check} and \eqref{z.beta.check}, and \emph{does not use} any of the messages  $\beta_{n}(\theta)$ (or $\alpha_n(\theta)$). Thus, the \gls{ep} algorithm uses a more ``complete'' information which increases its robustness to phase-slip.

\item In the \gls{skr} algorithm, any phase slip in $\alpha_{n-1}(\theta)$  will affect (propagate to) $\alpha_{n}(\theta)$ and  $\alpha_{n+1}(\theta)$, etc. (the same reasoning applies to the messages $\beta_n(\theta)$). In contrast, the \gls{ep} algorithm finds the projections $\tilde\gamma^{(i)}_n(\theta)$ independently for all $n$. Of course, there is some dependence between the projections because they are based on the same estimates $\alpha^{(i-1)}_n(\theta)$ and $\beta^{(i-1)}_n(\theta)$ obtained in the previous iteration but it does not lead to the propagation of the errors which must  happen in the \gls{skr} algorithm. 
\end{itemize}

\item 
The results obtained using the \gls{skr} algorithm but where the \gls{cmm} is implemented using the formulas from \cite[Appendix A]{Shayovitz16} indicate that  \cite[Eq.~(102)]{Shayovitz16} should be avoided. On the other hand, the approximation  \cite[Eq.~(101)]{Shayovitz16} produces results equivalent to the algorihtm \gls{skr} we show.
\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Phase-slip effect}\label{Sec:Phase.slip}

%%%%%%%%%%%%%%
\begin{figure}[bt]
\begin{center}
\psfrag{DMPXXXX.XXXX.XXXX}[lc][lc][\siz]{DMP}
\psfrag{CBC}[lc][lc][\siz]{CBC [$\delta_n=0.43$]}
\psfrag{SKR}[lc][lc][\siz]{\gls{skr} [$\delta_n=0.58$]}
\psfrag{EP2}[lc][lc][\siz]{EP, $I_\tr{ep}=2$ [$\delta_n=0.05$]}
\psfrag{EP3}[lc][lc][\siz]{EP, $I_\tr{ep}=3$ [$\delta_n=4\!\cd\!10^{-4}$]}
\psfrag{xlabel}[lc][lc][\siz]{$\theta_n$}
\psfrag{ylabel}[lc][lc][\siz]{$f(\theta_n)$}
\scalebox{\sizf}{\includegraphics[width=\linewidth]{./figures/PDF_Rev.eps}}
\end{center}
\caption{Example of the \gls{pdf}s obtained using one-shot phase tracking algorithms and $L=25$. The values of the \gls{kl} divergence \eqref{DKL} obtained for each of the \gls{pdf} are shown in brackets; the true value of the phase noise, $\theta_n\approx0.12$, is indicated by the position of the black circle on the axis of $\theta$.}\label{fig:PhaseSlip}
\end{figure}
%%%%%%%%%%%%%%

It is interesting to obtain further insight into the very concept of the phase-slip considering the probabilistic models we use. To illustrate the difficulty of grasping this idea, we show in \figref{fig:PhaseSlip} an example of the \gls{pdf}s 
\begin{align}
\nonumber
f^{\tr{Alg}}(\theta_n)&\propto \alpha_n(\theta)\beta_n(\theta)\\
&\propto f^{\tr{Alg}}(\theta_n|y_0,\ld,y_{n-1},y_{n+1},\ld,y_N)
\end{aling}
obtained using different phase tracking algorithms \mbox{$\tr{Alg}\in\set{\tr{DMP},\tr{CBC},\tr{EP},\tr{SKR}}$}. 

We also show the true value of the phase $\theta_n\approx0.12$ (a black circle on the axis) and,  
at first sight, it may seem that the \gls{pdf} of the \gls{skr} algorithm provides the more accurate estimation than the \gls{pdf} of the \gls{cbc} algorithm: $\pdf^{\tr{SKR}}(\theta_n)>\pdf^{\tr{CBC}}(\theta_n)$. However, such simplified analysis\footnote{Analysis which is equivalent to the evaluation of the mean square estimation error: if we approximate the \gls{pdf} by a Gaussian, then $\log\pdf^{\tr{Alg}}(\theta_n)\propto -|\theta_n-\mu_n |^2$, where $\mu_n=\angle ( z^\tr{Alg}_{\alpha,n}+z^\tr{Alg}_{\beta,n})$ is the point-estimate of the phase obtained using the phase tracking ``Alg".} misses the fact that the ``exactl'' \gls{pdf} is represented by the \gls{dmp} curve.

%%% DKL
We can thus calculate the \gls{kl} distance between to the exact distribution provided by the \gls{dmp},  algorithm, $f^\tr{DMP}_n(\theta)$, and the \gls{pdf} estimated using the given phase-tracking algorithm 
\begin{align}\label{DKL}
\delta^{\tr{Alg}}_n = \int f^\tr{DMP}_n(\theta)\log\frac{f^\tr{DMP}_n(\theta)}{f^{\tr{Alg}}_n(\theta)} \dd \theta.
\end{align}

Following with the example shown in \figref{fig:PhaseSlip}, the value of $\delta^{\tr{Alg}}_n$ is shown in the legend indicating that the \gls{pdf}s obtained via \gls{skr} is actually slightly worse (in the sense of the \gls{kl} distance) that the \gls{pdf} provided by the \gls{cbc} algorithms. This is, of course, just an example shown for a particular realization of the data so,  to obtain a better insight into the phase tracking results, we find the average \gls{kl} distance 
\begin{align}\label{av.DKL}
\Delta^{\tr{Alg}} = \frac{1}{\Ns}\sum_{n\in\Natural_{\tr{payload}}} \delta^{\tr{Alg}}_{n},
\end{align}
and next, via simulations we obtain the empirical distribution of $\Delta^{\tr{Alg}}$ which is shown in \figref{fig:PDP.DKL}.


%%%%%%%%%%%%%%
\begin{figure}[bt]
\begin{center}
\psfrag{CBC.XXX}[lc][lc][\siz]{CBC}
\psfrag{SKR}[lc][lc][\siz]{SKR}
\psfrag{EP2}[lc][lc][\siz]{EP, $I_\tr{ep}=2$}
\psfrag{EP3}[lc][lc][\siz]{EP, $I_\tr{ep}=3$}
\psfrag{xlabel}[lc][lc][\siz]{$\Delta$}
\psfrag{ylabel}[lc][lc][\siz]{$f(\Delta)$}
\scalebox{\sizf}{\includegraphics[width=\linewidth]{./figures/PDF_DKL_L25_SNR=20_Rev.eps}}
\end{center}
\caption{Empirical \gls{pdf}s of the average \gls{kl} distance \eqref{av.DKL} obtained using one-shot phase tracking algorithms; $L=25$, $\SNRrv=20$dB.}\label{fig:PDP.DKL}
\end{figure}
%%%%%%%%%%%%%%

This example illustrates the propensity of the algorithms to produce a phase-slip: while, the algorithm \gls{skr} is very likely to yield small values of $\Delta$,  it also displays the heavy tail so it is more likely to produce large deviation of the phase estimation than does the \gls{ep} algorithm. 

We also note that the same phenomenon happens for \gls{ep} algorithm, when we change $I_\tr{ep}=2$ to $I_\tr{ep}=3$, which may be related to the fact that the performance of the \gls{ep} algorithm is better (for \gls{snr} larger than $16$dB) when $I_\tr{ep}=2$ is used rather than $I_\tr{ep}=3$.

While the qualitative behaviour of the propensity to the phase-slip may be evaluated from the \gls{kl} distance distribution shown in \figref{fig:PDP.DKL}, it does not lead to a \emph{quantitative} assessment of its impact taking into account the transmission parameters defined by the modulation type and the coding rate. 

In fact, the relationship between the phase estimation accuracy and the decoding errors is difficult to evaluate. However, noting that the \gls{pdf} estimation errors must translate into errors of the \glspl{llr},  we propose to calculate here the \gls{gmi} \cite[(4.90)]{Szczecinski_Alvarado_book}, \cite{Alvarado15}
\begin{align}\label{GMI}
\mf{GMI} \approx 1- \min_{s}\frac{1}{\Nc}\sum_{k=1}^m\sum_{n=1}^{\Ns}\log_2\big(1+\e^{s\lambda_{n,k}(1-2c_{n,k})}\big),
\end{align}
where $\lambda_{n,k}$ are the \glspl{llr} given by \eqref{lambda.n.l}. The minimization over $s$ is requires since, in general, the \glspl{llr} are not correctly calculated and thus we deal with the so-called mismatched decoding: here, this happens due to the errors in the estimation of the \gls{pdf} $\pdf(\theta_n)$.\footnote{The minimization yields $\mf{GMI}=1$ if all the terms $\lambda_{n,k}(1-2c_{n,k})$ are negative; this simply means that if all bits $c_{n,k}$ can be estimated without errors before decoding, the decoding errors is unlikely.}  

The \gls{gmi} should be interpreted as the achievable transmission rate  based on the \glspl{llr} $\lambda_{n,k}$ assuming infinite-length coding/decoding \cite[Sec.~4.3.1]{Szczecinski_Alvarado_book}. More interestingly, this metric allows us to predict reliably the performance of the practical encoders/decoders \cite[Sec.~IV]{Alvarado15} with the main idea being that the decoder's performance may be uniquely defined using the \gls{gmi} which summarizes the behaviour of any demodulation scheme.  The \gls{per} curve of the decoder, $\PER^\tr{dec}(\mf{GMI})$ may be thus obtained independently of a particular processing at the demodulator, and here, we obtain it from the transmission without phase noise and the 4-\gls{qam} modulation.

Since, in the finite-length coding regime, the \gls{gmi} depends on the realizations of the signals, we treat it as a random variable and the \gls{per} has to be estimated by averaging 
\begin{align}
\PER &=\int \pdf(\mf{GMI}) \PER^\tr{dec}(\mf{GMI}) \dd \mf{GMI}\\
&\approx \cdf(\mf{GMI}_\tr{th}),
\end{align}
where $\mf{GMI}_\tr{th}$ is the decoding threshold and $\cdf(\mf{GMI})$ is the empirical \gls{cdf} of the \gls{gmi} which is shown in \figref{fig:PDP.GMI} for different phase tracking algorithms; the decoding curve $\PER^\tr{dec}(\mf{GMI})$ is also shown. 

The decoding threshold, defined as $\mf{GMI}_\tr{th}=\argmin_\mf{GMI} \set{\PER^\tr{dec}(\mf{GMI})>0.9}$ is indicated therein with a dashed line. In other words, the value of the empirical \gls{cdf} calculated at the \gls{gmi} threshold, $\cdf(\mf{GMI}_\tr{th})$, predicts the performance of the entire transmission scheme. Here we observe that $\mf{GMI}_\tr{th}\approx 0.91$ and the difference $\mf{GMI}_\tr{th}-r\approx 0.035$ is the \gls{gmi} penalty due to imperfect encoding/decoding.


 %%%%%%%%%%%%%%
\begin{figure}[bt]
\begin{center}
\psfrag{CBC.XXX}[lc][lc][\siz]{CBC}
\psfrag{SKR}[lc][lc][\siz]{SKR}
\psfrag{EP2}[lc][lc][\siz]{EP, $I_\tr{ep}=2$}
\psfrag{EP3}[lc][lc][\siz]{EP, $I_\tr{ep}=3$}
\psfrag{xlabel}[lc][lc][\siz]{$1-\mf{GMI}$}
\psfrag{ylabel}[cc][cc][\siz]{$\cdf(\mf{GMI})$, $\PER^\tr{dec}(\mf{GMI})$}
\begin{tabular}{c}
\scalebox{\sizf}{\includegraphics[width=\linewidth]{./figures/PDF_GMI_L25_SNR=16_Rev.eps}}\\
a)  \\
~\\
\scalebox{\sizf}{\includegraphics[width=\linewidth]{./figures/PDF_GMI_L17_SNR=18_Rev.eps}}
~\\
b)\\
\end{tabular}
\end{center}
\caption{Empirical \gls{cdf}s of the \gls{gmi} \eqref{GMI} obtained using one-shot phase tracking algorithms for a) $L=25$ and $\SNRrv=16$dB; b) $L=17$ and $\SNRrv=18$dB.}\label{fig:PDP.GMI}
\end{figure}
%%%%%%%%%%%%%%

The examples  in \figref{fig:PDP.GMI} are chosen to provide explanation of the results from \figref{fig:PER.OneShot}. In particular in \figref{fig:PDP.GMI}a shows that the \gls{cdf}s of the \gls{ep} algorithms with $I_\tr{ep}=2$ and $I_\tr{ep}=3$ cross close to the \gls{gmi} threshold; this should be seen as the equivalent performance in terms of the \gls{per} for $\SNRrv=16$dB. This is, indeed, the case as observed in \figref{fig:PER.OneShot} ($L=25$). Similarly, \figref{fig:PDP.GMI}b  result indicates that the performance of the algorithms \gls{cbc}  and \gls{skr} should be similar for $L=17$ and $\SNRrv=18$dB which, again, can be read from \figref{fig:PER.OneShot}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Iterative receivers}
%%%%%%%%%%%%%%
\begin{figure}[bt]
\begin{center}
\psfrag{DMP-T}[lc][lc][\siz]{DMP}
\psfrag{DMP10XXX.XXX.X}[lc][lc][\siz]{DMP one-shot}
\psfrag{CBC1S}[lc][lc][\siz]{CBC one-shot}
\psfrag{CBC+GA}[lc][lc][\siz]{CBC+GA \cite{Colavolpe05}}
\psfrag{CBC+CMM}[lc][lc][\siz]{CBC+CMM}
%\psfrag{AWGN}[lc][lc][\siz]{AWGN}
\psfrag{All-pilots}[lc][lc][\siz]{All-pilots}
\psfrag{\gls{skr}}[lc][lc][\siz]{\gls{skr}}
\psfrag{EP2}[lc][lc][\siz]{EP, $I_\tr{ep}=2$}
\psfrag{EP3}[lc][lc][\siz]{EP, $I_\tr{ep}=3$}
\psfrag{ylabel}[lc][lc][\siz]{$\PER$}
\psfrag{xlabel}[lc][lc][\siz]{$\SNRrv$ [dB]}
\scalebox{\sizf}{\includegraphics[width=\linewidth]{./figures/PER_Tikh_CBC_turbo_Rev.eps}}
\end{center}
\caption{Performance of the \gls{cbc} algorithm with two different projection methods: the \acrfull{ga} and the \acrfull{cmm}; the one-shot \gls{cbc} algorithm is also shown for reference; two pilot spacings $L=17$ (dashed) and $L=25$ (solid), are considered. The  ``All pilots'' curve is the performance limits for any joint phase tracking and decoding.}\label{fig:PER.Iterative.CBC}
\end{figure}
%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Closer look at the \gls{cbc} algorithm}
We start with a short analysis of the results obtained using the canonical \gls{cbc} algorithm. They are shown in \figref{fig:PER.Iterative.CBC}, where two ways of carrying out the projection are considered: the \gls{ga} (results denoted by \gls{cbc}+\gls{ga}) and the \gls{cmm} (\gls{cbc}+\gls{cmm}).

While the  difference between the \gls{cbc}+\gls{ga} and the \gls{cbc}+\gls{cmm} algorithms is well notable (which indicates the importance of the approximations/projection we make in the phase tracking), the qualitative behaviour of the \gls{cbc} algorithms is the same and the gap to the \gls{dmp} remains large. More importantly, the error floor appears in the \gls{per} curve which was already observed, \eg in \cite[Fig.~8]{Kreimer18}.

Unlike in the one-shot algorithms we discussed before, where the error floor was due to the phase slip or the uncertainty of the phase estimation, here, the appearance of the error floor is of a different nature and can be understood rather by analyzing the way the demodulator and the decoder exchange information. 

To this end we show in \figref{} the \gls{exit} charts of the demodulator and the decoder; this is a well-known visualization tool \cite{Brink01} providing an intuitive insight into the results of the iterative algorithms. Namely, the \gls{exit} charts assumes that the messages (the \glspl{llr}) exchanged beween the decoder and the demodulator may be characterized by a single parameter: the mutual information between the \glspl{llr}, $\set{\lambda_{n,k}}$, see \eqref{lambda.n.l}, and the coded bits, $\set{c_{n,k}}$. We can thus characterize the modulator and the decoder by their own \gls{exit} transfer functions and, in the iterative process the output of one becomes the input to the another. In this way, the iterative process can be though of as an trajectory bounded by the \gls{exit} functions, and the intersection of the functions indicates the convergence.

To understand this 
 The original \gls{cbc} algorithm from \cite{Colavolpe05} (CBC+GA) tends to saturate for high \gls{snr}, \ie where the phase noise dominates the \gls{awgn}. We attribute this behaviour, observed already \eg in \cite[Fig.~8]{Kreimer18}, to the particular form of scheduling, where, after each decoding iteration, $\tilde{\gamma}_n(\theta)$ is estimated afresh even if the first decoding iterations do not provide reliable estimates of the coded bits. This, in turn, may yield unreliable $\hat{P}^\tr{a}(a)$, hence unreliable $\tilde{\gamma}_n(\theta)$ which, in turn stalls the convergence. 



%%%%%%%%%%%%%%
\begin{figure}[bt]
\begin{center}
\psfrag{DMP-T}[lc][lc][\siz]{DMP}
\psfrag{DMP10XXX.XXX.X}[lc][lc][\siz]{DMP one-shot}
%\psfrag{AWGN}[lc][lc][\siz]{AWGN}
\psfrag{All-pilots}[lc][lc][\siz]{All-pilots}
\psfrag{Intra-MP}[lc][lc][\siz]{\gls{skr}}
\psfrag{EP2}[lc][lc][\siz]{EP, $I_\tr{ep}=2$}
\psfrag{EP3}[lc][lc][\siz]{EP, $I_\tr{ep}=3$}
\psfrag{ylabel}[lc][lc][\siz]{$\PER$}
\psfrag{xlabel}[lc][lc][\siz]{$\SNRrv$ [dB]}
\scalebox{\sizf}{\includegraphics[width=\linewidth]{./figures/PER_Tikh_turbo_Rev.eps}}
\end{center}
\caption{Performance of the iterative phase tracking algorithms: \acrfull{ep} (\secref{Sec:It.EP}) and \acrfull{skr} (\secref{Sec:Intra-MP}); two pilot spacings $L=17$ (dashed) and $L=25$ (solid), are considered. The  ``All pilots'' curve is the performance limits for any joint phase tracking and decoding.}\label{fig:PER.Iterative.all}
\end{figure}
%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{\gls{ep} and \gls{skr} }

We compare the iterative \gls{ep} and the \gls{skr} algorithms in \figref{fig:PER.Iterative.all}.


%%%%%%%%%%%%%%%%%%%%
\subsection{Scheduling and complexity}\label{Sec:Sch.Cplx}

It may, therefore, be useful to define a \emph{scheduling} which specifies the number of iterations the \gls{ldpc} decoder executes before its outputs are transformed into $\hat{P}_n(a)$ and used again by the phase tracking \gls{mp}. 

Let the scheduling defined by $\set{I_{\tr{loop}}\times I_\tr{dec} }$ means the following: after each passage of the \gls{cbc} phase tracking, the decoder executes $I_{\tr{dec}}$ elementary decoding iterations\footnote{Defined as one check-nodes message update and one bit-nodes message update.}, then the phase tracking is implemented again and the results are used by the decoder executing $I_{\tr{dec}}$ elementary decoding iterations. This is repeated $I_\tr{loop}$ times so the total number of decoding iterations is given by $I^{\Sigma}_\tr{dec}=I_\tr{loop}\cd I_\tr{dec}$.

The scheduling from \cite{Colavolpe05} is defined by $\set{200 \times 1}$ meaning that the phase-tracking was executed $I_\tr{loop}=200$ times and, each phase-tracking was followed by one elementary decoding iterations; the total number of decoding iterations if thus $I_\tr{dec}^\Sigma=200$.

A ``one-shot'' phase tracking is denoted by the scheduling $\set{1\times I^{\Sigma}_\tr{dec}}$, and means that the phase tracking is carried out once and then all the decoding iterations are executed.

%In other words, the phase tracking is executed $I_\tr{loop}$ times, and the decoder executes $I_{\tr{loop}}} I_{\tr{dec}}$ elementary decoding iterations and, with that notation, the scheduling from \cite{Colavolpe05} is defined by ${200 \times 1}$ meaning that the phase-tracking was executed $200$ times and, each phase-tracking was followed by one elementary decoding iterations of the \gls{ldpc} decoder , while the scheduling $\set{2\times 100}$ from \cite{Alfredsson19} means that the \gls{cbc} phase tracking was executed twice and each was followed by $100$ decoding iterations. 

There are clearly many other possibilities to schedule the operations and they may affect the performance and the complexity. However,  caution should be applied when talking about the implementation complexity because it is difficult to compare  different operations: counting the additions/multiplications may be misleading especially when targeting implementation on the specialized circuits. 

For example, the operations necessary in the \gls{cmm} do not have the same implementation ``complexity'' as those required by the \gls{mp} \eqref{z.alpha.init}-\eqref{z.beta}; and it is difficult to compare any of these to the operations required by the elementary decoding iteration. However,  when operations are of the same type, they can be compared and provide a general idea about the complexity.



%%%%%%%%%%%%%%
%\subsection{Impact of large-argument approximations}\label{Sec:Simplifications}
%
%The non-linear operations in the algorithm appear mostly due to the use of the Bessel function, and may be implemented via look-up tables or replaced by easy-to-implement approximations. These non-linearities are present i)~in the calculation of $\hat{I}_0 (x)$, see \eqref{hat.I0} and ii)~when implementing the \gls{cmm}, where the function $B(x)=\frac{I_1(x)}{I_0(x)}$ must be evaluated; this is necessary to implement the projection operation $\mcF[\cd]$ and to calculate the result of the convolution between the Gaussian and the Tikhonov distributions.
%
%As for the point i), we may actually implement exactly the function $\hat{I}_0 (x)$ or use the \gls{laa} which was already proposed in the previous works, \eg \cite{Colavolpe05,Pecorino15,Shayovitz16}. This amount to using $\hat{I}_0 (x)\approx x $.
%
%As for the points ii) we already abandoned the idea of exact implementation of $B(x)$ (\eg via look-up tables) and instead use the approximation valid for the entire range of its argument, see \appref{}. However, it is still interesting to see the impact of the \gls{lla} in this case, especially that it was previously used for the very same purpose in the literature, \eg \cite[Appendix~A]{Shayovitz16}.
%
%We show in \figref{} how the \gls{per} is affected when the \gls{laa} is applied in different parts of the algorithms.







==> Includes/Introduction.R1.v1.tex <==
%!TEX root =  ../Phase.Tracking.R1.v1.tex
\section{Introduction}

In this work we propose and analyze a simple algorithm for signal detection in single-carrier transmission affected by the phase noise. The proposed algorithm is based on parametric \gls{mp} and is  shown to outperform the state-of-the-art algorithms both in terms of attainable error rates and of the complexity.

%% the justification of the sigle-carrier + phase noise
The single-carrier transmission, considered here, is often used for high speed communication in frequency non-selective channels \eg in satellite channels \cite{Colavolpe05}, wireless backhaul \cite{ShahMohammadian18}, or optical communications \cite{Millar16,Alfredsson19}. The limiting factor in achieving a high spectral efficiency is then not only due to the presence of the \gls{awgn} but also due to the phase-noise which is caused by the instability of the phase reference (such as a laser or an RF oscillator). 

Although sometimes the concept of ``strong'' phase noise is used, it merely depends on the constellation size: with sufficiently large modulation, the phase noise becomes a limiting factor for reliable communications. It is especially true for the wireless backhaul and optical channel which aggressively increase the modulation size \cite{Millar16,ShahMohammadian18,Alfredsson19}. The wireless backhaul, for example, calls for the use of constellation which may contain thousands of points \cite{ShahMohammadian18}. 

Since the phase noise is a random process with memory, the term ``phase tracking'' is often used and the common strategy relies on pilots symbols which, providing reliable reference, facilitate the tracking of the phase for payload symbols.  Increasing the density of the pilots, usually improves the performance  at the cost of decreased spectral efficiency. Therefore, the challenge of the phase tracking is not to eliminate the pilots altogether but rather to attain desirable performance (\eg as measured by the errors rates) with the limited number of pilots. 

The problem of phase tracking can be conveniently formulated using the graph relating all the involved variables \cite{Dauwels04,Colavolpe05}, which also leads to optimal solution defined by the \gls{mp} defined over the graph. It allows us to track the distribution of the phase at each symbol but, to represent accurately the distributions, a large number of samples may be required \cite{Colavolpe05,Shayovitz16} even if  simplifications may be sought by truncating the support of the distributions \cite{ShahMohammadian18}.

Therefore, many works looked into the possibility of \emph{parametric} phase tracking, where the distributions of the phase is assumed to belong to a predefined family;  Tikhonov distributions \cite{Colavolpe05,Shayovitz16} or Gaussians \cite{Kreimer18,Alfredsson19} are the most popular choices. Then, instead of estimating the samples of the distributions, only a few parameters need to be tracked. 

The distributions in the \gls{mp} are naturally mixtures (result of  averaging the contribution of the unknown payload symbols over the entire constellation), with potentially large number of elements. The mixture reduction is thus at the heart of any parametric phase tracking, and consists in replacing the mixture with a member from the adopted family of distributions. While in most works the mixture reduction consists in replacing the mixture with one distribution, the notable difference is \cite{Shayovitz16} which proposes to replace the mixture with another mixture but which contains a small number of elements. The improvements are thus obtained by making the parametrization  more involved both in terms of the number of required parameters and of their estimation.

The main challenge of the mixture reduction resides in finding a right balance between the implementation complexity and the performance of the resulting algorithm. With that regard, the \gls{cbc} algorithm \cite{Colavolpe05} makes uttermost simplification: the mixture reduction is performed \emp{before} the \gls{mp} recursion is invoked. This yields a very simple \gls{mp} algorithm which, due to its simplicity and ensuing popularity, should be considered ``canonical''. However, the cost is paid with relatively poor performance which must be improved  by leveraging the presence of the decoder as only in this way the \gls{cbc} algorithm can exploit the information about the modulation constellation. The resulting joint phase tracking and decoding  relies thus on the iterative exchange of information between the phase tracking and the decoder. This approach has been often reused, \eg \cite{Pecorino15,Alfredsson19}.

It is not without the pitfalls, however, and it was shown in \cite{Kreimer18} that, for large coding rates the \gls{cbc} algorithm introduces an error floor in high \gls{snr}. The remedy is then sought in \cite{Shayovitz16,Kreimer18} by performing the mixture reduction \emph{within} the recursive equations of the \gls{mp}; in this way, exploiting the form of the constellation, the performance is largely improved but the resulting \gls{mp} is also more complex. 
%%contributions

What the \gls{cbc} algorithm and many works on parametric \gls{mp} have in common is to rely heavily on the decoder to improve the estimation of the phase via joint decoding - phase tracking. And while it is clear that such a joint operation improves the performance, much less attention was  paid to the performance of ``one-shot'' phase tracking (meaning that the latter is decoupled from the decoder's outcome). This is a relevant issue not only because it is compatible with a current industrial practice\footnote{To our best knowledge, current phase tracking algorithm used in industrial products do not use decoder's feedback.} but also because good one-shot algorithm should yield larger improvement when operating jointly with the decoder.

The above considerations explain our take on the problem:  we want to exploit the form of the constellation \emph{without} relying on the decoder's feedback. In principle, this is also done in the algorithms of  \cite{Shayovitz16,Kreimer18} but, here we will take advantage of the simplicity of the \gls{cbc} algorithm and make projections before the \gls{mp} recursion is invoked. As we said, the original \gls{cbc} algorithm does not exploit the constellation form so we will refine it iteratively using the \gls{ep} \cite{Minka01} which is a general framework for iterative refinement of the approximations in parametric \gls{mp}s.  The \gls{ep} phase tracking algorithm we derive, preserves the simplicity characteristic of the \gls{mp} in the \gls{cbc} algorithm. We will compare our results to those proposed in \cite{Kreimer18}.

%and yet outperforms the \gls{dmp}, which is often treated as a performance limit for the phase tracking algorithms.

%%organization
The rest of the paper is organized as follows. In~\secref{sec:model}, we introduce the adopted system model, in \secref{sec:phase.track} we outline the fundamentals of the Bayesian phase tracking while its parametric formulation is explained in \secref{Sec:Parametric.MP}, where we also show how the the ``canonical'' algorithm from \cite{Colavolpe05} may be significantly improved by considering explicitly the circular nature of the involved distributions.

The main contribution lies in \secref{Sec:It.EP} which explains how the \gls{ep} framework may be used to derive a new phase tracking algorithm which, as shown in numerical examples, improves the performance without any help from the decoder. We also show that, when combined with the decoder, the new algorithms surpasses the \gls{dmp} limits conventionally used to evaluate the phase tracking algorithms. The conclusions are drawn in \secref{sec:Conclusions}. 

The appendices complete the picture analyzing the requirements for the discretization in the \gls{dmp}, showing the details of the operations on the circular distributions and providing new approximations required in the  latter.






==> Includes/Introduction.R1.v2.tex <==
%!TEX root =  ../Phase.Tracking.R1.v2.tex
\section{Introduction}

In this work we propose and analyze a simple algorithm for signal detection in single-carrier transmission affected by the phase noise. The proposed algorithm is based on parametric \gls{mp} and is  shown to outperform the state-of-the-art algorithms both in terms of attainable error rates and of the complexity.

%% the justification of the sigle-carrier + phase noise
The single-carrier transmission, considered here, is often used for high speed communication in frequency non-selective channels \eg in satellite channels \cite{Colavolpe05}, wireless backhaul \cite{ShahMohammadian18}, or optical communications \cite{Millar16,Alfredsson19}. The limiting factor in achieving a high spectral efficiency is then not only due to the presence of the \gls{awgn} but also due to the phase-noise which is caused by the instability of the phase reference (such as a laser or an RF oscillator). 

Although sometimes the concept of ``strong'' phase noise is used, it merely depends on the constellation size: with sufficiently large modulation, the phase noise becomes a limiting factor for reliable communications. It is especially true for the wireless backhaul and optical channel which aggressively increase the modulation size \cite{Millar16,ShahMohammadian18,Alfredsson19}. The wireless backhaul, for example, calls for the use of constellation which may contain thousands of points \cite{ShahMohammadian18}. 

Since the phase noise is a random process with memory, the term ``phase tracking'' is often used and the common strategy relies on pilots symbols which, providing reliable reference, facilitate the tracking of the phase for payload symbols.  Increasing the density of the pilots, usually improves the performance  at the cost of decreased spectral efficiency. Therefore, the challenge of the phase tracking is not to eliminate the pilots altogether but rather to attain desirable performance (\eg as measured by the errors rates) with the limited number of pilots. 

The problem of phase tracking can be conveniently formulated using the graph relating all the involved variables \cite{Dauwels04,Colavolpe05}, which also leads to optimal solution defined by the \gls{mp} defined over the graph. It allows us to track the distribution of the phase at each symbol but, to represent accurately the distributions, a large number of samples may be required \cite{Colavolpe05,Shayovitz16} even if  simplifications may be sought by truncating the support of the distributions \cite{ShahMohammadian18}.

Therefore, many works looked into the possibility of \emph{parametric} phase tracking, where the distributions of the phase is assumed to belong to a predefined family;  Tikhonov distributions \cite{Colavolpe05,Shayovitz16} or Gaussians \cite{Kreimer18,Alfredsson19} are the most popular choices. Then, instead of estimating the samples of the distributions, only a few parameters need to be tracked. 

The distributions in the \gls{mp} are naturally mixtures (result of  averaging the contribution of the unknown payload symbols over the entire constellation), with potentially large number of elements. The mixture reduction is thus at the heart of any parametric phase tracking, and consists in replacing the mixture with a member from the adopted family of distributions. While in most works the mixture reduction consists in replacing the mixture with one distribution, the notable difference is \cite{Shayovitz16} which proposes to replace the mixture with another mixture but which contains a small number of elements. The improvements are thus obtained by making the parametrization  more involved both in terms of the number of required parameters and of their estimation.

The main challenge of the mixture reduction resides in finding a right balance between the implementation complexity and the performance of the resulting algorithm. With that regard, the \gls{cbc} algorithm \cite{Colavolpe05} makes uttermost simplification: the mixture reduction is performed \emp{before} the \gls{mp} recursion is invoked. This yields a very simple \gls{mp} algorithm which, due to its simplicity and ensuing popularity, should be considered ``canonical''. However, the cost is paid with relatively poor performance which must be improved  by leveraging the presence of the decoder as only in this way the \gls{cbc} algorithm can exploit the information about the modulation constellation. The resulting joint phase tracking and decoding  relies thus on the iterative exchange of information between the phase tracking and the decoder. This approach has been often reused, \eg \cite{Pecorino15,Alfredsson19}.

It is not without the pitfalls, however, and it was shown in \cite{Kreimer18} that, for large coding rates the \gls{cbc} algorithm introduces an error floor in high \gls{snr}. The remedy is then sought in \cite{Shayovitz16,Kreimer18} by performing the mixture reduction \emph{within} the recursive equations of the \gls{mp}; in this way, exploiting the form of the constellation, the performance is largely improved but the resulting \gls{mp} is also more complex. 
%%contributions

What the \gls{cbc} algorithm and many works on parametric \gls{mp} have in common is to rely heavily on the decoder to improve the estimation of the phase via joint decoding - phase tracking. And while it is clear that such a joint operation improves the performance, much less attention was  paid to the performance of ``one-shot'' phase tracking (meaning that the latter is decoupled from the decoder's outcome). This is a relevant issue not only because it is compatible with a current industrial practice\footnote{To our best knowledge, current phase tracking algorithm used in industrial products do not use decoder's feedback.} but also because good one-shot algorithm should yield larger improvement when operating jointly with the decoder.

The above considerations explain our take on the problem:  we want to exploit the form of the constellation \emph{without} relying on the decoder's feedback. In principle, this is also done in the algorithms of  \cite{Shayovitz16,Kreimer18} but, here we will take advantage of the simplicity of the \gls{cbc} algorithm and make projections before the \gls{mp} recursion is invoked. As we said, the original \gls{cbc} algorithm does not exploit the constellation form so we will refine it iteratively using the \gls{ep} \cite{Minka01} which is a general framework for iterative refinement of the approximations in parametric \gls{mp}s.  The \gls{ep} phase tracking algorithm we derive, preserves the simplicity characteristic of the \gls{mp} in the \gls{cbc} algorithm. We will compare our results to those proposed in \cite{Kreimer18}.

%and yet outperforms the \gls{dmp}, which is often treated as a performance limit for the phase tracking algorithms.

%%organization
The rest of the paper is organized as follows. In~\secref{sec:model}, we introduce the adopted system model, in \secref{sec:phase.track} we outline the fundamentals of the Bayesian phase tracking while its parametric formulation is explained in \secref{Sec:Parametric.MP}, where we also show how the the ``canonical'' algorithm from \cite{Colavolpe05} may be significantly improved by considering explicitly the circular nature of the involved distributions.

The main contribution lies in \secref{Sec:It.EP} which explains how the \gls{ep} framework may be used to derive a new phase tracking algorithm which, as shown in numerical examples, improves the performance without any help from the decoder. We also show that, when combined with the decoder, the new algorithms surpasses the \gls{dmp} limits conventionally used to evaluate the phase tracking algorithms. The conclusions are drawn in \secref{sec:Conclusions}. 

The appendices complete the picture analyzing the requirements for the discretization in the \gls{dmp}, showing the details of the operations on the circular distributions and providing new approximations required in the  latter.






==> Includes/Introduction.v1.tex <==
%!TEX root =  ../Phase.Track.HARQ.v2.tex
\section{Introduction}

This work proposes simple and efficient algorithms to track  the phase noise when multiple replicas of the same transmitted signal are available. Such a situation occurs when \gls{harq} is employed, \ie when, in response to the detected transmission error, the receiver requests the retransmission of the packet.

The \gls{harq} protocols are commonly used, particularly in wireless communications to guarantee a reliable transmission over error-prone channels. They rely on a feedback channel which is used by the receiver to inform the transmitter about a decoding success (via \gls{ack} message) or a failure (via \gls{nack} message). After each \gls{nack} message, the same information packet is retransmitted until successful decoding is declared or the maximum number of retransmission is attained. The sequence of transmission rounds of the same packet is called a cycle.

A well-know retransmission strategy--\gls{rrharq}--relies on transmitting  exactly the same signal in each transmission round \cite{Caire01,Larsson14}. Then, under assumption of channel being memoryless, the receiver may decode the information packet from the weighted sum of  the signals received in all transmission rounds; this approach is also known as Chase combining \cite{Larsson14} after \cite{Chase84,Chase85}. %The suboptimal alternative is based on the bit-level combining, where the reliability metrics are calculated for the bits in  each transmission and then are added before the decoding. The suboptimality comes from the fact the the product of the marginals is not the marginal of the product, unless particular assumptions are made.

In this work, we consider the receivers affected by a ``strong'' phase-noise. The resulting channels are not memoryless so the conventional Chase combining cannot be used. In practice, some form of the phase tracking or, at least, phase variation compensation based on the pilot symbols must be used. Indeed, the issue of phase tracking has been dealt with already \eg in \cite{}. These previous works present many elegant solutions with different approaches to the parameterization of distribution of the phase. The common part is that they are based on the single transmission and do not deal with multivariate phase-distribution which appears in the problem formulation proper to the \gls{rrharq}.

The  main objectif of this work is to address the issue of phase tracking for \gls{rrharq} transmission;  the contributions are the following:
\begin{itemize}
\item We explain how the phase tracking should be done in the presence of repetition redundancy \gls{harq} and the main conclusions is that, a multi-variate distributions of the phase is necessary to take direct advantage of the retransmissions. This approach stands in contrast with the \gls{irharq}, where the redundancy is not explicitly exploited in the phase tracking.
\item We propose a simple parametric model to track the phase and we show the resulting update/tracking equations. Unlike \cite{} which used the Tikhonov distributions to approximate the phase noise, we use the Gaussian approximations. Our work goes beyond the framework of \cite{} showing the pitfalls of using Gaussian to represent the circular distributions. Not only, taking care of they non-circular nature, the Gaussian approximations produce results comparable to those based on Tikhonov functions but, more importantly they are simple to deal with in the multivariate situation characteristic of the \gls{harq}.
\item We present numerical examples comparing various strategies for decoding in \gls{rrharq} when phase noise is present.
\end{itemize}

The rest of the paper is organized as follows. In~\secref{sec:model}, we introduce the adopted system model.











==> Includes/Introduction.v4.tex <==
%!TEX root =  ../Phase.Tracking.v4.tex
\section{Introduction}

In this work we propose a simple algorithms for signal detection in transmission corrupted by a phase noise. The proposed parametric solution is  shown to outperform the state-of-the-art parametric algorithms both in terms of attainable error rates and  of the complexity.

%% the justification of the sigle-carrier + phase noise
We consider here the single-carrier transmission which is often used for high speed communication in frequency non-selective medium \eg in satellite channels \cite{Colavolpe05}, wireless backhaul \cite{ShahMohammadian18} or optical communications \cite{Millar16,Alfredsson19}. The limiting factor in achieving a high spectral efficiency is then not only the \gls{awgn} but also the phase-noise which is caused by the instability of the phase reference (such as a laser or an RF oscillator). 

Although sometimes the concept of ``strong'' phase noise is used, it merely depends on the constellation size: with sufficiently large modulation, the phase noise becomes a limiting factor for reliable communications. It is especially true for the wireless backhaul and optical channel which aggressively increase the modulation size \cite{ShahMohammadian18}\cite{Millar16}\cite{Alfredsson19}. The wireless backhaul, for example, calls for the use of constellation which may contain thousands of points \cite{ShahMohammadian18}. 

Since the phase noise is a random process with memory, the term ``phase tracking'' is often used and the common strategy relies on pilots symbols which, providing reliable reference, facilitate the tracking of the phase for payload symbols.  Increasing the density of the pilots, usually improves the performance  at the cost of decreased spectral efficiency. Therefore, the challenge of the phase tracking is not to eliminate the pilots altogether but rather to attain desirable performance (as measured by the errors rates) with the limited number of pilots. 

The problem of phase tracking can be solved optimally (in the probabilistic sense) via the \gls{mp} defined over the graph relating all the involved variables \cite{Colavolpe05}. It allows us to track the distribution of the phase at each symbol but, to represent accurately the distributions, a large number of samples may be required \cite{Colavolpe05}\cite{Shayovitz16} even if  simplifications may be sought by truncating the support of the distributions \cite{ShahMohammadian18}.

Therefore, many works looked into the possibility of \emph{parametric} phase tracking, where the distributions of the phase is assumed to belong to a predefined family;  Tikhonov distributions \cite{Colavolpe05}\cite{Shayovitz16} or Gaussians \cite{Kreimer18}\cite{Alfredsson19} are the most popular choices. Then, instead of estimating the distribution, only a few parameters need to be tracked. 

The distributions in the \gls{mp} are naturally mixtures (result of  averaging the contribution of the unknown payload symbols over the entire constellation), with potentially large number of elements. The mixture reduction is thus at the heart of any parametric phase tracking, and consists in replacing the mixture with a member from the adopted family of distributions. The way in which  the mixture reduction is done, affects the implementation complexity and performance.  Thus, the art of parametric \gls{mp} resides in finding a right balance between these two, often, contradictory criteria.

With that regard, the \gls{cbc} algorithm \cite{Colavolpe05} makes uttermost simplification of the mixtures that produces a very simple \gls{mp}; due to its simplicity it should be considered ``canonical'' in that context. However, the cost is paid with relatively poor performance which must be improved  by leveraging the presence of the decoder as only in this way the \gls{cbc} algorithm can exploit the information about the modulation constellation. The resulting joint phase tracking and decoding  relies on the iterative exchange of information between the phase tracking and the decoder. This approach has been often reused, \eg \cite{Pecorino15}\cite{Alfredsson19}.

It is not without the pitfalls, however, and it was shown in \cite{Kreimer18} that, for large coding rates the \gls{cbc} algorithm introduces an error floor. The remedy is then sought in \cite{Shayovitz16}\cite{Kreimer18} by exploiting explicitly the form of the constellation and changing the way the mixture reduction is performed: the performance is improved but the resulting \gls{mp} is also more complex.
%%contributions

What the \gls{cbc} algorithm and many  previous works on the parametric \gls{mp} have in common is to rely heavily on the decoder to improve the estimation of the phase via joint decoding - phase tracking. The notable difference is \cite{Shayovitz16} which mimics the behaviour of the \gls{dmp}. However,  the improvement is attained by making the parametrization much more involved both in terms of the number of required parameters and their estimation.

In that regard, our take on this problem is different: we want to i) leverage the simplicity inherent in the \gls{mp} of the \gls{cbc} algorithm, and ii) exploit the structure of the constellation \emph{without} relying \emph{only} on the decoder's feedback; in fact, this is what the \gls{dmp} actually does and yet its performance is often taken as the reference for the phase tracking algorithm which \emph{do use} the decoder's feedback.

We propose to apply the \gls{ep} \cite{Minka01} which is a general framework for iterative refinement of the approximations in parametric \gls{mp}s.  The \gls{ep} phase tracking algorithm we derive, preserves the simplicity characteristic of the \gls{mp} of the \gls{cbc} algorithm, is thus simpler than the alternative proposed in \cite{Kreimer18}, and yet outperforms the \gls{dmp}, which is often treated as a performance limit for the phase tracking algorithms.

%%organization
The rest of the paper is organized as follows. In~\secref{sec:model}, we introduce the adopted system model, in \secref{sec:phase.track} we outline the fundamentals of the Bayesian phase tracking while its parametric formulation is explained in \secref{Sec:Parametric.MP}, where we also show how the the ``canonical'' algorithm from \cite{Colavolpe05} may be significantly improved by considering explicitly the circular nature of the involved distributions.

The main contribution lies in \secref{Sec:It.EP} which explains how the \gls{ep} framework may be used to derive a new phase tracking algorithm which, as shown in numerical examples, improves the performance without any help from the decoder. We also show that, when combined with the decoder, the new algorithms surpasses the \gls{dmp} limits conventionally used to evaluate the phase tracking algorithms. The conclusions are drawn in \secref{sec:Conclusions} and the appendices show the details of the operations on the circular distributions, clarifying the analytical details and providing new approximations.






==> Includes/Model.R1.v1.tex <==
%!TEX root =  ../Phase.Tracking.R1.v1.tex
\section{System Model}\label{sec:model}

We consider transmission over a channel corrupted by the additive noise and phased noise 
\begin{align}\label{y.kn}
y_{n} =  x_{n}\e^{\jj \theta_{n}} + v_{n},\quad n=0,\ld, N
\end{align}
where $x_n\in\mcA$ is the transmitted complex symbol drawn from the $M$-ary constellation $\mcA$, \ie $|\mcA|=M$, $y_{n}$ are samples of the received signal, $v_{n}$ is the additive noise, and $\theta_n$ is the phase noise. 

We assume the constellation $\mcA$ is zero mean and energy normalized so, modelling $x_n$ as random variable obtained by uniform sampling of  $\mcA$, we have $\Ex[x_n]=0$ and \mbox{$\Ex[x^2_n]=1$}. We model $v_{n}$ as complex \gls{iid} Gaussian variables with zero mean and variance $\No$ (\gls{awgn} model); $\theta_{n}$ is modelled as a Wiener process
\begin{align}\label{theta.Wiener}
\theta_{n}=\theta_{n-1}+w_{n}, \quad n=1,\ld,N,
\end{align}
where $w_{n}$ are \gls{iid}  zero-mean, real Gaussian variables with variance $\sigma_w^2$; the initial value $\theta_{0}$  is modelled as uniformly distributed over the interval $(-\pi, \pi]$.

This model is popular in wireless and optical communications, \eg \cite{Colavolpe05,Alfredsson19}. The variance of the additive noise $v_n$ is determined by the thermal/optical noise at the receiver and the attenuation on the propagation path; the \gls{snr} is defined as $\SNRrv=\frac{1}{\No}$. The variance of the phase noise $w_{n}$ reflects the (in)stability of the oscillator used in the demodulation process. We suppose that both, $\sigma_w^2$ and $\SNRrv$, are known at the receiver. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Coding and decoding}\label{Sec:cod.decod.}
The transmitted symbols $x_n$ are obtained via \gls{bicm} \cite[Chap.~1.4]{Szczecinski_Alvarado_book} in two steps: 1) the information bits $\set{b_n}_{n=1}^{\Nb}$ are encoded using the binary encoder of rate $r$ into the coded bits $\set{c_n}_{n=1}^{\Nc}$, where $\Nb=r\Nc$ (in the numerical examples we use the \gls{ldpc} codes, and 2) the coded bits $\set{c}$ are regrouped into length-$m$ labels $\tilde{\bc}_n=[c_{n,1},\ld, c_{n,m}]$ which are mapped onto the symbols from the  $\mcA$
\begin{align}\label{s.n.c}
s_{n}&=\MODwo\big[\tilde{\bc}_n\big], \quad n=1,\ld, \Ns,
\end{align} 
where $\MODwo[\cd]: \set{0,1}^m\mapsto \mcA$ is the mapping; in this work, $\mcA$ is $M$-ary \gls{qam} and $\MODwo[\cd]$ is the Gray mapping \cite[Sec.~2.5.2]{Szczecinski_Alvarado_book}.
Finally, reference symbols (pilots) are interleaved with the payload $\set{s_n}_{n=1}^\Ns$ so the transmitted sequence can be presented as
\begin{align}
\label{payload.1}
\set{x_n}_{n=1}^{N}
&=\set{ \underset{\uparrow}{x_0},x_1,\ld, x_{L-1},\underset{\uparrow}{x_L},x_{L+1},\ld, \underset{\uparrow}{x_N} },
\end{align}
where we indicate with arrows the pilot symbols $x_{l L}, l=0,\ld, F$, while $x_n, n\neq lF$ are payload symbols, that is, $x_{n'}=s_n, n=1,\ld,\Ns$ where the mapping $n'=n'(n)$ allows to index the symbols in $\set{x_n}$ by skipping the pilots. We will use the values of $L$ which satisfy $\Ns=F (L-1)$ for integer $F$.

Similarly, the \gls{bicm} decoding is carried out  in two steps \cite[Chap.~1.4]{Szczecinski_Alvarado_book}
\begin{enumerate}
\item \emph{Demodulation}: consists in finding the marginal conditional probability of the coded bits
\begin{align}\label{p.nk.c}
&\PR{c_{n,k}=c|\by}\\
\label{demodulation}
&\qquad ~ \quad 
\propto \sum_{a\in\mcA_{k,c}}\PR{s_{n}=a|\by},
\end{align}
where $\by=\set{y_n}_{n=1}^N$ gathers all the channel outcomes and 
\begin{align}
\mcA_{k,c}=\set{ \MOD{\bc}, \bc=[c_1,\ld, c_{k-1},c,c_{k+1},\ld, c_m]}
\end{align}
is a sub-constellation comprising only the symbols labeled by the bit with value $c\in\set{0,1}$ at the position $k=1,\ld,m$;  $\propto$ will be used in the text to indicate that the distributions are defined up to a multiplicative factor which is independent of the distribution argument (here $c$). 

%The marginalization \eqref{demodulation} done over the coded bits which label the same symbol $s_{n}$, is known as \gls{bicm} demodulation.

Since $s_n=x_{n'}$, to obtain \eqref{p.nk.c} we have to calculate the conditional distribution of the symbols $x_n$
\begin{align}\label{P.n.a.x}
P_n(a)\triangleq\PR{x_{n}=a|\by}, \quad a\in\mcA;
\end{align} 
this operation involves marginalization over the phase $\theta_{n}$ and the transmitted symbols $x_l, l\neq n$, and is a ``phase tracking'' since, as a byproduct of \eqref{P.n.a.x}, we will obtain the distribution of the phase $\pdf(\theta_n|\set{y_l}_{l=1}^N)$.

\item \emph{Soft-input decoding}: using \eqref{P.n.a.x} and \eqref{p.nk.c} we calculate the \glspl{llr} for the coded bits $c_{n,k}$, \ie 
\begin{align}\nonumber
\lambda_{n,k}&=\log\frac{\PR{c_{n,k}=1|\by}}{\PR{c_{n,k}=0|\by}}\\
\label{lambda.n.l}
&\approx
\max_{a\in\mcA_{k,1}}\hat{P}_{n'}(a) - \max_{a\in\mcA_{k,0}}\hat{P}_{n'}(a),
\end{align}
where we applied the max-log simplification using the log-probability, $\hat{P}_n(a)=\log P_n(a)$; the logarithmic domain eases implementation and will appear in all parametric derivations; we use again the mapping $n'=n'(n)$. 
\end{enumerate}

The \gls{llr}s, $\lambda_{n,k}$,  are fed to the binary decoder which operates in abstraction of how they were  calculated. This very separation of the operation of the decoder and the demodulator is the distinctive feature of the \gls{bicm} which made it, de facto, a standard approach to design spectrally efficient transceivers. The obvious advantage is that both, the demodulator (comprising the phase-tracking) and the decoder may be designed and implemented independently of each other. Such an operation is characteristic of ``one-shot'' demodulators which are the most common solutions in the \gls{bicm} transceivers. 

On the other hand, the inherent simplicity of one-shot demodulators is a source of performance limitation which may be overcome by forcing the two-way exchange between the demodulator and the decoder. We also consider this option and we will assume that the decoder provides the demodulator with the a priori symbol probabilities $P^\tr{a}_n(a)=\PR{x_n=a}$ which may be used in the phase tracking. On the other hand, we decide to preserve the \gls{llr} calculation in \eqref{lambda.n.l} which does not take advantage of the information provided by the decoder.\footnote{It is possible, however: in such a case, the decoder would have to provide the a priori probabilities of the bits and not only the probabilities of the symbols. This approach is known to provides little gain in the case of the Gray-mapped constellations we use here \cite{Schreckenbach03} but yields gains with appropriately designed mapping \cite{Szczecinski05e}.}






==> Includes/Model.R1.v2.tex <==
%!TEX root =  ../Phase.Tracking.R1.v2.tex
\section{System Model}\label{sec:model}

We consider transmission over a channel corrupted by the additive noise and phased noise 
\begin{align}\label{y.kn}
y_{n} =  x_{n}\e^{\jj \theta_{n}} + v_{n},\quad n=0,\ld, N
\end{align}
where $x_n\in\mcA$ is the transmitted complex symbol drawn from the $M$-ary constellation $\mcA$, \ie $|\mcA|=M$, $y_{n}$ are samples of the received signal, $v_{n}$ is the additive noise, and $\theta_n$ is the phase noise. 

We assume the constellation $\mcA$ is zero mean and energy normalized so, modelling $x_n$ as random variable obtained by uniform sampling of  $\mcA$, we have $\Ex[x_n]=0$ and \mbox{$\Ex[x^2_n]=1$}. We model $v_{n}$ as complex \gls{iid} Gaussian variables with zero mean and variance $\No$ (\gls{awgn} model); $\theta_{n}$ is modelled as a Wiener process
\begin{align}\label{theta.Wiener}
\theta_{n}=\theta_{n-1}+w_{n}, \quad n=1,\ld,N,
\end{align}
where $w_{n}$ are \gls{iid}  zero-mean, real Gaussian variables with variance $\sigma_w^2$; the initial value $\theta_{0}$  is modelled as uniformly distributed over the interval $(-\pi, \pi]$.

This model is popular in wireless and optical communications, \eg \cite{Colavolpe05,Alfredsson19}. The variance of the additive noise $v_n$ is determined by the thermal/optical noise at the receiver and the attenuation on the propagation path; the \gls{snr} is defined as $\SNRrv=\frac{1}{\No}$. The variance of the phase noise $w_{n}$ reflects the (in)stability of the oscillator used in the demodulation process. We suppose that both, $\sigma_w^2$ and $\SNRrv$, are known at the receiver. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Coding and decoding}\label{Sec:cod.decod.}
The transmitted symbols $x_n$ are obtained via \gls{bicm} \cite[Chap.~1.4]{Szczecinski_Alvarado_book} in two steps: 1) the information bits $\set{b_n}_{n=1}^{\Nb}$ are encoded using the binary encoder of rate $r$ into the coded bits $\set{c_n}_{n=1}^{\Nc}$, where $\Nb=r\Nc$ (in the numerical examples we use the \gls{ldpc} codes, and 2) the coded bits $\set{c_n}$ are regrouped into length-$m$ labels $\tilde{\bc}_n=[c_{n,1},\ld, c_{n,m}]$ which are mapped onto the symbols from the constellation $\mcA$
\begin{align}\label{s.n.c}
s_{n}&=\MODwo\big[\tilde{\bc}_n\big], \quad n=1,\ld, \Ns,
\end{align} 
where $\MODwo[\cd]: \set{0,1}^m\mapsto \mcA$ is the mapping; in this work, $\mcA$ is $M$-ary \gls{qam} and $\MODwo[\cd]$ is the Gray mapping \cite[Sec.~2.5.2]{Szczecinski_Alvarado_book}.
Finally, reference symbols (pilots) are interleaved with the payload $\set{s_n}_{n=1}^\Ns$ so the transmitted sequence can be presented as
\begin{align}
\label{payload.1}
\set{x_n}_{n=1}^{N}
&=\set{ \underset{\uparrow}{x_0},x_1,\ld, x_{L-1},\underset{\uparrow}{x_L},x_{L+1},\ld, \underset{\uparrow}{x_N} },
\end{align}
where we indicate with arrows the pilot symbols $x_{l L}, l=0,\ld, F$, while $x_n, n\neq lF$ are payload symbols, that is, $x_{n'}=s_n, n=1,\ld,\Ns$ where the mapping $n'=n'(n)$ allows to index the symbols in $\set{x_n}$ by skipping the pilots. We will use the values of $L$ which satisfy $\Ns=F (L-1)$ for integer $F$.

Similarly, the \gls{bicm} decoding is carried out  in two steps \cite[Chap.~1.4]{Szczecinski_Alvarado_book}
\begin{enumerate}
\item \emph{Demodulation}: consists in finding the marginal conditional probability of the coded bits
\begin{align}\label{p.nk.c}
&\PR{c_{n,k}=c|\by}\\
\label{demodulation}
&\qquad ~ \quad 
\propto \sum_{a\in\mcA_{k,c}}\PR{s_{n}=a|\by},
\end{align}
where $\by=\set{y_n}_{n=1}^N$ gathers all the channel outcomes and 
\begin{align}
\mcA_{k,c}=\set{ \MOD{\bc}, \bc=[c_1,\ld, c_{k-1},c,c_{k+1},\ld, c_m]}
\end{align}
is a sub-constellation comprising only the symbols labeled by the bit with value $c\in\set{0,1}$ at the position $k=1,\ld,m$;  $\propto$ will be used in the text to indicate that the distributions are defined up to a multiplicative factor which is independent of the distribution argument (here $c$ or $a$). 

%The marginalization \eqref{demodulation} done over the coded bits which label the same symbol $s_{n}$, is known as \gls{bicm} demodulation.

Since $s_n=x_{n'}$, to obtain \eqref{p.nk.c} we have to calculate the conditional distribution of the symbols $x_n$
\begin{align}\label{P.n.a.x}
P_n(a)\triangleq\PR{x_{n}=a|\by}, \quad a\in\mcA;
\end{align} 
this operation involves marginalization over the phase $\theta_{n}$ and the transmitted symbols $x_l, l\neq n$, and is a ``phase tracking'' since, as a byproduct of \eqref{P.n.a.x}, we will obtain the distribution of the phase $\pdf(\theta_n|\set{y_l}_{l=1}^N)$.

\item \emph{Soft-input decoding}: using \eqref{P.n.a.x} and \eqref{p.nk.c} we calculate the \glspl{llr} for the coded bits $c_{n,k}$, \ie 
\begin{align}\nonumber
\lambda_{n,k}&=\log\frac{\PR{c_{n,k}=1|\by}}{\PR{c_{n,k}=0|\by}}\\
\label{lambda.n.l}
&\approx
\max_{a\in\mcA_{k,1}}\hat{P}_{n'}(a) - \max_{a\in\mcA_{k,0}}\hat{P}_{n'}(a),
\end{align}
where we applied the max-log simplification using the log-probability, $\hat{P}_n(a)=\log P_n(a)$; the logarithmic domain eases implementation and will appear in all parametric derivations; we use again the mapping $n'=n'(n)$. 
\end{enumerate}

The \gls{llr}s, $\lambda_{n,k}$,  are fed to the binary decoder which operates in abstraction of how they were  calculated. This very separation of the operation of the decoder and the demodulator is the distinctive feature of the \gls{bicm} which made it, de facto, a standard approach to design spectrally efficient transceivers. The obvious advantage is that both, the demodulator (comprising the phase-tracking) and the decoder may be designed and implemented independently of each other. Such an operation is characteristic of ``one-shot'' demodulators which are the most common solutions in the \gls{bicm} transceivers. 

On the other hand, the inherent simplicity of one-shot demodulators is a source of performance limitation which may be overcome by forcing the two-way exchange between the demodulator and the decoder. We also consider this option and we will assume that the decoder provides the demodulator with the a priori symbol probabilities $P^\tr{a}_n(a)=\PR{x_n=a}$ which may be used in the phase tracking. On the other hand, we decide to preserve the \gls{llr} calculation in \eqref{lambda.n.l} which does not take advantage of the information provided by the decoder.\footnote{It is possible, however: in such a case, the decoder would have to provide the a priori probabilities of the bits and not only the probabilities of the symbols. This approach is known to provides little gain in the case of the Gray-mapped constellations we use here \cite{Schreckenbach03} but yields gains with appropriately designed mapping \cite{Szczecinski05e}.}






==> Includes/Model.v1.tex <==
%!TEX root =  ../Phase.Tracking.v3.tex
\section{System Model}\label{sec:model}

We consider transmission over \gls{awgn} channel corrupted by the phased noise 
\begin{align}\label{y.kn}
y_{n} =  x_{n}\e^{\jj \theta_{n}} + z_{n},\quad n=0,\ld, N
\end{align}
where $x_n$ is the transmitted complex symbol, $y_{n}$ are samples of the received signal, $z_{n}$ is the additive noise, and $\theta_n$ is the phase noise. We model $z_{n}$ as \gls{iid} complex Gaussian variables with zero mean and variance $\No$; $\theta_{n}$ is modelled as a Wiener process
\begin{align}\label{theta.Wiener}
\theta_{n}=\theta_{n-1}+w_{n}, \quad n=1,\ld,N,
\end{align}
where $w_{n}$ are \gls{iid}  zero-mean, real Gaussian variables with variance $\sigma_w^2$; the initial values $\theta_{0}$  are modelled as uniformly distributed over the interval $(-\pi, \pi]$.

The variance of the additive noise $z_n$ is determined by the thermal noise at the receiver and the attenuation on the propagation path;\footnote{The attenuation is considered unitary in \eqref{y.kn} but any signal attenuation can be factored into $\No$.} it is customary to use the \gls{snr}, $\SNR=1/\No$ to define the model \eqref{y.kn}. The variance of the phase noise $w_{n}$ reflects the (in)stability of the oscillator used in the demodulation process \cite{}. We suppose that both, $\sigma_w^2$ and $\No$, are known at the receiver, \eg through estimation.

\subsection{Coding and decoding}\label{Sec:cod.decod.}
The transmitted symbols may be obtained via three steps we show in the following, where the first two define how the payload symbols are obtained from the information bits via the \gls{bicm} encoding  \cite[Chap.~1.4]{Szczecinski_Alvarado_book}, and the third step defines the pilots.
\begin{enumerate}

\item \emph{Binary encoding}: the information bits $\bb=[b_1,\ld, b_{\Nb}]$ are encoded using the binary encoder of rate $r$ into the sequence of coded bits $\bc=[c_1,\ld, c_{\Nc}]$, where $\Nb=r\Nc$. In the numerical examples we use the \gls{ldpc} codes.

\item \emph{$M$-ary modulation}: the coded bits $\bc$ are regrouped into length-$m$ labels $\tilde{\bc}_n=[c_{n,1},\ld, c_{n,m}]$, \ie $\bc=[\tilde{\bc}_1,\ld,\tilde{\bc}_{\Ns}]$ (so $\Ns=\Nc/m$ ), and each label is mapped onto the symbols from the  $\mcA$, where $|\mcA|=M=2^m$
\begin{align}\label{}
s_{n}&=\MODwo\big[\tilde{\bc}_n\big], \quad n=1,\ld, \Ns.
\end{align} 

In the numerical examples, $\mcA$ is the well-known $M$-ary \gls{qam} constellations, such as $4$-\gls{qam} or 16-\gls{qam}.  We quickly note that the interleaving of the coded bits, $\bc$, prior to the modulation, often seen as  an inherent part of  \gls{bicm}, is not necessary if the encoder has the interleaving-like property, as is the case of the \gls{ldpc} encoder that we use in numerical examples.\footnote{In general, the interleaving is useful in the diversity-inducing (\eg fading) channels. In our case, the channel is \gls{awgn} so, unlike in fading channels, the propagation-related diversity does not exist. On the other hand, the phase-tracking may provoke bursts of phase-errors (by which we mean having the a posteriori distribution of the phase concentrated at the arguments which are far from the actual phase); this will corrupt the reliability metrics calculated for the (successive) bits affected by the burst is a manner somewhat similar to the fading. Thus  the interleaving is recommended and is implicitly implemented with the \gls{ldpc} encoder.}
\item \emph{Pilot insertion}: The common approach to deal with time-varying channel (that requires estimation of the phase noise or the channel gain) is to use the known/reference symbols (or, pilots), interleaved with the payload $\bs$; the sequence of transmitted symbols can be presented as
\begin{align}
\label{payload.1}
\bx
&=[\underset{\uparrow}{x_0},x_1,\ld, x_{L-1},\underset{\uparrow}{x_L},x_{L+1},\ld, \underset{\uparrow}{x_N} ]
%\\
%\label{payload.2}
%&=[s^{\tr{p}}_0,s_1,\ld, s_{L-1},v_1, s_{L},\ld, s_{\Ns},v_F ],
\end{align}
where $N=F L +1$ and we indicate with arrows the pilot symbols $x_{l L}, l=0,\ld, F$. We will use the values of $L$ which satisfy $\Ns=F (L-1)$ for integer $F$ and thus no dummy symbols are needed to fill the frame and $x_n, n\neq lF$ are payload symbols from $\bs$.
\end{enumerate}

Similarly, the \gls{bicm} decoding is carried out  in two steps \cite[Chap.~1.4]{Szczecinski_Alvarado_book}
\begin{enumerate}
\item \emph{Phase tracking and demodulation}: consists in finding the marginal conditional probability of the coded bits
\begin{align}\label{p.nk.c}
&\PR{c_{n,k}=c|\by}\\
\label{demodulation}
&\qquad ~ \quad 
\propto \sum_{a\in\mcA_{k,c}}\PR{s_{n}=a|\by},  \quad c\in\set{0,1},
\end{align}
where $\by=[y_0,\ld,y_{N}]$ gathers all the channel outcomes and $\mcA_{k,c}=\set{ \MOD{\bc}, \bc=[c_1,\ld, c_{k-1},c,c_{k+1},\ld, c_m]}$ is a sub-constellation comprising only the symbols labeled by the bit with value $c$ at the position $k$;  $\propto$ will be used in the text to indicate that the distributions are defined up to a multiplicative factor which is independent of the distribution argument (here $c$). 

The marginalization \eqref{demodulation} done over the coded bits which label the same symbol $s_{n}$, is known as \gls{bicm} demodulation.

Since $s_n$ are uniquely related to $x_n$ (via mapping $\bs \rightarrow \bx$, see \eqref{payload.1}, to obtain \eqref{p.nk.c} we have to calculate the conditional distribution of the symbols $x_n$
\begin{align}\label{track.phase}
P_n(a)\triangleq\PR{x_{n}=a|\by}, \quad a\in\mcA;
\end{align} 
this operation involves marginalization over the phase $\theta_{n}$ and the transmitted symbols $x_t, t\neq n$. This is what we call a ``phase tracking'' since, as we will see later, as a byproduct of \eqref{track.phase}, we will obtain the distribution of the phase $\pdf(\theta_n|\by)$.

%This logical separation of demodulation and phase tracking emphasizes that \eqref{track.phase} is necessary only in the presence of the phase noise. Without the phase noise which introduced memory in \eqref{y.kn}, it would be possible to abandon the dependence on the whole sequence and rewrite \eqref{track.phase} as $P_n(a)=\PR{x_{n}=a|y_n}$ and use it directly in \eqref{demodulation}.

\item \emph{Soft-input decoding}: the probabilities \eqref{p.nk.c} are fed to the decoder which operates in abstraction of how they were  calculated. %In the numerical examples we use the \gls{ldpc} decoder based on a sum-product algorithm with ten iterations.
\end{enumerate}

%\subsection{Pilots}\label{sec:pilots}





==> Includes/Model.v4.tex <==
%!TEX root =  ../Phase.Tracking.v4.tex
\section{System Model}\label{sec:model}

We consider transmission over a channel corrupted by the additive noise and phased noise 
\begin{align}\label{y.kn}
y_{n} =  x_{n}\e^{\jj \theta_{n}} + v_{n},\quad n=0,\ld, N
\end{align}
where $x_n$ is the transmitted complex symbol, $y_{n}$ are samples of the received signal, $v_{n}$ is the additive noise, and $\theta_n$ is the phase noise. We model $v_{n}$ as \gls{awgn}, \ie a complex \gls{iid} Gaussian variables with zero mean and variance $\No$; $\theta_{n}$ is modelled as a Wiener process
\begin{align}\label{theta.Wiener}
\theta_{n}=\theta_{n-1}+w_{n}, \quad n=1,\ld,N,
\end{align}
where $w_{n}$ are \gls{iid}  zero-mean, real Gaussian variables with variance $\sigma_w^2$; the initial values $\theta_{0}$  are modelled as uniformly distributed over the interval $(-\pi, \pi]$.

This model is popular in wireless and optical communications, \eg \cite{Colavolpe05} \cite{Alfredsson19}. The variance of the additive noise $v_n$ is determined by the thermal/optical noise at the receiver and the attenuation on the propagation path; the \gls{snr} is defined as $\SNR=\frac{1}{\No}$. The variance of the phase noise $w_{n}$ reflects the (in)stability of the oscillator used in the demodulation process. We suppose that both, $\sigma_w^2$ and $\SNR$, are known at the receiver. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Coding and decoding}\label{Sec:cod.decod.}
The transmitted symbols $x_n$ are obtained via \gls{bicm} \cite[Chap.~1.4]{Szczecinski_Alvarado_book}. That is, i) the information bits $\bb=[b_1,\ld, b_{\Nb}]$ are encoded using the binary encoder of rate $r$ into the sequence of coded bits $\bc=[c_1,\ld, c_{\Nc}]$, where $\Nb=r\Nc$; in the numerical examples we use the \gls{ldpc} codes, ii) the coded bits $\bc$ are regrouped into length-$m$ labels $\tilde{\bc}_n=[c_{n,1},\ld, c_{n,m}]$, \ie $\bc=[\tilde{\bc}_1,\ld,\tilde{\bc}_{\Ns}]$ which are mapped onto the symbols from the  $\mcA$, where $|\mcA|=M=2^m$
\begin{align}\label{}
s_{n}&=\MODwo\big[\tilde{\bc}_n\big], \quad n=1,\ld, \Ns.
\end{align} 
Finally, reference symbols (pilots) are interleaved with the payload $\bs$ so the sequence of transmitted symbols can be presented as
\begin{align}
\label{payload.1}
\bx
&=[\underset{\uparrow}{x_0},x_1,\ld, x_{L-1},\underset{\uparrow}{x_L},x_{L+1},\ld, \underset{\uparrow}{x_N} ]
\end{align}
where we indicate with arrows the pilot symbols $x_{l L}, l=0,\ld, F$ and $x_n, n\neq lF$ are payload symbols from $\bs$. That is, $x_{n'}=s_n, n=1,\ld,\Ns$ where the mapping $n\rightarrow n'$ allows to index the symbols in $\bx$ by skipping the pilots. We will use the values of $L$ which satisfy $\Ns=F (L-1)$ for integer $F$.

Similarly, the \gls{bicm} decoding is carried out  in two steps \cite[Chap.~1.4]{Szczecinski_Alvarado_book}
\begin{enumerate}
\item \emph{Phase tracking and demodulation}: consists in finding the marginal conditional probability of the coded bits
\begin{align}\label{p.nk.c}
&\PR{c_{n,k}=c|\by}\\
\label{demodulation}
&\qquad ~ \quad 
\propto \sum_{a\in\mcA_{k,c}}\PR{s_{n}=a|\by},  \quad c\in\set{0,1},
\end{align}
where $\by=[y_0,\ld,y_{N}]$ gathers all the channel outcomes and 
\begin{align}
\mcA_{k,c}=\set{ \MOD{\bc}, \bc=[c_1,\ld, c_{k-1},c,c_{k+1},\ld, c_m]}
\end{align}
is a sub-constellation comprising only the symbols labeled by the bit with value $c$ at the position $k$;  $\propto$ will be used in the text to indicate that the distributions are defined up to a multiplicative factor which is independent of the distribution argument (here $c$). 

%The marginalization \eqref{demodulation} done over the coded bits which label the same symbol $s_{n}$, is known as \gls{bicm} demodulation.

Since $s_n=x_{n'}$, to obtain \eqref{p.nk.c} we have to calculate the conditional distribution of the symbols $x_n$
\begin{align}\label{P.n.a.x}
P_n(a)\triangleq\PR{x_{n}=a|\by}, \quad a\in\mcA;
\end{align} 
this operation involves marginalization over the phase $\theta_{n}$ and the transmitted symbols $x_t, t\neq n$, and is a ``phase tracking'' since, as a byproduct of \eqref{P.n.a.x}, we will obtain the distribution of the phase $\pdf(\theta_n|\by)$.

\item \emph{Soft-input decoding}: using \eqref{P.n.a.x} and \eqref{p.nk.c} we calculate the \glspl{llr} for the coded bits $c_{n,k}$ 
\begin{align}\nonumber
\lambda_{n,k}&=\log\frac{\PR{c_{n,k}=1|\by}}{\PR{c_{n,k}=0|\by}}\\
\label{lambda.n.l}
&\approx
\max_{a\in\mcA_{k,1}}\hat{P}_{n'}(a) - \max_{a\in\mcA_{k,0}}\hat{P}_{n'}(a),
\end{align}
where we applied the max-log simplification using the log-probability, $\hat{P}_n(a)=\log P_n(a)$; the logarithmic domain simplifies implementation and will appear in all parametric derivations; we use again the mapping $n\rightarrow n'$. 

The \gls{llr}s are fed to the binary decoder which operates in abstraction of how they were  calculated.
\end{enumerate}






==> Includes/Tracking.R1.v1.tex <==
%!TEX root =  ../Phase.Tracking.R1.v1.tex
\section{Phase tracking}\label{sec:phase.track}
%%%%%
%\subsection{Message passing on the graph}\label{Sec:MP.graph}
%%%%%%%%%%%%%%
\begin{figure}[bt]
\begin{center}
\scalebox{0.8}{\input{./figures/Graph.RRHARQ.x.2D.tex}}
\end{center}
\caption{Graph defining the relationship between the variables in the phase tracking problem used previously \eg in \cite[Fig.~2]{Colavolpe05}, \cite[Fig.~2]{Shayovitz16}; the messages exchanged between the nodes are shown together with the arrows indicating the direction of the exchange. When variable is connected to two functions, the message passes transparently through the variable node as in the case of probability $P_n(a)=\PR{x_n=a|\by}, a\in\mcA$ defining the distribution of the symbol $x_n$ via phase tracking, and its priori distribution $P_n^{\tr{a}}(a), a\in\mcA$  (obtained from the decoder).}
\label{fig:graph.tracking}
\end{figure}
%%%%%%%%%%%%%%%

Our goal now is to find $P_n(a), a\in\mcA$ exploiting the relationships between the involved random variables.  

As in \cite{Colavolpe05,Kreimer18}, we show in \figref{fig:graph.tracking} a graph which captures these relationships: the squares represent the functions taking as arguments the variables which, in turn, are represented by the directly connected circles. In particular
\begin{align}
\label{f.n.x}
g_n(\theta_n,x_n)  & \propto f(y_n|x_n,\theta_n) \\
&\propto \exp\left(-\SNRrv\Big|y_n-x_n\e^{\jmath\theta_n}\Big|^2\right)
\end{align}
corresponds to the relationship defined in \eqref{y.kn}, where we use $\pdf(\cd|\cd)$ to denote the conditional \gls{pdf}; the model \eqref{theta.Wiener} yields 
\begin{align}\label{p.w}
q(\theta_n,\theta_{n+1}) &\propto \pdf(\theta_n|\theta_{n+1})\propto\pdf( \theta_{n+1} | \theta_{n} )\\
&=\omega(\theta_n-\theta_{n+1}),
\end{align}
with
\begin{align}\label{Normal.pdf}
\omega(\theta)=\frac{1}{\sqrt{2\pi \sigma^2_w}}\sum_{k=-\infty}^{\infty}\exp\left(-\frac{(\theta-k2\pi)^2}{2\sigma^2_w}\right)
\end{align}
being a zero-mean, wrapped Gaussian distribution defined over any interval of length $2\pi$.

In \figref{fig:graph.tracking} we also show a shaded rectangle labeled as ``modulation/coding graph''; it also contains a graph which describes the relationship $\set{x_n}  \rightarrow \set{s_n} \rightarrow \set{c_n} \rightarrow \set{b_n}$, and its knowledge is used for the demodulation (to implement \eqref{lambda.n.l}) and for the decoding.

If the phase tracking has to be carried out and no decoding was not yet executed,  the payload symbols $x_n$ are assumed to be \gls{iid}, with non-informative a priori distribution over the transmitted symbols, \ie $P^{\tr{a}}_n(a)\propto 1$. In a case we would like  to perform the joint decoding/demodulation/phase tracking, as done, \eg in \cite{Colavolpe05,Kreimer18,Alfredsson19}, we use $P^{\tr{a}}_n(a)$ obtained from the decoding results. 

Thus, from the point of view of the phase tracking, the relationships induced by the modulation/coding graph are summarized by $P^{\tr{a}}_n(a)$. As a direct consequence, the graph we deal with in \figref{fig:graph.tracking} is a tree, \ie contain no loops. Therefore, the efficient marginalization can be done exactly by the \gls{mp} algorithm as follows \cite{Colavolpe05}, \cite{Shayovitz16}, \cite{Kreimer18}
\begin{align}\label{P.n.x}
P_n(a) \propto\int_{-\pi}^{\pi}  \alpha_n(\theta)  \beta_n(\theta) g_n(\theta,a ) \dd \theta,\quad a\in\mcA,
\end{align}
where
\begin{align}\label{alpha}
\alpha_n(\theta)&\propto \big(\alpha_{n-1}(\theta)  \gamma_{n-1}(\theta)\big) \convop 
\omega(\theta),\\
\label{beta}
\beta_n(\theta)&\propto \big(\beta_{n+1}(\theta) \gamma_{n+1}(\theta) \big) \convop 
\omega(\theta),\\
\label{gamma}
\gamma_n(\theta)&\propto\sum_{a\in\mcA} P^{\tr{a}}_n(a) g_{n}(\theta,a ),%=\sum_{x\in\mcA}  g_{n}(\theta,a ),
\end{align}
are (proportional to) the marginal distributions of the phase $\theta_n$ conditioned, respectively, on $y_0,\ld,y_{n-1}$, on $y_{n+1},\ld,y_{N}$, and  on $y_n$.\footnote{That is,
\begin{align}
\alpha_n(\theta)&\propto\pdf(\theta_n| y_0,\ld,y_{n-1})\\
\beta_n(\theta)&\propto\pdf(\theta_n| y_{n+1},\ld,y_{N})\\
g_n(\theta,a)&\propto\pdf(\theta_n| y_{n},a)
\end{align}
and thus the integrand in \eqref{P.n.x} is the posterior distribution of the phase
\begin{align}
\pdf(\theta_n | \by, a)&\propto
 \alpha_n(\theta)  \beta_n(\theta) g_n(\theta,a ) 
\end{align}
while $P_n(a)$ is given by \eqref{P.n.a.x}.

} All the distributions of the phase are periodic and so is the convolution in \eqref{alpha} and \eqref{beta}. 
%These equations are practically the same as those appearing in the \gls{bcjr} recursion \cite{BCJR} well known in the area of decoding of convolutional codes to obtain the distribution of the bits, which has discrete argument. Here, derived from the graph representation, they are applied to calculate the continuous-argument distributions of the phase. 

%%%%%%%%%
\section{Parametric message passing}\label{Sec:Parametric.MP}
The operations \eqref{P.n.x}-\eqref{gamma} which allow us to calculate $P_n(a)$ may be implemented on the discretized versions of the distributions $\alpha_n(\theta)$, $\beta_n(\theta)$, and $\gamma_n(\theta)$ defined over the samples of $\theta\in(-\pi, \pi]$. In such a \gls{dmp} the multiplications and additions are straightforward to implemented and the convolution is efficiently implemented via \gls{fft}. 

However, to ensure sufficient precision of the discretization, a large number of samples, $N_{\theta}$, may be needed.\footnote{\label{foot:N8} The literature often used $N_\theta=8M$ \eg \cite{Peleg00,Colavolpe05,Shayovitz16,Kreimer18} but finding the smallest $N_{\theta}$ which ensures the sufficient accuracy of the \gls{mp}, \eqref{alpha}-\eqref{gamma}, is difficult. 

The general rule is that all the distributions involved in the \gls{mp} should be represented without ``significant'' loss of accuracy so the sampling step should decrease when the spectral support of the distributions increases. 

Then, by approximating the distributions by Gaussians, we know that their spectral support is proportional to their precision (inverse of the variance). Thus, observing that the precision of $g_n(\theta,a)$ increases with the \gls{snr}, see also \eqref{f.n.x.Tikh}-\eqref{z.fn}, and the precision of $\omega(\theta)$ decreases with $\sigma_w^2$, we may conclude that the number of samples will grow when we increase the \gls{snr} or when we decrease the phase-noise level. These operational conditions are also required to transmit reliably high-order constellations. So, indeed, we should expect that the $N_\theta$ will grow with $M$ but we are not aware of any formal study backing up the heuristics $N_\theta=8M$ (that turned out unnecessarily conservative in our case, see Footnote~\ref{foot:DMP32} in \secref{example.start}.).
%, which is where the impact of the \gls{dmp} complexity will be the most notable. In such a case, the simplification may be sought by limiting the period over which the distribution must be represented \cite{ShahMohammadian18}.
}  Since this implies a large computational complexity as well as a storage requirements, many previous works have gone in the direction of parametric representation of the involved periodic distributions. Then, instead of tracking the samples in \gls{dmp}, we only need to track (a few) parameters which represent the distributions. 

We thus should find a family of the distributions, $\mcF$, on which the operations defined in \eqref{P.n.x}-\eqref{gamma} are easily dealt with. In particular, we have to handle multiplication of the periodic functions as well as, the convolution in \eqref{alpha} and \eqref{beta}; the integration in \eqref{P.n.x}, when done on the parametric forms of distributions, is usually straightforward.

In other words, if $\alpha_n(\theta), \beta_n(\theta), \gamma_n(\theta), \omega(\theta)\in\mcF$  and $\mcF$ is closed under  multiplication and convolution, the parametric \gls{mp} will be immediately obtained. This condition,  however, does not materialize with the most popular circular distributions such as the wrapped Gaussian distributions or  the Tikhonov distributions \cite{Kurz16}. Namely, the space of wrapped Gaussian distributions is not closed under multiplications, while the Tikhonov space is not closed under convolution. Thus, independently of the choice we make, approximations will be necessary.

%%%%%%%%%
%\subsection{Tikhonov distributions}\label{Sec:Tikh.dist}
In this work we consider a family of  Tikhonov distributions which were already used, \eg in \cite{Colavolpe05,Barbieri07,Shayovitz16}, and are defined as
\begin{align}\label{Tikh.definition}
\mcT(\theta; z)= \frac{\e^{\Re[z\e^{-\jj \theta}]}}{2\pi I_0(|z|)},
\end{align}
where $\Re[\cd]$ denotes the real part and $I_0(\cd)$ is the zero-th order modified Bessel function; $z$ is a complex parameter whose phase is the circular mean of the underlying variable and the value of $|z|$ is, approximatively, a measure of precision \cite{Kurz16}.

The closeness of $\mcF$ under multiplication is then obvious
\begin{align}\label{Tikh.multiplication}
\mcT(\theta; z_1)\mcT(\theta; z_2)
&=\frac{I_0(|z_1+z_2|)}{2\pi I_0(|z_1|)I_0(|z_2|)}
\mcT(\theta; z_1+z_2),
\end{align}
while the convolution with the Gaussian, appearing in \eqref{alpha} and \eqref{beta}, must be treated via  approximations as done before \cite[Appendix]{Colavolpe05} and also explained using the concept of a \gls{cmm} in \appref{conv.T.G}
\begin{align}\label{Tik.h.Normal.convolution}
\mcT(\theta; z)&\convop\omega(\theta)
\approx  \mcT\Big( \theta; \frac{z}{1+\sigma_w^2|z|} \Big).
\end{align}

We also note that $g_n(\theta,a) \in \mcF$, so \eqref{f.n.x} can be rewritten as
\begin{align}\label{f.n.x.Tikh}
g_n(\theta,a)&\propto \e^{\xi_{g,n}(a)}\mcT\big(\theta; z_{g,n}(a)\big) \\
\label{z.fn}
z_{g,n}(a)&=2\frac{y_n a^{*}}{\No}\\
\label{xi.f.n}
\xi_{g,n}(a)&=%\e^{ -\frac{|a|^2}{\No} }I_0\big(|z_{g,n}(a)|\big)=
-\frac{|a|^2}{\No} +\hat{I}_0(|z_{g,n}(a)|),
%\eta_{g,n}(a)&=-\frac{|a|^2}{\No} + |z_{g,n}(a)| + \hat{I}_0\big(|z_{g,n}(a)|\big),
\end{align}
where, to avoid numerical issues due to the exponential grows of $I_0(\cd)$ we use its log-version
\begin{align}\label{hat.I0}
\hat{I}_0(x) &= \log I_0(x) = x  + \Delta(x),
\end{align}
with $\Delta(x)$ being the log-domain corrective factor.\footnote{The approximation $\Delta(x)\approx -\frac{1}{2}\log(2\pi x)$ is tight for large $x$ \cite[Eq.~(96)]{Shayovitz16}\cite[Eq.~(18)]{Pecorino15}  but does not apply for small arguments because $\Delta( 0 )=0$. Thus, for a better accuracy, $\Delta(x)$ may be implemented via lookup table. On the other hand, it is also possible to simply set $\Delta(x)\approx 0$.}

Instead of Tikhonov family we might opt for the wrapped Gaussians \eqref{Normal.pdf} but 
\begin{itemize}
\item We have to start using approximations already for $g_n(\theta,a)$ which is naturally represented by a Tikhonov distribution in \eqref{f.n.x.Tikh} but would have to be replaced by the approximating Gaussian; this can be done, of course, \eg as in \cite{Kreimer18}, but requires the introduction of additional layer of approximations before the \gls{mp} is derived;
\item To  take care of their periodic nature, particular attention is required when dealing with multiplication  \cite[Sec.~II.B]{Kurz16}; this aspect is not always emphasized in the literature: in some works,  the Gaussian distributions are used without explicit wrapping. Ignoring the circularity, it produces an apparent closeness under multiplication but may lead to interpretation errors when ``locking'' on the wrong phase, see example in \cite[Fig.~1]{Kurz16}; and 
\item Comparing to the Tikhonov distributions, Gaussians are less well suited to represent the uniform or almost-uniform distributions of the phase.\end{itemize}


%%%%%%%%%
Having defined the family $\mcF$ we want to use, we have to recognize that the main difficulty of the parametric \gls{mp} stems from the presence of $\gamma_n(\theta)$  which is a mixture of Tikhonov distributions which  we rewrite as
\begin{align}\label{gamma.def.mixture}
\gamma_n(\theta)&\propto\sum_{a\in\mcA}\e^{\eta_{g,n}(a)}\mcT\big(\theta;z_{g,n}(a )\big),\\
\label{eta.f.n}
\eta_{g,n}(a)&=-\frac{|a|^2}{\No}+ \hat{I}_0\big(|z_{g,n}(a)|\big)+\hat{P}^{\tr{a}}_n(a),
\end{align}
where we again use $\hat{P}^{\tr{a}}_n(a)=\log P^{\tr{a}}_n(a)$ because the logarithmic representation simplifies the implementation.

There are essentially two approaches that have been used in the literature to deal with this issues and we compare them in the following.

%%%
\subsection{Pre-MP approximation: \acrshort{cbc} algorithm}\label{Sec:Pre-MP}

In this approach, taking advantage of the fact that $\gamma_n(\theta)$ is not obtained recursively, its approximation, $\tilde{\gamma}_n(\theta)$ is obtained \emph{before} the steps of \gls{mp} \eqref{alpha}-\eqref{beta} are executed. This may be seen as the following approximate ``projection'' of the \gls{rhs} of \eqref{alpha} on $\mcF$:
\begin{align}
\label{alpha.projection.preMP}
\alpha_n(\theta)&\propto \mcF\left[\big(\alpha_{n-1}(\theta)  \gamma_{n-1}(\theta)\big) \convop  \omega(\theta)\right]\\
\label{alpha.projection.preMP.1}
&\approx \mcF\left[\alpha_{n-1}(\theta)  \gamma_{n-1}(\theta)\right] \convop  \omega(\theta)\\
\label{alpha.projection.preMP.2}
&\approx \big(\alpha_{n-1}(\theta)  \mcF[\gamma_{n-1}(\theta)]\big) \convop  \omega(\theta)\\
\label{alpha.projection.preMP.3}
&= \big(\alpha_{n-1}(\theta)  \tilde\gamma_{n-1}(\theta)\big) \convop  \omega(\theta)
\end{align}
where, 
\begin{align}\label{gamma.projection.first}
\tilde{\gamma}_n(\theta)
&=\mcF[\gamma_n(\theta)]=\mcT\Big(\theta;  z_{\tilde{\gamma},n} \Big)\\
&=\mcF\Big[ \sum_{a\in\mcA}\e^{\eta_{g,n}(a)}\mcT\big(\theta;z_{g,n}(a )\big) \Big],
\end{align}
and, with a slight abuse of notation we use $\mcF[\cd]$ to denote the operator which  projects $\gamma_n(\theta)$ onto the Tikhonov family $\mcF$. To pass from \eqref{alpha.projection.preMP} to \eqref{alpha.projection.preMP.1} we used (approximate) closeness of $\mcF$ with respect to convolution and this approximation holds well. On the other hand, to pass from  \eqref{alpha.projection.preMP} to \eqref{alpha.projection.preMP.1} we used the   approximation $\mcF\left[\alpha_{n-1}(\theta)  \gamma_{n-1}(\theta)\right]\approx \alpha_{n-1}(\theta)\mcF\left[\gamma_{n-1}(\theta) \right]$ that holds only if $\gamma_n(\theta)\in\mcF$. This is not the case, of course, but in this way we can precalculate $\tilde{\gamma}_n(\theta)$ before the \gls{mp} recursion starts.

To carry out the projection in \eqref{gamma.projection.first} Colavolpe, Barbieri and Caire \cite{Colavolpe05} proposed to approximate $\gamma_n(\theta)$ with $\tilde{\gamma}_n(\theta)\in\mcF$ by,  first matching a Gaussian to $\pdf(y_n|\theta_n,a)\propto g_n(\theta,a)$ from which a Tikhonov distribution was derived as \cite[Sec.~IV.B]{Colavolpe05}
\begin{align}
\label{hat.z.gamma}
\tilde{\gamma}_n(\theta)
&=\mcT\Big(\theta;  z_{\tilde{\gamma},n} \Big)\\
z_{\tilde{\gamma},n}&=
\begin{cases}
z_{g,n}(x_n)  & \text{if}\quad n= l L\\
2\frac{y_n\mfm_n^{*}}{\No+ \mfv_n}, & \text{if}\quad n\neq l L
\end{cases}
\end{align}
where 
\begin{align}
\label{m.n.A}
\mfm_n&=\sum_{a\in\mcA}  a P^{\tr{a}}_n(a) ,\quad%\label{v.n.A}
\mfv_n=\sum_{a\in\mcA}  |a|^2 P^{\tr{a}}_n(a)   -  |\mfm_n|^2,
\end{align}
are the mean and the variance of $x_n$. 

The approximation is needed only for the payload positions, $n\neq lL$. For the pilots $x_n, n=lL$, we have $\gamma_n(\theta)=g_{n}(\theta, x_{n} )$ so we can use directly the parameter of the Tikhonov distribution $z_{g,n}(x_n)$.

This \gls{ga} approach was often reused in the literature, \eg \cite{Barbieri07,Pecorino15,Alfredsson19} as the integral part of the \gls{cbc} algorithm. 

On the other hand, recognizing that the distribution \eqref{gamma.def.mixture} is circular, instead of the \gls{ga}  we may apply the \gls{cmm}. It relies on minimization of the \gls{kl} distance between $\tilde{\gamma}_n(\theta)$ and the mixture $\gamma_n(\theta)$, and changes the way the parameter $z_{\tilde{\gamma},n}$ is calculated, which we express as follows
\begin{align}
%\tilde{\gamma}_n(\theta)
%&=\mcT\Big(\theta;  z_{\tilde{\gamma},n} \Big)\\
%&=\mcF\Big[ \sum_{a\in\mcA}\e^{\eta_{g,n}(a)}\mcT\big(\theta;z_{g,n}(a )\big) \Big],\\
\label{gamma.projection.first.cases}
z_{\tilde{\gamma},n}
&=
\begin{cases}
z_{g,n}(x_{n}) &\text{if}\quad n= l L\\
\mf{CMM}\Big[ \big\{\eta_{g,n}(a), z_{g,n}(a)\big\}_{a\in\mcA}  \Big]&\text{if}\quad n\neq l L,
\end{cases}
\end{align}
where the dependence of $z_{\tilde{\gamma},n}$ on  $\eta_{g,n}(a)$ and $z_{g,n}(a)$, indexed by $a\in\mcA$  is defined in closed-form by a function $\mf{CMM}[\cd]$ shown in \appref{Sec:CMM}. %and which  follow closely \cite[Appendix~A]{Shayovitz16}. 

Next, since all the distributions are from the Tikhonov family, \ie $\alpha_n(\theta)=\mcT(\theta;z_{\alpha,n})$ and $\beta_n(\theta)=\mcT(\theta;z_{\beta,n})$, replacing $\gamma_n(\theta)$ with $\tilde{\gamma}_{n}(\theta)$ (as defined in \eqref{hat.z.gamma} or \eqref{gamma.projection.first})  and applying \eqref{Tikh.multiplication} and \eqref{Tik.h.Normal.convolution}, we obtain the following parametric \gls{mp} :
\begin{align}
\label{z.alpha.init}
z_{\alpha,0}&=0,\\
\label{z.alpha}
z_{\alpha,n}&= \frac{z_{\alpha,n-1} + z_{\tilde{\gamma},n-1}}{1+|z_{\alpha,n-1} + z_{\tilde{\gamma},n-1}|\sigma_w^2}, \quad n=1, \ld,N-1\\
\label{z.beta.init}
z_{\beta,N}&=0,\\
\label{z.beta}
z_{\beta,n}&= \frac{z_{\beta,n+1} + z_{\tilde{\gamma},n+1}}{1+|z_{\beta,n+1} + z_{\tilde{\gamma},n+1}|\sigma_w^2}, \quad n=N-1,\ld,1,
\end{align}
which is exactly equivalent to the \gls{cbc} algorithm defined in \cite[Eq.~(36)-(37)]{Colavolpe05} and  is provided for completeness and as a starting point for the discussion.

Using \eqref{Tikh.multiplication}  and \eqref{f.n.x.Tikh}--\eqref{xi.f.n} in \eqref{P.n.x}, the ``extrinsic'' symbol probabilities are also calculated as \cite[Eq.~(35)]{Colavolpe05}
\begin{align}\label{P.a.final}
P_n( a )&\propto \int_{0}^{2\pi} \mcT(\theta;z_{\Sigma,n}(a))\frac{\e^{\xi_{g,n}(a)} I_0\big(|z_{\Sigma,n}(a) |\big)}{I_0\big(|z_{g,n}(a)|\big)}\dd \theta,\\
\label{P.a.final.2}
\hat{P}_n( a )&=-\frac{|a|^2}{\No} + \hat{I}_0\big(|z_{\Sigma,n}(a)|\big),\\
\label{z.Sigma.n}
z_{\Sigma,n}(a)&=z_{\alpha,n}+z_{\beta,n}+2\frac{y_n a^{*}}{\No},
\end{align}
and the log-probability $\hat{P}_n( a )=\log P_n( a )$ should be next used in \eqref{lambda.n.l}.

Due to its simplicity, the \gls{cbc} algorithm \eqref{z.alpha.init}-\eqref{z.beta}, should be treated as a ``canonical'' solution to the problem of phase tracking: it is explicit and requires no fine-tuning. This explains the considerable attention it received up to now.

Before going further, we note that the difference between the original formulation of the \gls{cbc} algorithm in \cite{Colavolpe05} and this work appears in the way the approximate distribution $\tilde{\gamma}_n(\theta)$ is obtained, that is, whether we opt for the \gls{ga} \eqref{hat.z.gamma}-\eqref{m.n.A}, or we use the \gls{cmm} from \eqref{gamma.projection.first}-\eqref{gamma.projection.first.cases}. 

Although the \gls{cmm} was already used in the context of the phase tracking by \cite{Shayovitz16}, we are not aware of it being applied as a part of the \gls{cbc} algorithm. And while the implementation of the function $\mf{CMM}[\cd]$ is slightly less straightforward\footnote{Approximations of non-linear functions are involved, see \appref{Sec:CMM} and \appref{Sec:Bx}.} than the \gls{ga} shown in \eqref{hat.z.gamma}-\eqref{m.n.A}, we will soon compare the \gls{cmm} to the \gls{ga} and show the obvious advantage produced by the former. 


%we clarify its impact in \secref{example.start} and show that  the important improvement in performance justifies the use of the \gls{cmm} in the \gls{cbc} algorithms.

An important observation, already made \eg in \cite[Sec.~I]{Shayovitz16} or \cite[Sec.~IV]{Pecorino15}, is that, using a non-informative prior $\hat{P}^{\tr{a}}(a)\propto 0$,  the approximation $\tilde{\gamma}_n(\theta)$ is also non-informative for the payload symbols; that is, \mbox{$z_{\tilde{\gamma},n}=0, n\neq lL$}.\footnote{If  the \gls{ga} \eqref{hat.z.gamma}-\eqref{m.n.A}, is used,  this is true, if the constellation $\mcA$ is zero mean, which is obvious from \eqref{m.n.A}. On the other hand, if the \gls{cmm} approach is used, this is true for constellations $\mcA$ which may be decomposed into constant modulus zero-mean sub-constellations; the demonstration is easy and omitted for sake of space. For the most popular constellations such as $M$-\gls{qam}, both conditions hold.} 

Since then, the only useful information is obtained from the non-zero $z_{\tilde{\gamma},n}$ (\ie from the pilots), the \gls{mp} in \eqref{z.alpha.init}-\eqref{z.beta} may be then seen as a \emph{pilot-only} based recursive estimation of the phase. 

In fact, it is independent of the form of the constellation $\mcA$ used to modulate the payload symbols and this is why, in order to exploit the knowledge of $\mcA$, the \gls{cbc} phase tracking must be placed in the ``decoding-loop''. Known also as the joint phase tracking and decoding, it consists in alternate execution of  i)~the \gls{mp}  \eqref{z.alpha.init}-\eqref{z.beta} and ii)~the demodulation/decoding; the latter, providing an informative prior $\hat{P}^{\tr{a}}_n(a)$ on the payload symbols, improves the phase tracking, see \eg \cite{Colavolpe05,Barbieri07,Alfredsson19}.

\subsection{Intra-MP projection}\label{Sec:Intra-MP}

As we said, the disadvantage of the pre-\gls{mp} projection from \secref{Sec:Pre-MP} is that, without the decoder's feedback, the structure of the constellation $\mcA$ is ignored. In order to exploit the form of $\mcA$, \cite{Shayovitz16,Kreimer18} perform the projection on $\mcF$ \emph{after} the multiplications in \eqref{alpha}-\eqref{beta} are executed. In other words,  the approximations \eqref{alpha.projection.preMP.1} is used
\begin{align}\label{alpha.projection}
\alpha_n(\theta)&\propto 
\label{alpha.projection.3}
 \mcF\big[\alpha_{n-1}(\theta)\gamma_{n-1}(\theta)\big]\convop \omega(\theta)\\
&\approx \check{\alpha}_{n-1}(\theta) \convop \omega(\theta),\\
\label{beta.projection}
\beta_n(\theta)&\propto 
\mcF\big[\beta_{n+1}(\theta)\gamma_{n+1}(\theta)\big]  \convop  \omega(\theta)\\
&\approx\check{\beta}_{n+1}(\theta)\convop  \omega(\theta),
\end{align} 
where we define the ``auxiliary'' distributions obtained via projections
\begin{align}
\nonumber
\check{\alpha}_{n}(\theta)&=\mcT\big(\theta; z_{\check{\alpha},n}\big)\\%\mcF\big[\alpha_{n-1}(\theta)\gamma_{n-1}(\theta)\big]\\
\label{check.alpha}
&=\mcF\left[\sum_{a\in\mcA} P^{\tr{a}}_{n}(a) \alpha_{n}(\theta)g_{n}(\theta, a )\right]\\
\label{z.alpha.check}
z_{\check{\alpha},n}&=\mf{CMM}\Big[\big\{\eta_{g,n}(a), z_{\alpha,n}+z_{g,n}(a)\big\}_{a\in\mcA} \Big].
\end{align}
and
\begin{align}
\nonumber
\check{\beta}_{n}(\theta)&=\mcT\big(\theta; z_{\check{\beta},n}\big)\\%\mcF\big[\beta_{n+1}(\theta)\gamma_{n+1}(\theta)\big]\\
\label{check.beta}
&=\mcF\left[ \sum_{a\in\mcA} P^{\tr{a}}_{n}(a) \beta_{n}(\theta)g_{n}(\theta, a )  \right],\\
\label{z.beta.check}
z_{\check{\beta},n}&=\mf{CMM}\Big[\big\{\eta_{g,n}(a), z_{\beta,n}+z_{g,n}(a)\big\}_{a\in\mcA} \Big].
\end{align}

Using \eqref{Tik.h.Normal.convolution} in \eqref{alpha.projection.3} and \eqref{beta.projection} we obtain the following parametric \gls{mp}:
\begin{align}
z_{\alpha,0}&=0,\\
z_{\alpha,n}&= \frac{z_{\check{\alpha},n-1}}{1+|z_{\check{\alpha},n-1}| \sigma_w^2}, \quad n=1, \ld,N-1\\
z_{\beta,N}&=0,\\
z_{\beta,n}&= \frac{z_{\check{\beta},n-1}}{1+|z_{\check{\beta},n-1}| \sigma_w^2}, \quad n=N-1,\ld,1.
\end{align}

We need to carry now the projection twice for each time $n$ which increases the computational burden comparing to the \gls{cbc} algorithm. The hope is that, introducing approximations (projection) inside the \gls{mp} recursion we minimize the approximation error.



%%%%%%%%%%%%%%
\begin{figure}[bt]
\begin{center}
\psfrag{DMPXXX}[lc][lc][\siz]{DMP}
\psfrag{CBC+GA}[lc][lc][\siz]{CBC+GA \cite{Colavolpe05}}
\psfrag{CBC+CMM}[lc][lc][\siz]{CBC}
\psfrag{AWGN}[lc][lc][\siz]{AWGN}
\psfrag{All-pilots}[lc][lc][\siz]{All-pilots}
\psfrag{ylabel}[lc][lc][\siz]{$\PER$}
\psfrag{xlabel}[lc][lc][\siz]{$\SNRrv$ [dB]}
\scalebox{\sizf}{\includegraphics[width=\linewidth]{./figures/PER_Tikh_Ex1_Rev.eps}}
\end{center}
\caption{\gls{per} vs. \gls{snr} obtained using  \gls{cbc} algorithm with the projection based on the \acrfull{ga} originally proposed in \cite{Colavolpe05} (CBC+GA) or, on the \gls{cmm} explained in \appref{Sec:CMM} (CBC), both shown for the scheduling $\set{I_\tr{dec}\times 1}$ with $I_\tr{dec}=10$ (filled markers, solid lines) and $I_\tr{dec}=30$ (hollow markers, dashed lines); the encoding rate of the \gls{ldpc} is $r=\frac{7}{8}$.  The \acrfull{dmp} is implemented using $N_{\theta}=64$ samples, the ``AWGN" curve assumes no phase noise, and ``All pilots'' curve is the performance limits for any joint phase tracking and decoding, see explanation in \secref{example.start}.}\label{fig:PER.preMP}
\end{figure}
%%%%%%%%%%%%%%

\section{Example: Phase tracking reference results}\label{example.start}
%\begin{example}[Phase tracking: reference scenario]
This separate section discusses properties of the previously deployed algorithms especially comparing their one-shot operation to the iterative processing (joint demodulation and decoding).

We considers transmission based on $16$-\gls{qam} constellation with Gray mapping \cite[Sec.~2.5.2]{Szczecinski_Alvarado_book}; the proprietary \gls{ldpc} encoder with the rate $r=\frac{7}{8}$ produces the block of $\Nc=4032$ bits. The pilot symbols are pseudo-randomly drawn from a $4$-\gls{qam} constellation; the pilot spacing is set to $L=25$ which allows us to place $L-1=24$ payload symbols between pilots, see \eqref{payload.1}, so dummy symbols are not needed to fill the frame of transmitted symbols $\bx$; we thus have $F=43$ pilots and total $N=1051$ symbols. The phase noise is generated with $\sigma_w^2=0.01~\tr{rad}^2$ or--equivalently, $\sigma_w=0.1~\tr{rad}\approx 5.7~\tr{deg}$. This test scenario  will be also reused later.

The \acrfull{per}, shown in \figref{fig:PER.preMP} is estimated after transmitting $10^5$ blocks or after occurence of $100$ blocks in error, whichever comes first. In all cases the total number of decoding iterations is or $I^{\Sigma}_\tr{dec}=10$ (solid markers) or $I^{\Sigma}_\tr{dec}=30$ (hollow markers); the decoding is based on the min-sum algorithm.\footnote{With scaling of the check-nodes messages by a constant factor equal to $\rho=0.7$, see \cite{Xu14}; then, a fraction of dB loss was observed when comparing to the sum-product algorithm in the \gls{awgn} channel.}   

The \gls{dmp} is implemented using $N_\theta=64$ samples\footnote{\label{foot:DMP32}The numerical results obtained for $N_\theta\in\set{32,64,128}$ were practically indistinguishable but a significant deterioration of the results was observed for $N_\theta=16$. This seems to indicate that the heuristics  $N_\theta=8M$ used \eg in \cite{Peleg00,Colavolpe05,Kreimer18} may be too conservative but solving this issue is out of scope of our work.} and its \gls{per} curve is the performance limit for all ``one-shot'' phase tracking algorithms, \ie those defined by the scheduling \mbox{$\set{1\times I_\tr{dec}}$}.

The curve ``All-pilots'' is obtained assuming that, during the phase-tracking, all the symbols in $\bx$ are pilots. This corresponds to a situation when the output of the decoder provides highly reliable information about the bits which gives certainty about the symbols $\bx$ (that is, $P^{\tr{a}}_n(a)\approx 1$ for $a=x_n$); these, in turn, become de facto pilots allowing for the best possible phase tracking. 

Then, when calculating $\hat{P}_n(a)$, the only uncertainty about the symbol $x_n$ is caused by the \gls{awgn} as well as  by the residual phase noise -- this part of it which cannot be estimated from other symbols $x_l, l\neq n$. The ``All-pilots" curve is a performance limit for all joint phase-tracking and demodulation/decoding algorithms we study here.\footnote{More precisely, for all those algorithms which do not use the decoder's feedback in the \gls{llr} calculation in \eqref{lambda.n.l}; see comments at the end of \secref{sec:model}.} If the \gls{dmp} is too complex to implement, the ``All-pilots" curve may be treated as its proxy. 

On the other hand, the ``AWGN'' curve corresponds to a hypothetical scenario when the phase-noise is removed and we only deal with the \gls{awgn}. Such results are unattainable no matter how sophisticated the phase-tracking and decoding strategy are, and we show them to illustrate the impact of the phase noise.

The demodulation/phase-tracking algorithms which use the decoder's feedback are referred to as ``iterative'' and those which don't as ''one shot" algorithms. \ls{Unless stated otherwise} in the iterative algorithms we deliberately limit our considerations to the particular form of scheduling of operations between the demodulator and the decoder: each demodulation operation is followed by one decoding iteration. This is not necessarily the best solution but was extensively used in the literature, \eg \cite{Colavolpe05,Shayovitz16,Kreimer18}. The decoder's state (captured by the internal messages from the check to variables nodes) is, of course, preserved between iterations. 

We observe the following
\begin{itemize}
\item The (\gls{per} of the) original \gls{cbc} algorithm from \cite{Colavolpe05} (CBC+GA) tends to saturate for high \gls{snr}, \ie where the phase noise dominates the \gls{awgn}. This effect seems to be difficult to remove by increasing the number of iterations (by changin $I_\tr{dec}=10$ to $I_\tr{dec}=30$ the error floor remained the same, \cite[Fig.~2]{Szczecinski20b}). We attribute this behaviour, observed already \eg in \cite[Fig.~8]{Kreimer18}, to the particular form of scheduling, where, after each decoding iteration, $\tilde{\gamma}_n(\theta)$ is estimated afresh even if the first decoding iterations do not provide reliable estimates of the coded bits. This, in turn, may yield unreliable $\hat{P}^\tr{a}(a)$, hence unreliable $\tilde{\gamma}_n(\theta)$ which, in turn stalls the convergence. %\ls{To verify this hypothesis, we show the \gls{per} for the scheduling $\mfS=\set{1\times \I_\tr{dec}}$. For low \gls{snr}, it is obviously worse than the \gls{cbc} (+GA) algorithm. On the other hand, it does not display the error floor at the same level as the \gls{cbc}.}
\item The notable difference between the original \gls{cbc} algorithm (\gls{cbc}+\gls{ga}) and the \gls{cbc} algorithm based on the \gls{cmm} (\gls{cbc}) emphasizes the importance of the approximations we make in the phase tracking: by using the \gls{cmm}, we significantly lower the operational \gls{snr}\footnote{The \gls{snr} necessary to attain a given \gls{per} target, \eg for  $\PER_\tr{t}=10^{-2}$, the \gls{snr} decreases by $2$dB.} and  the error floor in the high \gls{snr}.  Thus, all the remaining results are based on the \gls{cmm}. 
\item Irrespectively of the valuable improvement due to the application of the \gls{cmm}, the qualitative behaviour of the \gls{cbc} algorithms is the same: the error floor appears in the \gls{per} curve and the gap to the \gls{dmp} remains large.
\end{itemize}


%%%%%%%%%%%%%%%%%%%%
\subsection{Scheduling and complexity}\label{Sec:Sch.Cplx}

It may, therefore, be useful to define a \emph{scheduling} which specifies the number of iterations the \gls{ldpc} decoder executes before its outputs are transformed into $\hat{P}_n(a)$ and used again by the phase tracking \gls{mp}. 

Let the scheduling defined by $\set{I_{\tr{loop}}\times I_\tr{dec} }$ means the following: after each passage of the \gls{cbc} phase tracking, the decoder executes $I_{\tr{dec}}$ elementary decoding iterations\footnote{Defined as one check-nodes message update and one bit-nodes message update.}, then the phase tracking is implemented again and the results are used by the decoder executing $I_{\tr{dec}}$ elementary decoding iterations. This is repeated $I_\tr{loop}$ times so the total number of decoding iterations is given by $I^{\Sigma}_\tr{dec}=I_\tr{loop}\cd I_\tr{dec}$.

The scheduling from \cite{Colavolpe05} is defined by $\set{200 \times 1}$ meaning that the phase-tracking was executed $I_\tr{loop}=200$ times and, each phase-tracking was followed by one elementary decoding iterations; the total number of decoding iterations if thus $I_\tr{dec}^\Sigma=200$.

A ``one-shot'' phase tracking is denoted by the scheduling $\set{1\times I^{\Sigma}_\tr{dec}}$, and means that the phase tracking is carried out once and then all the decoding iterations are executed.

%In other words, the phase tracking is executed $I_\tr{loop}$ times, and the decoder executes $I_{\tr{loop}}} I_{\tr{dec}}$ elementary decoding iterations and, with that notation, the scheduling from \cite{Colavolpe05} is defined by ${200 \times 1}$ meaning that the phase-tracking was executed $200$ times and, each phase-tracking was followed by one elementary decoding iterations of the \gls{ldpc} decoder , while the scheduling $\set{2\times 100}$ from \cite{Alfredsson19} means that the \gls{cbc} phase tracking was executed twice and each was followed by $100$ decoding iterations. 

There are clearly many other possibilities to schedule the operations and they may affect the performance and the complexity. However,  caution should be applied when talking about the implementation complexity because it is difficult to compare  different operations: counting the additions/multiplications may be misleading especially when targeting implementation on the specialized circuits. 

For example, the operations necessary in the \gls{cmm} do not have the same implementation ``complexity'' as those required by the \gls{mp} \eqref{z.alpha.init}-\eqref{z.beta}; and it is difficult to compare any of these to the operations required by the elementary decoding iteration. However,  when operations are of the same type, they can be compared and provide a general idea about the complexity.


%The scheduling $I_{\tr{loop}}\times I_{\tr{dec}}$, means that  the \gls{ldpc} decoder carries out $I_{\tr{dec}}$ iterations and $I_{\tr{loop}}$ is the number of outer-loop iterations, \ie the number of times the phase tracking results are fed to the decoder.



%%%%%%%%%%%%%%%%%%%%%
\section{Expectation Propagation:\\Self-iterations in the phase-tracking}\label{Sec:It.EP}

The example in \secref{example.start}, showing the improvement in performance obtained by replacing the \gls{ga} proposed originally in \cite{Colavolpe05} with the \gls{cmm}, demonstrates that a reliable phase-tracking may significantly improve the performance (\ie decrease the \gls{per}). 

Along the same light of thought, comparing the performance of the \gls{cbc} algorithm with the one-shot phase-tracking of the \gls{dmp}, indicates that satisfactory solutions may be obtained without relying on the decoders' feedback. Therefore, our goal now is to develop a  reliable and ``standalone'' (which can operate without decoder's feedback) phase tracking by exploiting the form of the constellation $\mcA$.

A similar idea was followed in  \cite{Shayovitz16} where the original mixture  $\gamma_n(\theta)$ \eqref{gamma} was used in \eqref{alpha} and \eqref{beta} and the results of multiplication $\alpha_n(\theta)\gamma_n(\theta)$ and $\beta_n(\theta)\gamma_n(\theta)$  were  projected on the space of Tikhonov mixtures $\mcF$. In this way, the projection $\mcF[\cd]$ is moved ``inside" the \gls{mp}; this improves the performance but, requires more projetions and thus increases the complexity comparing to the \gls{cbc} algorithm. Similar principle was explored in \cite{Kreimer18} but using the Gaussian family $\mcF$.

Here, we follow the idea of the \gls{cbc} algorithm motivated by the extreme simplicity of the forward-backward \gls{mp} \eqref{z.alpha.init}-\eqref{z.beta} which amounts to non-linear recursive filtering. Thus, unlike  \cite{Shayovitz16,Kreimer18}, rather than moving the projection inside the \gls{mp}, we want to enhance the approximations $\tilde{\gamma}_n(\theta)$ and preserve the structure of the \gls{mp} \eqref{z.alpha.init}-\eqref{z.beta}.

To do this, we will improve $\tilde{\gamma}_n(\theta)$ iteratively; this will be done with ``self-iterations", that is without any help from the decoder: the priors $\hat{P}^\tr{a}(a)$ will not change during the self-iterations. 

To explain why this can be done we note that, although the phase tracking \gls{mp} is defined on the tree (graph) that is known to yield the optimal solution in one run (backward-forward processing),  this is only  true for the \gls{dmp} which tracks the entire (discretized) distributions. On the other hand, the \gls{mp} in the \gls{cbc} algorithm is based on approximated distribution $\tilde{\gamma}_n(\theta)$ and, therefore, such a guarantee of optimality does not exist.

We follow here the \gls{ep} idea \cite[Ch.~3.2]{Minka01} which addresses the very problem of using approximate distributions in the \gls{mp}. We will apply the projection $\mcF[\cd]$ many times (iteratively) taking into account the results obtained in previous iterations.  Since most of the resulting operations are almost identical to those we already defined in the \gls{cbc} algorithm, we will use the parenthesized superscript $^{(i)}$ to denote the variables/functions obtained in the $i$-th iteration, where $i=1,\ld, I_\tr{ep}$ and $I_\tr{ep}$ is the maximum number of \gls{ep} iterations.


\subsection{Expectation Propagation for the Phase Tracking}\label{Sec:EP.Ph.Track}
The \gls{ep} applied to our problem relies on the following idea: in the iteration $i$,  we find the approximation $\tilde{\gamma}^{(i)}_n(\theta)$ using the distributions $\alpha^{(i-1)}_n(\theta)$ and $ \beta^{(i-1)}_n(\theta)$ calculated in the previous iterations. This is done by  matching the posterior distribution of $\theta_n$, that would be obtained using $\tilde{\gamma}^{(i)}_n(\theta)$ to the one calculated from the original distribution $\gamma_n(\theta)$ 
\begin{align}
\nonumber
\tilde{\gamma}^{(i)}_n(\theta)\big(\alpha^{(i-1)}_n(\theta)&\beta^{(i-1)}_n(\theta)\big)\\
\label{equal.proba.approx}
&\approx
\gamma_n(\theta)\big(\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)\big)
\end{align}
and requires the projection  operation, $\mcF[\cd]$ to be applied to both sides of \eqref{equal.proba.approx}. 

Since the \gls{lhs} contains the three terms from the family  $\mcF$, it is not affected by the projection (remember, the product of the Tikhonov distributions is a also a Tikhonov distribution), we obtain
\begin{align}\label{equal.proba.approx.2}
\tilde{\gamma}^{(i)}_n(\theta)
&\propto
\frac{\mcF\Big[\gamma_n(\theta)\big(\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)\big)\Big]}
{\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)}.
\end{align}

Of course, for $i=1$, we deal with non-informative distributions $\alpha^{(0)}(\theta)\propto 1$ and $\beta^{(0)}(\theta)\propto 1$, which reduces \eqref{equal.proba.approx.2} to  $\tilde{\gamma}^{(1)}_n(\theta)=\mcF\big[ \gamma_n(\theta)\big]$; this is what was done in \secref{Sec:Parametric.MP}, \ie  $\tilde{\gamma}_n^{(1)}(\theta)$ is the same as $\tilde{\gamma}_n(\theta)$ obtained in \eqref{gamma.projection.first}.\footnote{Similarly, if we want to apply the projection operator, $\mcF[\cd]$, to each of the terms under multiplication in the numerator in \eqref{equal.proba.approx.2}, the result will be the same as the original \gls{cbc} algorithm: the projection  $\mcF\Big[\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)\Big]=\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)$ will cancel out with the denominator and iterative improvement will not be possible. This ``transparency" to the presence of $\alpha_n(\theta)$ and $\beta_n(\theta)$ is thus nothing but the conventional projection characteristic of the \gls{cbc} and here it is not useful, although it may provide satisfactory results in other context, \eg \cite{Vannucci20}.}

For $i>1$, the informative distributions, $\alpha^{(i-1)}_n(\theta)$ and $\beta^{(i-1)}_n(\theta)$ are available so we have to calculate the \gls{rhs} of \eqref{equal.proba.approx}
\begin{align}
%\nonumber
\gamma_n(\theta)\Big(\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)\Big)
\label{apost.theta.i1}
&=
\sum_{a\in\mcA} \e^{\eta^{(i-1)}_{\Sigma,n}(a)} \mcT\big(\theta; z^{(i-1)}_{\Sigma,n}(a) \big),
\end{align}
where, with proper sup-indexing in \eqref{z.Sigma.n},  we have $z_{\Sigma,n}^{(i-1)}(a)=z_{\alpha,n}^{(i-1)}+z_{\beta,n}^{(i-1)}+z_{g,n}(a)$ and
\begin{align}
\label{eta.Sigma.n.i1}
\eta^{(i-1)}_{\Sigma,n}(a)&=-\frac{|a|^2}{\No}+ \hat{I}_0\big(|z^{(i-1)}_{\Sigma,n}(a)|\big)+\hat{P}^{\tr{a}}_n(a)\\
&=\hat{P}^{(i-1)}_n(a)+\hat{P}^{\tr{a}}(a)
\end{align}
represents the posterior log-probability of the symbols obtained in the iteration $i-1$.

Using \eqref{apost.theta.i1} in the numerator of \eqref{equal.proba.approx.2} yields
\begin{align}\label{EP.iterations}
\tilde{\gamma}^{(i)}_n(\theta) 
&=\mcT(\theta; z^{(i)}_{\tilde{\gamma},n})\\
\label{EP.division}
&\propto \frac
{\mcF\Big[\sum_{a\in\mcA} \e^{\eta^{(i-1)}_{\Sigma,n} (a)} \mcT\big(\theta; z^{(i-1)}_{\Sigma,n}(a) \big)\Big] }
{\mcT\big(\theta; z^{(i-1)}_{\alpha,n}+z^{(i-1)}_{\beta,n} \big)}\\
\label{EP.division.2}
&= \frac{ \mcT\Big(\theta; z^{(i)}_{\tr{post},n}\Big)  }{ \mcT\Big(\theta; z^{(i-1)}_{\alpha,n}+z^{(i-1)}_{\beta,n} \Big)},
\end{align}
where 
\begin{align}
z^{(i)}_{\tr{post},n} &=\mf{CMM}\Big[ \eta^{(i-1)}_{\Sigma,n}(a), z^{(i-1)}_{\Sigma,n}(a)\big| a\in\mcA  \Big]
\end{align}
and thus
\begin{align}
\label{z.gamma.i}
z^{(i)}_{\tilde{\gamma},n}&= z^{(i)}_{\tr{post},n}  - \big(z^{(i-1)}_{\alpha,n} + z^{(i-1)}_{\beta,n}\big).
\end{align}

%%%%%%%%%%%%%%%
\subsection{Pitfalls  and solutions}\label{Sec:Pitfalls}
The elegant formulation of  the \gls{ep} is indeed appealing but occasionally runs into difficulty due to the division of the distributions in \eqref{EP.division.2}, or equivalently, due to subtraction of the coefficients in \eqref{z.gamma.i}. The existence of a similar problem has been acknowledged in \cite[Sec.~3.2]{Minka01} in the context of the Gaussian \gls{ep}, where the division of the distributions may yield a ``Gaussian'' with negative variance, see also \cite[Sec.~IV.B]{Senst11} \cite[Sec.~IV.A]{Cespedes14}. Such results are usually uninterpretable so a workaround is needed. 

In the context of the \gls{ep} based on Tikhonov distributions $\mcT(\theta;z)$ which are defined by complex parameters $z$, the purely numerical issue of invalid parameters (such as a negative variance in  the Gaussian case) is avoided but the problem remains. To understand intuitively its source and devise a solution, we may look at the scenario where the problems materialize. 

\begin{example}[Pitfalls of EP]\label{Ex:Pitfall}
Assume that 
\begin{itemize}
\item The circular means of the approximate posterior distribution, $\mcT\big(\theta; z^{(i)}_{\tr{post},n}\big) $ and of the ``extrinsic'' distribution (defined by  the product $\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)$) coincide, that is,  $\angle z^{(i)}_{\tr{post},n} =\angle (z^{(i-1)}_{\alpha,n}+z^{(i-1)}_{\beta,n})$; (remember, the phase $\angle z^{(i)}_{\tr{post},n}$ defines the circular mean); and that
\item The variance of the posterior distribution is larger than the variance of the extrinsic distribution, \ie $|z^{(i)}_{\tr{post},n}|<|z^{(i-1)}_{\alpha,n}+z^{(i-1)}_{\beta,n}|$; this may occur because the distribution in the argument of $\mcF[\cd]$ in \eqref{EP.division} is obtained multiplying  the extrinsic distribution $\mcT\big(\theta; z^{(i-1)}_{\alpha,n}+z^{(i-1)}_{\beta,n}\big)$ with a mixture $\gamma_n(\theta)$; the variance of the resulting mixture (and thus of its projection result as well) may be larger than the variance of the extrinsic distribution. 
\end{itemize}

Then, carrying out the subtraction in \eqref{z.gamma.i} we will obtain
\begin{align}
z^{(i)}_{\tilde{\gamma},n}
&= (|z^{(i)}_{\tr{post},n}|  - |z^{(i-1)}_{\alpha,n} + z^{(i-1)}_{\beta,n}|\big)\e^{\jj \angle z^{(i)}_{\tr{post},n}}\\
&=|z^{(i-1)}_{\tilde{\gamma},n}|\e^{\jj(\angle z^{(i)}_{\tr{post},n}+\pi)}.
\end{align}
That is, the circular mean of the new distribution $\mcT(\theta; z^{(i)}_{\tilde{\gamma},n})$ will be  in disagreement (by the largest possible value of $\pi$) with the mean of the posterior and extrinsic distributions obtained from the previous iteration. Such a results, being an artefact of the way the \gls{ep} is defined \cite[Sec.~3.2]{Minka01} is clearly counterintuitive and simply wrong. 
\end{example}

This problem, characteristic of the \gls{ep} will affect first $\tilde{\gamma}_n(\theta)$ and,  propagating via the \gls{mp}, will have detrimental affects on $\alpha_n(\theta)$ and $\beta_n(\theta)$.

Heuristics were devised for the Gaussian \gls{ep} where the problem is clearly identified, \ie the variance of the distributions after division becomes negative. For example, \cite[Sec.~3.2]{Minka01} constrains the variance to be positive, while other proposed to identify the problematic cases (\ie the negative variance) and then, if necessary i)~eliminate the division of the distributions \cite[Sec.~IV.B]{Senst11}, which here would mean $z^{(i)}_{\tilde{\gamma},n}=z^{(i)}_{\tr{post},n}$, or ii)~remove the update \cite[Sec.~IV.A]{Cespedes14}, \ie $z^{(i)}_{\tilde{\gamma},n}=z^{(i-1)}_{\tilde{\gamma},n}$. 

On the other hand, instead of testing for the compliance with our prior requirements (that are not necessarily obvious to define),  we might ``smooth'' the obtained parameters via recursive filter \cite[Sec.~IV.A]{Cespedes14} , which would mean  replacing \eqref{z.gamma.i} with
\begin{align}\nonumber
z_{\tilde{\gamma},n}^{(i)} = \zeta \Big(z^{(i)}_{\tr{post},n}  - z^{(i-1)}_{\alpha,n} - z^{(i-1)}_{\beta,n}\Big)
&+(1-\zeta) z_{\tilde{\gamma},n}^{(i-1)}\\
\label{z.smoothing}
& i=2,\ld, I_\tr{ep},
\end{align}
where $\zeta<1$ must be chosen heuristically to strike a balance between the new solution and the history accumulated in the previous estimate. In this way we avoid rapid changes in the the parameters $z_{\tilde{\gamma},n}^{(i)}$, regularizing the final solution. Note that the smoothing is not necessary in the first iteration, $i=1$, which is based solely on the information obtained from the pilots and from the decoder (if such option is allowed). 

We applied this smoothing solution in our numerical experiments, and found $\zeta\approx 0.4$ yielding satisfactory results. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
\subsection{Summary of the algorithm}\label{Sec:Summary}
The proposed \gls{ep} phase tracking algorithm is now summarized as Algorithm~\ref{Algo:EP} where for simplicity we defined the set of indices to the payload symbols and to the pilots as
\begin{align}
\Natural_{\tr{pilots}}&=\set{0,L,2L,\ld, FL}\\
\Natural_{\tr{payload}}&=\set{1,\ld, N} \setminus \Natural_{\tr{pilots}}.
\end{align}
We also integrated the notation so that the \gls{cbc} algorithm is naturally the first iteration ($i=1$) of the \gls{ep} algorithm, \ie $z^{(0)}_{\Sigma,n}(a)=z_{g,n}(a)$ and thus $\eta^{(0)}_{\Sigma,n}(a)=\eta_{g,n}(a)$, see \eqref{gamma.projection.first.cases}; 
the main distinction we need to make is that the smoothing \eqref{z.smoothing} is not applied for $i=1$, see lines \ref{i.if}--\ref{i.endif} of the algorithm. Note that the notation with the iteration index $^{(i)}$ may be removed (and the in-place calculation carried out) but we kept it for compatibility with the equations in the paper.

Last but not least, and at the risk of stating the obvious, we want to emphasize what the \gls{ep} algorithm is \emph{not} doing. Namely, it is not reusing the output ``extrinsic'' log-probabilities $\hat{P}_n(a)$ as if they were newly calculated prior log-probabilities $\hat{P}^{\tr{a}}_n(a)$. This is clearly seen in the description of the algorithm: plugging $\hat{P}_n(a)$ calculated at line \ref{P.n.a} into the line \ref{eta.Sigma.n} will \emph{not} yield the same results $\eta^{(i-1)}_{\Sigma,n}(a)$.

Since the \gls{ep} phase tracking is an iterative process itself, the notion of scheduling has to be revised; we use now the notation $\set{I_\tr{loop}\times (I_\tr{ep}, I_\tr{dec})}$ which takes into account the fact that within each loop the phase tracking may execute $I_\tr{ep}$ \gls{ep} iterations. With this notation, the original \gls{cbc} algorithm is denoted as $I_\tr{dec}\times (1, 1)$ and  one-shot \gls{ep} phase tracking is identified by the scheduling $1\times(I_\tr{ep}, I_\tr{dec} )$

% ------------------------------- algorithm -----------------------
\begin{algorithm}
    \caption{EP phase tracking} \label{Algo:EP}
\begin{algorithmic}[1]
\State Inputs:
\State $y_n, n\in\set{0,\ld,N}$ \Comment Received signal 
\State $x_n, n\in\Natural_{\tr{pilots}}$  \Comment Pilot symbols
\State $\hat{P}^{\tr{a}}_n(a)$\Comment Log-probabilities from the decoder
\State Initialization:
\State $z^{(i)}_{\tilde{\gamma},n}\gets 2\frac{y_n x_n^*}{\No},    n\in \Natural_{\tr{pilots}}, i\in{1,\ld, I_\tr{ep}}$
\State $z_{g,n}(a)\gets 2\frac{y_n a^*}{\No},\quad a\in\mcA, n\in\Natural_{\tr{payload}}$
\State $z_{\Sigma,n}^{(0)}(a) \gets z_{g,n}(a), \quad n\in\Natural_{\tr{payload}}$
\State EP iterations:
\For{ $i\gets1,\ld, I_\tr{ep}$ }
	\For {$n\gets \Natural_{\tr{payload}}$} \Comment Finds $\tilde{\gamma}_n(\theta)$:
		\State $\eta^{(i-1)}_{\Sigma,n}(a) \gets -\frac{|a|^2}{\No}+ \hat{I}_0\big(|z^{(i-1)}_{\Sigma,n}(a)|\big)+\hat{P}^{\tr{a}}_n(a)$ \label{eta.Sigma.n}
		\State $z^{(i)}_{\tr{post},n}  \gets \mf{CMM}\Big[ \eta^{(i-1)}_{\Sigma,n}(a), z^{(i-1)}_{\Sigma,n}(a)\big| a\in\mcA  \Big]$
	\If {$i=1$} \label{i.if}
		\State $z^{(i)}_{\tilde{\gamma},n}\gets z^{(i)}_{\tr{post},n}  - z^{(i-1)}_{\alpha,n} - z^{(i-1)}_{\beta,n}$
	\Else
		\State $z_{\tilde{\gamma},n}^{(i)} \gets \zeta \Big(z^{(i)}_{\tr{post},n}  - z^{(i-1)}_{\alpha,n} - z^{(i-1)}_{\beta,n}\Big)$
		\State \qquad~ \qquad  ~ \qquad~ \qquad~ \qquad$+(1-\zeta) z_{\tilde{\gamma},n}^{(i-1)}$
	\EndIf  \label{i.endif}
	\EndFor
	\State $z^{(i)}_{\alpha,0}\gets 0$	
	\For {$n\gets 1,\ld,N$} \Comment Finds $\alpha^{(i)}_n(\theta)$:
		\State $z^{(i)}_{\alpha,n} \gets \frac{z^{(i)}_{\alpha,n-1} + z^{(i)}_{\tilde{\gamma},n-1}}{1+\big|z^{(i)}_{\alpha,n-1} + z^{(i)}_{\tilde{\gamma},n-1}\big|\sigma_w^2}$
	\EndFor
   	\State $z^{(i)}_{\beta,N} \gets 0$
	\For {$n\gets N-1,\ld,0$} \Comment Finds $\beta^{(i)}_n(\theta)$:
		\State $z^{(i)}_{\beta,n} \gets  \frac{z^{(i)}_{\beta,n+1} + z^{(i)}_{\tilde{\gamma},n+1}}{1+\big|z^{(i)}_{\beta,n+1} + z^{(i)}_{\tilde{\gamma},n+1}\big|\sigma_w^2}$
	\EndFor
	\For {$n\gets \Natural_{\tr{payload}}$} %\Comment Prepare outputs
	\State $z^{(i)}_{\Sigma,n} \gets  z_{g,n}(a) +z^{(i)}_{\alpha,n}+ z^{(i)}_{\beta,n}$
	\EndFor
\EndFor % i
\State Output: log-probabilities to be used in \eqref{lambda.n.l}
\For {$n \gets \Natural_{\tr{payload}}$}
\State $\hat{P}_{n}( a ) \gets -\frac{|a|^2}{\No} + \hat{I}_0\big(|z^{(I_{\tr{ep}})}_{\Sigma,n}(a)|\big)$\label{P.n.a}
\EndFor
\end{algorithmic}
\end{algorithm}
% ------------------------------- end algorithm -------------------

\subsection{Numerical results}\label{Example.EP} 
Considering the transmission scenario from \secref{example.start} we evaluate the \gls{per} in the one-shot phase tracking (the scheduling $1\times (I_\tr{ep}, I_\tr{dec})$); as discussed in \secref{example.start}, the performance limit for one-shot phase tracking is the \gls{dmp} (with $I_\tr{dec}$ decoding operations).

The results are shown in \figref{fig:PER.EP} and we observe the following:
\begin{itemize}
\item The one-shot \gls{ep} phase tracking with the scheduling \mbox{$\set{1\times (2, 10)}$} outperforms the \gls{cbc} algorithm (scheduling, $\set{30\times 1}$) notably, despite the fact that the later requires $20$ more decoding iterations and $28$  more \gls{mp}s (and, of course, $28$ more projections \eqref{gamma.projection.first.cases}). The same comparison can be made with the \gls{cbc} (scheduling $\set{10\times 1}$): although the complexity measured by the number of decoding iteration is the same, the number of \gls{mp}s is still larger in the \gls{cbc} algorithm. Using the \gls{ep} we thus gain, both in terms of complexity and performance. Moreover, the \gls{ep} phase tracking operates independently of the decoder which is a significant advantage.
\item Increasing the number of \gls{ep} iterations from $I_\tr{ep}=2$ to $I_\tr{ep}=3$ improves the performance in low \gls{snr} at the cost of the \gls{per} saturating in high \gls{snr}. However, the choice of the operating point may be different between applications so the ``optimal'' choice of the parameters is on open issue.
\item Some gain is further obtained by increasing the number of operations from $I_\tr{dec}=10$ to $I_\tr{dec}=30$, yet the qualitative behaviour remains the same.
\end{itemize}

Despite a notable improvement in terms of complexity and performance when comparing to the \gls{cbc} algorithm, we still observe the saturation of the \gls{per} for high \gls{snr}. 

While this may be an acceptable solution at least in a context where only one-shot phase tracking is allowed, putting the \gls{ep} phase-tracking  in the decoding loop, changes the picture even more notably as shown in \figref{fig:PER.EP.DEC}. Since we consider the scheduling $3\times(I_\tr{ep},10)$, the reference curves are those obtained with  $I^{\Sigma}_\tr{dec}=30$ decoding iterations. We observe that
\begin{itemize}
\item The saturation of the \gls{per} disappears thanks to the feedback from the decoder which, already after the first \gls{ep} phase-tracking and $I_\tr{dec}=10$ decoding iterations provides a reliable  prior $\hat{P}^{\tr{a}}_n(a)$.
\item The \gls{ep} results are better than those yield by the \gls{dmp} (with $I_\tr{dec}=30$); this is quite an impressive results as we are not aware of the results in the literature which would show such a performance; and while it might be surprising at the first sight, it is also correct: remember, the performance limit for the joint decoding-phase tracking is defined by the ``All-pilots'' curve ($I_\tr{dec}=30$).
\item As for the complexity, the \gls{ep} phase tracking with a scheduling $\set{3\times(I_\tr{ep},10)}$ requires the same number of decoding iterations as the \gls{cbc} algorithm ($I_\tr{dec}=30$). The result of the latter appear only for  high \gls{snr} and thus, due to the change in the \gls{snr} axis range, they are not plotted in \figref{fig:PER.EP.DEC}. Still, the number of  the \gls{mp} is much lower in the case of the proposed \gls{ep} algorithm so again, we not only gained  notably in performance comparing to the \gls{cbc} algorithm but also preserved the lower complexity.
\end{itemize}

%%%%%%%%%%%%%%
\begin{figure}[bt]
\begin{center}
\psfrag{DMPXXX.XXX}[lc][lc][\siz]{DMP: $I_{\tr{dec}}=10$}
\psfrag{DMP30}[lc][lc][\siz]{DMP: $I_{\tr{dec}}=30$}
\psfrag{CBC10}[lc][lc][\siz]{CBC:$\set{10\times 1}$}
\psfrag{CBC30}[lc][lc][\siz]{CBC:$\set{30\times 1}$}
\psfrag{EP2.10}[lc][lc][\siz]{EP:$\set{1\times(2,10)}$}
\psfrag{EP3.10}[lc][lc][\siz]{EP:$\set{1\times(3,10)}$}
\psfrag{EP2.30}[lc][lc][\siz]{EP:$\set{1\times(2,30)}$}
\psfrag{EP3.30}[lc][lc][\siz]{EP:$\set{1\times(3,30)}$}
\psfrag{ylabel}[lc][lc][\siz]{$\PER$}
\psfrag{xlabel}[lc][lc][\siz]{$\SNRrv$ [dB]}
\scalebox{\sizf}{\includegraphics[width=\linewidth]{./figures/PER_Tikh_EP.eps}}
\end{center}
\caption{\gls{per} vs. \gls{snr} obtained using  the \gls{ep} one-shot phase tracking, that is, the scheduling \mbox{$\set{1\times(I_{\tr{ep}}, I_\tr{dec})}$}, and the \gls{cbc} algorithm ( scheduling $\set{I_{\tr{dec}}\times 1}$). The \gls{dmp} results are obtained with $I_\tr{dec}=10$ (filled markers, solid lines) and $I_\tr{dec}=30$ (hollow markers, dashed lines).}\label{fig:PER.EP}
\end{figure}
%%%%%%%%%%%%%%

%%%%%%%%%%%%%%
\begin{figure}[bt]
\begin{center}
\psfrag{DMP10XXX.XXX.X}[lc][lc][\siz]{DMP: $I_\tr{dec}=10$}
\psfrag{DMP30X}[lc][lc][\siz]{DMP: $I_\tr{dec}=30$}
\psfrag{All-pilots10}[lc][lc][\siz]{``All-pilots'': $I_\tr{dec}=10$}
\psfrag{All-pilots30}[lc][lc][\siz]{``All-pilots'': $I_\tr{dec}=30$}
\psfrag{EP3x(2,10)}[lc][lc][\siz]{EP: $\set{3\times(2,10)}$}
\psfrag{EP3x(3,10)}[lc][lc][\siz]{EP: $\set{3\times(3,10)}$}
\psfrag{ylabel}[lc][lc][\siz]{$\PER$}
\psfrag{xlabel}[lc][lc][\siz]{$\SNRrv$ [dB]}
\scalebox{\sizf}{\includegraphics[width=\linewidth]{./figures/PER_Tikh_EP_turbo.eps}}
\end{center}
\caption{\gls{per} vs. \gls{snr} obtained using the \gls{ep} algorithm in the joint decoding-phase tracking algorithm,  with  the scheduling \mbox{$\set{3\times(I_{\tr{ep}}, 10)}$} . The \gls{dmp} and ``All-pilots" results are obtained with $I_\tr{dec}=10$ (filled markers, solid lines) and $I_\tr{dec}=30$ (hollow markers, dashed lines)}\label{fig:PER.EP.DEC}
\end{figure}
%%%%%%%%%%%%%%

%%%%%%%%%%%%%%
%\subsection{Complexity estimation}\label{Sec:Complexity}
%
%To evaluate the complexity and compare it eventually to the methods from the literature we propose to split the complexity into three parts related respectively to the decoding, \acrlong{mp}, and \gls{cmm}.


%%%%%%%%%%%%%%
%\subsection{Impact of large-argument approximations}\label{Sec:Simplifications}
%
%The non-linear operations in the algorithm appear mostly due to the use of the Bessel function, and may be implemented via look-up tables or replaced by easy-to-implement approximations. These non-linearities are present i)~in the calculation of $\hat{I}_0 (x)$, see \eqref{hat.I0} and ii)~when implementing the \gls{cmm}, where the function $B(x)=\frac{I_1(x)}{I_0(x)}$ must be evaluated; this is necessary to implement the projection operation $\mcF[\cd]$ and to calculate the result of the convolution between the Gaussian and the Tikhonov distributions.
%
%As for the point i), we may actually implement exactly the function $\hat{I}_0 (x)$ or use the \gls{laa} which was already proposed in the previous works, \eg \cite{Colavolpe05,Pecorino15,Shayovitz16}. This amount to using $\hat{I}_0 (x)\approx x $.
%
%As for the points ii) we already abandoned the idea of exact implementation of $B(x)$ (\eg via look-up tables) and instead use the approximation valid for the entire range of its argument, see \appref{}. However, it is still interesting to see the impact of the \gls{lla} in this case, especially that it was previously used for the very same purpose in the literature, \eg \cite[Appendix~A]{Shayovitz16}.
%
%We show in \figref{} how the \gls{per} is affected when the \gls{laa} is applied in different parts of the algorithms.







==> Includes/Tracking.v1.tex <==
%!TEX root =  ../Phase.Tracking.v2.tex
\section{Phase tracking}\label{sec:phase.track}

\subsection{Message passing on the graph}\label{Sec:MP.graph}
%%%%%%%%%%%%%%
\begin{figure}[bt]
\begin{center}
\scalebox{0.8}{\input{./figures/Graph.RRHARQ.x.2D.tex}}
\end{center}
\caption{Graph defining the relationship between the variables in the phase tracking problem; the messages exchanged between the nodes are shown together with the arrows indicating the direction of the exchange.}
\label{fig:graph.tracking}
\end{figure}
%%%%%%%%%%%%%%%

Our goal now is to find 
\begin{align}\label{Px}
P_n(a)=\PR{x_{n}=a|\by}, \quad a\in\mcA.
\end{align} 
and this is done exploiting the relationships between the involved random variable. 

As in \cite{Colavolpe05,Kreimer18} we show in \figref{fig:graph.tracking} a graph which captures this relationship: the squares represent the functions taking as arguments the variables which, in turn, are represented by the directly connected circles. In particular
\begin{align}
\label{f.n.x}
f_n(\theta_n,x_n)  & \propto \exp\left(-\SNR\Big|y_n-x_n\e^{\jmath\theta_n}\Big|^2\right)
\end{align}
corresponds to the relationship defined in \eqref{y.kn} and
\begin{align}\label{p.w}
p_w(\theta_n,\theta_{n+1}) =\omega(\theta_n-\theta_{n+1})
%& \propto \mcN(\theta_n; \theta_{n+1},\sigma_w^2)
%\exp\left(-\frac{(\theta_n-\theta_{n+1})^2}{\sigma_w^2}\right)
\end{align}
corresponds to \eqref{theta.Wiener} and thus $\omega(\theta)=\mcN(\theta;0,\sigma_w^2)$, where we use the Gaussian distribution defined as
\begin{align}\label{Normal.pdf}
\mcN(\theta;m,v)=\frac{1}{\sqrt{2\pi v}}\exp\left(-\frac{(\theta-m)^2}{2v}\right).
\end{align}

Although \eqref{p.w} is used very often in the literature, we want to emphasize that it is a proxy to a more precise notation which reflects the periodicity of the phase $\theta_n$, \ie
\begin{align}
\omega(\theta)= \tilde{\mcN}(\theta; 0,\sigma_w^2),
\end{align}
where tilde will be henceforth used to denote the ``periodicization'' of a function which is not periodic by definition
\begin{align}\label{definition.periodic}
\tilde{g}(\theta)
&=\sum_{k=-\infty}^{\infty}
g(\theta-k2\pi).
\end{align}

In \figref{fig:graph.tracking} we also show a shaded rectangle labeled as ``modulation/coding graph''; it hides the graph which describes the relationship $\bx  \rightarrow \bs \rightarrow \bc \rightarrow \bb$, and its knowledge is used for the demodulation (to implement \eqref{demodulation}) and for the decoding \eg to implement a sum-product algorithm for \gls{ldpc} decoding \cite[]{}.

What is important to note at this point is  that the relationships induced by the modulation/coding graph are ignored during the phase tracking, which essentially means that the symbols $x_n$ are assumed to be a priori \gls{iid}, with non-informative distribution, \ie $P^{\tr{a}}_n(a)\propto 1$.

As a direct consequence of ignoring the relationship between $x_n$ (which are induced by the coding), the graph we deal with in \figref{fig:graph.tracking} is a tree, \ie contain no loops. Therefore, the efficient marginalization can be done exactly by the \gls{mp} algorithm as follows \cite{Colavolpe05,Shayovitz16,Kreimer18}
\begin{align}\label{P.n.x}
P_n(a) \propto\int_{-\pi}^{\pi}  \alpha_n(\theta)  \beta_n(\theta) f_n(\theta,a ) \dd \theta,\quad a\in\mcA,
\end{align}
where
\begin{align}\label{alpha}
\alpha_n(\theta)&\propto \left(\alpha_{n-1}(\theta)  \gamma_{n-1}(\theta)\right) \convop 
\omega(\theta)\\
%\mcN(\theta;0,\sigma_w^2),\\
\label{beta}
\beta_n(\theta)&\propto \left(\beta_{n+1}(\theta) \gamma_{n+1}(\theta) \right) \convop 
\omega(\theta)\\
%\mcN(\theta;0,\sigma_w^2),\\
\label{gamma}
\gamma_n(\theta)&\propto\sum_{a\in\mcA} P^{\tr{a}}_n(a) f_{n}(\theta,a )=\sum_{x\in\mcA}  f_{n}(\theta,a ),
\end{align}
are (proportional to) the marginal distributions of the phase $\theta_n$ conditioned, respectively, on $y_0,\ld,y_{n-1}$, on $y_{n+1},\ld,y_{N}$, and  on $y_n$. All the distributions of the phase are periodic and so is the convolution in \eqref{alpha} and \eqref{beta}. \footnote{In a case we would like  to perform the joint decoding/demodulation/phase tracking, as done, \eg in \cite{Kreimer18}, we would have to use non-uniform distribution $P^{\tr{a}}_n(x)$ based on the decoding results;  however, we do not follow this path here.}

These equations are practically the same as those appearing in the \gls{bcjr} recursion \cite{BCJR} well known in the area of decoding of convolutional codes. Here, derived from the graph representation, they are applied to calculate the continuous-argument distributions of the phase. 

\subsection{Parametric message passing strategies}\label{Sec:Parametric.MP}
The operations \eqref{P.n.x}-\eqref{gamma} which allow us to calculate $P_n(a)$ may be implemented on the discretized versions of the distributions $\alpha_n(\theta)$, $\beta_n(\theta)$, and $\gamma_n(\theta)$ defined over samples of $\theta\in(-\pi, \pi]$. In such a \gls{dmp} the multiplications and additions are straightforward to implemented and the convolution is efficiently implemented via \gls{fft}. 

However, to ensure sufficient precision,  large number of samples may be necessary implying possibly a large complexity and storage burden. Therefore, many previous works have gone in the direction of parametric representation of the involved periodic distributions. Then, instead of tracking the samples in \gls{dmp}, we only need to track (a few) parameters which represent the distributions.

We thus have to find a family of the distributions, $\mcF$, on which the operations defined in \eqref{P.n.x}-\eqref{gamma} are easily dealt with. In particular, we have to handle multiplication of the periodic functions as well as, the convolution in \eqref{alpha} and \eqref{beta}; the integration in \eqref{P.n.x}, when done on the parametric forms of distributions, is usually straightforward. In other words, if $\alpha_n(\theta), \beta_n(\theta), \gamma_n(\theta), \omega(\theta)\in\mcF$  and $\mcF$ is closed under  multiplication and convolution, the parametric \gls{mp} will be immediately obtained. 

Of course, if  some distribution $g(\theta)$ which is obtained implementing \eqref{alpha}-\eqref{gamma} (as the final, or an intermedia result) is not in $\mcF$, we need to \emph{project} it onto $\mcF$, as $\hat{g}(\theta)=\mcP[g(\theta)]$. This may be done using some easy-to-implement approximations or, more formally, optimizing a well defined criterion, such as the Kulhback-Leiber divergence between $g(\theta)$ and a member of $\mcF$, which we express as
\begin{align}\label{projection}
\hat{g}(\theta)=\mcP[ g(\theta) ] &= \argmax_{ \xi(\theta)\in\mcF } \int g(\theta)\log \xi(\theta) \dd \theta.
\end{align}
If $\mcF$ is an exponential family, \eqref{projection} can be often solved analytically.\footnote{The best example is a Gaussian family $\mcF$, where the projection \eqref{projection} boils down to calculation of the mean and the variance of $g(\theta)$.} 

Henceforth, when it is clear how the projection is carried out, we make no distinction between the projected function and the original one.

Depending how the projection is applied in  \gls{mp}, we obtain different parametric \gls{mp} algorithms. Among main strategies we may specify two which cover most of the approaches used in the literature up to now

\begin{enumerate}
%%
\item \textbf{Pre-\gls{mp} projection}; this approach was used in \cite{Colavolpe05}\cite{Barbieri07}\cite{Alfredsson19}, where the distributions $\gamma_n(\theta)$ are obtained before the steps of \gls{mp} \eqref{alpha}-\eqref{gamma} are executed, that is
\begin{align}\label{gamma.projection.first}
\gamma_n(\theta)=\mcP\Big[\sum_{a\in\mcA} f_{n}(\theta,a )\Big].
\end{align}

While this may be appealing (the obvious advantage is that \gls{mp} is easily implemented without further approximations if we ensure that $\alpha(\theta), \beta(\theta), \gamma(\theta), \omega(\theta) \in\mcF$), it is not very useful if no feedback from the decoder is available (as we assumed in this work).

To understand this we note that, in most practical cases, the constellation $\mcA=\set{a_0,\ld,a_{M-1}}$ contains symbols with the phase uniformly set in the interval $(-\pi, \pi]$. For example, in \gls{psk}, $a_m=a_0\e^{\jj m2\pi/M}$  and we may write $f_n(\theta, a_m)=f_n(\theta+m\frac{2\pi}{M},a_0)$; the sum of these uniformly separated  replicas of $f_n(\theta, a_0)$, projected on $\mcF$ yields a trivial, zero-mean  distribution $\gamma_n(\theta)$ which is, de facto, useless for the phase tracking.

To make $\gamma_n(\theta)$ useful, we may introduce  a prior on $\theta$ which is discussed in \secref{}, or provide a prior on the symbols $a\in\mcA$, via $P^{\tr{a}}_n(a)$ that may be obtained from the modulation/coding graph; however,  this requires the iteration between the phase tracking and the demodulation/decoding. As we said, this cases is not considered here, \ie we assume $P^{\tr{a}}_n(a)\propto 1$.
%%
\item \textbf{Intra-\gls{mp} projection}; in this approach  we decide to operate only on the functions from the family $\mcF$ thus  we use approximations $\hat{f}_n(\theta)$ and  $\hat{\omega}_n(\theta)$ instead of $f_n(\theta,a)$ and $\omega(\theta)$ in \eqref{alpha}-\eqref{gamma}. Next we apply the projection after all the operations in \eqref{alpha}-\eqref{beta} are executed 
\begin{align}\label{alpha.projection}
\alpha_n(\theta)&\propto \mcP\left[ \sum_{a\in\mcA}  \Big( \alpha_{n-1} (\theta) \hat{f}_{n-1}(\theta,a ) \Big)\convop 
\hat{\omega}(\theta)\right]\\
%\label{alpha.projection.2}
%\alpha_n(\theta)&= \mcP\left[\mcP\bigg[ \sum_{a\in\mcA}  \alpha_{n-1}(\theta)\hat{f}_{n-1}(\theta,a ) \bigg]\convop \hat{\omega}(\theta)\right]\\
\label{alpha.projection.3}
&= \mcP\left[ \sum_{a\in\mcA}  \alpha_{n-1}(\theta) \hat{f}_{n-1}(\theta, a ) \right]\convop 
\hat{\omega}(\theta)\\
\label{beta}
\beta_n(\theta)&\propto \mcP\left[\sum_{a\in\mcA}\beta_{n+1}(\theta) \hat{f}_{n+1}(\theta, a ) \right] \convop 
\hat{\omega}(\theta),
\end{align}
where \eqref{alpha.projection} simplifies to \eqref{alpha.projection.3} due to $\mcF$ being closed under multiplication and convolution. 

Comparing to ``pre-\gls{mp}'' projection, we need to carry out the projection for each time $n$; this increases the computational burden but the hope is that, introducing approximations (projection) at the later stage, we minimize the approximation error which will be propagated through the time-recursive calculations.

\end{enumerate}

In this work we will consider two parametric distributions adopted in the literature for the purpose of phase tracking:
\begin{itemize}
\item The Gaussian distribution $\tilde{\mcN}(\theta;m,v)$ -- a periodic version of \eqref{Normal.pdf} defined via \eqref{definition.periodic}.
\begin{align}\label{}
\tilde{\mcN}(\theta;m,v)=\sum_{l=-\infty}^{\infty}\mcN(\theta-l2\pi;m,v),
\end{align}
used, \eg in \cite{Kreimer18}. In that case we have $\hat{\omega}(\theta)=\omega(\theta)$ and the challenge is to find $\hat{f}_n(\theta,a)$; more on that in \secref{}.
\item The Tiknonov distributions defined as 
\begin{align}\label{}
\mcT(\theta; m, \kappa)= \frac{\e^{\Re[\kappa\e^{-\mathj (\theta-m)}]}}{2\pi I_0(\kappa)},
\end{align}
where $I_0(\cd)$ is the zero-th order modified Bessel function, $m\in(-\pi,\pi]$ is the circular mean, and $\kappa$ is a measure of precision. 
For large $\kappa$ (\eg, $\kappa>2)$ we can approximate the Tiknonov distribution with a Gaussian 
\begin{align}
\mcT(\theta; m, \kappa)\approx \tilde{\mcN}(\theta;m, 1/\kappa).
\end{align}

Since Tiknonov distribution is periodic by definition, it seems well suited to represent the distributions of the phase and was already used, \eg in \cite{Colavolpe05}\cite{Barbieri07}\cite{Shayovitz16}. In particular, it is easy to see that \eqref{f.n.x} can be written as
\begin{align}\label{f.n.x.Tikh}
f_n(\theta,a)\propto&  \mcT\Big(\theta; m_a,\kappa_a), \Big) \\
m_a&=\angle \frac{y_n}{a},\\
\kappa_a&=2\SNR |y_n||a|,\\
\xi_a&=\exp\big(-\SNR|a|^2\big)I_0\big(2\SNR |y_n||a|\big)
\end{align}
\end{itemize}


%The parametric representations will yield approximate solution not only because of the assumptions we made regarding the particular form of the distribution.\footnote{Which may be more or less adequate in the case we deal with; the choice of the parametric family will be resolved via implementation and comparison of the results as we do in \secref{}.} There are also additional approximations which need to be made in order to implement the equations \eqref{alpha}-\eqref{gamma}. The issue will appear depending on the type of parametric form we will use. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Gaussian approximation in one-dimensional case}\label{Sec:messages.1D}

In particular, noting that \eqref{f.n.x} defines the Tikhonov (or von Mises) distribution, the latter was used to approximate also $\alpha(\theta)$ and $\beta(\theta)$ \cite{Colavolpe05}. Indeed, the advantage is that the periodic property is automatically taken care of, and that the product of the Tikhonov distributions is also in the  Tikhonov family. On the other hand, the convolution in \eqref{alpha}-\eqref{beta}, requires approximating of the Tikhonov distribution with a Gaussian. Finally, approximation is also necessary when the sum of the distributions, which appears in \eqref{gamma}, is projected onto the space of Tiknonov distributions.\footnote{This is a must: keeping all the terms of the sum in $\gamma_n$, would increase their number exponentially with $n$.} Because of the latter, the approximations will be always necessary.

Here, as in \cite{Kreimer18} we use the Gaussian family to approximate $\alpha_n(\theta)$ and $\beta_n(\theta)$. The disadvantage is that we have to deal with their non-periodic behaviour as well as derive suitable approximation for $f_n(\theta_n,x_n)$. On the other the convolution is straightforward. What motivates us the most, however, is the possibility of applying the Gaussian parametrization in the case of multivariate distributions, which appear in the case of \gls{rrharq} as we explained in \secref{Sec:rrharq}; this will be detailed in \secref{sec:RR.phase.track}.

\subsection{Approximation of $f_n(\theta,x)$}\label{sec:approx.f.theta.x}
To obtain the parametric representation of \eqref{P.n.x}-\eqref{gamma} we start linearizing the relationship \eqref{y.kn} using $\e^{\jj \theta}\approx \e^{\jj \hat{\theta}}(1+\jj ( \theta-\hat{\theta} ))$, where the choice of suitable $\hat{\theta}$ will be discussed shortly. This approximation transforms \eqref{f.n.x} into a Gaussian \cite{Kreimer18}
\begin{align}\label{f.Gauss}
f_n(\theta,x)
&\approx \xi_{x,n}\mcN\Big(\theta; m_{x,n}, v_{x,n}\Big),
\end{align}
where
\begin{align}\label{}
m_{x,n} &= \frac{\Im[y x^* \e^{-\jj \hat{\theta} }] }{|x|^2}+\hat{\theta}\\
v_{x,n}&=\frac{\No}{2|x|^2}\\
\xi_{x,n}&=\exp\left(-\frac{\Big(|x|^2-\Re[yx^*\e^{-\jj \hat{\theta}}]\Big)^2}{\No|x|^2}\right)\frac{\sqrt{\pi\No}}{|x|}\\
&=\exp\left(-\frac{\Big(|x|-|y|\cos(\delta-\hat{\theta})\Big)^2}{\No}\right)\frac{\sqrt{\pi\No}}{|x|}
\end{align}
where $\delta=\angle y -\angle x$, and$\Re[\cd]$ $\Im[\cd]$ are, respectively, the real and the imaginary parts of their argument.



Various approaches to find the parameters $m_{x,n}$, $v_{x,n}$  and $\xi_{x,n}$ may be used and, here, we compare two; both use  
\begin{align}\label{m.f}
m_{x,n}&=\angle y-\angle x,\\
\label{xi.f}
\xi_{x,n}&=\mcN(|y_n|;|x|,\No/2)\pi\sqrt{2\No v_{x,n}},
\end{align}
where $\angle a \in(-\pi, \pi]$ denotes the phase of the complex variable $a$.
The two approaches differ in the way the variance is defined; the first one uses
\begin{align}
\label{v1.f}
v_{x,n}&=\frac{\No}{2|x|^2},
\end{align}
while the second,
\begin{align}
\label{v2.f}
v_{x,n}&=\frac{\No}{2|x||y_n|};
\end{align}
 the details of derivation are shown in Appendix A. The Gaussian with observation-dependent variance \eqref{v2.f} provides a better fit to $f_n(\theta,x)$ but requires additional safeguard for small values of $|y_n|$. In fact, we always have to be aware of the periodic property of the distributions involved in the calculations; the period-based integration/convolution over $(-\pi, \pi]$ may be replaced by their simple infinite-domain counterparts (carried over the interval $(-\infty,\infty)$) only if the distributions are sufficiently ``narrow'', \ie when their support is much smaller than $2\pi$. The extreme scenario occurs when $y_n=0$ as then, from \eqref{f.n.x}, $f_n(\theta_n,x_n)\propto 1$. This non-informative distribution, under a Gaussian modelling, is obtained with infinite variance,\footnote{In the implementation, instead of variance, we might prefer to work with its inverse, know as a \emph{precision}.} \ie
 \begin{align}\label{v.th.cond}
 v_{x,n}&>v_\tr{th} \implies v_{x,n}=\infty,
\end{align}
where $v_\tr{th}$ is chosen somewhat arbitrary; here, we decide to set it so that
\begin{align}\label{}
\int_{-\pi+m_{x,n}}^{\pi+m_{x,n}}  \mcN\Big(\theta; m_{x,n}, v_{x,n}\Big) \dd \theta <1-\epsilon_\tr{th},
\end{align}
\ie when the integral of the \gls{pdf}  over the period centered at the mean $m_{x,n}$ is decreased by $\epsilon_\tr{th}$; we set $\epsilon_\tr{th}=0.2$ which yields $v_\tr{th}= (\pi/Q^{-1}(\epsilon/2))^2\approx 6$. While the condition \eqref{v.th.cond} does not materialize frequently, this approach will be also helpful in other approximation steps. 

%%%%-----
\subsection{Approximation of $\alpha_n(\theta)$ and $\beta_n(\theta)$}\label{sec:mult.alpha.f}
Next, our goal is to find recursively the parameters of the Gaussians representing $\alpha_n(\theta)\propto\mcN(\theta; m_{\alpha,n}, v_{\alpha,n})$ and $\beta_n(\theta)\propto\mcN(\theta; m_{\beta,n}, v_{\beta,n})$, where we assume that
\begin{align}\label{}
m_{\alpha,n}\in(-\pi,\pi], \quad m_{\beta,n}\in(-\pi,\pi];
\end{align}
\ie $\alpha_n(\theta)$ and $\beta_n(\theta)$ are the ``prototype'' functions whose means are in the reference interval $(-\pi, \pi]$. The periodic version of the prototype function, is denoted using tilde, \ie
\begin{align}\label{}
\tilde{\alpha}_n(\theta)=\sum_{k=-\infty}^{\infty} \mcN(\theta-k2\pi; m_{\alpha,n}, v_{\alpha,n}).
\end{align}
This periodic form is convenient to resolve the issues of the representation ambiguity. 

We will rewrite \eqref{alpha} as follows 
\begin{align}\label{tilde.alpha.projection}
\tilde{\alpha}_n(\theta)&\propto \mcP\left[\sum_{x\in\mcA}\left(\tilde{\alpha}_{n-1}(\theta) \cd\tilde{f}_{n-1}(\theta,x)\right)\right] \convop \mcN(\theta;0,\sigma_w^2)
\end{align}
which reflects the steps we are going to make, namely to i)~find the product of $\tilde{\alpha}_{n-1}(\theta)$ and $\tilde{f}_{n-1}(\theta,x)$, ii)~``project'' the sum (over $x$) of the results on a Gaussian function; the projection is denoted by $\mcP[\cd]$, and  then ii)~convolve the results with the Gaussian $\mcN(\theta;0;\sigma_w^2)$. The derivations will be done for $\alpha_n(\theta)$; they can be straightforwardly applied to calculate $\beta_n(\theta)$.

As we will see the approximations will be necessary even in the step i) above, but the most important approximation appears in the projection $\mcP[\cd]$. To avoid accumulation of approximation errors, the projection should be carried out as late in the process as possible. This is what \cite{Kreimer18} also does and it may be contrasted with \cite{Colavolpe05} which used the projection very early in the calculation. In fact, it projected the discrete distribution of the symbols $x$ given by $P^{\tr{a}}_n(x)\propto\sum_{a\in\mcA}\delta(x-a)$ on the Gaussian
\begin{align}\label{}
\hat{P}^{\tr{a}}_n(x)\propto \mcP\big[P^{\tr{a}}_n(x)\big]= \mcN(x;0,1);
\end{align}
such an approach suppresses information about the constellation form\footnote{Because all constellations used in practice have zero mean and are normalized to unitary energy.} so the improvement can be then sought from $P^{\tr{a}}_n (x)$ obtained after the decoding, \ie iterating between the decoder and the phase tracking as done also in \cite{Kreimer18}. 

%before the multiplication, which here (in the context of Gaussian approximations) would mean 
%\begin{align}\label{alpha.Colavolpe}
%\tilde{\alpha}_n(\theta)&\propto \left(\tilde{\alpha}_{n-1}(\theta)  \mcP_\mcN\left[\sum_{x\in\mcA}\tilde{f}_{n-1}(\theta,x)\right]\right) \convop \tilde{\mcN}(\theta;0,\sigma_w^2)
%\end{align}
%The issue with \eqref{alpha.Colavolpe} is that it 


%%%%%-----
\subsubsection{Multiplication  $\tilde{\alpha}_{n-1}(\theta) \cd\tilde{f}_{n-1}(\theta,x)$}\label{sec:mult}

We  note that \cite{Kreimer18} implements \eqref{alpha} as 
\begin{align}\label{alpha.Kreimer}
\alpha_n(\theta)&\propto \mcP\left[\sum_{x\in\mcA}\left(\alpha_{n-1}(\theta)  f_{n-1}(\theta,x)\right) \convop \mcN(\theta;0,\sigma_w^2)\right],
\end{align}
where the difference with \eqref{tilde.alpha.projection} is in the position of the projection operation before the convolution; as we will see this is irrelevant from the point of view of the final results. The more important difference, however, is that \eqref{alpha.Kreimer} operates on the prototype distributions instead of their periodic versions. 

To understand the difference we have to recall that the prototype functions $\alpha(\theta)$ and $f(\theta,x)$ have the infinite support, where, for clarity, we skip indexing $(\cd)_n$. Thus the multiplication of their periodic versions $\tilde{\alpha}(\theta)$ and $\tilde{f}(\theta,x)$ produces infinite number of terms in each of the periods. Namely
\begin{align}\nonumber
&\tilde{\kappa}(\theta,x)=\tilde{\alpha}(\theta) \tilde{f}(\theta,x) \\
\nonumber
&= 
 \sum_{k=-\infty}^{\infty} \xi_{x}\mcN(\theta-k2\pi; m_{\alpha}, v_{\alpha})
\sum_{l=-\infty}^{\infty} \mcN\Big(\theta-l2\pi; m_{x}, v_{x}\Big)\\
\label{alpha.beta}
&=\sum_{k=-\infty}^{\infty} \kappa(\theta-k 2 \pi,x),
\end{align}
with
\begin{align}\label{kappa}
 \kappa(\theta,x)=
\xi_{x} \mcN(\theta; m_{\alpha}, v_{\alpha})
 \sum_{l=-\infty}^{\infty} \mcN\Big(\theta; m_{x} + l2\pi, v_{x}\Big).
\end{align}

%%%%%%%%%%%%%%
\begin{figure}[bt]
\begin{center}
\psfrag{mx}[ct][cb][\siz]{$0.9\pi$}
\psfrag{ma}[ct][cb][\siz]{$-0.12\pi$}
\psfrag{m1}[ct][cb][\siz]{$0.39\pi$}
\psfrag{m2}[ct][cb][\siz]{$-0.61\pi$}
\scalebox{\sizf}{\includegraphics[width=\linewidth]{./figures/Gauss.Mult.Ambiguity.eps}}
\end{center}
\caption{Ambiguity appearing when the periodic Gaussians are multiplied; shown using the circular axis of the arguments. Two Gaussians plotted with solid (black) lines are multiplied yielding the Gaussians shown with with dotted (green) lines; these have the same variance $v=v_{\alpha}v_{x}/(v_{\alpha}+v_x)=0.05$ but different means $m_1=0.39\pi$ and $m_2=-0.61\pi$. Resolving the ambiguity consists in choosing the Gaussians with the largest weighting factor.}\label{fig:Gauss.Ambiguity}
\end{figure}
%%%%%%%%%%%%%%

\begin{example}[Multiplication of periodic Gaussians]\label{ex:multiplication.Gaussians}
The multiplication of periodic Gaussians is illustrated in \figref{fig:Gauss.Ambiguity} where $\tilde{\alpha}(\theta)$ and  $\tilde{f}(\theta,x) $ are shown with solid (black) lines; $m_{\alpha}=-0.12\pi$, $m_x=0.9\pi$, $v_x=v_{\alpha}=0.1$. The multiplication result, $\kappa(\theta,x)$, is shown with dotted lines where we see that many Gaussians (two are shown as others are negligible) are created in the reference period. This phenomenon,  well perceived thanks to the particular values of the parameters chosen in this example, $|m_\alpha - m_x|\approx \pi$, causes an ambiguity in the interpretation of the multiplication results. 
\end{example}


The multiplication of the Gaussians in \eqref{kappa} is done using \cite[Ch.~8.4]{Barber12_Book}\cite[Sec.~III.B]{Kreimer18}
\begin{align}
 \mcN(\theta; m_1, v_1) &\mcN(\theta; m_2, v_2)\\
 \label{Gauss.operations}
 &= \mcN(\theta; m_3, v_3)\mcN(m_1;m_2,v_1+v_2)\\
 m_3&=\frac{m_1 v_2+m_2 v_1}{v_1+v_2},\quad v_3 = \frac{v_1 v_2}{v_1 + v_2},
\end{align}
\ie the mean $m_3$ is the linear combination of $m_1$ and $m_2$; the weighting factor $\mcN(m_1;m_2,v_1+v_2)$ decreases exponentially with the squared difference $(m_1-m_2)^2$. 

In the spirit of the simplifications, we would like to approximate $\kappa(\theta,x)$ with a single Gaussian term chosen among those defined for different $l$. This is possible, because the case shown in \figref{fig:Gauss.Ambiguity}, leading to the ambiguity (more than one Gaussian appears as a result of the multiplication), occurs rarely; in fact, the appearance of multiple significant Gaussians is an artefact which would not be present if truly periodic distributions (such as Tikhonov) were used.

Using \eqref{Gauss.operations}, we see that all the Gaussian terms in \eqref{kappa} have the same variance, so we select the one with the largest weighting factor
\begin{align}\label{kappa.simple}
\kappa(\theta,x)
&\approx
\xi_{x}\mcN(\theta; m_{\alpha}, v_{\alpha})\mcN\Big(\theta; m_{x} + \hat{l}2\pi, v_{x}\Big)\\
&=\eta_{x} \mcN(\theta; m_{\kappa,x}, v_{\kappa,x})\\
\label{hat.l}
\hat{l}&=\argmin_{l\in\set{-1,0,1}}  |m_{\alpha}-m_x- l2\pi|,
\end{align}
where, using \eqref{Gauss.operations},
\begin{align}\label{}
\eta_{x}&=\xi_{x}\mcN(m_{\alpha};m_{x} + \hat{l}2\pi, v_{\alpha} +v_{x})\\
v_{\kappa,x} &= \frac{v_{\alpha} v_x}{v_{\alpha} + v_{x}}\\
\label{m.kappa}
m_{\kappa,x}&=\mcB_{[-\pi]}\left(\frac{m_{\alpha} v_{x} +(m_{x}+\hat{l}2\pi) v_{\alpha}}{v_{\alpha} + v_{x}}\right)
\end{align}
and
\begin{align}\label{B.folding}
\mcB_{[a]}(z)=  z+k2\pi, \quad k\in\Natural : z+k2\pi\in(a,a+2\pi]
\end{align}
is the folding operation returning the angle in the interval $(a,a+2\pi]$. In particular,  $\mcB_{[-\pi]}(z)$ returns $z$ to the reference interval which makes $\kappa(\theta)$ the prototype distribution. 

If $\hat{l}=0$, \eqref{kappa.simple} is identical  to what is done in \cite{Kreimer18} but, in general  \eqref{hat.l} allows us to deal with the ambiguity of the definition of the reference period; it acts as the phase disambiguation which guarantees that the absolute difference between two phases is smaller than $\pi$.

%%%%---
\subsubsection{Projection  $\mcP[\cd]$ and convolution}\label{Sec:conv.proj}

We want now to calculate the projection in \eqref{tilde.alpha.projection} $\mcP[\tilde{\phi}_{n-1}(\theta)]$, where the argument is the periodic distribution constructed from the prototype  we found above
\begin{align}\label{phi.n}
\phi_{n-1}(\theta)
&\propto \sum_{x\in\mcA}\kappa(\theta;  x)\\
&=\sum_{x\in\mcA}\eta_{x,n-1}\mcN(\theta; m_{\kappa,x,n-1}, v_{\kappa,x,n-1}).
%\label{sorted.means}
%\phi(\theta)
%&=\sum_{l=1}^{M} \hat{\eta}_l\mcN(\theta; \hat{m}_l, \hat{v}_l),
\end{align}
%where in \eqref{sorted.means} we use the \emph{sorted} means $m_{\kappa,x,n-1}$ denoted by $-\pi<\hat{m}_1< \hat{m}_2<\ld< \hat{m}_M\le \pi$; the corresponding weighting factors $\eta_{x,n-1}$ and variances are denoted, respectively, by $\hat{\eta}_l$ and $\hat{v}_l, l=1, \ld, M$. We skipped again the indexing with $n$ and $(t)$.

The projection on the space of Gaussian function requires calculation of the mean and the variance; this is done easily directly from on \eqref{phi.n}, yielding \cite{Kreimer18}
\begin{align}\label{}
\mc{N}(\theta; m_{\phi}, v_{\phi} ) &= \mcP\left[ \sum_{x\in\mcA}\eta_{x}\mcN(\theta; m_{\kappa,x}, v_{\kappa,x}) \right]\\
\label{m.phi}
m_{\phi}&=\frac{\sum_{x\in\mcA}\eta_{x} m_{\kappa,x}}{\sum_{x\in\mcA}\eta_{x}}\\
\label{v.phi}
v_{\phi} &=    \frac{\eta_{x}\big(v_{\kappa,x}+m^2_{\kappa,x}\big)}{\sum_{x\in\mcA}\eta_{x}}-m^2_{\phi},
\end{align}
where we skipped again the indexing $(\cd)_{n-1}$.

We argue, however, that the projection of the prototype is not (always) the best solution; again this is due to the very fact that it depends on a particular choice of $(-\pi, \pi]$ as the reference period. The question is how many different periods we should look at to obtain the alternative solutions?

Recall that any period $(a-\pi,a+\pi]$ will contain all the Gaussians or their images; using different $a$ we will look at different images of the Gaussians. Since there are $M=|\mcA|$ Gaussian representing $\tilde{\phi}_{n-1}(\theta)$, there are at most $M$ different periods containing different means of $M$ Gaussian.  

Let $-\pi\le a_1\le \ld, \le a_M\le\pi$ be the \emph{sorted} sequence of means $m_{\kappa,x,n-1}$; for convenience we define $a_0=-\pi$. It is easy to see that the interval $(a_j, a_j+2\pi]$, contains $M-j$ means $a_{j+1},\ld, a_M\in(-\pi,\pi]$ and $j$ means $a_1+2\pi, \ld, a_j+2\pi$. Alternatively, we can say that, independently of $a_j$, the Gaussians with means $\mcB_{[a_j]}(m_{\kappa,x}), x\in\mcA$, are sufficient to represent $\phi_{n-1}(\theta)$.

We can now generalize the projection \eqref{m.phi}-\eqref{v.phi} so that it can be calculated over arbitrarily defined period $(a_j,a_j+2\pi], j=0,\ld, M-1$. Namely,
\begin{align}\label{projection.j}
\mc{N}(\theta; \hat{m}_{\phi,j}, \hat{v}_{\phi,j} ) &= \mcP\left[ \sum_{x\in\mcA}\eta_{x}\mcN(\theta; \mcB_{[a_j]}(m_{\kappa,x}), v_{\kappa,x}) \right], \\
\label{m.phi}
\hat{m}_{\phi,j}&=\frac{\sum_{x\in\mcA}\eta_{x} \mcB_{[a_j]}(m_{\kappa,x})}{\sum_{x\in\mcA}\eta_{x})}\\
\label{v.phi}
\hat{v}_{\phi,j} &=    \frac{\eta_{x}\big(v_{\kappa,x}+m^2_{\kappa,x}\big)}{\sum_{x\in\mcA}\eta_{x}}-\hat{m}^2_{\phi,j}.
\end{align}
Among the projections defined for $j=0,\ld,M-1$, we choose the most representative/informative one, \ie the one with the smallest variance; the similar idea has been used in a different context in \cite{Shayovitz16}.

%%%%%%
\begin{example}[Projection] \label{ex:projection}
Suppose four Gaussians are present with the means $m_1=-0.75\pi$, $m_2=-0.25\pi$, $m_3=0.25\pi$, and $m_4=0.75\pi$, the variances $v_1=\ld =v_4=0.05$, and the weighting factors  $\eta_1=0.69$, $\eta_2=0.07$, $\eta_3=0.03$,  $\eta_4=0.21$. They are shown in \figref{fig:Gauss.Projection} using solid lines together with the three ``images'' from the period $(\pi,3\pi]$, which are shown with dotted lines. The four different projections obtained via \eqref{projection.j} for $j=0,\ld, 3$ are shown with dashed lines, where  \eqref{v.phi} yields  $\hat{v}_{\phi,1}=3.73$, $\hat{v}_{\phi,2}=1.86$, $\hat{v}_{\phi,3}=0.96$, and $\hat{v}_{\phi,4}=1.05$. Thus,  the  third Gaussian is the most informative representation and we show it  with a thick line; note that, since $\hat{m}_{\phi,3}=1.15\pi$, we return the mean to the reference period $(-\pi,\pi]$ via folding $\mcB_{[-\pi]}(\hat{m}_{\phi,3})=-0.85\pi$. The projection for $j=0$, \ie the one obtained from the reference period has a very large variance as it ignores the fact that the Gaussians with means $m_1=-0.75\pi$ and $m_4=0.75\pi$, which have large weighting factors, $\eta_1+\eta_4=0.9$, are close to each other on the circular axis.
\end{example}
%%%%%%

%%%%%%%%%%%%%%
\begin{figure}[bt]
\begin{center}
\psfrag{p1}[ct][cb][\siz]{$-\pi$}
\psfrag{p2}[ct][cb][\siz]{$\pi$}
\psfrag{p3}[ct][cb][\siz]{$3\pi$}
\scalebox{\sizf}{\includegraphics[width=\linewidth]{./figures/Gauss.Projection.eps}}
\end{center}
\caption{The projections of the Gaussian mixture (solid and dotted lines; black) are obtained using different intervals $(a_j,a_j+2\pi], j=0,\ld, M-1$, and are shown with dashed (green) line. The most informative Gaussian (with the minimum variance) is plotted using the thick dashed (green) line. }\label{fig:Gauss.Projection}
\end{figure}
%%%%%%%%%%%%%%

The somewhat cumbersome notation based on the intervals and  folding \eqref{B.folding} may be simplified but it will be useful to explain the approach in the case of multi-dimensional phase tracking.

Recapitulating, the whole projection is done in the following steps:
\begin{enumerate}
\item Sort the means $\set{m_{\kappa,x,n-1}}_{x\in\mcA}$ into $\set{a_j}_{j=0}^{M-1}$.
\item Find the projection via \eqref{projection.j}
\begin{align}\label{}
\mcN(\theta; \hat{m}_{\phi,j},\hat{v}_{\phi,j}),\quad j=0,\ld, M-1.
\end{align}
\item Pick the most informative one
\begin{align}\label{hat.j}
\hat{j}= \argmin_{j} \hat{v}_{\phi,j}.
\end{align}
\item Recover the prototype of the projection $\mcN(\theta; m_{\phi,n-1}, v_{\phi,n-1})$ via 
\begin{align}\label{}
 m_{\phi,n-1}=\mcB_{[-\pi]}( \hat{m}_{\phi,\hat{j}} ),\quad v_{\phi,n-1}  =\hat{v}_{\phi,\hat{j}},
\end{align}
where the folding $\mcB_{[-\pi]}(\cd)$ is necessary to ensure that the mean returns to the reference period $(-\pi, \pi]$; see also \exref{ex:projection}.
\end{enumerate}

Finally, to obtain $\alpha_n(\theta)\propto\mcN(\theta; m_{\alpha,n}, v_{\alpha,n})$ we have to convolve the projection results $\mcN(\theta; m_{\phi,n-1}, v_{\phi,n-1})$ with the periodic version of the Gaussian $\tilde{\mcN}(\theta;0,\sigma_w^2)$. This yields the final result
\begin{align}\label{}
m_{\alpha,n} & =  m_{\phi,n-1}\\
\label{v.alpha.n}
v_{\alpha,n}  &  = v_{\phi,n-1} +\sigma_w^2.
\end{align}

At this point it is easy to see that if the convolution was done before the projection, the variances $\hat{v}_{\phi,j}$ would be replaced by $\hat{v}_{\phi,j}+\sigma_w^2$. Adding the constant value $\sigma_w^2$ to all terms $\hat{v}_{\phi,j}$ is equivalent to \eqref{v.alpha.n} and, of course, would not change  the results of the search for the most informative representation in \eqref{hat.j}.

\subsection{Approximation of $P_n(x) $}\label{sec:P.x}

The final step which involves the Gaussian approximations and thus requires some care is given by \eqref{P.n.x} which we rewrite using explicit periodic notation
\begin{align}\label{P.n.x.tilde}
P_n(x) \propto\int_{-\pi}^{\pi}  \tilde{\alpha}_n(\theta)  \tilde{\beta}_n(\theta) \tilde{f}_n(\theta,x ) \dd \theta,\quad x\in\mcA.
\end{align}
We do it merely to emphasize again the possibility of ambiguity in the multiplication of the involved Gaussians. Instead of formal derivations we will take advantage of the lesson learnt in \secref{sec:mult}: multiplying two Gaussians we should look at two images and pick the one with the largest weighting factor; this is what \eqref{hat.l} does and the weighting factor depends on the difference between the means of the Gaussians. 

The situation is slightly different in \eqref{P.n.x.tilde} because we multiply three Gaussians. Thus, after multiplying $\alpha_n(\theta)$ and $\beta_n(\theta)$ 
\begin{align}\label{}
\alpha_n(\theta)\beta_n(\theta)
&\propto \xi_{\alpha\beta x,l}\mcN(\theta; m_{\alpha\beta,l}, v_{\alpha\beta}),\\
\xi_{\alpha\beta x,l}&=\mcN(m_{\alpha};m_\beta+l 2\pi, v_{\alpha}+v_{\beta}),\\
m_{\alpha\beta,l}&=v_{\alpha\beta} \big(m_\alpha/v_\alpha + (m_\beta+l 2\pi)/v_\beta \big),\\
1/v_{\alpha\beta} & = 1/v_\alpha+1/ v_\beta,
\end{align}
we keep temporarily two the most relevant terms (as shown in \figref{fig:Gauss.Ambiguity}), \ie those identified by two values of $l$ with the smallest difference $|m_{\alpha}-m_\beta+l 2\pi|$. Both terms are multiplied by $\tilde{f}_n(\theta,x )$ yielding 
\begin{align}\label{abx}
\alpha_n(\theta)\beta_n(\theta)&f_n(\theta,x )
\propto \xi_{\alpha\beta x,l,k}\mcN(\theta; m_{\alpha\beta x,l,k}, v_{\alpha\beta x}),\\
\label{xi.abx}
\xi_{\alpha\beta x,l,k}&=\xi_{\alpha\beta x,l}\mcN(m_{\alpha\beta,l}; m_x+k 2\pi; v_{\alpha\beta}+v_x),
%\label{m.abx}
%m_{\alpha\beta x,l,k}&=v_{\alpha\beta x} \big(m_{\alpha\beta,l}/v_{\alpha\beta} + (m_x+k 2\pi)/v_x \big),\\
%\label{v.abx}
%1/v_{\alpha\beta x} & = 1/v_\alpha+1/v_\beta + 1/v_x.
\end{align}
where
out of the terms $\xi_{\alpha\beta x,l,k}$  indexed with $l$ and $k$, we then choose the one with maximum value of $\xi_{\alpha\beta x,l,k}$, which also becomes the final result of the integration \eqref{P.n.x.tilde}
\begin{align}\label{}
P_n(x) \propto \xi_{\alpha\beta x,l,k},
\end{align}
and thus the mean $m_{\alpha\beta x,l,k}$ and the variance $v_{\alpha\beta x}$ are irrelevant.

The immediate simplification which gets rid of the \emph{joint} search over $l$ and $k$ consists in two separate search steps: first, we choose one Gaussian to represent the product $\alpha_n(\theta)\beta_n(\theta)$; this determines $l$. Next we perform the multiplication with $f_n(\theta,x )$ searching for $k$. 

What can we say about this simplification? The ultimate objective is to calculate the bit-level message by averaging $P_n(x)$ over different $x\in\mcA$, see \eqref{demodulation}. The phases of all $x$ are spread uniformly on the reference period; thus, for some $x=x_0$ the term $f_n(\theta, x_0 )$ will be always much larger than the terms produced by other $x\neq x_0$ even without the shift by $k$ as defined in \eqref{abx}-\eqref{xi.abx}. Therefore, the separate search should not affect the results significantly.  

Finally, if the iterative decoding/phase tracking is targeted, the joint search over $l$ and $k$ may be important: averaging over $x$ we must take into account the  priori terms $P^{\tr{a}}_n(x)$ and not only $f_n(\theta, x_0 )$.  






==> Includes/Tracking.v2.tex <==
%!TEX root =  ../Phase.Tracking.v2.tex
\section{Phase tracking}\label{sec:phase.track}
%%%%%
%\subsection{Message passing on the graph}\label{Sec:MP.graph}
%%%%%%%%%%%%%%
\begin{figure}[bt]
\begin{center}
\scalebox{0.8}{\input{./figures/Graph.RRHARQ.x.2D.tex}}
\end{center}
\caption{Graph defining the relationship between the variables in the phase tracking problem; the messages exchanged between the nodes are shown together with the arrows indicating the direction of the exchange.}
\label{fig:graph.tracking}
\end{figure}
%%%%%%%%%%%%%%%

Our goal now is to find 
\begin{align}\label{Px}
P_n(a)=\PR{x_{n}=a|\by}, \quad a\in\mcA.
\end{align} 
and this is done exploiting the relationships between the involved random variable. 

As in \cite{Colavolpe05,Kreimer18} we show in \figref{fig:graph.tracking} a graph which captures this relationship: the squares represent the functions taking as arguments the variables which, in turn, are represented by the directly connected circles. In particular
\begin{align}
\label{f.n.x}
f_n(\theta_n,x_n)  & \propto \exp\left(-\SNR\Big|y_n-x_n\e^{\jmath\theta_n}\Big|^2\right)
\end{align}
corresponds to the relationship defined in \eqref{y.kn} and 
\begin{align}\label{p.w}
p_w(\theta_n,\theta_{n+1}) =\omega(\theta_n-\theta_{n+1})
%& \propto \mcN(\theta_n; \theta_{n+1},\sigma_w^2)
%\exp\left(-\frac{(\theta_n-\theta_{n+1})^2}{\sigma_w^2}\right)
\end{align}
corresponds to \eqref{theta.Wiener} and thus $\omega(\theta)=\mcN(\theta;0,\sigma_w^2)$, where we use the wrapped Gaussian distribution defined as\
\begin{align}\label{Normal.pdf}
\mcN(\theta;m,v)=\frac{1}{\sqrt{2\pi v}}\sum_{k=-\infty}^{\infty}\exp\left(-\frac{(\theta-m-k2\pi)^2}{2v}\right).
\end{align}

In \figref{fig:graph.tracking} we also show a shaded rectangle labeled as ``modulation/coding graph''; it also contains a graph which describes the relationship $\bx  \rightarrow \bs \rightarrow \bc \rightarrow \bb$, and its knowledge is used for the demodulation (to implement \eqref{demodulation}) and for the decoding \eg to implement a sum-product algorithm for \gls{ldpc} decoding \cite[]{}.

What is important to note at this point is  that the relationships induced by the modulation/coding graph are ignored during the phase tracking; essentially, this means that the symbols $x_n$ are assumed to be a priori \gls{iid}, with non-informative distribution, \ie $P^{\tr{a}}_n(a)\propto 1$. 

In a case we would like  to perform the joint decoding/demodulation/phase tracking, as done, \eg in \cite{Colavolpe05}\cite{Kreimer18}\cite{Alfredsson19}, we would have to use non-uniform distribution $P^{\tr{a}}_n(x)$ based on the decoding results. While this is not our concern, we preserve the notation $P^{\tr{a}}_n(\cd)$ which allows for the application of this iterative approach on the top of the algorithms we will propose.

As a direct consequence of ignoring the structure imposed on $x_n$ (by the coding), the graph we deal with in \figref{fig:graph.tracking} is a tree, \ie contain no loops. Therefore, the efficient marginalization can be done exactly by the \gls{mp} algorithm as follows \cite{Colavolpe05,Shayovitz16,Kreimer18}
\begin{align}\label{P.n.x}
P_n(a) \propto\int_{-\pi}^{\pi}  \alpha_n(\theta)  \beta_n(\theta) f_n(\theta,a ) \dd \theta,\quad a\in\mcA,
\end{align}
where
\begin{align}\label{alpha}
\alpha_n(\theta)&\propto \left(\alpha_{n-1}(\theta)  \gamma_{n-1}(\theta)\right) \convop 
\omega(\theta)\\
%\mcN(\theta;0,\sigma_w^2),\\
\label{beta}
\beta_n(\theta)&\propto \left(\beta_{n+1}(\theta) \gamma_{n+1}(\theta) \right) \convop 
\omega(\theta)\\
%\mcN(\theta;0,\sigma_w^2),\\
\label{gamma}
\gamma_n(\theta)&\propto\sum_{a\in\mcA} P^{\tr{a}}_n(a) f_{n}(\theta,a ),%=\sum_{x\in\mcA}  f_{n}(\theta,a ),
\end{align}
are (proportional to) the marginal distributions of the phase $\theta_n$ conditioned, respectively, on $y_0,\ld,y_{n-1}$, on $y_{n+1},\ld,y_{N}$, and  on $y_n$. All the distributions of the phase are periodic and so is the convolution in \eqref{alpha} and \eqref{beta}. 
%These equations are practically the same as those appearing in the \gls{bcjr} recursion \cite{BCJR} well known in the area of decoding of convolutional codes to obtain the distribution of the bits, which has discrete argument. Here, derived from the graph representation, they are applied to calculate the continuous-argument distributions of the phase. 

%%%%%%%%%
\section{Parametric message passing strategies}\label{Sec:Parametric.MP}
The operations \eqref{P.n.x}-\eqref{gamma} which allow us to calculate $P_n(a)$ may be implemented on the discretized versions of the distributions $\alpha_n(\theta)$, $\beta_n(\theta)$, and $\gamma_n(\theta)$ defined over the samples of $\theta\in(-\pi, \pi]$. In such a \gls{dmp} the multiplications and additions are straightforward to implemented and the convolution is efficiently implemented via \gls{fft}. 

However, to ensure sufficient precision,  large number of samples may be necessary implying possibly a large complexity and storage burden.\footnote{The number of sample, $N_{\theta}$, required to represent the distributions over the interval of length $2\pi$ may be estimated from their approximate Nyquist frequency, $F_{\tr{Nyq.}}$, as $N_{\theta}>4\pi F_{\tr{Nyq.}}$. To find the latter we approximate the function $f_n(\theta,x)$ as a Gaussian with the variance $\No/(2|x|^2)$, see \cite[Eq.~(XXX)]{Shayovitz16}, so its (approximate) Nyquist frequency is $F_{f,\tr{Nyq.,}}=c|x|\sqrt{2/\No}$ (where $c$ depends on how we define the frequency support of the spectrum, \eg $c=1.5$ for 10\% spectral overlap.). Similarly, for the Gaussian distribution $\omega(\theta)$ the respective value is $F_{\omega,\tr{Nyq.}}\approx c/\sigma_w$ . Thus the rule of thumb requirement is $N_{\theta}>10\pi/\min\set{\sigma_2 , \sqrt{\No/2}  } $ so the number of samples is inversely proportional to the level of the phase noise $w_n$ or the level of the additive noise $z_n$. Since decreasing the levels of the noise is required for large constellations, this is where the \gls{dmp} will be suffer the most from the complexity issues. For example, in the examples based on $16$-\gls{qam}, we have $\SNR\approx 13$dB and $\sigma_w^2=0.01$, which requires $N_\theta>125$. Of course, this ballpark number does not take into all effects, \eg due to multiplications of the distributions.} Therefore, many previous works have gone in the direction of parametric representation of the involved periodic distributions. Then, instead of tracking the samples in \gls{dmp}, we only need to track (a few) parameters which represent the distributions.

We thus have to find a family of the distributions, $\mcF$, on which the operations defined in \eqref{P.n.x}-\eqref{gamma} are easily dealt with. In particular, we have to handle multiplication of the periodic functions as well as, the convolution in \eqref{alpha} and \eqref{beta}; the integration in \eqref{P.n.x}, when done on the parametric forms of distributions, is usually straightforward. 

In other words, if $\alpha_n(\theta), \beta_n(\theta), \gamma_n(\theta), \omega(\theta)\in\mcF$  and $\mcF$ is closed under  multiplication and convolution, the parametric \gls{mp} will be immediately obtained. This condition,  however, does not materialize with the most popular circular distributions such as the wrapped Gaussian distributions or  the Tikhonov distributions \cite{Kurz16}. Namely, the space of wrapped Gaussian distributions is not closed under multiplications, while the Tikhonov space is not closed under convolution. Thus, independently of the choice we make, approximations will be necessary.

In this work we consider a family of  Tiknonov distributions which were already used, \eg in \cite{Colavolpe05}\cite{Barbieri07}\cite{Shayovitz16}, and are defined as
\begin{align}\label{Tikh.definition}
\mcT(\theta; z)= \frac{\e^{\Re[z\e^{-\jj \theta}]}}{2\pi I_0(|z|)},
\end{align}
where $I_0(\cd)$ is the zero-th order modified Bessel function and $z$ is a complex parameter whose phase is the circular mean of the underlying variable and the value of $|z|$ is, approximatively, a measure of precision.

We note that $f_n(\theta,a) \in \mcF$, that is, we can write \eqref{f.n.x} as
\begin{align}\label{f.n.x.Tikh}
f_n(\theta,a)&\propto \xi_{f,n}(a)\mcT\big(\theta; z_{f,n}(a)\big) \\
\label{z.fn}
z_{f,n}(a)&=2\frac{y_n a^{*}}{\No}\\
\label{xi.f.n}
\xi_{f,n}(a)&=\e^{ -\frac{|a|^2}{\No} }I_0\big(|z_{f,n}(a)\big)=\e^{-\frac{|a|^2}{\No} +\hat{I}_0(|z_{f,n}(a)|)}
%\eta_{f,n}(a)&=-\frac{|a|^2}{\No} + |z_{f,n}(a)| + \hat{I}_0\big(|z_{f,n}(a)|\big),
\end{align}
where, to avoid numerical issues due to the exponential grows of $I_0(\cd)$, we use its log-version
\begin{align}
\hat{I}_0(x) &= \log I_0(x) = x  + \Delta(x),
\end{align}
with $\Delta(x)$ being the log-domain corrective factor. The approximation $\Delta(x)\approx -\frac{1}{2}\log(2\pi x)$ already shown in \cite[Eq.~(96)]{Shayovitz16}\cite[Eq.~(18)]{Pecorino15} is tight for large $x$ but does not apply for small arguments because $\Delta( 0 )=0$. Thus, for a better accuracy, $\Delta(x)$ may be implemented via lookup table. 


Instead of Tikhnov functions we might opt for the wrapped Gaussian family \eqref{Normal.pdf} but, to  take care of their periodic nature, particular attention is required when dealing with multiplication  \cite[Sec.~II.B]{Kurz16}.\footnote{This aspect is not always emphasized in the literature: in some works,  \eg \cite{Kreimer18}, the Gaussian distributions are used without explicit wrapping. Ignoring the circularity, it produces an apparent closeness under multiplication but may lead to interpretation errors when ``locking'' on the wrong phase, see \cite[Fig.~1]{Kurz16}.} Moreover, comparing to the Tikhonov distributions, Gaussians are less well suited to represent the uniform or almost-uniform distributions of the phase; a case which occurs, \eg when using high order \gls{qam} constellations for which $|a|$ may be small in \eqref{z.fn} yielding small $|z_{f,n}(a)|$.

From \eqref{Tikh.definition} we obtain
\begin{align}\label{Tikh.multiplication}
\mcT(\theta; z_1)\mcT(\theta; z_2)
&=\frac{I_0(|z_1+z_2|)}{2\pi I_0(|z_1|)I_0(|z_2|)}
\mcT(\theta; z_1+z_2),
\end{align}
while the convolution with the Gaussian, appearing in \eqref{alpha} and \eqref{beta}, must be treated via  approximations. It is done using moment-matching explained in \appref{conv.T.G} and which we summarize as follows:
\begin{align}\label{Tik.h.Normal.convolution}
\mcT(\theta; z)&\convop\mcN(\theta; 0,v)
\approx  \mcT\big( \theta; C(z,v) \big)\\
\label{C.zv}
C(z,v)&=
\frac{z}{1+v(|z|-0.5)}\IND{|z|>1}+
z(1-\frac{v}{2})\IND{|z| \leq 1}.
\end{align}

The main need for approximations, however,  stems from  the presence of $\gamma_n(\theta)$ which, being a mixture of distributions from $\mcF$,  see \eqref{gamma}, does not belong itself to $\mcF$.  And there are essentially two approaches which may be used to deal with this issue; we compare them in the following. 

%%%%%%%
\section{Pre-MP approximation}\label{pre.MP}
In this approach, the approximate distributions $\hat{\gamma}_n(\theta)$ are obtained \emph{before} the steps of \gls{mp} \eqref{alpha}-\eqref{beta} are executed, that is
\begin{align}\label{gamma.projection.first}
\hat{\gamma}_n(\theta)
&=\mcT\Big(\theta;  z_{\gamma,n} \Big)\\
\label{gamma.projection.first.cases}
&=
\begin{cases}
\mcT\big(\theta; z_{f,n}(x_{n})\big) &\text{if}\quad n= l L\\
\mcF\Big[ \sum_{a\in\mcA}\eta_{f,n}(a)\mcT\big(\theta;z_{f,n}(a )\big) \Big]&\text{if}\quad n\neq l L
\end{cases}\\
\label{eta.f.n}
\eta_{f,n}(a)&=\exp\left(-\frac{|a|^2}{\No}+ \hat{I}_0\big(|z_{f,n}(a)|\big)+\log P^{\tr{a}}_n(a)\right)
\end{align}
where,  at the pilot positions  $n=lL$, we use directly the parameter of the Tikhonov distribution $f_{n}(\theta, x_{n} )$. Otherwise, we project $\gamma_n(\theta)$ onto $\mcF$ via circular moment matching, as denoted by $\mcF[\cd]$. \appref{Sec:CMM} explains how $z_{\gamma,n}$ is obtained from the series $\bset{z_{f,n}(a)}_{a\in\mcA}$ and $\bset{P^{\tr{a}}_n(a)}_{a\in\mcA}$;  we use there the same approach as in \cite[Appendix~A]{Shayovitz16} removing oversimplifications, whose impact will be shown later in \secref{}.

A similar projection approach as in \eqref{gamma.projection.first} was used previously in \cite{Colavolpe05}\cite{Barbieri07}\cite{Alfredsson19} but instead of circular moment matching, a  Gaussian was first matched to $\pdf(y_n|\theta_n,a)\propto f_n(\theta,a)$ from which a Tiknonov distribution was derived as
\begin{align}
\label{hat.z.gamma}
\hat{z}_{\gamma,n}&=2\frac{y_n\mfm_n^{*}}{\No+ \mfv_n},\\
\label{m.n.A}
\mfm_n&=\sum_{a\in\mcA}  a P^{\tr{a}}_n(a) ,\\
\label{v.n.A}
\mfv_n&=\sum_{a\in\mcA}  |a|^2 P^{\tr{a}}_n(a)   -  |\mfm_n|^2,
\end{align}
where  $\mfm_n$ and $\mfgv_n$ are the mean and the variance of the symbol at time $n$. 

Next, if all the distributions are from the Tikhonov family, \ie $\alpha_n(\theta)=\mcT(\theta;z_{\alpha,n})$ and $\beta_n(\theta)=\mcT(\theta;z_{\beta,n})$, using $\hat{\gamma}_{n}(\theta)$ instead of $\gamma_n(\theta)$ in \eqref{Tikh.multiplication} and \eqref{Tik.h.Normal.convolution}, we obtain the following parametric \gls{mp} :
\begin{align}
\label{z.alpha.init}
z_{\alpha,0}&=0\\
\label{z.alpha}
z_{\alpha,n}&= C(z_{\alpha,n-1} + z_{\gamma,n-1}, \sigma_w^2), \quad n=1, \ld,N-1\\
\label{z.beta.init}
z_{\beta,N}&=0\\
\label{z.beta}
z_{\beta,n}&= C(z_{\beta,n+1} + z_{\gamma,n+1}, \sigma_w^2), \quad n=N-1,\ld,1,
\end{align}
where $C(z,v)$ is defined in \eqref{C.zv}. 

The \gls{mp} in \eqref{z.alpha.init}-\eqref{z.beta} is exactly equivalent to the \gls{mp} defined in \cite[Eq.~(36)-(37)]{Colavolpe05} if we assume $|z|>1$ and  is provided as a starting point for the discussion.

Using \eqref{Tikh.multiplication}  and \eqref{f.n.x.Tikh}--\eqref{xi.f.n} in \eqref{P.n.x}, the extrinsic symbol probabilities are calculated as \cite[Eq.~(35)]{Colavolpe05}
\begin{align}\label{P.a.final}
P_n( a )&\propto \int_{0}^{2\pi} \mcT(\theta;z_{\Sigma,n}(a))\frac{\xi_{f,n}(a) I_0\big(|z_{\Sigma,n}(a) |\big)}{I_0\big(|z_{f,n}(a)|\big)}\dd \theta\\
%&=I_0\big(|z_{\Sigma,n}(a)|\big)\e^{-\frac{|a|^2}{\No}}\\
\label{P.a.final.2}
&=\exp\left(-\frac{|a|^2}{\No} + \hat{I}_0\big(|z_{\Sigma,n}(a)|\big)\right)\\
\label{z.Sigma.n}
z_{\Sigma,n}(a)&=z_{\alpha,n}+z_{\beta,n}+2\frac{y_n a^{*}}{\No}.
\end{align}


The simplicity of the \gls{mp} defined by \eqref{z.alpha.init}-\eqref{z.beta} is very appealing but the problem stems from the following: 

\begin{proposition}\label{lemma.z0} If the constellations $\mcA$ may be decomposed into constant-modulus, zero-mean sub-constellations, then, using non-informative prior $P^{\tr{a}}(a)\propto 1$,  the projection results of \eqref{gamma.projection.first} are non-informative for payload symbols, that is, $z_{\gamma,n}=0, n\neq lL$.
\end{proposition}
\begin{proof} See \appref{Sec:Proof.lemma.z0}.
\end{proof}

A similar observation was made before, \eg in \cite[Sec.~I]{Shayovitz16} or \cite[Sec.~IV]{Pecorino15}, but was based on the approximation  introduced in \cite[Sec.]{Colavolpe05} for which, a non-informative $\hat{\gamma}_n(\theta)$ was obtained whenever $\mcA$ was zero-mean. Here, using the projection based on moment-matching the zero-mean condition is necessary but not sufficient; for details see \appref{Sec:Proof.lemma.z0}. 

For the most popular \gls{psk} and \gls{qam} constellation (which may be decomposed into constant modulus, zero-mean sub-constellations) we still obtain the non-informative $\hat{\gamma}_n(\theta)$. Nevertheless, with the moment matching approach, we might construct zero-mean constellations which will provide the informative distribution $\hat{\gamma}_n(\theta)$; of course, this potentially interesting issue is out of scope of this work.

%%%%%%%%%%%%%%%%%%%%%
\section{Pre-MP with iterative refinement}\label{Sec:It.EP}

Since $\hat{\gamma}_n(\theta)\propto 1$ is non-informative, it does not help in the phase estimation. This is also why, the previous works based on this approach combined it with the feedback from the decoder, \eg \cite{Colavolpe05}\cite{Barbieri07}\cite{Alfredsson19}. Such a feedback, \ie non-uniform $P^{\tr{a}}(a)$, provides prior on the constellation that  transforms $\hat{\gamma}_n(\theta)$ into a non-uniform (thus, informative) distribution.

The feedback from the decoder may be  definitely useful but, as already said, we cannot always rely on it so our objective is to obtain the most efficient ``stand-alone'' phase-tracking algorithm. To exploit the constraints imposed by the discrete constellation and to take advantage of the extreme simplicity of \eqref{z.alpha.init}-\eqref{z.beta} we need to implement the projection taking advantage of the phase tracking results in an iterative manner; hence we will use the parenthesized superscript $^{(i)}$ to denote the variables/functions obtained in the $i$-th iteration, where $i=1,\ld, I$ and $I$ is the maximum iteration number;  superscripting the distributions with $^{(0)}$ means that they are non-informative.

%Literature proposes different approaches to define the iterations and the one suggested in \cite[Sec.~III.C]{Alfredsson19} postulates, for each iteration $i=1,\ld, I$, to replace the prior $P^{\tr{a}}_n(a)$  with the extrinsic probability from the previous iteration $P^{(i-1)}_n(a)$. For example, this can be done by recalculating the projection \eqref{gamma.projection.first.cases} in the $i$-th iteration using weighting coefficients
%\begin{align}
%\eta^{(i)}_{f,n}(a)&=\exp\left(-\frac{|a|^2}{\No}+ \hat{I}_0\big(|z_{f,n}(a)|\big)+\log P^{(i-1)}_n(a)\right);
%\end{align}
%similarly we may replace $P^{\tr{a}}_n(a)$ with $P^{(i-1)}_n(a)$ in \eqref{hat.z.gamma}-\eqref{v.n.A}. 
%
%And while  reusing the outgoing message from the node goes against the \gls{mp} principle, we have to remember that the projection on $\mcF$, which yields $\hat{\gamma}_n(\theta)$, is very crude. Thus, even violating the fundamental principles of  the \gls{mp} may yield improvements.

We will follow the approach postulated by the \gls{ep} \cite[Ch.~3.2]{Minka01}, which tries to ``match'' the distributions before and after the projection taking into account the results from the previous iteration. In our case this would mean matching the posterior distributions of $\theta$, calculated from the projection $\hat{\gamma}^{(i)}_n(\theta)$ and from the original distribution $\gamma_n(\theta)$
\begin{align}
\nonumber
\hat{\gamma}^{(i)}_n(\theta)\Big[\alpha^{(i-1)}_n(\theta)&\beta^{(i-1)}_n(\theta)\Big]\\
\label{equal.proba.approx}
&\approx
\gamma_n(\theta)\Big[\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)\Big].
\end{align}
Of course, for $i=1$, using  non-informative distributions $\alpha^{(0)}(\theta)\propto 1$ and $\beta^{(0)}(\theta)\propto 1$, reduces \eqref{equal.proba.approx} to  $\hat{\gamma}^{(1)}_n(\theta)\approx \gamma_n(\theta)$; this is what was done in \secref{pre.MP}.

We can calculate the \gls{rhs} of \eqref{equal.proba.approx} as
\begin{align}
\nonumber
\gamma_n(\theta)\Big[\alpha^{(i-1)}_n(\theta)&\beta^{(i-1)}_n(\theta)\Big]\\
\label{apost.theta.i1}
&=
\sum_{a\in\mcA} \eta^{(i-1)}_{\Sigma,n} (a) \mcT\big(\theta; z^{(i-1)}_{\Sigma,n}(a) \big),
\end{align}
where
\begin{align}
\label{eta.Sigma.n.i1}
\eta^{(i-1)}_{\Sigma,n}(a)&=\e^{-\frac{|a|^2}{\No}+ \hat{I}_0\big(|z^{(i-1)}_{\Sigma,n}(a)|\big)+\log P^{\tr{a}}_n(a)}\\
&=P^{(i-1)}_n(a)P^{\tr{a}}(a)
\end{align}
represents the posterior probability of the symbols obtained in the iteration $i-1$, and $z^{(i-1)}_{\Sigma,n}(a)$ is the same as \eqref{z.Sigma.n} calculated in the iteration \mbox{$i-1$}. 

The remaining question is how to obtain $\hat{\gamma}_n^{(i)}(\theta)$ from \eqref{apost.theta.i1} and \eqref{equal.proba.approx} which we address in the following.

%%%%%%%%%%%%%%%
\subsection{Pitfalls of Expectation Propagation}
Since we have started iterative improvements considerations in the spirit of the \gls{ep}, it is natural to apply it to the problem at hand. This means concretely that i)~the projection  operation, $\mcF[\cd]$, is applied to the \gls{lhs} and \gls{rhs}  sides of \eqref{equal.proba.approx} and ii)~the approximation sign is replaced with equality (or rather, proportionality $\propto$), yielding
\begin{align}\label{EP.iterations}
\hat{\gamma}^{(i)}_n(\theta) 
&=\mcT(\theta; z^{(i)}_{\gamma,n})\\
\label{EP.division}
&\propto \frac
{\mcF\Big[\sum_{a\in\mcA} \eta^{(i-1)}_{\Sigma,n} (a) \mcT\big(\theta; z^{(i-1)}_{\Sigma,n}(a) \big)\Big] }
{\mcT\big(\theta; z^{(i-1)}_{\alpha,n}+z^{(i-1)}_{\beta,n} \big)}\\
\label{EP.division.2}
&\propto \frac{ \mcT\Big(\theta; z^{(i-1)}_{\tr{post},n}\Big)  }{ \mcT\Big(\theta; z^{(i-1)}_{\alpha,n}+z^{(i-1)}_{\beta,n} \Big)}\\
\label{z.gamma.i}
z^{(i)}_{\gamma,n}&= z^{(i-1)}_{\tr{post},n}  - z^{(i-1)}_{\alpha,n} - z^{(i-1)}_{\beta,n}.
\end{align}

The elegant formulation of  the \gls{ep} is indeed appealing but suffers from a problem due to the division of the distributions in \eqref{EP.division.2}, or equivalently, due to subtraction of the coefficients in \eqref{z.gamma.i}. This problem has been already recognized in the literature, particularly in the context of the Gaussian \gls{ep}, where the division of the distributions may yield a ``Gaussian'' with negative variance, \eg \cite[Sec.~IV.B]{Senst11} \cite[Sec.~IV.A]{Cespedes14}; such distributions are uninterpretable in our application. 

In the context of the Tikhnov distribution we are using, there is no problem of the parameters which would yield uninterpretable distributions, nevertheless, the problem remains. To understand intuitively its source we may assume that i)~$\angle z^{(i-1)}_{\tr{post},n} =\angle (z^{(i-1)}_{\alpha,n}+z^{(i-1)}_{\beta,n})$, and ii)~$|z^{(i-1)}_{\tr{post},n}|<|z^{(i-1)}_{\alpha,n}+z^{(i-1)}_{\beta,n}|$. This means that i)~the circular means of the approximate posterior distribution, $\mcT\big(\theta; z^{(i-1)}_{\tr{post},n}\big) $ and of the ``extrinsic'' distribution (defined by  the product $\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)$) coincide (remember, the phase $\angle z^{(i-1)}_{\tr{post},n}$ defines the circular mean), and ii)~the posterior distribution is ``larger" than the extrinsic distribution.\footnote{This may occur because the projection takes into account the symbols which widen the distribution.} 

Then, carrying out the subtraction in \eqref{z.gamma.i} we will obtain
\begin{align}
z^{(i)}_{\gamma,n}
&= (|z^{(i-1)}_{\tr{post},n}|  - |z^{(i-1)}_{\alpha,n} + z^{(i-1)}_{\beta,n}|\big)\e^{\jj \angle z^{(i-1)}_{\tr{post},n}}\\
&=|z^{(i-1)}_{\tr{post},n}|\e^{\jj(\angle z^{(i-1)}_{\tr{post},n}+\pi)}.
\end{align}
That is, the circular mean of the new distribution $\mcT(\theta; z^{(i)}_{\gamma,n})$ will be  in disagreement (by the largest possible value of $\pi$) with the mean of the posterior and extrinsic distributions obtained from the previous iteration. This is clearly wrong.

To deal with this \gls{ep}-typical problem,  heuristics were devised for the Gaussian \gls{ep} where the problem is clearly identified, \ie the variance becomes negative. For example, \cite[Sec.~IV.B]{Senst11} proposed to eliminate the division, which here would mean $z^{(i)}_{\gamma,n}=z^{(i-1)}_{\tr{post},n}$ , while \cite[Sec.~IV.A]{Cespedes14} removed the update, \ie $z^{(i)}_{\gamma,n}=z^{(i-1)}_{\gamma,n}$ .  

However, to apply such heuristics in our case we would have to i)~devise a strategy to identify the problem for the Tikhnov distribution in the case which is more general than the equal-phase example we gave above, and ii)~rely on many iterations to overcome the disruptions in the convergence introduced by these heuristics. 

Moreover, it simply seems that the generic \gls{ep} may not be the best solution for the case we deal with. Hence we propose to go back to the very principle of distribution matching defined in \eqref{equal.proba.approx} taking into account the structure of $\gamma_n(\theta)$.

%%%%%
\subsection{Mixture-oriented projection}\label{Sec:Constr.Proj.}

The principal observation is that, although  $\gamma_n(\theta)$ defined in \eqref{gamma} is a mixture of the Tikhonov distributions $\mcT\big(\theta; z_{f,n}(a)\big)$ with weighting factors $\xi_{f,n}(a)$ (see \eqref{z.fn}-\eqref{xi.f.n}), after the multiplication with the extrinsic distribution in \eqref{apost.theta.i1} (defined by the product $\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)$), only some of the mixture terms are relevant in the posteriori distribution, \ie those with ``sufficiently'' large values of $\eta^{(i-1)}_{\Sigma,n}(a)$. Removing these irrelevant terms will not change (significantly) nor the posterior distribution itself, nor its projection on the Tikhnov space $\mcT\big(\theta; z^{(i-1)}_{\tr{post},n}\big)$.

The idea is thus, to remove the irrelevant terms from the mixture $\gamma_n(\theta)$ \emph{before} the projection on the space $\mcF$, using, as a criterion, the weighting coefficients of the posterior  distribution. The resulting procedure will i) keep the spirit of \eqref{equal.proba.approx}, ii) be simple to implement, and iii) avoid the division of distribution which is at the root of the problem in the \gls{ep}. 

In fact, with the proposed approach, we focus on the fact that the distribution $\gamma_{n}(\theta)$ is a mixture of distributions with well-defined meaning: each term is related to the particular symbol in the constellation. By allowing to change the weights of the mixture terms (here, removing the term may be seen as zeroing of its weight, but more sophisticated versions might be devised) we keep the parameters of the distributions in the mixture (the terms $z_{f,n}(a)$) unaltered. This is why we dub this approach ``mixture-oriented" (MO) projection which  stands in contrast with the \gls{ep} which ignores the structure of $\gamma_n(\theta)$; in particular, the fact that $\gamma_n(\theta)$ is a mixture.

We can reformulate the above idea replacing $\mcA$ with the ``trimmed'' constellation $\mcA^{(i)}_n\subset \mcA$,  trimming/removing these symbols $a$ whose contribution to the posterior distribution \eqref{apost.theta.i1} is negligible as judged by the posterior symbol probability $\eta^{(i-1)}_{\Sigma,n}(a)$. 

For example, the weights are first ordered, $\eta^{(i-1)}_{\Sigma,n}(a_0)>\eta^{(i-1)}_{\Sigma,n}(a_1)>\ld>\eta^{(i-1)}_{\Sigma,n}(a_{M-1})$, and then normalized, $\sum_{m=0}^{M-1} \eta^{(i-1)}_{\Sigma,n}(a_m)=1$.\footnote{The ordering and normalization must be carried our for each time $n$ and each iteration $i>1$.} Next, we the trimmed constellation is defined as $\mcA^{(i)}_n=\set{a_0,\ld,a_{M'-1}}$ where 
\begin{align}
M'= \argmin_{k}\set{ k : \sum_{m=0}^{k-1} \eta^{(i-1)}_{\Sigma,n}(a_m) \ge 1-\epsilon}
\end{align}
where $\epsilon$ is arbitrarily set, \eg $\epsilon=0.05$.

Since in practice, the cardinality of  $\mcA^{(i)}_n$ is quite small, and to avoid cumbersome trimming of the constellation,  we might opt for the extreme simplification of taking only one symbol with a maximum posterior, that is $\mcA^{(i)}_n=\set{a_0$}; since normalization is not necessary, we may operate directly in the logarithmic scale so, from \eqref{eta.Sigma.n.i1}, we have
\begin{align}\label{a.0}
a_{0,n}^{(i)} = \argmax_{a \in\mcA} \SET{  -\frac{|a|^2}{\No}  + \hat{I}_0(|z^{(i-1)}_{\Sigma,n}(a)|) +P^{\tr{a}}(a) }
\end{align}
and, the projection being not necessary, we have
\begin{align}\label{z.gamma.a.0}
 z_{\gamma,n}^{(i)}&=z_{f,n}\big(a_{0,n}^{(i)}\big).
\end{align}

Of course, such crude approximation affects accuracy. On the other hand, dealing with one symbol, we get rid of all the operations such as moving from the logarithmic to the linear scale, the normalization of the weighting coefficients, or the projection. From the implementation perspective, this huge advantage may outweigh some performance loss. 

In order to deal with imperfections related to these (or other) approximations, the parameters $z_{\gamma,n}^{(i)}$ obtained in the $i$-the projection may be smoothed
\begin{align}\label{z.smoothing}
\tilde{z}_{\gamma,n}^{(i)} = \zeta z_{\gamma,n}^{(i)} +(1-\zeta) \tilde{z}_{\gamma,n}^{(i-1)},
\end{align}
where $\zeta<1$ must be chosen to strike a balance between the new update and the history accumulated in the previous estimate ; this is a usual heuristics in the \gls{ep}, \eg \cite[Sec.~IV.A]{Cespedes14} and, here, \ls{we choose $\zeta=0.2$.} 



%We will thus keep the symbols $a$ in the trimmed constellation $\mcA^{(i)}_n$ when
%\begin{align}
%-\frac{|a|^2}{\No} +\hat{I}_0\big(|z_{\Sigma,n}^{(i-1)}(a)|\big) > -\frac{|\hat{a}_n|^2}{\No} +\hat{I}_0\big(|z_{f,n}(\hat{a}_n)|\big).
%\end{align}
%or, using $\hat{I}_0(x)\approx x$ (valid for large $x$ hence for small $\No$)  when
%\begin{align}
%|y_n|>\frac{1}{2}(|a|+|\hat{a}_n|).
%\end{align}


%%%%%%%%%%%%%%%
\section{Intra-MP projection}\label{Sec:Intra-MP}

Since the projection (mixture reduction) in at heart of the parametric \gls{mp} and it critically affects the accuracy of the estimation we obtain, it may be beneficial to perform the projection only when it does not allow for the \gls{mp} algorithm to proceed in the parametric fashion we defined. 

In particular, we may accept the auxiliary variables to deviate from the Tikhonov distribution as long as the ultimate results are projected again on the Tikhnov family.  This is the spirit of the intra-\gls{mp} approach: we will perform the projection \emph{after} the operations in \eqref{alpha}-\eqref{beta} are executed 
\begin{align}\label{alpha.projection}
\alpha_n(\theta)&\propto 
%\mcP\left[ \sum_{a\in\mcA}  \Big( \alpha_{n-1} (\theta) \hat{f}_{n-1}(\theta,a ) \Big)\convop 
%\hat{\omega}(\theta)\right]\\
%\label{alpha.projection.2}
%\alpha_n(\theta)&= \mcP\left[\mcP\bigg[ \sum_{a\in\mcA}  \alpha_{n-1}(\theta)\hat{f}_{n-1}(\theta,a ) \bigg]\convop \hat{\omega}(\theta)\right]\\
\label{alpha.projection.3}
\mcF\big[ \check{\alpha}_{n-1}(\theta) \big]\convop 
\omega(\theta),\\
\label{beta.projection}
\beta_n(\theta)&\propto 
\mcF\big[\check{\beta}_{n+1}(\theta)  \big] \convop 
\omega(\theta),
\end{align} 
where the intermediate results are given by
\begin{align}
\nonumber
\check{\alpha}_{n-1}(\theta)&=\alpha_{n-1}(\theta)\gamma_{n-1}(\theta)\\
\label{check.alpha}
&=\sum_{a\in\mcA} P^{\tr{a}}_{n-1}(a) \alpha_{n-1}(\theta) f_{n-1}(\theta, a )\\
\nonumber
\check{\beta}_{n+1}(\theta)&=\beta_{n+1}(\theta)\gamma_{n+1}(\theta)\\
\label{check.beta}
&=\sum_{a\in\mcA} P^{\tr{a}}_{n+1}(a) \beta_{n+1}(\theta) f_{n+1}(\theta, a )
\end{align}

We need to carry now the projection twice for each time $n$; this increases the computational burden but the hope is that, introducing approximations (projection) at the later stage, we minimize the approximation error which will be propagated through the time-recursive calculations.

The projection will be done in the same manner as defined before
\begin{align}
\check{\alpha}_{n}(\theta)
&=\mcT\big(\theta; z_{\check{\alpha},n}\big),\\
&=\mcF\left[ \sum_{a\in\mcA} \eta_{\alpha,n}(a) \mcT\big(\theta; z_{\alpha,n}+z_{f,n}(a)\big)  \right],\\
\eta_{\alpha,n}(a)
&=
\e^{-\frac{|a|^2}{\No}+ \hat{I}_0\big(|z_{\alpha,n}+z_{f,n}(a)|\big)+\log P^{\tr{a}}_n(a)}\\
\check{\beta}_{n}(\theta)
&=\mcT\big(\theta; z_{\check{\beta},n}\big)\\
&=\mcF\left[ \sum_{a\in\mcA} \eta_{\beta,n}(a) \mcT\big(\theta; z_{\beta,n}+z_{f,n}(a)\big)  \right],\\
\eta_{\beta,n}(a)
&=
\e^{-\frac{|a|^2}{\No}+ \hat{I}_0\big(|z_{\beta,n}+z_{f,n}(a)|\big)+\log P^{\tr{a}}_n(a)}
\end{align}
and the \gls{mp} follows from \eqref{z.alpha} and \eqref{z.beta}
 we obtain the following parametric \gls{mp} :
\begin{align}
\label{z.alpha.check}
z_{\alpha,n}&= C(z_{\check{\alpha},n-1}, \sigma_w^2), \quad n=1, \ld,N-1\\
\label{z.beta.check}
z_{\beta,n}&= C(z_{\check{\beta},n+1} , \sigma_w^2), \quad n=N-1,\ld,1,
\end{align}
where $C(z,v)$ is defined in \eqref{C.zv}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> Includes/Tracking.v3.tex <==
%!TEX root =  ../Phase.Tracking.v3.tex
\section{Phase tracking}\label{sec:phase.track}
%%%%%
%\subsection{Message passing on the graph}\label{Sec:MP.graph}
%%%%%%%%%%%%%%
\begin{figure}[bt]
\begin{center}
\scalebox{0.8}{\input{./figures/Graph.RRHARQ.x.2D.tex}}
\end{center}
\caption{Graph defining the relationship between the variables in the phase tracking problem; the messages exchanged between the nodes are shown together with the arrows indicating the direction of the exchange.}
\label{fig:graph.tracking}
\end{figure}
%%%%%%%%%%%%%%%

Our goal now is to find 
\begin{align}\label{Px}
P_n(a)=\PR{x_{n}=a|\by}, \quad a\in\mcA.
\end{align} 
and this is done exploiting the relationships between the involved random variable. 

As in \cite{Colavolpe05,Kreimer18} we show in \figref{fig:graph.tracking} a graph which captures this relationship: the squares represent the functions taking as arguments the variables which, in turn, are represented by the directly connected circles. In particular
\begin{align}
\label{f.n.x}
f_n(\theta_n,x_n)  & \propto \exp\left(-\SNR\Big|y_n-x_n\e^{\jmath\theta_n}\Big|^2\right)
\end{align}
corresponds to the relationship defined in \eqref{y.kn} and 
\begin{align}\label{p.w}
p_w(\theta_n,\theta_{n+1}) =\omega(\theta_n-\theta_{n+1})
%& \propto \mcN(\theta_n; \theta_{n+1},\sigma_w^2)
%\exp\left(-\frac{(\theta_n-\theta_{n+1})^2}{\sigma_w^2}\right)
\end{align}
corresponds to \eqref{theta.Wiener} and thus $\omega(\theta)=\mcN(\theta;0,\sigma_w^2)$, where we use the wrapped Gaussian distribution defined as\
\begin{align}\label{Normal.pdf}
\mcN(\theta;m,v)=\frac{1}{\sqrt{2\pi v}}\sum_{k=-\infty}^{\infty}\exp\left(-\frac{(\theta-m-k2\pi)^2}{2v}\right).
\end{align}

In \figref{fig:graph.tracking} we also show a shaded rectangle labeled as ``modulation/coding graph''; it also contains a graph which describes the relationship $\bx  \rightarrow \bs \rightarrow \bc \rightarrow \bb$, and its knowledge is used for the demodulation (to implement \eqref{demodulation}) and for the decoding.

What is important to note at this point is  that the relationships induced by the modulation/coding graph are ignored during the phase tracking; essentially, this means that the symbols $x_n$ are assumed to be a priori \gls{iid}, with non-informative distribution, \ie $P^{\tr{a}}_n(a)\propto 1$. 

In a case we would like  to perform the joint decoding/demodulation/phase tracking, as done, \eg in \cite{Colavolpe05}\cite{Kreimer18}\cite{Alfredsson19}, we would have to use non-uniform distribution $P^{\tr{a}}_n(x)$ obtained from the decoding results. While this is not our concern, we preserve the notation $P^{\tr{a}}_n(\cd)$ which immediately indicate how this iterative approach may be used on top of the phase tracking algorithms we propose.

As a direct consequence of ignoring the structure imposed on $x_n$ (by the coding), the graph we deal with in \figref{fig:graph.tracking} is a tree, \ie contain no loops. Therefore, the efficient marginalization can be done exactly by the \gls{mp} algorithm as follows \cite{Colavolpe05}, \cite{Shayovitz16}, \cite{Kreimer18}
\begin{align}\label{P.n.x}
P_n(a) \propto\int_{-\pi}^{\pi}  \alpha_n(\theta)  \beta_n(\theta) f_n(\theta,a ) \dd \theta,\quad a\in\mcA,
\end{align}
where
\begin{align}\label{alpha}
\alpha_n(\theta)&\propto \left(\alpha_{n-1}(\theta)  \gamma_{n-1}(\theta)\right) \convop 
\omega(\theta)\\
%\mcN(\theta;0,\sigma_w^2),\\
\label{beta}
\beta_n(\theta)&\propto \left(\beta_{n+1}(\theta) \gamma_{n+1}(\theta) \right) \convop 
\omega(\theta)\\
%\mcN(\theta;0,\sigma_w^2),\\
\label{gamma}
\gamma_n(\theta)&\propto\sum_{a\in\mcA} P^{\tr{a}}_n(a) f_{n}(\theta,a ),%=\sum_{x\in\mcA}  f_{n}(\theta,a ),
\end{align}
are (proportional to) the marginal distributions of the phase $\theta_n$ conditioned, respectively, on $y_0,\ld,y_{n-1}$, on $y_{n+1},\ld,y_{N}$, and  on $y_n$. All the distributions of the phase are periodic and so is the convolution in \eqref{alpha} and \eqref{beta}. 
%These equations are practically the same as those appearing in the \gls{bcjr} recursion \cite{BCJR} well known in the area of decoding of convolutional codes to obtain the distribution of the bits, which has discrete argument. Here, derived from the graph representation, they are applied to calculate the continuous-argument distributions of the phase. 

%%%%%%%%%
\section{Parametric message passing strategies}\label{Sec:Parametric.MP}
The operations \eqref{P.n.x}-\eqref{gamma} which allow us to calculate $P_n(a)$ may be implemented on the discretized versions of the distributions $\alpha_n(\theta)$, $\beta_n(\theta)$, and $\gamma_n(\theta)$ defined over the samples of $\theta\in(-\pi, \pi]$. In such a \gls{dmp} the multiplications and additions are straightforward to implemented and the convolution is efficiently implemented via \gls{fft}. 

However, to ensure sufficient precision,  large number of samples may be necessary implying possibly a large complexity and storage burden.\footnote{It is hard to estimate exactly the number of sample, $N_{\theta}$, required to represent the distributions over the interval of length $2\pi$. We observe that to we should represent all the distributions involved in the \gls{mp}, and the sampling step should decrease when the precision (inverse of the variance) increases. Thus, observing that the precision of $f_n(\theta,x)$ increases with the \gls{snr}, see also \eqref{f.n.x.Tikh}-\eqref{z.fn}, and the precision of $\omega(\theta)$ decreases with $\sigma_w^2$, we may conclude that the number of samples will grow when we increase the \gls{snr} and when we decrease the phase-noise level. These operational conditions are also required to transmit reliably high-order constellations, which is where the impact of the \gls{dmp} complexity will be the most notable.} Therefore, many previous works have gone in the direction of parametric representation of the involved periodic distributions. Then, instead of tracking the samples in \gls{dmp}, we only need to track (a few) parameters which represent the distributions. We thus have to find a family of the distributions, $\mcF$, on which the operations defined in \eqref{P.n.x}-\eqref{gamma} are easily dealt with. %In particular, we have to handle multiplication of the periodic functions as well as, the convolution in \eqref{alpha} and \eqref{beta}; the integration in \eqref{P.n.x}, when done on the parametric forms of distributions, is usually straightforward. 

In other words, if $\alpha_n(\theta), \beta_n(\theta), \gamma_n(\theta), \omega(\theta)\in\mcF$  and $\mcF$ is closed under  multiplication and convolution, the parametric \gls{mp} will be immediately obtained. This condition,  however, does not materialize with the most popular circular distributions such as the wrapped Gaussian distributions or  the Tikhonov distributions \cite{Kurz16}. Namely, the space of wrapped Gaussian distributions is not closed under multiplications, while the Tikhonov space is not closed under convolution. Thus, independently of the choice we make, approximations will be necessary.

In this work we consider a family of  Tiknonov distributions which were already used, \eg in \cite{Colavolpe05}\cite{Barbieri07}\cite{Shayovitz16}, and are defined as
\begin{align}\label{Tikh.definition}
\mcT(\theta; z)= \frac{\e^{\Re[z\e^{-\jj \theta}]}}{2\pi I_0(|z|)},
\end{align}
where $I_0(\cd)$ is the zero-th order modified Bessel function and $z$ is a complex parameter whose phase is the circular mean of the underlying variable and the value of $|z|$ is, approximatively, a measure of precision.

We note that $f_n(\theta,a) \in \mcF$, that is, we can write \eqref{f.n.x} as
\begin{align}\label{f.n.x.Tikh}
f_n(\theta,a)&\propto \xi_{f,n}(a)\mcT\big(\theta; z_{f,n}(a)\big) \\
\label{z.fn}
z_{f,n}(a)&=2\frac{y_n a^{*}}{\No}\\
\label{xi.f.n}
\xi_{f,n}(a)&=\e^{ -\frac{|a|^2}{\No} }I_0\big(|z_{f,n}(a)\big)=\e^{-\frac{|a|^2}{\No} +\hat{I}_0(|z_{f,n}(a)|)}
%\eta_{f,n}(a)&=-\frac{|a|^2}{\No} + |z_{f,n}(a)| + \hat{I}_0\big(|z_{f,n}(a)|\big),
\end{align}
where, to avoid numerical issues due to the exponential grows of $I_0(\cd)$, we use its log-version
\begin{align}
\hat{I}_0(x) &= \log I_0(x) = x  + \Delta(x),
\end{align}
with $\Delta(x)$ being the log-domain corrective factor. The approximation $\Delta(x)\approx -\frac{1}{2}\log(2\pi x)$ already shown in \cite[Eq.~(96)]{Shayovitz16}\cite[Eq.~(18)]{Pecorino15} is tight for large $x$ but does not apply for small arguments because $\Delta( 0 )=0$. Thus, for a better accuracy, $\Delta(x)$ may be implemented via lookup table. 


Instead of Tikhnov functions we might opt for the wrapped Gaussian family \eqref{Normal.pdf} but, to  take care of their periodic nature, particular attention is required when dealing with multiplication  \cite[Sec.~II.B]{Kurz16}.\footnote{This aspect is not always emphasized in the literature: in some works,  \eg \cite{Kreimer18}, the Gaussian distributions are used without explicit wrapping. Ignoring the circularity, it produces an apparent closeness under multiplication but may lead to interpretation errors when ``locking'' on the wrong phase, see \cite[Fig.~1]{Kurz16}.} Moreover, comparing to the Tikhonov distributions, Gaussians are less well suited to represent the uniform or almost-uniform distributions of the phase; a case which occurs, \eg when using high order \gls{qam} constellations for which $|a|$ may be small in \eqref{z.fn} yielding small $|z_{f,n}(a)|$.

From \eqref{Tikh.definition} we obtain
\begin{align}\label{Tikh.multiplication}
\mcT(\theta; z_1)\mcT(\theta; z_2)
&=\frac{I_0(|z_1+z_2|)}{2\pi I_0(|z_1|)I_0(|z_2|)}
\mcT(\theta; z_1+z_2),
\end{align}
while the convolution with the Gaussian, appearing in \eqref{alpha} and \eqref{beta}, must be treated via  approximations. It is done using moment-matching explained in \appref{conv.T.G} and which we summarize as follows:
\begin{align}\label{Tik.h.Normal.convolution}
\mcT(\theta; z)&\convop\mcN(\theta; 0,v)
\approx  \mcT\big( \theta; C(z,v) \big)\\
\label{C.zv}
C(z,v)&=
\frac{z}{1+v(|z|-0.5)}\IND{|z|>1}+
z(1-\frac{v}{2})\IND{|z| \leq 1}.
\end{align}

The main need for approximations, however,  stems from  the presence of $\gamma_n(\theta)$ which, being a mixture of distributions from $\mcF$,  see \eqref{gamma}, does not belong itself to $\mcF$.  There are essentially two approaches which have been used in the literature to deal with this issue; we compare them in the following. 

%%%%%%%
\subsection{Pre-MP approximation}\label{pre.MP}
In this approach, taking advantage of the fact that $\gamma_n(\theta)$ is not obtained recursively, its approximation, $\hat{\gamma}_n(\theta)$ is obtained \emph{before} the steps of \gls{mp} \eqref{alpha}-\eqref{beta} are executed, that is
\begin{align}\label{gamma.projection.first}
\hat{\gamma}_n(\theta)
&=\mcT\Big(\theta;  z_{\gamma,n} \Big)\\
\label{gamma.projection.first.cases}
&=
\begin{cases}
\mcT\big(\theta; z_{f,n}(x_{n})\big) &\text{if}\quad n= l L\\
\mcF\Big[ \sum_{a\in\mcA}\eta_{f,n}(a)\mcT\big(\theta;z_{f,n}(a )\big) \Big]&\text{if}\quad n\neq l L
\end{cases}\\
\label{eta.f.n}
\eta_{f,n}(a)&=\exp\left(-\frac{|a|^2}{\No}+ \hat{I}_0\big(|z_{f,n}(a)|\big)+\log P^{\tr{a}}_n(a)\right)
\end{align}
where,  at the pilot positions  $n=lL$, we use directly the parameter of the Tikhonov distribution $f_{n}(\theta, x_{n} )$. Otherwise, we project $\gamma_n(\theta)$ onto $\mcF$ via circular moment matching, as denoted by $\mcF[\cd]$. \appref{Sec:CMM} explains how $z_{\gamma,n}$ is obtained from the series $\bset{z_{f,n}(a)}_{a\in\mcA}$ and $\bset{P^{\tr{a}}_n(a)}_{a\in\mcA}$;  we use there the same approach as in \cite[Appendix~A]{Shayovitz16} removing oversimplifications, whose impact will be shown later in \secref{}.

A similar projection approach as in \eqref{gamma.projection.first} was used previously in \cite[Sec.~IV.B]{Colavolpe05}\cite{Barbieri07}\cite{Alfredsson19} but instead of circular moment matching, a  Gaussian was first matched to $\pdf(y_n|\theta_n,a)\propto f_n(\theta,a)$ from which a Tiknonov distribution was derived as
\begin{align}
\label{hat.z.gamma}
\hat{z}_{\gamma,n}&=2\frac{y_n\mfm_n^{*}}{\No+ \mfv_n},\\
\label{m.n.A}
\mfm_n&=\sum_{a\in\mcA}  a P^{\tr{a}}_n(a) ,\quad%\label{v.n.A}
\mfv_n=\sum_{a\in\mcA}  |a|^2 P^{\tr{a}}_n(a)   -  |\mfm_n|^2,
\end{align}
where  $\mfm_n$ and $\mfv_n$ are the mean and the variance of the symbol at time $n$. 

Next, if all the distributions are from the Tikhonov family, \ie $\alpha_n(\theta)=\mcT(\theta;z_{\alpha,n})$ and $\beta_n(\theta)=\mcT(\theta;z_{\beta,n})$, using $\hat{\gamma}_{n}(\theta)$ instead of $\gamma_n(\theta)$ in \eqref{Tikh.multiplication} and \eqref{Tik.h.Normal.convolution}, we obtain the following parametric \gls{mp} :
\begin{align}
\label{z.alpha.init}
z_{\alpha,0}&=0\\
\label{z.alpha}
z_{\alpha,n}&= C(z_{\alpha,n-1} + z_{\gamma,n-1}, \sigma_w^2), \quad n=1, \ld,N-1\\
\label{z.beta.init}
z_{\beta,N}&=0\\
\label{z.beta}
z_{\beta,n}&= C(z_{\beta,n+1} + z_{\gamma,n+1}, \sigma_w^2), \quad n=N-1,\ld,1,
\end{align}
where $C(z,v)$ is defined in \eqref{C.zv}. 

The \gls{mp} in \eqref{z.alpha.init}-\eqref{z.beta} is exactly equivalent to the \gls{mp} defined in \cite[Eq.~(36)-(37)]{Colavolpe05} if we assume $|z|>1$ and  is provided as a starting point for the discussion.

Using \eqref{Tikh.multiplication}  and \eqref{f.n.x.Tikh}--\eqref{xi.f.n} in \eqref{P.n.x}, the ``extrinsic'' symbol probabilities are calculated as \cite[Eq.~(35)]{Colavolpe05}
\begin{align}\label{P.a.final}
P_n( a )&\propto \int_{0}^{2\pi} \mcT(\theta;z_{\Sigma,n}(a))\frac{\xi_{f,n}(a) I_0\big(|z_{\Sigma,n}(a) |\big)}{I_0\big(|z_{f,n}(a)|\big)}\dd \theta\\
\label{P.a.final.2}
&=\exp\left(-\frac{|a|^2}{\No} + \hat{I}_0\big(|z_{\Sigma,n}(a)|\big)\right)\\
\label{z.Sigma.n}
z_{\Sigma,n}(a)&=z_{\alpha,n}+z_{\beta,n}+2\frac{y_n a^{*}}{\No}.
\end{align}

The simplicity of the \gls{mp} defined by \eqref{z.alpha.init}-\eqref{z.beta} is very appealing but the problem stems from the observation made, \eg in \cite[Sec.~I]{Shayovitz16} or \cite[Sec.~IV]{Pecorino15}: using non-informative prior $P^{\tr{a}}(a)\propto 1$,  the projection results of \eqref{gamma.projection.first} are non-informative for payload symbols; that is, $z_{\gamma,n}=0, n\neq lL$.\footnote{If circular moment-matching approach is used, this is true for constellations $\mcA$ which may be decomposed into constant modulus zero-mean sub-constellations. On the other hand, using the Gaussian approximation \eqref{hat.z.gamma}-\eqref{m.n.A}, it is enough for $\mcA$ is zero-mean, which is immediate from \eqref{m.n.A}.}

In fact, with $z_{\gamma,n}=0$, the \gls{mp} in \eqref{z.alpha.init}-\eqref{z.beta}, maybe seen as a pilot-only based recursive estimation of the phase which serves later as the reference for detection in \eqref{P.a.final}.

Since $\hat{\gamma}_n(\theta)\propto 1$ is non-informative, it does not help in the phase estimation. This is also why, the previous works based on this approach combined it with the feedback from the decoder, \eg \cite{Colavolpe05}\cite{Barbieri07}\cite{Alfredsson19}. Such a feedback, \ie non-uniform $P^{\tr{a}}(a)$, provides prior on the constellation that  transforms $\hat{\gamma}_n(\theta)$ into a non-uniform (thus, informative) distribution.

The feedback from the decoder may be  definitely useful but, as already said, we cannot always rely on it so our objective is to obtain the most efficient ``stand-alone'' phase-tracking algorithm. 

%%%%%%%%%%%%%%%
\subsection{Intra-MP projection}\label{Sec:Intra-MP}

%Since the projection (mixture reduction) which in at heart of the parametric \gls{mp} and it critically affects the accuracy of the estimation we obtain, it may be beneficial to perform the projection only when it does not allow for the \gls{mp} algorithm to proceed in the parametric fashion we defined. 

The disadvantage of the pre-\gls{mp} projection from \secref{pre.MP} is that the structure of the constellation $\mcA$, reflected in $\gamma_n(\theta)$ is not taken into consideration. Thus, in order to exploit the form of the constellation, \cite{Shayovitz16} proposed to perform the projection on $\mcF$ \emph{after} the multiplications in \eqref{alpha}-\eqref{beta} are executed, that is
\begin{align}\label{alpha.projection}
\alpha_n(\theta)&\propto 
\label{alpha.projection.3}
 \mcF\big[\alpha_{n-1}(\theta)\gamma_{n-1}(\theta)\big]\convop \omega(\theta)\\
&\propto \check{\alpha}_{n-1}(\theta) \convop \omega(\theta),\\
\label{beta.projection}
\beta_n(\theta)&\propto 
\mcF\big[\beta_{n+1}(\theta)\gamma_{n+1}(\theta)\big]  \convop  \omega(\theta)\\
&\propto\check{\beta}_{n+1}(\theta)\convop  \omega(\theta),
\end{align} 
where the ``auxiliary'' distributions 
\begin{align}
\nonumber
\check{\alpha}_{n-1}(\theta)&=\mcF\big[\alpha_{n-1}(\theta)\gamma_{n-1}(\theta)\big]\\
\label{check.alpha}
&=\sum_{a\in\mcA} P^{\tr{a}}_{n-1}(a) \alpha_{n-1}(\theta) f_{n-1}(\theta, a )\\
\nonumber
\check{\beta}_{n+1}(\theta)&=\mcF\big[\beta_{n+1}(\theta)\gamma_{n+1}(\theta)\big]\\
\label{check.beta}
&=\sum_{a\in\mcA} P^{\tr{a}}_{n+1}(a) \beta_{n+1}(\theta) f_{n+1}(\theta, a )
\end{align}

We need to carry now the projection twice for each time $n$ which increases the computational burden. The hope is that, introducing approximations (projection) we minimize the approximation error which will be propagated through the time-recursive calculations.

The projection will be done in the same manner as defined before
\begin{align}
\check{\alpha}_{n}(\theta)
&=\mcT\big(\theta; z_{\check{\alpha},n}\big),\\
&=\mcF\left[ \sum_{a\in\mcA} \eta_{\alpha,n}(a) \mcT\big(\theta; z_{\alpha,n}+z_{f,n}(a)\big)  \right],\\
\eta_{\alpha,n}(a)
&=
\e^{-\frac{|a|^2}{\No}+ \hat{I}_0\big(|z_{\alpha,n}+z_{f,n}(a)|\big)+\log P^{\tr{a}}_n(a)}\\
\check{\beta}_{n}(\theta)
&=\mcT\big(\theta; z_{\check{\beta},n}\big)\\
&=\mcF\left[ \sum_{a\in\mcA} \eta_{\beta,n}(a) \mcT\big(\theta; z_{\beta,n}+z_{f,n}(a)\big)  \right],\\
\eta_{\beta,n}(a)
&=
\e^{-\frac{|a|^2}{\No}+ \hat{I}_0\big(|z_{\beta,n}+z_{f,n}(a)|\big)+\log P^{\tr{a}}_n(a)}
\end{align}
and the \gls{mp} follows from \eqref{z.alpha} and \eqref{z.beta}
 we obtain the following parametric \gls{mp} :
\begin{align}
\label{z.alpha.check}
z_{\alpha,n}&= C(z_{\check{\alpha},n-1}, \sigma_w^2), \quad n=1, \ld,N-1\\
\label{z.beta.check}
z_{\beta,n}&= C(z_{\check{\beta},n+1} , \sigma_w^2), \quad n=N-1,\ld,1,
\end{align}
where $C(z,v)$ is defined in \eqref{C.zv}. 

\begin{example}[Pre-MP vs Intra-MP]
To compare the Pre-MP and Intra-MP projections, we consider transmission of $16$-\gls{qam} constellation with Gray mapping \cite[Sec.~2.5.2]{Szczecinski_Alvarado_book}; the proprietary \gls{ldpc} encoder with rate $R=\frac{3}{4}$ is applied to the block of $\Nb=4032$ bits; the \gls{ldpc} decoder executes 10 iterations. The \gls{dmp} is implemented using 64 samples. The noise level is set at $\sigma_w^2=0.01$ and we use the pilot spacing of $L\in\set{17,25}$ (these values allow us to place $L-1$ payload symbols between pilots, see \eqref{payload.1}, so that dummy symbols are not needed). 

The \gls{per} estimated after transmitting $10^4$ blocks is shown in \figref{fig:PER.preMP}. The performance loss is measured, as the \gls{snr} gap to the \gls{dmp} curve  at the target $\PER_\tr{t}$, typically $\PER_\tr{t}=10^{-2}$ or $\PER_\tr{t}=10^{-3}$. 

The results in \figref{fig:PER.preMP} illustrate what has been, to a large extend stated in the literature.\foontnote{However, it is not so easy to find such results compared side-by-side in the same transmission setup, so we provided them as a reference.} In particular, it is obvious that the performance loss of the approximate methods (Pre- and Intra-\gls{mp} projections) grows with the pilot spacing, $L$. On the other hand, it is less obvious that for the large \gls{snr} and $L$ (\ie in phase-noise dominated scenarios), the simple Pre-\gls{mp} approach may outperform the more complex Intra-\gls{mp}.

The degradation of the Intra-\gls{mp} should be attributed to the ``phase slip": following the locally most likely phase and excluding the less-likely but true phase shift leads to unrecoverable errors. As this is caused by assumed unimodal (Tikhnonov) distribution of the phase, as a remedy \cite{Shayovitz16} proposes to enrich the space $\mcF$ by  including the mixtures of the distributions. In this way the phase less likely but close to true elements of the distribution are preserved at the cost of greater phase tracking complexity.  

\end{example}

%%%%%%%%%%%%%%
\begin{figure}[bt]
\begin{center}
\psfrag{DMPXXX}[lc][lc][\siz]{DMP}
\psfrag{CBC}[lc][lc][\siz]{Pre-MP}
\psfrag{MP}[lc][lc][\siz]{Intra-MP}
\psfrag{xlabel}[lc][lc][\siz]{$\SNR$}
\scalebox{\sizf}{\includegraphics[width=\linewidth]{./figures/PER_Tikh.eps}}
\end{center}
\caption{\gls{per} vs. \gls{snr} for the ``exact'' \gls{mp} (\gls{dmp}), and approximate \gls{mp}s based on the Pre- and Intra-\gls{mp} projections, for pilot spacing $L=17$ (solid) and $L=25$ (dashed).}\label{fig:PER.preMP}
\end{figure}
%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%
\section{Iterative refinement}\label{Sec:It.EP}


\subsection{Pre-MP with}
To exploit the constraints imposed by the discrete constellation and to take advantage of the extreme simplicity of \eqref{z.alpha.init}-\eqref{z.beta} we need to implement the projection taking advantage of the phase tracking results in an iterative manner; hence we will use the parenthesized superscript $^{(i)}$ to denote the variables/functions obtained in the $i$-th iteration, where $i=1,\ld, I$ and $I$ is the maximum iteration number;  superscripting the distributions with $^{(0)}$ means that they are non-informative.

%Literature proposes different approaches to define the iterations and the one suggested in \cite[Sec.~III.C]{Alfredsson19} postulates, for each iteration $i=1,\ld, I$, to replace the prior $P^{\tr{a}}_n(a)$  with the extrinsic probability from the previous iteration $P^{(i-1)}_n(a)$. For example, this can be done by recalculating the projection \eqref{gamma.projection.first.cases} in the $i$-th iteration using weighting coefficients
%\begin{align}
%\eta^{(i)}_{f,n}(a)&=\exp\left(-\frac{|a|^2}{\No}+ \hat{I}_0\big(|z_{f,n}(a)|\big)+\log P^{(i-1)}_n(a)\right);
%\end{align}
%similarly we may replace $P^{\tr{a}}_n(a)$ with $P^{(i-1)}_n(a)$ in \eqref{hat.z.gamma}-\eqref{v.n.A}. 
%
%And while  reusing the outgoing message from the node goes against the \gls{mp} principle, we have to remember that the projection on $\mcF$, which yields $\hat{\gamma}_n(\theta)$, is very crude. Thus, even violating the fundamental principles of  the \gls{mp} may yield improvements.

We will follow the approach postulated by the \gls{ep} \cite[Ch.~3.2]{Minka01}, which tries to ``match'' the distributions before and after the projection taking into account the results from the previous iteration. In our case this would mean matching the posterior distributions of $\theta$, calculated from the projection $\hat{\gamma}^{(i)}_n(\theta)$ and from the original distribution $\gamma_n(\theta)$
\begin{align}
\nonumber
\hat{\gamma}^{(i)}_n(\theta)\Big[\alpha^{(i-1)}_n(\theta)&\beta^{(i-1)}_n(\theta)\Big]\\
\label{equal.proba.approx}
&\approx
\gamma_n(\theta)\Big[\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)\Big].
\end{align}
Of course, for $i=1$, using  non-informative distributions $\alpha^{(0)}(\theta)\propto 1$ and $\beta^{(0)}(\theta)\propto 1$, reduces \eqref{equal.proba.approx} to  $\hat{\gamma}^{(1)}_n(\theta)\approx \gamma_n(\theta)$; this is what was done in \secref{pre.MP} where the approximation is meant to be carried by projection the \gls{rhs} on the space $\mcF$.

We can calculate the \gls{rhs} of \eqref{equal.proba.approx} as
\begin{align}
\nonumber
\gamma_n(\theta)\Big[\alpha^{(i-1)}_n(\theta)&\beta^{(i-1)}_n(\theta)\Big]\\
\label{apost.theta.i1}
&=
\sum_{a\in\mcA} \eta^{(i-1)}_{\Sigma,n} (a) \mcT\big(\theta; z^{(i-1)}_{\Sigma,n}(a) \big),
\end{align}
where
\begin{align}
\label{eta.Sigma.n.i1}
\eta^{(i-1)}_{\Sigma,n}(a)&=\e^{-\frac{|a|^2}{\No}+ \hat{I}_0\big(|z^{(i-1)}_{\Sigma,n}(a)|\big)+\log P^{\tr{a}}_n(a)}\\
&=P^{(i-1)}_n(a)P^{\tr{a}}(a)
\end{align}
represents the posterior probability of the symbols obtained in the iteration $i-1$, and $z^{(i-1)}_{\Sigma,n}(a)$ is the same as \eqref{z.Sigma.n} calculated in the iteration \mbox{$i-1$}. 

The remaining question is how to obtain $\hat{\gamma}_n^{(i)}(\theta)$ from \eqref{apost.theta.i1} and \eqref{equal.proba.approx} which we address in the following.

%%%%%%%%%%%%%%%
\subsection{Pitfalls of Expectation Propagation}
Since we have started iterative improvements considerations in the spirit of the \gls{ep}, it is natural to apply it to the problem at hand. This means concretely that i)~the projection  operation, $\mcF[\cd]$, is applied to the \gls{lhs} and \gls{rhs}  sides of \eqref{equal.proba.approx} and ii)~the approximation sign is replaced with equality (or rather, proportionality $\propto$), yielding
\begin{align}\label{EP.iterations}
\hat{\gamma}^{(i)}_n(\theta) 
&=\mcT(\theta; z^{(i)}_{\gamma,n})\\
\label{EP.division}
&\propto \frac
{\mcF\Big[\sum_{a\in\mcA} \eta^{(i-1)}_{\Sigma,n} (a) \mcT\big(\theta; z^{(i-1)}_{\Sigma,n}(a) \big)\Big] }
{\mcT\big(\theta; z^{(i-1)}_{\alpha,n}+z^{(i-1)}_{\beta,n} \big)}\\
\label{EP.division.2}
&\propto \frac{ \mcT\Big(\theta; z^{(i-1)}_{\tr{post},n}\Big)  }{ \mcT\Big(\theta; z^{(i-1)}_{\alpha,n}+z^{(i-1)}_{\beta,n} \Big)}\\
\label{z.gamma.i}
z^{(i)}_{\gamma,n}&= z^{(i-1)}_{\tr{post},n}  - z^{(i-1)}_{\alpha,n} - z^{(i-1)}_{\beta,n}.
\end{align}

The elegant formulation of  the \gls{ep} is indeed appealing but suffers from a problem due to the division of the distributions in \eqref{EP.division.2}, or equivalently, due to subtraction of the coefficients in \eqref{z.gamma.i}. This problem has been already recognized in the literature, particularly in the context of the Gaussian \gls{ep}, where the division of the distributions may yield a ``Gaussian'' with negative variance, \eg \cite[Sec.~IV.B]{Senst11} \cite[Sec.~IV.A]{Cespedes14}; such distributions are uninterpretable in our application. 

In the context of the Tikhnov distribution we are using, there is no problem of the parameters which would yield uninterpretable distributions, nevertheless, the problem remains. To understand intuitively its source we may assume that i)~$\angle z^{(i-1)}_{\tr{post},n} =\angle (z^{(i-1)}_{\alpha,n}+z^{(i-1)}_{\beta,n})$, and ii)~$|z^{(i-1)}_{\tr{post},n}|<|z^{(i-1)}_{\alpha,n}+z^{(i-1)}_{\beta,n}|$. This means that i)~the circular means of the approximate posterior distribution, $\mcT\big(\theta; z^{(i-1)}_{\tr{post},n}\big) $ and of the ``extrinsic'' distribution (defined by  the product $\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)$) coincide (remember, the phase $\angle z^{(i-1)}_{\tr{post},n}$ defines the circular mean), and ii)~the posterior distribution is ``larger" than the extrinsic distribution.\footnote{This may occur because the projection takes into account the symbols which widen the distribution.} 

Then, carrying out the subtraction in \eqref{z.gamma.i} we will obtain
\begin{align}
z^{(i)}_{\gamma,n}
&= (|z^{(i-1)}_{\tr{post},n}|  - |z^{(i-1)}_{\alpha,n} + z^{(i-1)}_{\beta,n}|\big)\e^{\jj \angle z^{(i-1)}_{\tr{post},n}}\\
&=|z^{(i-1)}_{\tr{post},n}|\e^{\jj(\angle z^{(i-1)}_{\tr{post},n}+\pi)}.
\end{align}
That is, the circular mean of the new distribution $\mcT(\theta; z^{(i)}_{\gamma,n})$ will be  in disagreement (by the largest possible value of $\pi$) with the mean of the posterior and extrinsic distributions obtained from the previous iteration. This is clearly wrong.

To deal with this \gls{ep}-typical problem,  heuristics were devised for the Gaussian \gls{ep} where the problem is clearly identified, \ie the variance becomes negative. For example, \cite[Sec.~IV.B]{Senst11} proposed to eliminate the division, which here would mean $z^{(i)}_{\gamma,n}=z^{(i-1)}_{\tr{post},n}$ , while \cite[Sec.~IV.A]{Cespedes14} removed the update, \ie $z^{(i)}_{\gamma,n}=z^{(i-1)}_{\gamma,n}$ .  

However, to apply such heuristics in our case we would have to i)~devise a strategy to identify the problem for the Tikhnov distribution in the case which is more general than the equal-phase example we gave above, and ii)~rely on many iterations to overcome the disruptions in the convergence introduced by these heuristics. 

Moreover, it simply seems that the generic \gls{ep} may not be the best solution for the case we deal with. Hence we propose to go back to the very principle of distribution matching defined in \eqref{equal.proba.approx} taking into account the structure of $\gamma_n(\theta)$.

%%%%%
\subsection{Mixture-oriented projection}\label{Sec:Constr.Proj.}

The principal observation is that, although  $\gamma_n(\theta)$ defined in \eqref{gamma} is a mixture of the Tikhonov distributions $\mcT\big(\theta; z_{f,n}(a)\big)$ with weighting factors $\xi_{f,n}(a)$ (see \eqref{z.fn}-\eqref{xi.f.n}), after the multiplication with the extrinsic distribution in \eqref{apost.theta.i1} (defined by the product $\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)$), only some of the mixture terms are relevant in the posteriori distribution, \ie those with ``sufficiently'' large values of $\eta^{(i-1)}_{\Sigma,n}(a)$. Removing these irrelevant terms will not change (significantly) nor the posterior distribution itself, nor its projection on the Tikhnov space $\mcT\big(\theta; z^{(i-1)}_{\tr{post},n}\big)$.

The idea is thus, to remove the irrelevant terms from the mixture $\gamma_n(\theta)$ \emph{before} the projection on the space $\mcF$, using, as a criterion, the weighting coefficients of the posterior  distribution. The resulting procedure will i) keep the spirit of \eqref{equal.proba.approx}, ii) be simple to implement, and iii) avoid the division of distribution which is at the root of the problem in the \gls{ep}. 

In fact, with the proposed approach, we focus on the fact that the distribution $\gamma_{n}(\theta)$ is a mixture of distributions with well-defined meaning: each term is related to the particular symbol in the constellation. By allowing to change the weights of the mixture terms (here, removing the term may be seen as zeroing of its weight, but more sophisticated versions might be devised) we keep the parameters of the distributions in the mixture (the terms $z_{f,n}(a)$) unaltered. This is why we dub this approach ``mixture-oriented" (MO) projection which  stands in contrast with the \gls{ep} which ignores the structure of $\gamma_n(\theta)$; in particular, the fact that $\gamma_n(\theta)$ is a mixture.

We can reformulate the above idea replacing $\mcA$ with the ``trimmed'' constellation $\mcA^{(i)}_n\subset \mcA$,  trimming/removing these symbols $a$ whose contribution to the posterior distribution \eqref{apost.theta.i1} is negligible as judged by the posterior symbol probability $\eta^{(i-1)}_{\Sigma,n}(a)$. 

For example, the weights are first ordered, $\eta^{(i-1)}_{\Sigma,n}(a_0)>\eta^{(i-1)}_{\Sigma,n}(a_1)>\ld>\eta^{(i-1)}_{\Sigma,n}(a_{M-1})$, and then normalized, $\sum_{m=0}^{M-1} \eta^{(i-1)}_{\Sigma,n}(a_m)=1$.\footnote{The ordering and normalization must be carried our for each time $n$ and each iteration $i>1$.} Next, we the trimmed constellation is defined as $\mcA^{(i)}_n=\set{a_0,\ld,a_{M'-1}}$ where 
\begin{align}
M'= \argmin_{k}\set{ k : \sum_{m=0}^{k-1} \eta^{(i-1)}_{\Sigma,n}(a_m) \ge 1-\epsilon}
\end{align}
where $\epsilon$ is arbitrarily set, \eg $\epsilon=0.05$.

Since in practice, the cardinality of  $\mcA^{(i)}_n$ is quite small, and to avoid cumbersome trimming of the constellation,  we might opt for the extreme simplification of taking only one symbol with a maximum posterior, that is $\mcA^{(i)}_n=\set{a_0$}; since normalization is not necessary, we may operate directly in the logarithmic scale so, from \eqref{eta.Sigma.n.i1}, we have
\begin{align}\label{a.0}
a_{0,n}^{(i)} = \argmax_{a \in\mcA} \SET{  -\frac{|a|^2}{\No}  + \hat{I}_0(|z^{(i-1)}_{\Sigma,n}(a)|) +P^{\tr{a}}(a) }
\end{align}
and, the projection being not necessary, we have
\begin{align}\label{z.gamma.a.0}
 z_{\gamma,n}^{(i)}&=z_{f,n}\big(a_{0,n}^{(i)}\big).
\end{align}

Of course, such crude approximation affects accuracy. On the other hand, dealing with one symbol, we get rid of all the operations such as moving from the logarithmic to the linear scale, the normalization of the weighting coefficients, or the projection. From the implementation perspective, this huge advantage may outweigh some performance loss. 

In order to deal with imperfections related to these (or other) approximations, the parameters $z_{\gamma,n}^{(i)}$ obtained in the $i$-the projection may be smoothed
\begin{align}\label{z.smoothing}
\tilde{z}_{\gamma,n}^{(i)} = \zeta z_{\gamma,n}^{(i)} +(1-\zeta) \tilde{z}_{\gamma,n}^{(i-1)},
\end{align}
where $\zeta<1$ must be chosen to strike a balance between the new update and the history accumulated in the previous estimate ; this is a usual heuristics in the \gls{ep}, \eg \cite[Sec.~IV.A]{Cespedes14} and, here, \ls{we choose $\zeta=0.2$.} 



%We will thus keep the symbols $a$ in the trimmed constellation $\mcA^{(i)}_n$ when
%\begin{align}
%-\frac{|a|^2}{\No} +\hat{I}_0\big(|z_{\Sigma,n}^{(i-1)}(a)|\big) > -\frac{|\hat{a}_n|^2}{\No} +\hat{I}_0\big(|z_{f,n}(\hat{a}_n)|\big).
%\end{align}
%or, using $\hat{I}_0(x)\approx x$ (valid for large $x$ hence for small $\No$)  when
%\begin{align}
%|y_n|>\frac{1}{2}(|a|+|\hat{a}_n|).
%\end{align}







==> Includes/Tracking.v4.tex <==
%!TEX root =  ../Phase.Tracking.v4.tex
\section{Phase tracking}\label{sec:phase.track}
%%%%%
%\subsection{Message passing on the graph}\label{Sec:MP.graph}
%%%%%%%%%%%%%%
\begin{figure}[bt]
\begin{center}
\scalebox{0.8}{\input{./figures/Graph.RRHARQ.x.2D.tex}}
\end{center}
\caption{Graph defining the relationship between the variables in the phase tracking problem; the messages exchanged between the nodes are shown together with the arrows indicating the direction of the exchange.}
\label{fig:graph.tracking}
\end{figure}
%%%%%%%%%%%%%%%

Our goal now is to find $P_n(a)$ exploiting the relationships between the involved random variable.  

As in \cite{Colavolpe05,Kreimer18}, we show in \figref{fig:graph.tracking} a graph which captures this relationship: the squares represent the functions taking as arguments the variables which, in turn, are represented by the directly connected circles. In particular
\begin{align}
\label{f.n.x}
g_n(\theta_n,x_n)  & \propto \exp\left(-\SNR\Big|y_n-x_n\e^{\jmath\theta_n}\Big|^2\right)
\end{align}
corresponds to the relationship defined in \eqref{y.kn} and 
\begin{align}\label{p.w}
p_w(\theta_n,\theta_{n+1}) =\omega(\theta_n-\theta_{n+1})
%& \propto \mcN(\theta_n; \theta_{n+1},\sigma_w^2)
%\exp\left(-\frac{(\theta_n-\theta_{n+1})^2}{\sigma_w^2}\right)
\end{align}
corresponds to \eqref{theta.Wiener} and thus $\omega(\theta)=\mcN(\theta;0,\sigma_w^2)$, where the wrapped Gaussian distribution is defined as
\begin{align}\label{Normal.pdf}
\mcN(\theta;m,v)=\frac{1}{\sqrt{2\pi v}}\sum_{k=-\infty}^{\infty}\exp\left(-\frac{(\theta-m-k2\pi)^2}{2v}\right).
\end{align}

In \figref{fig:graph.tracking} we also show a shaded rectangle labeled as ``modulation/coding graph''; it also contains a graph which describes the relationship $\bx  \rightarrow \bs \rightarrow \bc \rightarrow \bb$, and its knowledge is used for the demodulation (to implement \eqref{lambda.n.l}) and for the decoding.

If the phase tracking has to be carried out and no decoding was not yet executed,  the payload symbols $x_n$ are assumed to be \gls{iid}, with non-informative distribution, \ie $P^{\tr{a}}_n(a)\propto 1$. In a case we would like  to perform the joint decoding/demodulation/phase tracking, as done, \eg in \cite{Colavolpe05}\cite{Kreimer18}\cite{Alfredsson19}, we use $P^{\tr{a}}_n(x)$ obtained from the decoding results. 

Thus, from the point of view of the phase tracking, the relationships induced by the modulation/coding graph are summarized by $P^{\tr{a}}_n(a)$. As a direct consequence, the graph we deal with in \figref{fig:graph.tracking} is a tree, \ie contain no loops. Therefore, the efficient marginalization can be done exactly by the \gls{mp} algorithm as follows \cite{Colavolpe05}, \cite{Shayovitz16}, \cite{Kreimer18}
\begin{align}\label{P.n.x}
P_n(a) \propto\int_{-\pi}^{\pi}  \alpha_n(\theta)  \beta_n(\theta) g_n(\theta,a ) \dd \theta,\quad a\in\mcA,
\end{align}
where
\begin{align}\label{alpha}
\alpha_n(\theta)&\propto \big(\alpha_{n-1}(\theta)  \gamma_{n-1}(\theta)\big) \convop 
\omega(\theta)\\
%\mcN(\theta;0,\sigma_w^2),\\
\label{beta}
\beta_n(\theta)&\propto \big(\beta_{n+1}(\theta) \gamma_{n+1}(\theta) \big) \convop 
\omega(\theta)\\
%\mcN(\theta;0,\sigma_w^2),\\
\label{gamma}
\gamma_n(\theta)&\propto\sum_{a\in\mcA} P^{\tr{a}}_n(a) g_{n}(\theta,a ),%=\sum_{x\in\mcA}  g_{n}(\theta,a ),
\end{align}
are (proportional to) the marginal distributions of the phase $\theta_n$ conditioned, respectively, on $y_0,\ld,y_{n-1}$, on $y_{n+1},\ld,y_{N}$, and  on $y_n$.\footnote{That is,
\begin{align}
\alpha_n(\theta)&\propto\pdf(\theta_n| y_0,\ld,y_{n-1})\\
\beta_n(\theta)&\propto\pdf(\theta_n| y_{n+1},\ld,y_{N})\\
g_n(\theta,a)&\propto\pdf(\theta_n| y_{n},a)
\end{align}
and thus the integrand in \eqref{P.n.x} is the posterior distribution of the phase
\begin{align}
\pdf(\theta_n | \by, a)&\propto
 \alpha_n(\theta)  \beta_n(\theta) g_n(\theta,a ) 
\end{align}
} All the distributions of the phase are periodic and so is the convolution in \eqref{alpha} and \eqref{beta}. 
%These equations are practically the same as those appearing in the \gls{bcjr} recursion \cite{BCJR} well known in the area of decoding of convolutional codes to obtain the distribution of the bits, which has discrete argument. Here, derived from the graph representation, they are applied to calculate the continuous-argument distributions of the phase. 

%%%%%%%%%
\section{Parametric message passing}\label{Sec:Parametric.MP}
The operations \eqref{P.n.x}-\eqref{gamma} which allow us to calculate $P_n(a)$ may be implemented on the discretized versions of the distributions $\alpha_n(\theta)$, $\beta_n(\theta)$, and $\gamma_n(\theta)$ defined over the samples of $\theta\in(-\pi, \pi]$. In such a \gls{dmp} the multiplications and additions are straightforward to implemented and the convolution is efficiently implemented via \gls{fft}. 

However, to ensure sufficient precision,  large number of samples, $N_{\theta}$, may be necessary implying possibly a large complexity and storage burden.\footnote{The number of samples, $N_{\theta}$, required to represent the distributions over the interval of length $2\pi$ and to ensure the accuracy of the \gls{mp}, \eqref{alpha}-\eqref{gamma}, is difficult to estimate. Nevertheless,  all the distributions involved in the \gls{mp} should be represented without significant loss of accuracy so the sampling step should decrease when the spectrum support of the distributions increases. 

Approximating the distributions by Gaussians, the precision (inverse of the variance) is proportional to the spectral support. Thus, observing that the precision of $g_n(\theta,a)$ increases with the \gls{snr}, see also \eqref{f.n.x.Tikh}-\eqref{z.fn}, and the precision of $\omega(\theta)$ decreases with $\sigma_w^2$, we may conclude that the number of samples will grow when we increase the \gls{snr} or when we decrease the phase-noise level. These operational conditions are also required to transmit reliably high-order constellations, which is where the impact of the \gls{dmp} complexity will be the most notable. In such a case, the simplification may be sought by limiting the period over which the distribution must be represented \cite{ShahMohammadian18}.} \footnote{The number of samples, $N_{\theta}$, required to represent the distributions over the interval of length $2\pi$ may be estimated from their approximate Nyquist frequency, $F_{\tr{Nyq.}}$, as $N_{\theta}>4\pi F_{\tr{Nyq.}}$. To find the latter we approximate the function $f_n(\theta,x)$ as a Gaussian with the variance $\No/(2|x|^2)$, see \cite[Eq.~(XXX)]{Shayovitz16}, so its (approximate) Nyquist frequency is $F_{f,\tr{Nyq.,}}=c|x|\sqrt{2/\No}$ (where $c$ depends on how we define the frequency support of the spectrum, \eg $c=1.5$ for 10\% spectral overlap.). Similarly, for the Gaussian distribution $\omega(\theta)$ the respective value is $F_{\omega,\tr{Nyq.}}\approx c/\sigma_w$ . Thus the rule of thumb requirement is $N_{\theta}>10\pi/\min\set{\sigma_2 , \sqrt{\No/2}  } $ so the number of samples is inversely proportional to the level of the phase noise $w_n$ or the level of the additive noise $z_n$. Since decreasing the levels of the noise is required for large constellations, this is where the \gls{dmp} will be suffer the most from the complexity issues. For example, in the examples based on $16$-\gls{qam}, we have $\SNR\approx 13$dB and $\sigma_w^2=0.01$, which requires $N_\theta>125$. Of course, this ballpark number does not take into all effects, \eg due to multiplications of the distributions.}Therefore, many previous works have gone in the direction of parametric representation of the involved periodic distributions. Then, instead of tracking the samples in \gls{dmp}, we only need to track (a few) parameters which represent the distributions. We thus have to find a family of the distributions, $\mcF$, on which the operations defined in \eqref{P.n.x}-\eqref{gamma} are easily dealt with. %In particular, we have to handle multiplication of the periodic functions as well as, the convolution in \eqref{alpha} and \eqref{beta}; the integration in \eqref{P.n.x}, when done on the parametric forms of distributions, is usually straightforward. 

In other words, if $\alpha_n(\theta), \beta_n(\theta), \gamma_n(\theta), \omega(\theta)\in\mcF$  and $\mcF$ is closed under  multiplication and convolution, the parametric \gls{mp} will be immediately obtained. This condition,  however, does not materialize with the most popular circular distributions such as the wrapped Gaussian distributions or  the Tikhonov distributions \cite{Kurz16}. Namely, the space of wrapped Gaussian distributions is not closed under multiplications, while the Tikhonov space is not closed under convolution. Thus, independently of the choice we make, approximations will be necessary.

%%%%%%%%%
\subsection{Tikhonov distributions}\label{Sec:Tikh.dist}
In this work we consider a family of  Tikhonov distributions which were already used, \eg in \cite{Colavolpe05}\cite{Barbieri07}\cite{Shayovitz16}, and are defined as
\begin{align}\label{Tikh.definition}
\mcT(\theta; z)= \frac{\e^{\Re[z\e^{-\jj \theta}]}}{2\pi I_0(|z|)},
\end{align}
where $\Re[\cd]$ denotes the real part and $I_0(\cd)$ is the zero-th order modified Bessel function; $z$ is a complex parameter whose phase is the circular mean of the underlying variable and the value of $|z|$ is, approximatively, a measure of precision \cite{Kurz16}.

The closeness of $\mcF$ under multiplication is then obvious
\begin{align}\label{Tikh.multiplication}
\mcT(\theta; z_1)\mcT(\theta; z_2)
&=\frac{I_0(|z_1+z_2|)}{2\pi I_0(|z_1|)I_0(|z_2|)}
\mcT(\theta; z_1+z_2),
\end{align}
while the convolution with the Gaussian, appearing in \eqref{alpha} and \eqref{beta}, must be treated via  approximations as done before \cite[Appendix]{Colavolpe05} and also explained using the concept of a \gls{cmm} in \appref{conv.T.G}
\begin{align}\label{Tik.h.Normal.convolution}
\mcT(\theta; z)&\convop\mcN(\theta; 0,\sigma_w^2)
\approx  \mcT\Big( \theta; \frac{z}{1+\sigma_w^2|z|} \Big).
\end{align}

We also note that $g_n(\theta,a) \in \mcF$, that is, we can write \eqref{f.n.x} as
\begin{align}\label{f.n.x.Tikh}
g_n(\theta,a)&\propto \e^{\xi_{g,n}(a)}\mcT\big(\theta; z_{g,n}(a)\big) \\
\label{z.fn}
z_{g,n}(a)&=2\frac{y_n a^{*}}{\No}\\
\label{xi.f.n}
\xi_{g,n}(a)&=%\e^{ -\frac{|a|^2}{\No} }I_0\big(|z_{g,n}(a)|\big)=
-\frac{|a|^2}{\No} +\hat{I}_0(|z_{g,n}(a)|),
%\eta_{g,n}(a)&=-\frac{|a|^2}{\No} + |z_{g,n}(a)| + \hat{I}_0\big(|z_{g,n}(a)|\big),
\end{align}
where, to avoid numerical issues due to the exponential grows of $I_0(\cd)$ we use its log-version
\begin{align}\label{hat.I0}
\hat{I}_0(x) &= \log I_0(x) = x  + \Delta(x),
\end{align}
with $\Delta(x)$ being the log-domain corrective factor.\footnote{The approximation $\Delta(x)\approx -\frac{1}{2}\log(2\pi x)$ is tight for large $x$ \cite[Eq.~(96)]{Shayovitz16}\cite[Eq.~(18)]{Pecorino15}  but does not apply for small arguments because $\Delta( 0 )=0$. Thus, for a better accuracy, $\Delta(x)$ may be implemented via lookup table. On the other hand, it is also possible to simply set $\Delta(x)\approx 0$.}

Instead of Tikhonov family we might opt for the wrapped Gaussians \eqref{Normal.pdf} but i)~to  take care of their periodic nature, particular attention is required when dealing with multiplication  \cite[Sec.~II.B]{Kurz16},\footnote{This aspect is not always emphasized in the literature: in some works,  the Gaussian distributions are used without explicit wrapping. Ignoring the circularity, it produces an apparent closeness under multiplication but may lead to interpretation errors when ``locking'' on the wrong phase, see example in \cite[Fig.~1]{Kurz16}.} ii)~comparing to the Tikhonov distributions, Gaussians are less well suited to represent the uniform or almost-uniform distributions of the phase, and iii)~we have to start approximations already when representing $g_n(\theta,a)$ which is naturally represented by a Tikhonov distribution in \eqref{f.n.x.Tikh}; this can be done, of course, \eg as in \cite{Kreimer18}, but requires introduction of additional layer of approximations before the \gls{mp} is derived.


%%%%%%%%%
\subsection{Approximation of $\gamma_n(\theta)$}\label{Sec:App.gamma.n}

The main need for approximations stems from  the presence of $\gamma_n(\theta)$ which, being a mixture of Tikhonov distributions,  see \eqref{gamma}, does not belong itself to $\mcF$. Namely,  
\begin{align}\label{gamma.def.mixture}
\gamma_n(\theta)&=\sum_{a\in\mcA}\e^{\eta_{g,n}(a)}\mcT\big(\theta;z_{g,n}(a )\big),\\
\label{eta.f.n}
\eta_{g,n}(a)&=-\frac{|a|^2}{\No}+ \hat{I}_0\big(|z_{g,n}(a)|\big)+\hat{P}^{\tr{a}}_n(a),
\end{align}
where we again use $\hat{P}^{\tr{a}}_n(a)=\log P^{\tr{a}}_n(a)$ because the logarithmic representation simplifies the implementation.

To deal with this issue, Colavolpe, Barbieri and Caire \cite{Colavolpe05} proposed to approximate $\gamma_n(\theta)$ with $\tilde{\gamma}_n(\theta)\in\mcF$ by,  first matching a Gaussian to $\pdf(y_n|\theta_n,a)\propto g_n(\theta,a)$ from which a Tikhonov distribution was derived as \cite[Sec.~IV.B]{Colavolpe05}
\begin{align}
\label{hat.z.gamma}
\tilde{\gamma}_n(\theta)
&=\mcT\Big(\theta;  z_{\tilde{\gamma},n} \Big)\\
z_{\tilde{\gamma},n}&=
\begin{cases}
z_{g,n}(x_n)  & \text{if}\quad n= l L\\
2\frac{y_n\mfm_n^{*}}{\No+ \mfv_n}, & \text{if}\quad n\neq l L
\end{cases}
\end{align}
where 
\begin{align}
\label{m.n.A}
\mfm_n&=\sum_{a\in\mcA}  a P^{\tr{a}}_n(a) ,\quad%\label{v.n.A}
\mfv_n=\sum_{a\in\mcA}  |a|^2 P^{\tr{a}}_n(a)   -  |\mfm_n|^2,
\end{align}
are the mean and the variance of $x_n$. 

The approximation is needed only for the payload positions, $n\neq lL$. For the pilots $x_n, n=lL$, we have $\gamma_n(\theta)=g_{n}(\theta, x_{n} )$ so we can use directly the parameter of the Tikhonov distribution $z_{g,n}(x_n)$.

This \gls{ga} approach was often reused in the literature, \eg \cite{Barbieri07}\cite{Pecorino15}\cite{Alfredsson19} as the integral part of the \gls{cbc} algorithm. 

On the other hand, recognizing that the distribution \eqref{gamma.def.mixture} is circular, instead of the \gls{ga}  we may apply the \gls{cmm}. It relies on minimization of the \gls{kl} distance between $\tilde{\gamma}_n(\theta)$ and the mixture $\gamma_n(\theta)$, and changes the way the parameter $z_{\tilde{\gamma},n}$ is calculated
\begin{align}\label{gamma.projection.first}
\tilde{\gamma}_n(\theta)
%&=\mcT\Big(\theta;  z_{\tilde{\gamma},n} \Big)\\
&=\mcF\Big[ \sum_{a\in\mcA}\e^{\eta_{g,n}(a)}\mcT\big(\theta;z_{g,n}(a )\big) \Big],\\
\label{gamma.projection.first.cases}
z_{\tilde{\gamma},n}
&=
\begin{cases}
z_{g,n}(x_{n}) &\text{if}\quad n= l L\\
\mf{CMM}\Big[ \eta_{g,n}(a), z_{g,n}(a)\big| a\in\mcA  \Big]&\text{if}\quad n\neq l L.
\end{cases}
\end{align}
where, again, only the payload symbols, $x_n,  n\neq lL$ require the approximation. With a slight abuse of notation we use $\mcF[\cd]$ to denote the operator which  ``projects'' $\gamma_n(\theta)$ onto the Tikhonov family $\mcF$. As a result we obtain the distribution with the parameter $z_{\tilde{\gamma},n}$ which depends only on $\eta_{g,n}(a)$ and $z_{g,n}(a)$, where $a\in\mcA$; this dependence is defined in closed-form by a function $\mf{CMM}[\cd]$ shown in \appref{Sec:CMM}. %and which  follow closely \cite[Appendix~A]{Shayovitz16}. 



%%%%%%%
\subsection{Colavolpe--Barbieri--Caire algorithm \cite{Colavolpe05}}\label{Sec:CBC}

Next, if all the distributions are from the Tikhonov family, \ie $\alpha_n(\theta)=\mcT(\theta;z_{\alpha,n})$ and $\beta_n(\theta)=\mcT(\theta;z_{\beta,n})$, using $\tilde{\gamma}_{n}(\theta)$ instead of $\gamma_n(\theta)$ in \eqref{Tikh.multiplication} and \eqref{Tik.h.Normal.convolution}, we obtain the following parametric \gls{mp} :
\begin{align}
\label{z.alpha.init}
z_{\alpha,0}&=0,\\
\label{z.alpha}
z_{\alpha,n}&= \frac{z_{\alpha,n-1} + z_{\tilde{\gamma},n-1}}{1+|z_{\alpha,n-1} + z_{\tilde{\gamma},n-1}|\sigma_w^2}, \quad n=1, \ld,N-1\\
\label{z.beta.init}
z_{\beta,N}&=0,\\
\label{z.beta}
z_{\beta,n}&= \frac{z_{\beta,n+1} + z_{\tilde{\gamma},n+1}}{1+|z_{\beta,n+1} + z_{\tilde{\gamma},n+1}|\sigma_w^2}, \quad n=N-1,\ld,1,
\end{align}
which is exactly equivalent to the \gls{cbc} algorithm defined in \cite[Eq.~(36)-(37)]{Colavolpe05} and  is provided for completeness and as a starting point for the discussion.

Using \eqref{Tikh.multiplication}  and \eqref{f.n.x.Tikh}--\eqref{xi.f.n} in \eqref{P.n.x}, the ``extrinsic'' symbol probabilities are also calculated as \cite[Eq.~(35)]{Colavolpe05}
\begin{align}\label{P.a.final}
P_n( a )&\propto \int_{0}^{2\pi} \mcT(\theta;z_{\Sigma,n}(a))\frac{\e^{\xi_{g,n}(a)} I_0\big(|z_{\Sigma,n}(a) |\big)}{I_0\big(|z_{g,n}(a)|\big)}\dd \theta,\\
\label{P.a.final.2}
\hat{P}_n( a )&=-\frac{|a|^2}{\No} + \hat{I}_0\big(|z_{\Sigma,n}(a)|\big),\\
\label{z.Sigma.n}
z_{\Sigma,n}(a)&=z_{\alpha,n}+z_{\beta,n}+2\frac{y_n a^{*}}{\No},
\end{align}
and the log-probability $\hat{P}_n( a )=\log P_n( a )$ should be next used in \eqref{lambda.n.l}.

Due to its simplicity, the \gls{cbc} algorithm \eqref{z.alpha.init}-\eqref{z.beta}, should be treated as a ``canonical'' solution to the problem of phase tracking in the sense that it is can be implement without additional assumptions. This explains the considerable attention it received up to now.

Before going further, we note that the difference between the original formulation of the \gls{cbc} algorithm in \cite{Colavolpe05} and this work appears in the way the approximate distribution $\tilde{\gamma}_n(\theta)$ is obtained, that is, whether we opt for the \gls{ga} \eqref{hat.z.gamma}-\eqref{m.n.A}, or we use the \gls{cmm} from \eqref{gamma.projection.first.cases}. 

Although the \gls{cmm} was already used in the context of the phase tracking by \cite{Shayovitz16}, we are not aware of it being applied directly in the \gls{cbc} algorithm. And while the implementation of the function $\mf{CMM}[\cd]$ is less straightforward\footnote{Approximations of non-linear functions are involved, see \appref{Sec:CMM} and \appref{Sec:Bx}.} than the \gls{ga} shown in \eqref{hat.z.gamma}-\eqref{m.n.A}, we will soon compare the \gls{cmm} to the \gls{ga} and show the obvious advantage produced by the former. 


%we clarify its impact in \secref{example.start} and show that  the important improvement in performance justifies the use of the \gls{cmm} in the \gls{cbc} algorithms.

An important observation, already made \eg in \cite[Sec.~I]{Shayovitz16} or \cite[Sec.~IV]{Pecorino15}, is that, using a non-informative prior $\hat{P}^{\tr{a}}(a)\propto 0$,  the approximation $\tilde{\gamma}_n(\theta)$ is also non-informative for the payload symbols; that is, \mbox{$z_{\tilde{\gamma},n}=0, n\neq lL$}.\footnote{If  the \gls{ga} \eqref{hat.z.gamma}-\eqref{m.n.A}, is used,  this is true, if the constellation $\mcA$ is zero mean, which is obvious from \eqref{m.n.A}. On the other hand, if the \gls{cmm} approach is used, this is true for constellations $\mcA$ which may be decomposed into constant modulus zero-mean sub-constellations; the demonstration is easy and omitted for sake of space. For the most popular constellations such as $M$-\gls{qam}, both conditions hold.} 

Since then, the only useful information is obtained from the non-zero $z_{\tilde{\gamma},n}$, that is, from the pilots, the \gls{mp} in \eqref{z.alpha.init}-\eqref{z.beta}, may be then seen as a \emph{pilot-only} based recursive estimation of the phase. And it is independent of the form of the constellation $\mcA$ used to modulate the payload symbols.% which serves later as the reference for detection in \eqref{P.a.final.2}.

This is why, in order to exploit the form of the constellation $\mcA$, the \gls{cbc} phase tracking is put in the ``decoding-loop''. Known also as the joint phase tracking and decoding, it consists in alternate execution of  i)~the \gls{mp}  \eqref{z.alpha.init}-\eqref{z.beta} and ii)~the demodulation/decoding; the latter, providing an informative prior $\hat{P}^{\tr{a}}_n(a)$ on the payload symbols, improves the phase tracking, see \eg \cite{Colavolpe05}\cite{Barbieri07}\cite{Alfredsson19}.


%%%%%%%%%%%%%%%%%%%%
\subsection{Scheduling and complexity}\label{Sec:Sch.Cplx}

It may, therefore, be useful to define a \emph{scheduling} which specifies the number of iteration the \gls{ldpc} decoder executes before its outputs are transformed into $\hat{P}_n(a)$ and used again by the phase tracking \gls{mp}. 

Let the scheduling defined by $\set{I_{\tr{loop}}\times I_\tr{dec} }$ means the following: after each passage of the \gls{cbc} phase tracking, the decoder executes $I_{\tr{dec}}$ elementary decoding iterations\footnote{Defined as one check-nodes message update and one bit-nodes message update.}, then the phase tracking is implemented again and the results are used by the decoder executing $I_{\tr{dec}}$ elementary decoding iterations. This is repeated $I_\tr{loop}$ times so the total number of decoding iterations is given by $I^{\Sigma}_\tr{dec}=I_\tr{loop}\cd I_\tr{dec}$.

The scheduling from \cite{Colavolpe05} is defined by $\set{200 \times 1}$ meaning that the phase-tracking was executed $I_\tr{loop}=200$ times and, each phase-tracking was followed by one elementary decoding iterations; the total number of decoding iterations if thus $I_\tr{dec}^\Sigma=200$.

A ``one-shot'' phase tracking is denoted by the scheduling $\set{1\times I^{\Sigma}_\tr{dec}}$, and means that the phase tracking is carried out once and then all the decoding iterations are executed.

%In other words, the phase tracking is executed $I_\tr{loop}$ times, and the decoder executes $I_{\tr{loop}}} I_{\tr{dec}}$ elementary decoding iterations and, with that notation, the scheduling from \cite{Colavolpe05} is defined by ${200 \times 1}$ meaning that the phase-tracking was executed $200$ times and, each phase-tracking was followed by one elementary decoding iterations of the \gls{ldpc} decoder , while the scheduling $\set{2\times 100}$ from \cite{Alfredsson19} means that the \gls{cbc} phase tracking was executed twice and each was followed by $100$ decoding iterations. 

There are clearly many other possibilities to schedule the operations and they may affect the performance and the complexity. However,  caution should be applied when talking about the implementation complexity because it is difficult to compare  different operations: counting the additions/multiplications may be misleading especially when targeting implementation on the specialized circuits. 

For example, the operations necessary in the \gls{cmm} do not have the same implementation ``complexity'' as those required by the \gls{mp} \eqref{z.alpha.init}-\eqref{z.beta}; and it is difficult to compare any of these to the operations required by the elementary decoding iteration. However,  when operations are of the same type, they can be compared and provide a general idea about the complexity.


%The scheduling $I_{\tr{loop}}\times I_{\tr{dec}}$, means that  the \gls{ldpc} decoder carries out $I_{\tr{dec}}$ iterations and $I_{\tr{loop}}$ is the number of outer-loop iterations, \ie the number of times the phase tracking results are fed to the decoder.


%%%%%%%%%%%%%%
\begin{figure}[bt]
\begin{center}
\psfrag{DMPXXX}[lc][lc][\siz]{DMP}
\psfrag{CBC+GA}[lc][lc][\siz]{CBC+GA \cite{Colavolpe05}}
\psfrag{CBC+CMM}[lc][lc][\siz]{CBC}
\psfrag{AWGN}[lc][lc][\siz]{AWGN}
\psfrag{All-pilots}[lc][lc][\siz]{All-pilots}
\psfrag{ylabel}[lc][lc][\siz]{$\PER$}
\psfrag{xlabel}[lc][lc][\siz]{$\SNR$ [dB]}
\scalebox{\sizf}{\includegraphics[width=\linewidth]{./figures/PER_Tikh_Ex1.eps}}
\end{center}
\caption{\gls{per} vs. \gls{snr} obtained using  \gls{cbc} algorithm with the projection based on the \acrfull{ga} originally proposed in \cite{Colavolpe05} (CBC+GA) or, on the \acrfull{cmm} explained in \appref{Sec:CMM} (CBC), both shown for the scheduling $\set{I_\tr{dec}\times 1}$ with $I_\tr{dec}=10$ (filled markers, solid lines) and $I_\tr{dec}=30$ (hollow markers, dashed lines); the encoding rate of the \gls{ldpc} is $R=\frac{7}{8}$.  The \acrfull{dmp} is implemented using $N_{\theta}=64$ samples, the ``AWGN" curve assumes no phase noise, and ``All pilots'' curve is the performance limits for any joint phase tracking and decoding, see explanation in \secref{example.start}.}\label{fig:PER.preMP}
\end{figure}
%%%%%%%%%%%%%%

\subsection{Example: Phase tracking reference results}\label{example.start}
%\begin{example}[Phase tracking: reference scenario]
The test scenario that will be reused later considers transmission based on $16$-\gls{qam} constellation with Gray mapping \cite[Sec.~2.5.2]{Szczecinski_Alvarado_book}; the proprietary \gls{ldpc} encoder with the rate $R=\frac{7}{8}$ is applied to the block of $\Nb=4032$ bits. The pilot symbols are pseudo-randomly drawn from a $4$-\gls{qam} constellation; the pilot spacing is set to $L=25$ which allows us to place $L-1=24$ payload symbols between pilots, see \eqref{payload.1}, so dummy symbols are not needed to fill the frame of transmitted symbols $\bx$; we thus have $F=43$ pilots and total $N=1051$ symbols. The noise level is $\sigma_w^2=0.01$.

The \gls{per}, shown in \figref{fig:PER.preMP} is estimated after transmitting $10^5$ blocks or after occurence of $100$ blocks in error, whichever comes first. In all cases the total number of decoding iterations is or $I^{\Sigma}_\tr{dec}=10$ (solid markers) or $I^{\Sigma}_\tr{dec}=30$ (hollow markers); the decoding is based on the min-sum algorithm.\footnote{With scaling of the check-nodes messages by a constant factor equal to $\rho=0.7$, see \cite{Xu14}; then, a fraction of dB loss was observed when comparing to the sum-product algorithm in the \gls{awgn} channel.}  

The \gls{dmp} is implemented using $N_\theta=64$ samples and its \gls{per} curve is the performance limit for all ``one-shot'' phase tracking algorithms, \ie those defined by the scheduling \mbox{$\set{1\times I_\tr{dec}}$}.

The curve ``All-pilots'' is obtained assuming that, during the phase-tracking, all the symbols in $\bx$ are pilots. This correspond to a situation when the output of the decoder provides highly reliable information about the bits which gives certainty about the symbols $\bx$ (that is, $P^{\tr{a}}_n(a)\approx 1$ for $a=x_n$); these, in turn, become de facto pilots allowing for the best possible phase tracking. 

Then, when calculating $\hat{P}_n(a)$, the only uncertainty about the symbol $x_n$ is due to the \gls{awgn} noise and the residual phase noise -- this part of it which cannot be estimated from other symbols $x_l, l\neq n$. The ``All-pilots" curve is a performance limit for any joint phase-tracking and demodulation/decoding algorithms. If the \gls{dmp} is too complex to implement, the ``All-pilots" curve may be treated as the proxy for the \gls{dmp}. 

On the other hand, the ``AWGN'' curve corresponds to a hypothetical scenario when the phase-noise is removed and we only deal with the \gls{awgn}. Such results are unattainable no matter how sophisticated the phase-tracking and decoding strategy are, and we show them to illustrate the impact of the phase noise.

As for the \gls{cbc} phase tracking, we observe the following
\begin{itemize}
\item The \gls{per} of the original \gls{cbc} algorithm from \cite{Colavolpe05} (CBC+GA) tends to saturate for high \gls{snr}, \ie where the phase noise dominates the \gls{awgn}. This effect seems to be difficult to remove by increasing the number of iterations. We attribute this behaviour, observed already \eg in \cite[Fig.~8]{Kreimer18}, to the scheduling, where, after each decoding iteration, $\tilde{\gamma}_n(\theta)$ is estimated afresh even if the first decoding iterations do not provide reliable estimates of the coded bits. This, in turn, may yield unreliable $\hat{P}^\tr{a}(a)$, hence unreliable $\tilde{\gamma}_n(\theta)$ which, in turn stalls the convergence. %\ls{To verify this hypothesis, we show the \gls{per} for the scheduling $\mfS=\set{1\times \I_\tr{dec}}$. For low \gls{snr}, it is obviously worse than the \gls{cbc} (+GA) algorithm. On the other hand, it does not display the error floor at the same level as the \gls{cbc}.}
\item The notable difference between the original \gls{cbc} algorithm (\gls{cbc}+\gls{ga}) and the \gls{cbc} algorithm based on the \gls{cmm} (\gls{cbc}) emphasizes the importance of the approximations we make in the phase tracking: by using the \gls{cmm}, we significantly lower the operational \gls{snr}\footnote{The \gls{snr} necessary to attain a given \gls{per} target, \eg for  $\PER_\tr{t}=10^{-2}$, the \gls{snr} decreases by $2$dB.} and  the error floor in the high \gls{snr}.  Thus, all the remaining results are based on the \gls{cmm}. 
\item Irrespectively of the valuable improvement due to the application of the \gls{cmm}, the qualitative behaviour of the \gls{cbc} algorithms is the same: the error floor appears in the \gls{per} curve and the gap to the \gls{dmp} remains large even when we increase the number of iterations. We hasten to say, that it is possible that the error floor occurs also for the \gls{dmp} but it may be difficult to attain without excessively heavy simulations.
\end{itemize}


%%%%%%%%%%%%%%%%%%%%%
\section{Expectation Propagation:\\Self-iterations in the phase-tracking}\label{Sec:It.EP}

The example in \secref{example.start}, showing the improvement in performance obtained by replacing the \gls{ga} proposed originally in \cite{Colavolpe05} with the \gls{cmm}, demonstrates that the reliable phase-tracking results may improve the performance significantly. 

Along the same light of thought, comparing the performance of the \gls{cbc} algorithm with the one-shot phase-tracking of the \gls{dmp}, indicates that satisfactory solutions may be obtained without relying on the decoders' feedback. Therefore, our goal now is to develop a  reliable and ``standalone'' (which can operate without decoder's feedback) phase tracking by exploiting the form of the constellation $\mcA$.

A similar idea was followed in  \cite{Shayovitz16} where the original mixture  $\gamma_n(\theta)$ \eqref{gamma} was used in \eqref{alpha} and \eqref{beta} and the results of multiplication $\alpha_n(\theta)\gamma_n(\theta)$ and $\beta_n(\theta)\gamma_n(\theta)$  were  projected on the space of Tikhonov mixtures $\mcF$. In this way, the projection $\mcF[\cd]$ is moved ``inside" the \gls{mp}; this improves the performance but, requires more projetions and thus increases the complexity comparing to the \gls{cbc} algorithm. Similar principle was explored in \cite{Kreimer18} but using the Gaussian family $\mcF$.

Here, we follow the idea of the \gls{cbc} algorithm motivated by the extreme simplicity of the forward-backward \gls{mp} \eqref{z.alpha.init}-\eqref{z.beta} which amounts to non-linear recursive filtering. Thus, unlike  \cite{Shayovitz16}\cite{Kreimer18}, rather than moving the projection inside the \gls{mp}, we want to enhance the approximations $\tilde{\gamma}_n(\theta)$ and preserve the structure of the \gls{mp} \eqref{z.alpha.init}-\eqref{z.beta}.

To do this, we will improve $\tilde{\gamma}_n(\theta)$ iteratively; this will be done with ``self-iterations", that is without any help from the decoder: the priors $\hat{P}^\tr{a}(a)$ will not change during the self-iterations. 

To explain why this can be done we note that, although the phase tracking \gls{mp} is defined on the tree (graph) that is known to yield the optimal solution in one run (backward-forward processing),  this is only  true for the \gls{dmp} which tracks the entire (discretized) distributions. On the other hand, the \gls{mp} in the \gls{cbc} algorithm is based on approximated distribution $\tilde{\gamma}_n(\theta)$ and, therefore, such a guarantee of optimality does not exist.

We follow here the \gls{ep} idea \cite[Ch.~3.2]{Minka01} which addresses the very problem of using approximate distributions in the \gls{mp}. We will apply the projection $\mcF[\cd]$ many times (iteratively) taking into account the results obtained in previous iterations.  Since most of the resulting operations are almost identical to those we already defined in the \gls{cbc} algorithm, we will use the parenthesized superscript $^{(i)}$ to denote the variables/functions obtained in the $i$-th iteration, where $i=1,\ld, I_\tr{ep}$ and $I_\tr{ep}$ is the maximum number of \gls{ep} iterations.


\subsection{Expectation Propagation for the Phase Tracking}\label{Sec:EP.Ph.Track}
The \gls{ep} applied to our problem relies on the following idea: in the iteration $i$,  we find the approximation $\tilde{\gamma}^{(i)}_n(\theta)$ using the distributions $\alpha^{(i-1)}_n(\theta)$ and $ \beta^{(i-1)}_n(\theta)$ calculated in the previous iterations. This is done by  matching the posterior distribution of $\theta_n$, that would be obtained using $\tilde{\gamma}^{(i)}_n(\theta)$ to the one calculated from the original distribution $\gamma_n(\theta)$ 
\begin{align}
\nonumber
\tilde{\gamma}^{(i)}_n(\theta)\big(\alpha^{(i-1)}_n(\theta)&\beta^{(i-1)}_n(\theta)\big)\\
\label{equal.proba.approx}
&\approx
\gamma_n(\theta)\big(\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)\big)
\end{align}
and requires the projection  operation, $\mcF[\cd]$ to be applied to both sides of \eqref{equal.proba.approx}. 

Since the \gls{lhs} contains the three terms from the family  $\mcF$, it is not affected by the projection (remember, the product of the Tikhonov distributions is a also a Tikhonov distribution), we obtain
\begin{align}\label{equal.proba.approx.2}
\tilde{\gamma}^{(i)}_n(\theta)
&\propto
\frac{\mcF\Big[\gamma_n(\theta)\big(\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)\big)\Big]}
{\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)}.
\end{align}

Of course, for $i=1$, we deal with non-informative distributions $\alpha^{(0)}(\theta)\propto 1$ and $\beta^{(0)}(\theta)\propto 1$, which reduces \eqref{equal.proba.approx.2} to  $\tilde{\gamma}^{(1)}_n(\theta)=\mcF\big[ \gamma_n(\theta)\big]$; this is what was done in \secref{Sec:Parametric.MP}, \ie  $\tilde{\gamma}_n^{(1)}(\theta)$ is the same as $\tilde{\gamma}_n(\theta)$ obtained in \eqref{gamma.projection.first}.

For $i>1$, the informative distributions, $\alpha^{(i-1)}_n(\theta)$ and $\beta^{(i-1)}_n(\theta)$ are available so we have to calculate the \gls{rhs} of \eqref{equal.proba.approx}
\begin{align}
%\nonumber
\gamma_n(\theta)\Big(\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)\Big)
\label{apost.theta.i1}
&=
\sum_{a\in\mcA} \e^{\eta^{(i-1)}_{\Sigma,n}(a)} \mcT\big(\theta; z^{(i-1)}_{\Sigma,n}(a) \big),
\end{align}
where, with proper sup-indexing in \eqref{z.Sigma.n},  we have $z_{\Sigma,n}^{(i-1)}(a)=z_{\alpha,n}^{(i-1)}+z_{\beta,n}^{(i-1)}+z_{g,n}(a)$ and
\begin{align}
\label{eta.Sigma.n.i1}
\eta^{(i-1)}_{\Sigma,n}(a)&=-\frac{|a|^2}{\No}+ \hat{I}_0\big(|z^{(i-1)}_{\Sigma,n}(a)|\big)+\hat{P}^{\tr{a}}_n(a)\\
&=\hat{P}^{(i-1)}_n(a)+\hat{P}^{\tr{a}}(a)
\end{align}
represents the posterior log-probability of the symbols obtained in the iteration $i-1$.

Using \eqref{apost.theta.i1} in \eqref{equal.proba.approx.2} yields
\begin{align}\label{EP.iterations}
\tilde{\gamma}^{(i)}_n(\theta) 
&=\mcT(\theta; z^{(i)}_{\tilde{\gamma},n})\\
\label{EP.division}
&\propto \frac
{\mcF\Big[\sum_{a\in\mcA} \e^{\eta^{(i-1)}_{\Sigma,n} (a)} \mcT\big(\theta; z^{(i-1)}_{\Sigma,n}(a) \big)\Big] }
{\mcT\big(\theta; z^{(i-1)}_{\alpha,n}+z^{(i-1)}_{\beta,n} \big)}\\
\label{EP.division.2}
&= \frac{ \mcT\Big(\theta; z^{(i)}_{\tr{post},n}\Big)  }{ \mcT\Big(\theta; z^{(i-1)}_{\alpha,n}+z^{(i-1)}_{\beta,n} \Big)},
\end{align}
where 
\begin{align}
z^{(i)}_{\tr{post},n} &=\mf{CMM}\Big[ \eta^{(i-1)}_{\Sigma,n}(a), z^{(i-1)}_{\Sigma,n}(a)\big| a\in\mcA  \Big]
\end{align}
and thus
\begin{align}
\label{z.gamma.i}
z^{(i)}_{\tilde{\gamma},n}&= z^{(i)}_{\tr{post},n}  - \big(z^{(i-1)}_{\alpha,n} + z^{(i-1)}_{\beta,n}\big).
\end{align}

%%%%%%%%%%%%%%%
\subsection{Pitfalls  and solutions}\label{Sec:Pitfalls}
The elegant formulation of  the \gls{ep} is indeed appealing but occasionally runs into difficulty due to the division of the distributions in \eqref{EP.division.2}, or equivalently, due to subtraction of the coefficients in \eqref{z.gamma.i}. The existence of such a problem has been acknowledged in \cite[Sec.~3.2]{Minka01} in the context of the Gaussian \gls{ep}, where the division of the distributions may yield a ``Gaussian'' with negative variance, see also \cite[Sec.~IV.B]{Senst11} \cite[Sec.~IV.A]{Cespedes14}. Such results are usually uninterpretable so the workarounds are needed. 

In the context of the Tikhonov distributions $\mcT(\theta;z)$ defined by a complex parameter $z$, the purely numerical issue of invalid parameters (such as a negative variance in  the Gaussian case) is avoided but the problem remains. To understand intuitively its source and devise a solution, we may look at the scenario where the problems materialize. 

\begin{example}[Pitfalls of EP]\label{Ex:Pitfall}
Assume that 
\begin{itemize}
\item The circular means of the approximate posterior distribution, $\mcT\big(\theta; z^{(i)}_{\tr{post},n}\big) $ and of the ``extrinsic'' distribution (defined by  the product $\alpha^{(i-1)}_n(\theta)\beta^{(i-1)}_n(\theta)$) coincide, that is,  $\angle z^{(i)}_{\tr{post},n} =\angle (z^{(i-1)}_{\alpha,n}+z^{(i-1)}_{\beta,n})$; (remember, the phase $\angle z^{(i)}_{\tr{post},n}$ defines the circular mean); and that
\item The variance of the posterior distribution is larger than the variance of the extrinsic distribution, \ie $|z^{(i)}_{\tr{post},n}|<|z^{(i-1)}_{\alpha,n}+z^{(i-1)}_{\beta,n}|$; this may occur because the distribution in the argument of $\mcF[\cd]$ in \eqref{EP.division} is obtained multiplying  the extrinsic distribution $\mcT\big(\theta; z^{(i-1)}_{\alpha,n}+z^{(i-1)}_{\beta,n}\big)$ with a mixture $\gamma_n(\theta)$; the variance of the resulting mixture (and thus of its projection result as well) may be larger than the variance of the extrinsic distribution. 
\end{itemize}

Then, carrying out the subtraction in \eqref{z.gamma.i} we will obtain
\begin{align}
z^{(i)}_{\tilde{\gamma},n}
&= (|z^{(i)}_{\tr{post},n}|  - |z^{(i-1)}_{\alpha,n} + z^{(i-1)}_{\beta,n}|\big)\e^{\jj \angle z^{(i)}_{\tr{post},n}}\\
&=|z^{(i-1)}_{\tilde{\gamma},n}|\e^{\jj(\angle z^{(i)}_{\tr{post},n}+\pi)}.
\end{align}
That is, the circular mean of the new distribution $\mcT(\theta; z^{(i)}_{\tilde{\gamma},n})$ will be  in disagreement (by the largest possible value of $\pi$) with the mean of the posterior and extrinsic distributions obtained from the previous iteration. Such a results, being an artefact of the way the \gls{ep} is defined \cite[Sec.~3.2]{Minka01} is clearly counterintuitive and simply wrong. 
\end{example}

This problem, characteristic of the \gls{ep} occurs in $\tilde{\gamma}_n(\theta)$ and,  propagating via the \gls{mp}, affects $\alpha_n(\theta)$ and $\beta_n(\theta)$.

Heuristics were devised for the Gaussian \gls{ep} where the problem is clearly identified, \ie the variance of the distributions after division becomes negative. For example, \cite[Sec.~3.2]{Minka01} constrains the variance to be positive, while other proposed to identify the problematic cases (\ie the negative variance) and then, if necessary i)~eliminate the division of the distributions \cite[Sec.~IV.B]{Senst11}, which here would mean $z^{(i)}_{\tilde{\gamma},n}=z^{(i)}_{\tr{post},n}$, or ii)~remove the update \cite[Sec.~IV.A]{Cespedes14}, \ie $z^{(i)}_{\tilde{\gamma},n}=z^{(i-1)}_{\tilde{\gamma},n}$. 

On the other hand, instead of testing for the compliance with our prior requirements (that are not necessarily obvious to define),  we might ``smooth'' the obtained parameters via recursive filter \cite[Sec.~IV.A]{Cespedes14} , which would mean  replacing \eqref{z.gamma.i} with
\begin{align}\nonumber
z_{\tilde{\gamma},n}^{(i)} = \zeta \Big(z^{(i)}_{\tr{post},n}  - z^{(i-1)}_{\alpha,n} - z^{(i-1)}_{\beta,n}\Big)
&+(1-\zeta) z_{\tilde{\gamma},n}^{(i-1)}\\
\label{z.smoothing}
& i=2,\ld, I_\tr{ep},
\end{align}
where $\zeta<1$ must be chosen heuristically to strike a balance between the new solution and the history accumulated in the previous estimate. In this way we avoid rapid changes in the the parameters $z_{\tilde{\gamma},n}^{(i)}$, providing a sort of regularization which robustifies the final solution. Note that the smoothing is not necessary in the first iteration, $i=1$, which is based solely on the information obtained from the pilots and from the decoder (if such option is allowed). 

We applied this smoothing solution in our numerical experiments, and found $\zeta\approx 0.4$ yielding satisfactory results. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
\subsection{Summary of the algorithm}\label{Sec:Summary}
The entire algorithm is now summarized as Algorithm~\ref{Algo:EP} where for simplicity we defined the set of indices to the payload symbols and to the pilots as
\begin{align}
\Natural_{\tr{pilots}}&=\set{0,L,2L,\ld, FL}\\
\Natural_{\tr{payload}}&=\set{1,\ld, N} \setminus \Natural_{\tr{pilots}}.
\end{align}
We also integrated the notation so that the \gls{cbc} algorithm is naturally the first iteration ($i=1$) of the \gls{ep} algorithm, \ie $z^{(0)}_{\Sigma,n}(a)=z_{g,n}(a)$ and thus $\eta^{(0)}_{\Sigma,n}(a)=\eta_{g,n}(a)$, see \eqref{gamma.projection.first.cases}; 
the main distinction we need to make is that the smoothing \eqref{z.smoothing} is not applied for $i=1$, seelines \ref{i.if}--\ref{i.endif} of the algorithm. Note that the notation with the iteration index $^{(i)}$ may be removed (and the in-place calculation carried out) but we kept it for compatibility with the equations in the paper.

Last but not least, and at the risk of stating the obvious, we want to emphasize what the \gls{ep} algorithm is \emph{not} doing. Namely, it is not reusing the output ``extrinsic'' log-probabilities $\hat{P}_n(a)$ as if they were newly calculated prior log-probabilities $\hat{P}^{\tr{a}}_n(a)$. This is clearly seen in the description of the algorithm: plugging $\hat{P}_n(a)$ calculated at line \ref{P.n.a} into the line \ref{eta.Sigma.n} will \emph{not} yield the same results $\eta^{(i-1)}_{\Sigma,n}(a)$.

Since the \gls{ep} phase tracking is an iterative process itself, the notion of scheduling has to be revised; we use now the notation $\set{I_\tr{loop}\times (I_\tr{ep}, I_\tr{dec})}$ which takes into account the fact that within each loop the phase tracking may execute $I_\tr{ep}$ \gls{ep} iterations. With this notation, the original \gls{cbc} algorithm is denoted as $I_\tr{dec}\times (1, 1)$ and  one-shot \gls{ep} phase tracking is identified by the scheduling $1\times(I_\tr{ep}, I_\tr{dec} )$

% ------------------------------- algorithm -----------------------
\begin{algorithm}
    \caption{EP phase tracking} \label{Algo:EP}
\begin{algorithmic}[1]
\State Inputs:
\State $y_n, n\in\set{0,\ld,N}$ \Comment Received signal 
\State $x_n, n\in\Natural_{\tr{pilots}}$  \Comment Pilot symbols
\State $\hat{P}^{\tr{a}}_n(a)$\Comment Log-probabilities from the decoder
\State Initialization:
\State $z^{(i)}_{\tilde{\gamma},n}\gets 2\frac{y_n x_n^*}{\No},    n\in \Natural_{\tr{pilots}}, i\in{1,\ld, I_\tr{ep}}$
\State $z_{g,n}(a)\gets 2\frac{y_n a^*}{\No},\quad a\in\mcA, n\in\Natural_{\tr{payload}}$
\State $z_{\Sigma,n}^{(0)}(a) \gets z_{g,n}(a), \quad n\in\Natural_{\tr{payload}}$
\State EP iterations:
\For{ $i\gets1,\ld, I_\tr{ep}$ }
	\For {$n\gets \Natural_{\tr{payload}}$} \Comment Finds $\tilde{\gamma}_n(\theta)$:
		\State $\eta^{(i-1)}_{\Sigma,n}(a) \gets -\frac{|a|^2}{\No}+ \hat{I}_0\big(|z^{(i-1)}_{\Sigma,n}(a)|\big)+\hat{P}^{\tr{a}}_n(a)$ \label{eta.Sigma.n}
		\State $z^{(i)}_{\tr{post},n}  \gets \mf{CMM}\Big[ \eta^{(i-1)}_{\Sigma,n}(a), z^{(i-1)}_{\Sigma,n}(a)\big| a\in\mcA  \Big]$
	\If {$i=1$} \label{i.if}
		\State $z^{(i)}_{\tilde{\gamma},n}\gets z^{(i)}_{\tr{post},n}  - z^{(i-1)}_{\alpha,n} - z^{(i-1)}_{\beta,n}$
	\Else
		\State $z_{\tilde{\gamma},n}^{(i)} \gets \zeta \Big(z^{(i)}_{\tr{post},n}  - z^{(i-1)}_{\alpha,n} - z^{(i-1)}_{\beta,n}\Big)$
		\State \qquad~ \qquad  ~ \qquad~ \qquad~ \qquad$+(1-\zeta) z_{\tilde{\gamma},n}^{(i-1)}$
	\EndIf  \label{i.endif}
	\EndFor
	\State $z^{(i)}_{\alpha,0}\gets 0$	
	\For {$n\gets 1,\ld,N$} \Comment Finds $\alpha^{(i)}_n(\theta)$:
		\State $z^{(i)}_{\alpha,n} \gets \frac{z^{(i)}_{\alpha,n-1} + z^{(i)}_{\tilde{\gamma},n-1}}{1+|z^{(i)}_{\alpha,n-1} + z^{(i)}_{\tilde{\gamma},n-1}|\sigma_w^2}$
	\EndFor
   	\State $z^{(i)}_{\beta,N} \gets 0$
	\For {$n\gets N-1,\ld,0$} \Comment Finds $\beta^{(i)}_n(\theta)$:
		\State $z^{(i)}_{\beta,n} \gets  \frac{z^{(i)}_{\beta,n+1} + z^{(i)}_{\tilde{\gamma},n+1}}{1+|z^{(i)}_{\beta,n+1} + z^{(i)}_{\tilde{\gamma},n+1}|\sigma_w^2}$
	\EndFor
	\For {$n\gets \Natural_{\tr{payload}}$} %\Comment Prepare outputs
	\State $z^{(i)}_{\Sigma,n} \gets  z_{g,n}(a) +z^{(i)}_{\alpha,n}+ z^{(i)}_{\beta,n}$
	\EndFor
\EndFor % i
\State Output: log-probabilities to be used in \eqref{lambda.n.l}
\For {$n \gets \Natural_{\tr{payload}}$}
\State $\hat{P}_{n}( a ) \gets -\frac{|a|^2}{\No} + \hat{I}_0\big(|z^{(I_{\tr{ep}})}_{\Sigma,n}(a)|\big)$\label{P.n.a}
\EndFor
\end{algorithmic}
\end{algorithm}
% ------------------------------- end algorithm -------------------

\subsection{Numerical results}\label{Example.EP} 
Considering the transmission scenario from \secref{example.start} we evaluate the \gls{per} in the one-shot phase tracking (the scheduling $1\times (I_\tr{ep}, I_\tr{dec})$); as discussed in \secref{example.start}, the performance limit for one-shot phase tracking is the \gls{dmp} (with $I_\tr{dec}$ decoding operations).

The results are shown in \figref{fig:PER.EP} and we observe the following:
\begin{itemize}
\item The one-shot \gls{ep} phase tracking with the scheduling \mbox{$\set{1\times (2, 10)}$} outperforms the \gls{cbc} algorithm (scheduling, $\set{30\times 1}$) notably, despite the fact that the later requires $20$ more decoding iterations and $28$  more \gls{mp}s (and, of course, $28$ more projections \eqref{gamma.projection.first.cases}). The same comparison can be made with the \gls{cbc} (scheduling $\set{10\times 1}$): although the complexity measured by the number of decoding iteration is the same, the number of \gls{mp}s is still larger in the \gls{cbc} algorithm. Using the \gls{ep} we thus gain, both in terms of complexity and performance. Moreover, the \gls{ep} phase tracking operates independently of the decoder which is a significant advantage.
\item Increasing the number of \gls{ep} iterations from $I_\tr{ep}=2$ to $I_\tr{ep}=3$ improves the performance in low \gls{snr} at the cost of the \gls{per} saturating in high \gls{snr}. However, the choice of the operating point may be different between applications so the ``optimal'' choice of the parameters is on open issue.
\item Some gain is further obtained by increasing the number of operations from $I_\tr{dec}=10$ to $I_\tr{dec}=30$, yet the qualitative behaviour remains the same.
\end{itemize}

Despite a notable improvement in terms of complexity and performance when comparing to the \gls{cbc} algorithm, we still observe the saturation of the \gls{per} for high \gls{snr}. 

While this may be an acceptable solution at least in a context where only one-shot phase tracking is allowed, putting the \gls{ep} phase-tracking  in the decoding loop, changes the picture even more notably as shown in \figref{fig:PER.EP.DEC}. Since we consider the scheduling $3\times(I_\tr{ep},10)$, the reference curves are those obtained with  $I^{\Sigma}_\tr{dec}=30$ decoding iterations. We observe that
\begin{itemize}
\item The saturation of the \gls{per} disappears thanks to the feedback from the decoder which, already after the first \gls{ep} phase-tracking and $I_\tr{dec}=10$ decoding iterations provides a reliable  prior $\hat{P}^{\tr{a}}_n(a)$.
\item The \gls{ep} results are better than those yield by the \gls{dmp} (with $I_\tr{dec}=30$); this is quite an impressive results as we are not aware of the results in the literature which would show such a performance; and while it might be surprising at the first sight, it is also correct: remember, the performance limit for the joint decoding-phase tracking is defined by the ``All-pilots'' curve ($I_\tr{dec}=30$).
\item As for the complexity, the \gls{ep} phase tracking with a scheduling $\set{3\times(I_\tr{ep},10)}$ requires the same number of decoding iterations as the \gls{cbc} algorithm ($I_\tr{dec}=30$). The result of the latter appear only for  high \gls{snr} and thus, due to the change in the \gls{snr} axis range, they are not plotted in \figref{fig:PER.EP.DEC}. Still, the number of  the \gls{mp} is much lower in the case of the proposed \gls{ep} algorithm so again, we not only gained  notably in performance comparing to the \gls{cbc} algorithm but also preserved the lower complexity.
\end{itemize}

%%%%%%%%%%%%%%
\begin{figure}[bt]
\begin{center}
\psfrag{DMPXXX.XXX}[lc][lc][\siz]{DMP: $I_{\tr{dec}}=10$}
\psfrag{DMP30}[lc][lc][\siz]{DMP: $I_{\tr{dec}}=30$}
\psfrag{CBC10}[lc][lc][\siz]{CBC:$\set{10\times 1}$}
\psfrag{CBC30}[lc][lc][\siz]{CBC:$\set{30\times 1}$}
\psfrag{EP2.10}[lc][lc][\siz]{EP:$\set{1\times(2,10)}$}
\psfrag{EP3.10}[lc][lc][\siz]{EP:$\set{1\times(3,10)}$}
\psfrag{EP2.30}[lc][lc][\siz]{EP:$\set{1\times(2,30)}$}
\psfrag{EP3.30}[lc][lc][\siz]{EP:$\set{1\times(3,30)}$}
\psfrag{ylabel}[lc][lc][\siz]{$\PER$}
\psfrag{xlabel}[lc][lc][\siz]{$\SNR$ [dB]}
\scalebox{\sizf}{\includegraphics[width=\linewidth]{./figures/PER_Tikh_EP.eps}}
\end{center}
\caption{\gls{per} vs. \gls{snr} obtained using  the \gls{ep} one-shot phase tracking, that is, the scheduling \mbox{$\set{1\times(I_{\tr{ep}}, I_\tr{dec})}$}, and the \gls{cbc} algorithm ( scheduling $\set{I_{\tr{dec}}\times 1}$). The \gls{dmp} results are obtained with $I_\tr{dec}=10$ (filled markers, solid lines) and $I_\tr{dec}=30$ (hollow markers, dashed lines).}\label{fig:PER.EP}
\end{figure}
%%%%%%%%%%%%%%

%%%%%%%%%%%%%%
\begin{figure}[bt]
\begin{center}
\psfrag{DMP10XXX.XXX.X}[lc][lc][\siz]{DMP: $I_\tr{dec}=10$}
\psfrag{DMP30X}[lc][lc][\siz]{DMP: $I_\tr{dec}=30$}
\psfrag{All-pilots10}[lc][lc][\siz]{``All-pilots'': $I_\tr{dec}=10$}
\psfrag{All-pilots30}[lc][lc][\siz]{``All-pilots'': $I_\tr{dec}=30$}
\psfrag{EP3x(2,10)}[lc][lc][\siz]{EP: $\set{3\times(2,10)}$}
\psfrag{EP3x(3,10)}[lc][lc][\siz]{EP: $\set{3\times(3,10)}$}
\psfrag{ylabel}[lc][lc][\siz]{$\PER$}
\psfrag{xlabel}[lc][lc][\siz]{$\SNR$ [dB]}
\scalebox{\sizf}{\includegraphics[width=\linewidth]{./figures/PER_Tikh_EP_turbo.eps}}
\end{center}
\caption{\gls{per} vs. \gls{snr} obtained using the \gls{ep} algorithm in the joint decoding-phase tracking algorithm,  with  the scheduling \mbox{$\set{3\times(I_{\tr{ep}}, 10)}$} . The \gls{dmp} and ``All-pilots" results are obtained with $I_\tr{dec}=10$ (filled markers, solid lines) and $I_\tr{dec}=30$ (hollow markers, dashed lines)}\label{fig:PER.EP.DEC}
\end{figure}
%%%%%%%%%%%%%%

%%%%%%%%%%%%%%
%\subsection{Complexity estimation}\label{Sec:Complexity}
%
%To evaluate the complexity and compare it eventually to the methods from the literature we propose to split the complexity into three parts related respectively to the decoding, \acrlong{mp}, and \gls{cmm}.


%%%%%%%%%%%%%%
%\subsection{Impact of large-argument approximations}\label{Sec:Simplifications}
%
%The non-linear operations in the algorithm appear mostly due to the use of the Bessel function, and may be implemented via look-up tables or replaced by easy-to-implement approximations. These non-linearities are present i)~in the calculation of $\hat{I}_0 (x)$, see \eqref{hat.I0} and ii)~when implementing the \gls{cmm}, where the function $B(x)=\frac{I_1(x)}{I_0(x)}$ must be evaluated; this is necessary to implement the projection operation $\mcF[\cd]$ and to calculate the result of the convolution between the Gaussian and the Tikhonov distributions.
%
%As for the point i), we may actually implement exactly the function $\hat{I}_0 (x)$ or use the \gls{laa} which was already proposed in the previous works, \eg \cite{Colavolpe05}\cite{Pecorino15}\cite{Shayovitz16}. This amount to using $\hat{I}_0 (x)\approx x $.
%
%As for the points ii) we already abandoned the idea of exact implementation of $B(x)$ (\eg via look-up tables) and instead use the approximation valid for the entire range of its argument, see \appref{}. However, it is still interesting to see the impact of the \gls{lla} in this case, especially that it was previously used for the very same purpose in the literature, \eg \cite[Appendix~A]{Shayovitz16}.
%
%We show in \figref{} how the \gls{per} is affected when the \gls{laa} is applied in different parts of the algorithms.







==> figures/Frame.structure.tex <==
%!TEX root =  ../Phase.Track.HARQ.tex
\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

%=================
\begin{center}
\begin{tikzpicture}[trim left=0cm,node distance=3cm]

  %%%%%--------  Set nodes -------- %%%%%%%%%%%%%%%%  
\node[point_my]	(start_p) 				{};
\node[rect_my] 	(Enc) 	[right of=start_p,node distance=2cm]	{$\ENCwo$};
\node[rect_my]	(Chan1) 	[right of=Enc]	{Round $1$};
\node[rect_my]	(Chan2) 	[below of=Chan1,yshift=2cm]	{Round $2$};
\node[point_my]	(dots_etc) 	[below of=Chan2,yshift=2cm]			{$\vdots$};
\node[rect_my]	(Chank) 	[below of=dots_etc,yshift=2cm]  {Round $k$};
\node[square_my]	(Dem1) 	[right of=Chan1,node distance=3.5cm]	{$\DEMwo_1$};
\node[square_my]	(Dem2) 	[right of=Chan2,node distance=3.5cm]	{$\DEMwo_2$};
\node[square_my]	(Demk) 	[right of=Chank,node distance=3.5cm]	{$\DEMwo_k$};
\node[square_my]	(Agg) 	[right of=Dem1,node distance=2.5cm]	{$\Sigma$};
\node[rect_my]	(Dec) 	[right of=Agg,node distance=2.5cm]	{$\DECwo$};
\node[point_my]	(end_p)	[right of=Dec,node distance = 2cm]    {};    

 %%%%%--------    Draw Paths  -------- %%%%%%%%%%%%%%%%
\path[line_my]   (start_p)	-- node[above, near start]{$\bb$}	(Enc);
\path[line_my]   (Enc)		-- node[above, near start]{$\bx$} 	(Chan1) coordinate[pos=0.6](Temp1); 
\path[line_my]   (Temp1)		|- 	(Chan2);
\path[line_my]   (Temp1)		|- 	(Chank);
\path[line_my]   (Chan1)	-- node[above]{$\by_1$}	(Dem1); 
\path[line_my]   (Chan2)	-- node[above]{$\by_2$}	(Dem2); 
\path[line_my]   (Chank)	-- node[above]{$\by_k$}	(Demk); 
\path[line_my]   (Dem1)	-- node[above,near start]{$L_1$}	(Agg); 
\path[line_my]   (Dem2.east)	-- node[above,near start]{$L_2$}	(Agg);
\path[line_my]   (Demk.east)	-- node[below right,near start]{$L_k$}	(Agg);
\path[line_my]   (Agg)		-- node[above,near end]{$L^\Sigma$}	(Dec);
\path[line_my]   (Dec)		-- node[above, near end]{$\hat{\bb}$}	(end_p); 

%%%% %% --- Draw Big Box
\begin{pgfonlayer}{background}
\node[bigbox_my,fill=blue!20, fit=(Dem1)(Demk)(Agg),label=north:$\DEMwo$]   (Dem_tot) {};
\node[bigbox_my,fill=blue!20, fit=(Chan1)(Chank),label=north:Channel]   (Chan_tot) {};
%\node[below right] at (RX.north)  {Receiver};
\end{pgfonlayer}

%%%%
\end{tikzpicture}
\end{center}


==> figures/Graph.IRHARQ.tex <==
%!TEX root =  ../Phase.Track.HARQ.tex
\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

%=================
\begin{center}
\begin{tikzpicture}[trim left=0cm,node distance=3cm]

 %%%%%--------  Set nodes -------- %%%%%%%%%%%%%%%%  
 %  $n-1$
\node[circle_my_graph] 	(phase11) 		{$\theta^{(1)}_{n-1}$};
\node[square_my_graph]	(Chan11) 	[above of=phase11,node distance=1.5cm]	{$f_{n-1}^{(1)}$};
\node[circle_my_graph] 	(symbol11) 	[above of=Chan11,node distance=1.5cm]	{$x^{(1)}_{n}$};
\node[square_my_graph]	(MOD11) 	[above of=symbol11,node distance=1.5cm]	{$\MODwo$};
\node[circle_my_graph] 	(label11) 	[above of=MOD11,node distance=1.5cm]	{$\tilde{\bc}^{(1)}_{n-1}$};

%-- anchoring the graphs
\node[square_my_graph]	(Pw1) 	[below right of=phase11,node distance=2.5cm]	{$p_w$};
\node[square_my_graph]	(Pw2) 	[right of=Pw1,node distance=.7cm, yshift=-0.1cm]	{$p_w$};
%-

\node[circle_my_graph] 	(phase21) 	[above left of=Pw2,node distance=2.5cm]	{$\theta^{(2)}_{n-1}$};
\node[square_my_graph]	(Chan21) 	[above of=phase21,node distance=1.5cm]	{$f_{n-1}^{(2)}$};
\node[circle_my_graph] 	(symbol21) 	[above of=Chan21,node distance=1.5cm]	{$x^{(2)}_{n-1}$};
\node[square_my_graph]	(MOD21) 	[above of=symbol21,node distance=1.5cm]	{$\MODwo$};
\node[circle_my_graph] 	(label21) 	[above of=MOD21,node distance=1.5cm]	{$\tilde{\bc}^{(2)}_{n-1}$};

\node[point_my]	 		(point11) 	[below left of=phase11,node distance=1.5cm]	{};
\node[point_my]	 		(point21) 	[below left of=phase21,node distance=1.5cm]	{};
%%%%%--------    Draw Paths  -------- %%%%%%%%%%%%%%%%
\draw[--]   (Pw1)	  -- 	(phase11.south);   \draw[-]   (Pw2)	  -- 	(phase21.south);
\draw[--]   (phase11)  -- 	(Chan11);   \draw[--]   (phase21)  -- 	(Chan21);
\draw[--]   (Chan11) -- (symbol11);  \draw[--]   (Chan21) -- (symbol21);
\draw[--]    (symbol11) -- (MOD11); \draw[--]    (symbol21) -- (MOD21);
\draw[--]    (MOD11) --  (label11);   \draw[--   ](MOD21) --  (label21);
\draw[--,dashed]   (point11)	  -- 	(phase11);   \draw[--,dashed]   (point21)	  -- 	(phase21);
 %  $n$

\node[circle_my_graph] 	(phase1) 	[above right of=Pw1,node distance=2.5cm]	{$\theta^{(1)}_{n}$};
\node[square_my_graph]	(Chan1) 	[above of=phase1,node distance=1.5cm]	{$f_n^{(1)}$};
\node[circle_my_graph] 	(symbol1) 	[above of=Chan1,node distance=1.5cm]	{$x^{(1)}_{n}$};
\node[square_my_graph]	(MOD1) 	[above of=symbol1,node distance=1.5cm]	{$\MODwo$};
\node[circle_my_graph] 	(label1) 	[above of=MOD1,node distance=1.5cm]	{$\tilde{\bc}^{(1)}_{n}$};
%--

\node[circle_my_graph] 	(phase2) 	[above right of=Pw2,node distance=2.5cm]	{$\theta^{(2)}_{n}$};
\node[square_my_graph]	(Chan2) 	[above of=phase2,node distance=1.5cm]	{$f_n^{(2)}$};
\node[circle_my_graph] 	(symbol2) 	[above of=Chan2,node distance=1.5cm]	{$x^{(2)}_{n}$};
\node[square_my_graph]	(MOD2) 	[above of=symbol2,node distance=1.5cm]	{$\MODwo$};
\node[circle_my_graph] 	(label2) 	[above of=MOD2,node distance=1.5cm]	{$\tilde{\bc}^{(2)}_{n}$};
%%%%%--------    Draw Paths  -------- %%%%%%%%%%%%%%%%
\draw[--]   (Pw1)	  -- 	(phase1);   \draw[-]   (Pw2)	  -- 	(phase2);
\draw[--]   (phase1)  -- 	(Chan1);   \draw[--]   (phase2)  -- 	(Chan2);
\draw[--]   (Chan1) -- (symbol1);  \draw[--]   (Chan2) -- (symbol2);
\draw[--]    (symbol1) -- (MOD1); \draw[--]    (symbol2) -- (MOD2);
\draw[--   ](MOD1) --  (label1);   \draw[--   ](MOD2) --  (label2);


%  $n+1$
\node[square_my_graph]	(Pw13) 	[below right of=phase1,node distance=2.5cm]	{$p_w$};
\node[circle_my_graph] 	(phase13) 	[above right of=Pw13,node distance=2.5cm]	{$\theta^{(1)}_{n+1}$};
\node[square_my_graph]	(Chan13) 	[above of=phase13,node distance=1.5cm]	{$f_{n+1}^{(1)}$};
\node[circle_my_graph] 	(symbol13) 	[above of=Chan13,node distance=1.5cm]	{$x^{(1)}_{n+1}$};
\node[square_my_graph]	(MOD13) 	[above of=symbol13,node distance=1.5cm]	{$\MODwo$};
\node[circle_my_graph] 	(label13) 	[above of=MOD13,node distance=1.5cm]	{$\tilde{\bc}^{(1)}_{n+1}$};
%--
\node[square_my_graph]	(Pw23) 	[below right of=phase2,node distance=2.5cm]	{$p_w$};
\node[circle_my_graph] 	(phase23) 	[above right of=Pw23,node distance=2.5cm]	{$\theta^{(2)}_{n+1}$};
\node[square_my_graph]	(Chan23) 	[above of=phase23,node distance=1.5cm]	{$f_{n+1}^{(2)}$};
\node[circle_my_graph] 	(symbol23) 	[above of=Chan23,node distance=1.5cm]	{$x^{(2)}_{n+1}$};
\node[square_my_graph]	(MOD23) 	[above of=symbol23,node distance=1.5cm]	{$\MODwo$};
\node[circle_my_graph] 	(label23) 	[above of=MOD23,node distance=1.5cm]	{$\tilde{\bc}^{(2)}_{n+1}$};
%-
\node[point_my]	 		(point13) 	[below right of=phase13,node distance=1.5cm]	{};
\node[point_my]	 		(point23) 	[below right of=phase23,node distance=1.5cm]	{};
%%%%%--------    Draw Paths  -------- %%%%%%%%%%%%%%%%
\draw[--]   (Pw13)	  -- 	(phase1.south);   \draw[-]   (Pw23)	  -- 	(phase2.south);
\draw[--]   (Pw13)	  -- 	(phase13);   \draw[-]   (Pw23)	  -- 	(phase23);
\draw[--]   (phase13)  -- 	(Chan13);   \draw[--]   (phase23)  -- 	(Chan23);
\draw[--]   (Chan13) -- (symbol13);  \draw[--]   (Chan23) -- (symbol23);
\draw[--]    (symbol13) -- (MOD13); \draw[--]    (symbol23) -- (MOD23);
\draw[--]    (MOD13) --  (label13);   \draw[--   ](MOD23) --  (label23);

\draw[--,dashed]   (point13)	  -- 	(phase13.south);   \draw[--,dashed]   (point23)	  -- 	(phase23.south);

%%%% add the code constraints
\begin{pgfonlayer}{foreground}
\node[point_my]	 (label11H)	[above of=label11,node distance=1.5cm]	{};
\node[point_my]	 (label21H)	[above of=label21,node distance=1.5cm]	{};
\node[point_my]	 (label1H)	[above of=label1,node distance=1.5cm]	{};
\node[point_my]	 (label2H)	[above of=label2,node distance=1.5cm]	{};
\node[point_my]	 (label13H)	[above of=label13,node distance=1.5cm]	{};
\node[point_my]	 (label23H)	[above of=label23,node distance=1.5cm]	{};


\draw[--]    (label1) -- (label1H);   \draw[--]    (label2) -- (label2H);   
\draw[--]    (label11) -- (label11H);   \draw[--]    (label21) -- (label21H);   
\draw[--]    (label13) --  (label13H);  \draw[--]    (label23) --  (label23H);
\node[bigbox_my,fill=blue!20, fit=(label11H)(label23H)]   (ENCODER) {Channel code graph};
\end{pgfonlayer}
 
%\path[line_my]   (start_p)	-- node[above, near start]{$\bb$}	(Enc);
%\path[line_my]   (Enc)		-- node[above, near start]{$\bx$} 	(Chan1) coordinate[pos=0.6](Temp1); 
%\path[line_my]   (Temp1)		|- 	(Chan2);
%\path[line_my]   (Temp1)		|- 	(Chank);
%\path[line_my]   (Chan1)	-- node[above]{$\by_1$}	(Dem1); 
%\path[line_my]   (Chan2)	-- node[above]{$\by_2$}	(Dem2); 
%\path[line_my]   (Chank)	-- node[above]{$\by_k$}	(Demk); 
%\path[line_my]   (Dem1)	-- node[above,near start]{$L_1$}	(Agg); 
%\path[line_my]   (Dem2.east)	-- node[above,near start]{$L_2$}	(Agg);
%\path[line_my]   (Demk.east)	-- node[below right,near start]{$L_k$}	(Agg);
%\path[line_my]   (Agg)		-- node[above,near end]{$L^\Sigma$}	(Dec);
%\path[line_my]   (Dec)		-- node[above, near end]{$\hat{\bb}$}	(end_p); 

%%%% %% --- Draw Big Box
%\begin{pgfonlayer}{background}
%\node[bigbox_my,fill=blue!20, fit=(Dem1)(Demk)(Agg),label=north:$\DEMwo$]   (Dem_tot) {};
%\node[bigbox_my,fill=blue!20, fit=(Chan1)(Chank),label=north:Channel]   (Chan_tot) {};
%\node[below right] at (RX.north)  {Receiver};
%\end{pgfonlayer}

%%%%
\end{tikzpicture}
\end{center}


==> figures/Graph.IRHARQ.x.tex <==
%!TEX root =  ../Phase.Track.HARQ.tex
\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

%=================
\begin{tikzpicture}[trim left=0cm,node distance=3cm]

 %%%%%--------  Set nodes -------- %%%%%%%%%%%%%%%%  
 %  $n-1$
\node[circle_my_graph] 	(phase11) 		{$\theta^{(1)}_{n-1}$};
\node[square_my_graph]	(Chan11) 	[above of=phase11,node distance=2cm]	{$f_{n-1}^{(1)}$};
\node[circle_my_graph] 	(symbol11) 	[above of=Chan11,node distance=2cm]	{$x^{(1)}_{n-1}$};
%\node[square_my_graph]	(MOD11) 	[above of=symbol11,node distance=1.5cm]	{$\MODwo$};
%\node[circle_my_graph] 	(label11) 	[above of=MOD11,node distance=1.5cm]	{$\tilde{\bc}^{(1)}_{n-1}$};

%-- anchoring the graphs
\node[square_my_graph]	(Pw1) 	[below right of=phase11,node distance=2.5cm]	{$p_w$};
\node[square_my_graph]	(Pw2) 	[right of=Pw1,node distance=.7cm, yshift=-0.1cm]	{$p_w$};
%-

\node[circle_my_graph] 	(phase21) 	[above left of=Pw2,node distance=2.5cm]	{$\theta^{(2)}_{n-1}$};
\node[square_my_graph]	(Chan21) 	[above of=phase21,node distance=2cm]	{$f_{n-1}^{(2)}$};
\node[circle_my_graph] 	(symbol21) 	[above of=Chan21,node distance=2cm]	{$x^{(2)}_{n-1}$};
%\node[square_my_graph]	(MOD21) 	[above of=symbol21,node distance=1.5cm]	{$\MODwo$};
%\node[circle_my_graph] 	(label21) 	[above of=MOD21,node distance=1.5cm]	{$\tilde{\bc}^{(2)}_{n-1}$};

\node[point_my]	 		(point11) 	[below left of=phase11,node distance=1.5cm]	{};
\node[point_my]	 		(point21) 	[below left of=phase21,node distance=1.5cm]	{};
%%%%%--------    Draw Paths  -------- %%%%%%%%%%%%%%%%
\draw[-]   (Pw1)	  	--   (phase11.south);   \draw[-]   (phase21.south) -- (Pw2);
\draw[-]   (phase11)  -- 	(Chan11);   \draw[-]   (phase21)  -- 	(Chan21);
\draw[-]   (Chan11) -- (symbol11);  \draw[-]   (Chan21) -- (symbol21);
%\draw[-]    (symbol11) -- (MOD11); \draw[-]    (symbol21) -- (MOD21);
%\draw[-]    (MOD11) --  (label11);   \draw[--   ](MOD21) --  (label21);
\draw[-,dashed]   (point11)	  -- 	(phase11);   \draw[-,dashed]   (point21)	  -- 	(phase21);
%\draw[-]  (Xa)	 -- node[midway,below,sloped]{\tiny $\overrightarrow{\mu_{f_1\sra X_\tr{a}}}$} (fun_1);


%%%%%%%%% ----  $n$ -----

\node[circle_my_graph] 	(phase1) 	[above right of=Pw1,node distance=2.5cm]	{$\theta^{(1)}_{n}$};
\node[square_my_graph]	(Chan1) 	[above of=phase1,node distance=2cm]	{$f_n^{(1)}$};
\node[circle_my_graph] 	(symbol1) 	[above of=Chan1,node distance=2cm]	{$x^{(1)}_{n}$};
%\node[square_my_graph]	(MOD1) 	[above of=symbol1,node distance=1.5cm]	{$\MODwo$};
%\node[circle_my_graph] 	(label1) 	[above of=MOD1,node distance=1.5cm]	{$\tilde{\bc}^{(1)}_{n}$};
%--

\node[circle_my_graph] 	(phase2) 	[above right of=Pw2,node distance=2.5cm]	{$\theta^{(2)}_{n}$};
\node[square_my_graph]	(Chan2) 	[above of=phase2,node distance=2cm]	{$f_n^{(2)}$};
\node[circle_my_graph] 	(symbol2) 	[above of=Chan2,node distance=2cm]	{$x^{(2)}_{n}$};
%\node[square_my_graph]	(MOD2) 	[above of=symbol2,node distance=1.5cm]	{$\MODwo$};
%\node[circle_my_graph] 	(label2) 	[above of=MOD2,node distance=1.5cm]	{$\tilde{\bc}^{(2)}_{n}$};
%%%%%--------    Draw Paths  -------- %%%%%%%%%%%%%%%%
\draw[-]   (Pw1)	  --  node[midway,above,sloped]{$\underrightarrow{\alpha^{(t)}_{n}(\theta)}$}	(phase1);   
\draw[-]   (Pw2)	  --  (phase2);
\draw[-]   (Chan1) -- node[midway,below,sloped]{$\overrightarrow{\gamma^{(t)}_{n}(\theta)}$} (phase1);   
\draw[-]   (phase2)  -- 	(Chan2);
\draw[-]   (Chan1) -- node[midway,above,sloped]{$\underrightarrow{P^{(t)}_{n}(x)}$}   (symbol1);  
\draw[-]   (Chan2) -- (symbol2);
%\draw[-]    (symbol1) -- (MOD1); \draw[-]    (symbol2) -- (MOD2);
%\draw[--   ](MOD1) --  (label1);   \draw[--   ](MOD2) --  (label2);


%  $n+1$
\node[square_my_graph]	(Pw13) 	[below right of=phase1,node distance=2.5cm]	{$p_w$};
\node[circle_my_graph] 	(phase13) 	[above right of=Pw13,node distance=2.5cm]	{$\theta^{(1)}_{n+1}$};
\node[square_my_graph]	(Chan13) 	[above of=phase13,node distance=2cm]	{$f_{n+1}^{(1)}$};
\node[circle_my_graph] 	(symbol13) 	[above of=Chan13,node distance=2cm]	{$x^{(1)}_{n+1}$};
%\node[square_my_graph]	(MOD13) 	[above of=symbol13,node distance=1.5cm]	{$\MODwo$};
%\node[circle_my_graph] 	(label13) 	[above of=MOD13,node distance=1.5cm]	{$\tilde{\bc}^{(1)}_{n+1}$};
%--
\node[square_my_graph]	(Pw23) 	[below right of=phase2,node distance=2.5cm]	{$p_w$};
\node[circle_my_graph] 	(phase23) 	[above right of=Pw23,node distance=2.5cm]	{$\theta^{(2)}_{n+1}$};
\node[square_my_graph]	(Chan23) 	[above of=phase23,node distance=2cm]	{$f_{n+1}^{(2)}$};
\node[circle_my_graph] 	(symbol23) 	[above of=Chan23,node distance=2cm]	{$x^{(2)}_{n+1}$};
%\node[square_my_graph]	(MOD23) 	[above of=symbol23,node distance=1.5cm]	{$\MODwo$};
%\node[circle_my_graph] 	(label23) 	[above of=MOD23,node distance=1.5cm]	{$\tilde{\bc}^{(2)}_{n+1}$};
%-
\node[point_my]	 		(point13) 	[below right of=phase13,node distance=1.5cm]	{};
\node[point_my]	 		(point23) 	[below right of=phase23,node distance=1.5cm]	{};
%%%%%--------    Draw Paths  -------- %%%%%%%%%%%%%%%%
\draw[-]   (Pw13)	  -- 	(phase1.south);   
\draw[-]   (Pw23)	  -- node[midway,above,sloped]{$\underleftarrow{\beta^{(t)}_{n}(\theta)}$}	(phase2.south);
\draw[-]   (Pw13)	  -- 	(phase13);   \draw[-]   (Pw23)	  -- 	(phase23);
\draw[-]   (phase13)  -- 	(Chan13);   \draw[-]   (phase23)  -- 	(Chan23);
\draw[-]   (Chan13) -- (symbol13);  \draw[-]   (Chan23) -- (symbol23);
%\draw[-]    (symbol13) -- (MOD13); \draw[-]    (symbol23) -- (MOD23);
%\draw[-]    (MOD13) --  (label13);   \draw[--   ](MOD23) --  (label23);
\draw[-,dashed]   (point13)	  -- 	(phase13.south);   \draw[-,dashed]   (point23)	  -- 	(phase23.south);

%%%% add the code constraints
\begin{pgfonlayer}{foreground}
\node[point_my]	 (label11H)	[above of=symbol11,node distance=2.5cm]	{};
\node[point_my]	 (label21H)	[above of=symbol21,node distance=2.5cm]	{};
\node[point_my]	 (label1H)	[above of=symbol1,node distance=2.5cm]	{};
\node[point_my]	 (label2H)	[above of=symbol2,node distance=2.5cm]	{};
\node[point_my]	 (label13H)	[above of=symbol13,node distance=2.5cm]	{};
\node[point_my]	 (label23H)	[above of=symbol23,node distance=2.5cm]	{};


\draw[-]    (symbol1) -- node[near start,above,sloped]{$\underrightarrow{P^{(t)}_{n}(x)}$} (label1H);   
\draw[-]    (symbol2) -- node[near start,below,sloped,xshift=0.2cm]{$\overleftarrow{P^{\tr{a},(t)}_{n}(x)}$} (label2H);   
\draw[-]    (symbol11) -- (label11H);   \draw[-]    (symbol21) -- (label21H);   
\draw[-]    (symbol13) --  (label13H);  \draw[-]    (symbol23) --  (label23H);
\node[bigbox_my,fill=blue!20, fit=(label11H)(label23H)]   (ENCODER) {modulation/coding graph};
\end{pgfonlayer}
 
%\path[line_my]   (start_p)	-- node[above, near start]{$\bb$}	(Enc);
%\path[line_my]   (Enc)		-- node[above, near start]{$\bx$} 	(Chan1) coordinate[pos=0.6](Temp1); 
%\path[line_my]   (Temp1)		|- 	(Chan2);
%\path[line_my]   (Temp1)		|- 	(Chank);
%\path[line_my]   (Chan1)	-- node[above]{$\by_1$}	(Dem1); 
%\path[line_my]   (Chan2)	-- node[above]{$\by_2$}	(Dem2); 
%\path[line_my]   (Chank)	-- node[above]{$\by_k$}	(Demk); 
%\path[line_my]   (Dem1)	-- node[above,near start]{$L_1$}	(Agg); 
%\path[line_my]   (Dem2.east)	-- node[above,near start]{$L_2$}	(Agg);
%\path[line_my]   (Demk.east)	-- node[below right,near start]{$L_k$}	(Agg);
%\path[line_my]   (Agg)		-- node[above,near end]{$L^\Sigma$}	(Dec);
%\path[line_my]   (Dec)		-- node[above, near end]{$\hat{\bb}$}	(end_p); 

%%%% %% --- Draw Big Box
%\begin{pgfonlayer}{background}
%\node[bigbox_my,fill=blue!20, fit=(Dem1)(Demk)(Agg),label=north:$\DEMwo$]   (Dem_tot) {};
%\node[bigbox_my,fill=blue!20, fit=(Chan1)(Chank),label=north:Channel]   (Chan_tot) {};
%\node[below right] at (RX.north)  {Receiver};
%\end{pgfonlayer}

%%%%
\end{tikzpicture}



==> figures/Graph.RRHARQ.x.tex <==
%!TEX root =  ../Phase.Track.HARQ.tex
\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

%=================
\begin{tikzpicture}[trim left=0cm,node distance=3cm]

 %%%%%--------  Set nodes -------- %%%%%%%%%%%%%%%%  
 %  $n-1$
\node[circle_my_graph] 	(phase11) 		{$\theta^{(1)}_{n-1}$};
\node[square_my_graph]	(Chan11) 	[above of=phase11,node distance=2cm]	{$f_{n-1}^{(1)}$};
\node[circle_my_graph] 	(symbol11) 	[above of=Chan11,node distance=2cm]	{$x_{n-1}$};
%\node[square_my_graph]	(MOD11) 	[above of=symbol11,node distance=1.5cm]	{$\MODwo$};
%\node[circle_my_graph] 	(label11) 	[above of=MOD11,node distance=1.5cm]	{$\tilde{\bc}^{(1)}_{n-1}$};

%-- anchoring the graphs
\node[square_my_graph]	(Pw1) 	[below right of=phase11,node distance=2.5cm]	{$p_w$};
\node[square_my_graph]	(Pw2) 	[right of=Pw1,node distance=.7cm, yshift=-0.1cm]	{$p_w$};
%-

\node[circle_my_graph] 	(phase21) 	[above left of=Pw2,node distance=2.5cm]	{$\theta^{(2)}_{n-1}$};
\node[square_my_graph]	(Chan21) 	[above of=phase21,node distance=2cm]	{$f_{n-1}^{(2)}$};
%\node[circle_my_graph] 	(symbol21) 	[above of=Chan21,node distance=1.5cm]	{$x^{(2)}_{n-1}$};
%\node[square_my_graph]	(MOD21) 	[above of=symbol21,node distance=1.5cm]	{$\MODwo$};
%\node[circle_my_graph] 	(label21) 	[above of=MOD21,node distance=1.5cm]	{$\tilde{\bc}^{(2)}_{n-1}$};

\node[point_my]	 		(point11) 	[below left of=phase11,node distance=1.5cm]	{};
\node[point_my]	 		(point21) 	[below left of=phase21,node distance=1.5cm]	{};
%%%%%--------    Draw Paths  -------- %%%%%%%%%%%%%%%%
\draw[-]   (Pw1)	  	--   (phase11.south);   \draw[-]   (phase21.south) -- (Pw2);
\draw[-]   (phase11)  -- 	(Chan11);   \draw[-]   (phase21)  -- 	(Chan21);
\draw[-]   (Chan11) -- (symbol11);  \draw[-]   (Chan21) -- (symbol11);
%\draw[-]    (symbol11) -- (MOD11); \draw[-]    (symbol21) -- (MOD21);
%\draw[-]    (MOD11) --  (label11);   \draw[--   ](MOD21) --  (label21);
\draw[-,dashed]   (point11)	  -- 	(phase11);   \draw[-,dashed]   (point21)	  -- 	(phase21);
%\draw[-]  (Xa)	 -- node[midway,below,sloped]{\tiny $\overrightarrow{\mu_{f_1\sra X_\tr{a}}}$} (fun_1);

%%%%%%%%% ----  $n$ -----

\node[circle_my_graph] 	(phase1) 	[above right of=Pw1,node distance=2.5cm]	{$\theta^{(1)}_{n}$};
\node[square_my_graph]	(Chan1) 	[above of=phase1,node distance=2cm]	{$f_n^{(1)}$};
\node[circle_my_graph] 	(symbol1) 	[above of=Chan1,node distance=2cm]	{$x_{n}$};
%\node[square_my_graph]	(MOD1) 	[above of=symbol1,node distance=1.5cm]	{$\MODwo$};
%\node[circle_my_graph] 	(label1) 	[above of=MOD1,node distance=1.5cm]	{$\tilde{\bc}^{(1)}_{n}$};
%--

\node[circle_my_graph] 	(phase2) 	[above right of=Pw2,node distance=2.5cm]	{$\theta^{(2)}_{n}$};
\node[square_my_graph]	(Chan2) 	[above of=phase2,node distance=2cm]	{$f_n^{(2)}$};
%\node[circle_my_graph] 	(symbol2) 	[above of=Chan2,node distance=1.5cm]	{$x^{(2)}_{n}$};
%\node[square_my_graph]	(MOD2) 	[above of=symbol2,node distance=1.5cm]	{$\MODwo$};
%\node[circle_my_graph] 	(label2) 	[above of=MOD2,node distance=1.5cm]	{$\tilde{\bc}^{(2)}_{n}$};
%%%%%--------    Draw Paths  -------- %%%%%%%%%%%%%%%%
\draw[-]   (Pw1)	  --  node[midway,above,sloped]{$\underrightarrow{\alpha^{(t)}_{n}(\theta)}$}	(phase1);   
\draw[-]   (Pw2)	  --  (phase2);
\draw[-]   (Chan1) -- node[midway,below,sloped]{$\overrightarrow{\gamma^{(t)}_{n}(\theta)}$} (phase1);   
\draw[-]   (phase2)  -- 	(Chan2);
\draw[-]   (Chan1) -- node[midway,above,sloped]{$\underrightarrow{P^{(1)}_{n}(x)}$} (symbol1);  
\draw[-]   (Chan2) -- node[midway,above,sloped]{$\underleftarrow{P^{(2)}_{n}(x)}$} (symbol1);
%\draw[-]    (symbol1) -- (MOD1); \draw[-]    (symbol2) -- (MOD2);
%\draw[--   ](MOD1) --  (label1);   \draw[--   ](MOD2) --  (label2);


%  $n+1$
\node[square_my_graph]	(Pw13) 	[below right of=phase1,node distance=2.5cm]	{$p_w$};
\node[circle_my_graph] 	(phase13) 	[above right of=Pw13,node distance=2.5cm]	{$\theta^{(1)}_{n+1}$};
\node[square_my_graph]	(Chan13) 	[above of=phase13,node distance=2cm]	{$f_{n+1}^{(1)}$};
\node[circle_my_graph] 	(symbol13) 	[above of=Chan13,node distance=2cm]	{$x_{n+1}$};
%\node[square_my_graph]	(MOD13) 	[above of=symbol13,node distance=1.5cm]	{$\MODwo$};
%\node[circle_my_graph] 	(label13) 	[above of=MOD13,node distance=1.5cm]	{$\tilde{\bc}^{(1)}_{n+1}$};
%--
\node[square_my_graph]	(Pw23) 	[below right of=phase2,node distance=2.5cm]	{$p_w$};
\node[circle_my_graph] 	(phase23) 	[above right of=Pw23,node distance=2.5cm]	{$\theta^{(2)}_{n+1}$};
\node[square_my_graph]	(Chan23) 	[above of=phase23,node distance=2cm]	{$f_{n+1}^{(2)}$};
%\node[circle_my_graph] 	(symbol23) 	[above of=Chan23,node distance=1.5cm]	{$x^{(2)}_{n+1}$};
%\node[square_my_graph]	(MOD23) 	[above of=symbol23,node distance=1.5cm]	{$\MODwo$};
%\node[circle_my_graph] 	(label23) 	[above of=MOD23,node distance=1.5cm]	{$\tilde{\bc}^{(2)}_{n+1}$};
%-
\node[point_my]	 		(point13) 	[below right of=phase13,node distance=1.5cm]	{};
\node[point_my]	 		(point23) 	[below right of=phase23,node distance=1.5cm]	{};
%%%%%--------    Draw Paths  -------- %%%%%%%%%%%%%%%%
\draw[-]   (Pw13)	  -- 	(phase1.south);   
\draw[-]   (Pw23)	  -- node[midway,above,sloped]{$\underleftarrow{\beta^{(t)}_{n}(\theta)}$}	(phase2.south);
\draw[-]   (Pw13)	  -- 	(phase13);   \draw[-]   (Pw23)	  -- 	(phase23);
\draw[-]   (phase13)  -- 	(Chan13);   \draw[-]   (phase23)  -- 	(Chan23);
\draw[-]   (Chan13) -- (symbol13);  \draw[-]   (Chan23) -- (symbol13);
%\draw[-]    (symbol13) -- (MOD13); \draw[-]    (symbol23) -- (MOD23);
%\draw[-]    (MOD13) --  (label13);   \draw[--   ](MOD23) --  (label23);
\draw[-,dashed]   (point13)	  -- 	(phase13.south);   \draw[-,dashed]   (point23)	  -- 	(phase23.south);

%%%% add the code constraints
\begin{pgfonlayer}{foreground}
\node[point_my]	 (label11H)	[above of=symbol11,node distance=2.5cm]	{};
%\node[point_my]	 (label21H)	[above of=symbol21,node distance=2.5cm]	{};
\node[point_my]	 (label1H)	[above of=symbol1,node distance=2.5cm]	{};
%\node[point_my]	 (label2H)	[above of=symbol2,node distance=2.5cm]	{};
\node[point_my]	 (label13H)	[above of=symbol13,node distance=2.5cm]	{};
\node[point_my]	 (label23H)	[above of=symbol23,node distance=2.5cm]	{};


\draw[-]    (symbol1) -- node[near start,above,sloped]{$\underrightarrow{P_{n}(x)}$} (label1H);   
%\draw[-]    (symbol2) -- node[near start,below,sloped,xshift=0.2cm]{$\overleftarrow{P^{\tr{a},(t)}_{n}(x)}$} (label2H);   
\draw[-]    (symbol11) -- (label11H);   %\draw[-]    (symbol21) -- (label21H);   
\draw[-]    (symbol13) --  (label13H);  %\draw[-]    (symbol23) --  (label23H);
\node[bigbox_my,fill=blue!20, fit=(label11H)(label23H)]   (ENCODER) {modulation/coding graph};
\end{pgfonlayer}
 
%\path[line_my]   (start_p)	-- node[above, near start]{$\bb$}	(Enc);
%\path[line_my]   (Enc)		-- node[above, near start]{$\bx$} 	(Chan1) coordinate[pos=0.6](Temp1); 
%\path[line_my]   (Temp1)		|- 	(Chan2);
%\path[line_my]   (Temp1)		|- 	(Chank);
%\path[line_my]   (Chan1)	-- node[above]{$\by_1$}	(Dem1); 
%\path[line_my]   (Chan2)	-- node[above]{$\by_2$}	(Dem2); 
%\path[line_my]   (Chank)	-- node[above]{$\by_k$}	(Demk); 
%\path[line_my]   (Dem1)	-- node[above,near start]{$L_1$}	(Agg); 
%\path[line_my]   (Dem2.east)	-- node[above,near start]{$L_2$}	(Agg);
%\path[line_my]   (Demk.east)	-- node[below right,near start]{$L_k$}	(Agg);
%\path[line_my]   (Agg)		-- node[above,near end]{$L^\Sigma$}	(Dec);
%\path[line_my]   (Dec)		-- node[above, near end]{$\hat{\bb}$}	(end_p); 

%%%% %% --- Draw Big Box
%\begin{pgfonlayer}{background}
%\node[bigbox_my,fill=blue!20, fit=(Dem1)(Demk)(Agg),label=north:$\DEMwo$]   (Dem_tot) {};
%\node[bigbox_my,fill=blue!20, fit=(Chan1)(Chank),label=north:Channel]   (Chan_tot) {};
%\node[below right] at (RX.north)  {Receiver};
%\end{pgfonlayer}

%%%%
\end{tikzpicture}

